Estimating Peer Effects Using Partial Network Data

We study the estimation of peer effects through social networks when researchers do not observe the entire network structure. Special cases include sampled networks, censored networks, and misclassified links. We assume that researchers can obtain a consistent estimator of the distribution of the network. We show that this assumption is sufficient for estimating peer effects using a linear-in-means model. We provide an empirical application to the study of peer effects on students' academic achievement using the widely used Add Health database, and show that network data errors have a large downward bias on estimated peer effects.

==> RestatRR1/OA_Bayesian_2.tex <==
\section{Bayesian estimator}\label{sec:OA_bayesian}

\input{appendix_bayesian}

\subsection{Network Sampling}\label{sec:networksampling}
This section explains how we sample the network in Algorithm \ref{algo:mcmc} using Gibbs sampling. As discussed above, a natural solution is to update only one entry of the adjacency matrix at every step $t$ of the MCMC. The entry $(i, j)$ is updated according to its conditional posterior distribution. For each entry, however, we need to compute $\mathcal{P}(\mathbf{y}|0,\mathbf{A}_{-ij})$ and $\mathcal{P}(\mathbf{y}|1,\mathbf{A}_{-ij})$, which are the respective likelihoods of replacing $a_{ij}$ by 0 or by 1. The likelihood computation requires the determinant of $(\mathbf{I}-\alpha\mathbf{G})$, which has a complexity $O(N^3)$ where N is the dimension of $\mathbf{G}$. This implies that we must compute $2N(N-1)$ times $\text{det}(\mathbf{I}-\alpha\mathbf{G})$ to update the adjacency matrix at each step of the MCMC. As $\bG$ is row-normalized, alternating any off-diagonal entry $(i,j)$ in $\bA$ between $0$ and $1$ perturbs all off-diagonal entries of the row $i$ in $(\mathbf{I}-\alpha\mathbf{G})$. We show that $\bA_{ij}$ and $\text{det}(\mathbf{I}-\alpha\mathbf{G})$ can be updated by computing a determinant of an auxiliary matrix that requires only updating two entries.

Assume that we want to update the entry $(i,j)$. Let $h$ be the function defined in $\mathbb{N}$ such that $\forall ~ x \in \mathbb{N}^*$, $h(x) = x$, and $h(0) = 1$. Let $\mathbf{L}$ be an N $\times$ N diagonal matrix, where $\mathbf{L}_{ii} = h(n_i)$, and $n_i$ stands for the degree of $i$, while $\mathbf{L}_{kk}=1$ for all $k\neq i$, and $\mathbf{W}$ is the matrix $\bG$ where the row $i$ of $\mathbf{W}$ is replaced by the row $i$ of $\bA$. Then, as the determinant is linear in each row, we can obtain $\mathbf{I}-\alpha\mathbf{G}$ by dividing the row $i$ of $\mathbf{L} - \alpha\mathbf{W}$ by $h(n_i)$. We get:
$$
\text{det}(\mathbf{I}-\alpha\mathbf{G}) = \dfrac{1}{h(n_i)}\text{det}(\mathbf{L}-\alpha\mathbf{W}).
$$
\noindent When $a_{ij}$ changes (from $0$ to $1$, or $1$ to $0$), note that only the entries $(i,i)$ and $(i,j)$ change in $\mathbf{L}-\alpha\mathbf{W}$. Two cases can be distinguished.
\begin{itemize}
    \item If $a_{ij} = 0$ before the update, then the new degree of $i$ will be $n_i + 1$. Thus, the entry $(i,i)$ in $\mathbf{L}-\alpha\mathbf{W}$ will change from $h(n_i)$ to $h(n_i + 1)$ (as the diagonal of $\mathbf{W}$ equals $0$), and the entry $(i,j)$ will change from $0$ to $-\alpha$. The new determinant is therefore given by
    $$\text{det}(\mathbf{I}-\alpha\mathbf{G}^*) = \dfrac{1}{h(n_i + 1)}\text{det}(\mathbf{L}^*-\alpha\mathbf{W}^*),$$ where $\mathbf{G}^*$, $\mathbf{L}^*$, and $\alpha\mathbf{W}^*$ are the new matrices once $a_{ij}$ has been updated.
    \item If $a_{ij} = 1$ before the update, then the new degree of $k$ will be $n_i - 1$. Thus, the entry $(i,i)$ in $\mathbf{L}-\alpha\mathbf{W}$ will change from $h(n_i)$ to $h(n_i - 1)$, and the entry $(i,j)$ will change from $-\alpha$ to $0$. The new determinant is therefore given by
    $$\text{det}(\mathbf{I}-\alpha\mathbf{G}^*) = \dfrac{1}{h(n_i - 1)}\text{det}(\mathbf{L}^*-\alpha\mathbf{W}^*).$$
\end{itemize}
\noindent Then, to update $\text{det}(\mathbf{L}-\alpha\mathbf{W})$ when only the entries $(i,i)$ and $(i,j)$ change, we adapt the Lemma 1 in \citeOA{hsieh2019structural} as follows:

\begin{proposition}\label{prop:det}
\noindent Let $\mathbf{e}_i$ be the $i$'th unit basis vector in $\mathbb{R}^N$. Let $\mathbf{M}$ denote an N $\times$ N matrix and $\mathbf{B}_{ij}(\mathbf{Q}, \epsilon)$ an N $\times$ N matrix as a function of an N $\times$ N matrix $\mathbf{Q}$ and a real value $\epsilon$, such that
\begin{equation}
    \mathbf{B}_{ij}(\mathbf{Q}, \epsilon) = \dfrac{\mathbf{Q} \mathbf{e}_i \mathbf{e}_j^{\prime} \mathbf{Q}}{1 + \epsilon \mathbf{e}_j^{\prime} \mathbf{Q} \mathbf{e}_i}.
\end{equation}
\noindent Adding a perturbation $\epsilon_1$ in the (i, i)th position and a perturbation $\epsilon_2$ in the (i, j)th position to the matrix $\mathbf{M}$ can be written as $\tilde{\mathbf{M}} = \mathbf{M} + \epsilon_1 \mathbf{e}_i \mathbf{e}_i^{\prime} +  \epsilon_2 \mathbf{e}_i \mathbf{e}_j^{\prime}$. 
\begin{enumerate}
    \item  The inverse of the perturbed matrix can be written as
    \begin{equation*}
    \tilde{\mathbf{M}}^{-1} = \mathbf{M}^{-1} - \epsilon_1\mathbf{B}_{ii}(\mathbf{M}^{-1}, \epsilon_1) -  \epsilon_2\mathbf{B}_{ij}\left(\mathbf{M}^{-1} - \epsilon_1\mathbf{B}_{ii}(\mathbf{M}^{-1}, \epsilon_1), \epsilon_2\right).
    \end{equation*}
    \item The determinant of the perturbed matrix can be written as
    \begin{equation*}
    \text{det}\left(\tilde{\mathbf{M}}\right) = \left(1 + \epsilon_2 \mathbf{e}_j^{\prime}\left(\mathbf{M}^{-1} - \epsilon_1\mathbf{B}_{ii}(\mathbf{M}^{-1}, \epsilon_1) \mathbf{e}_i\right)\right)(1 + \epsilon_1\mathbf{e}_i^{\prime}\mathbf{M}^{-1}\mathbf{e}_i)\text{det}\left(\mathbf{M}\right).
    \end{equation*}
\end{enumerate}
\end{proposition}
\begin{proof}
\begin{enumerate}
\item By the Sherman--Morrison formula \citepOA[][]{mele2017}, we have
\begin{equation*}
\left(\mathbf{M} + \epsilon \mathbf{e}_i \mathbf{e}_j^{\prime}\right)^{-1} = \mathbf{M}^{-1} - \epsilon \dfrac{\mathbf{M}^{-1} \mathbf{e}_i \mathbf{e}_j^{\prime} \mathbf{M}^{-1}}{1 + \epsilon \mathbf{e}_j^{\prime} \mathbf{M}^{-1} \mathbf{e}_i} = \mathbf{M}^{-1} - \epsilon\mathbf{B}_{ij}(\mathbf{M}, \epsilon).
\end{equation*}
Thus, 
\begin{eqnarray*}
 \tilde{\mathbf{M}}^{-1} &= \left((\mathbf{M} + \epsilon_1 \mathbf{e}_i \mathbf{e}_i^{\prime}) +  \epsilon_2 \mathbf{e}_i \mathbf{e}_j^{\prime}\right)^{-1},\\
 \tilde{\mathbf{M}}^{-1}   &= (\mathbf{M} + \epsilon_1 \mathbf{e}_i \mathbf{e}_i^{\prime})^{-1} - \epsilon_2\mathbf{B}_{ij}((\mathbf{M} + \epsilon_1 \mathbf{e}_i \mathbf{e}_i^{\prime})^{-1}, \epsilon_2),\\
 \tilde{\mathbf{M}}^{-1}   &=  \mathbf{M}^{-1} - \epsilon_1\mathbf{B}_{ii}(\mathbf{M}^{-1}, \epsilon_1) -  \epsilon_2\mathbf{B}_{ij}\left(\mathbf{M}^{-1} - \epsilon_1\mathbf{B}_{ii}(\mathbf{M}^{-1}, \epsilon_1), \epsilon_2\right).
\end{eqnarray*}
\item By the matrix determinant lemma \citepOA[][]{johnson1985matrix}, we have
\begin{equation*}
\text{det}\left(\mathbf{M} + \epsilon \mathbf{e}_i \mathbf{e}_j^{\prime}\right) = (1 + \epsilon \mathbf{e}_j^{\prime}\mathbf{M}^{-1}\mathbf{e}_i)\text{det}\left(\mathbf{M}\right).
\end{equation*}
\noindent It follows that
\begin{eqnarray*}
 \text{det}\left(\tilde{\mathbf{M}}\right) &= \text{det}\left((\mathbf{M} + \epsilon_1 \mathbf{e}_i \mathbf{e}_i^{\prime}) +  \epsilon_2 \mathbf{e}_i \mathbf{e}_j^{\prime}\right),\\
 \text{det}\left(\tilde{\mathbf{M}}\right)   &= (1 + \epsilon_2\mathbf{e}_j^{\prime} (\mathbf{M} + \epsilon_1 \mathbf{e}_i \mathbf{e}_i^{\prime})^{-1} \mathbf{e}_i) \text{det}\left(\mathbf{M} + \epsilon_1 \mathbf{e}_i \mathbf{e}_i^{\prime}\right),\\
 \text{det}\left(\tilde{\mathbf{M}}\right)  &=  \left(1 + \epsilon_2 \mathbf{e}_j^{\prime}\left(\mathbf{M}^{-1} - \epsilon_1\mathbf{B}_{ii}(\mathbf{M}^{-1}, \epsilon_1) \mathbf{e}_i\right)\right)(1 + \epsilon_1\mathbf{e}_i^{\prime}\mathbf{M}^{-1}\mathbf{e}_i)\text{det}\left(\mathbf{M}\right).
\end{eqnarray*}
\end{enumerate}
\end{proof}

\noindent The method proposed above becomes computationally intensive when many entries must be updated simultaneously.  We also propose an alternative method that allows updating the block for entries in $\bA$. Let $\mathbf{D}=(\mathbf{I}-\alpha\mathbf{G})$; we can write
\begin{equation}
\displaystyle \text{det}(\mathbf{D}) = \sum_{j = 1}^N(-1)^{i+j}\mathbf{D}_{\text{ij}}\delta_{\text{ij}},
\label{det}
\end{equation}
where $i$ denotes any row of $\mathbf{D}$ and $\delta_{ij}$ is the minor\footnote{The determinant of the submatrix of $\mathbf{M}$ by removing row $i$ and column $j$.} associated with the entry $(i, j)$. The minors of row $i$ do not depend on the values of entries in row $i$. To update any block in row $i$, we therefore compute the $N$ minors associated with $i$ and use this minor within the row. We can then update many entries simultaneously without increasing the number of times that we compute $\text{det}(\mathbf{D})$.

\noindent One possibility is to update multiple links simultaneously by randomly choosing the number of entries to consider and their position in the row. As suggested by \citeOA{chib2010tailored}, this method would help the Gibbs sampling to converge more quickly. We can summarize how we update the row $i$ as follows:
\begin{enumerate}
    \item Compute the $N$ minors $\delta_{i1}, \dots, \delta_{in}$ \label{update::minor}.
	\item Let $\Omega_{\bG}$ be the entries to update in the row $i$, and $n_{\bG} = |\Omega_{\bG}|$ the number of entries in $\Omega_{\bG}$.
	%Generally $\Omega_{\bG} = \{(i,1), (i,2), \dots, (i, N)\} \setminus \{(i, i)\}$ and $n_{\bG} = N - 1$, but sometimes we do not need to update some links (for example, the observed links).
	\begin{enumerate}
	    \item Choose $r$, the size of the block to update, as a random integer number such that $1 \leq r \leq  n_{\bG}$. In practice, we choose $r \leq \min(5, n_{\bG})$ because the number of possibilities of links to consider grows exponentially with $r$. \label{update::block::size}
    	\item Choose the $r$ random entries from $\Omega_{\bG}$. These entries define the block to update. \label{update::entries}
    	\item Compute the posterior probabilities of all possibilities of links inside the block and update the block (there are $2^r$ possibilities). Use the minors calculated at \ref{update::minor} and the formula (\ref{det}) to quickly compute $det(\mathbf{D})$.  \label{update::post::prob}
    	\item  Remove the $r$ drawn positions from $\Omega_{\bG}$ and let  $n_{\bG} = n_{\bG} - r$.  Replicate \ref{update::block::size},  \ref{update::entries}, and \ref{update::post::prob} until $n_{\bG} = 0$.
	\end{enumerate}
\end{enumerate}


\subsection{How to build prior distributions}\label{sec:appendix_prior}
The two following examples discuss how to construct prior distributions depending on whether the first stage is estimated by a classical or Bayesian estimator.

\begin{example}[Priors from the Asymptotic Distribution of $\boldsymbol{\rho}$]\label{ex:prior_distr}
In a classical setting, and under the usual assumptions, the estimation of (\ref{eq:gennetfor}) produces an estimator $\hat{\boldsymbol{\rho}}$ of $\boldsymbol{\rho}_0$ and an estimator of the asymptotic variance of $\hat{\boldsymbol{\rho}}$, i.e., $\hat{\mathbf{V}}(\hat{\boldsymbol{\rho}})$. In this case, we define the prior density $\pi(\boldsymbol{\rho})$ as the density of a multivariate normal distribution with mean $\hat{\boldsymbol{\rho}}$ and variance--covariance matrix $\hat{\mathbf{V}}(\hat{\boldsymbol{\rho}})$.
\end{example}

\begin{example}[Priors from the Posterior Distribution of $\boldsymbol{\rho}$]\label{ex:prior_post}
In a Bayesian setting, the estimation of $\boldsymbol{\rho}$ from the network formation model (\ref{eq:gennetfor}) results in draws from the posterior distribution of $\boldsymbol{\rho}$. It is therefore natural to use such a posterior distribution as the prior distribution of $\mathbf{A}$ for the estimation based on (\ref{eq:likelihood}). Performing such a sequential Bayesian updating approach comes with a well-known numerical issue.\footnote{See \citeOA{thijssen2020approximating} for a recent discussion.}

Indeed, the evaluation of the acceptance ratio in Step 1 of Algorithm \ref{algo:mcmc} below requires the evaluation of the density of $\boldsymbol{\rho}$ at different values. Ideally, one would use the draws from the posterior distribution of $\boldsymbol{\rho}$ from the first step (network formation model) and perform a nonparametric kernel density estimation of the posterior distribution. However, when the dimension of $\boldsymbol{\rho}$ is large, the kernel density estimation may be infeasible in practice.

This is especially true for very flexible network formation models, such as that proposed by \citeOA{breza2017using} for which the number of parameters to estimate is $O(N_m)$. In such a case, it might be more reasonable to use a more parametric approach or to impose additional restrictions on the dependence structure of $\boldsymbol{\rho}$ across dimensions.\footnote{For example, if we assume that the posterior distribution of $\boldsymbol{\rho}$ is jointly normal, the estimation of the mean and variance-covariance matrix is straightforward, even in a high-dimensional setting. Simulations suggest that this approach performs well in practice. See the Vignette accompanying our R package.}
\end{example}

==> RestatRR1/OA_THM1.tex <==
\section{Proof of Theorem 1: Additional Material}\label{sec:OA_thm1}
\begin{customthm}{\ref{lemma:continuity}}[Differentiability]
    $\mathbb{E}[\mathbf{m}_{m}(\boldsymbol{\theta},\boldsymbol{\rho})]$ is continuously differentiable in $(\boldsymbol{\theta}, \boldsymbol{\rho})$.
\end{customthm}

\begin{proof}
Since $\mathbf{m}_{m}(\boldsymbol{\theta},\boldsymbol{\rho})$ is continuously differentiable in $\boldsymbol{\theta}$ and absolutely integrable, along with its derivative with respect to $\boldsymbol{\theta}$, it follows that $\mathbb{E}[\mathbf{m}_{m}(\boldsymbol{\theta},\boldsymbol{\rho})]$ is continuously differentiable in $\boldsymbol{\theta}$ by the Leibniz integral rule. However, $\mathbf{m}_{m}(\boldsymbol{\theta},\boldsymbol{\rho})$ is continuously differentiable in $\boldsymbol{\rho}$ only for \emph{almost all} $\boldsymbol{\rho}$. We now show that $\mathbb{E}[\mathbf{m}_{m}(\boldsymbol{\theta},\boldsymbol{\rho})]$ is continuously differentiable for all $\boldsymbol{\rho}$.


Consider $\mathbf{B}_m\dot{\mathbf{G}}_m(\boldsymbol{\rho}) = \mathbf{B}_m f(\dot{\mathbf{A}}_m(\boldsymbol{\rho}))$ for some (conformable) matrix $\mathbf{B}_m$. We have:
\begin{equation}\label{eq:EB}
    \hat{\mathbb{E}}_m (\mathbf{B}_m\dot{\mathbf{G}}_m(\boldsymbol{\rho})) = \sum_{\hat{\mathbf{A}}_m} \mathbf{B}_m f(\hat{\mathbf{A}}_m) P (\mathbf{A}_m(\boldsymbol{\rho}) = \hat{\mathbf{A}}_m \mid \mathbf{X}_m, \kappa(\mathcal{A}_m)),
\end{equation}
where the sum is taken over all the possible network configurations $\hat{\mathbf{A}}_m$, and where \break$P(\mathbf{A}_m(\boldsymbol{\rho})=\hat{\mathbf{A}}_m|\mathbf{X}_m,\kappa(\mathcal{A}_m))=\Pi_{ij}P(a_{ij,m}(\boldsymbol{\rho})=\hat{a}_{ij,m}|\mathbf{X}_m,\kappa(\mathcal{A}_m))$, as defined in Equation (\ref{eq:gennetfor}). Thus $\hat{\mathbb{E}}_m (\mathbf{B}_m\dot{\mathbf{G}}_m(\boldsymbol{\rho}))$ is continuously differentiable in $\boldsymbol{\rho}$ by Assumption \ref{as:derivatives_P}.
By adapting this argument for the appropriate definition of the matrix $\mathbf{B}_m$, and for $\hat{\mathbb{E}}_m$, and $\mathbb{E}^{(0)}_m$, this shows that $\mathbb{E}[\mathbf{m}_{m,rst}(\boldsymbol{\theta},\boldsymbol{\rho})|\mathbf{X}_m,\kappa(\mathcal{A}_m)]$ is continuously differentiable in $(\boldsymbol{\theta}, \boldsymbol{\rho})$. As a result, $\mathbb{E}[\mathbf{m}_{m}(\boldsymbol{\theta},\boldsymbol{\rho})]$ is continuously differentiable in $(\boldsymbol{\theta}, \boldsymbol{\rho})$ by the Leibniz integral rule.\end{proof}


\begin{customthm}{\ref{lemma:uniformconvergence}}[Uniform convergence] We establish the following results.
\begin{enumerate}[label=(\alph*), nosep]
    \item $\mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},\hat{\boldsymbol{\rho}})] - \mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},{\boldsymbol{\rho}}_0)]$ converges uniformly to $\mathbf{0}$ in $\boldsymbol{\theta}$ as $M \to \infty$.
    \item $\bar{\mathbf{m}}_M(\boldsymbol{\theta},\hat{\boldsymbol{\rho}}) - \mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},\hat{\boldsymbol{\rho}})]$ converges uniformly in probability to $\mathbf{0}$ in $\boldsymbol{\theta}$ as $M \to \infty$.
    \item $\bar{\mathbf{m}}_M(\boldsymbol{\theta},\hat{\boldsymbol{\rho}}) - \mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},{\boldsymbol{\rho}}_0)]$ converges uniformly in probability to $\mathbf{0}$ in $\boldsymbol{\theta}$ as $M \to \infty$. 
\end{enumerate}
    
\end{customthm}


\begin{proof} 
As $\mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},\boldsymbol{\rho})]$ is nonstochastic and continuously differentiable in $\boldsymbol{\rho}$ (Lemma \ref{lemma:continuity}), it follows that $\mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},\hat{\boldsymbol{\rho}})] - \mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},{\boldsymbol{\rho}}_0)]$ converges to $\mathbf{0}$ pointwise for each $\boldsymbol{\theta}$, given that $\plim \hat{\boldsymbol{\rho}} = {\boldsymbol{\rho}}_0$. To establish uniform convergence, we apply Lemma 2.9 in  \cite{newey1994large}. The required conditions are satisfied: (i) the space of $\boldsymbol\theta$ is compact (Assumption \ref{as:regularity}), (ii) $\mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},\hat{\boldsymbol{\rho}})] - \mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},{\boldsymbol{\rho}}_0)]$ converges to $\mathbf{0}$ for all $\boldsymbol\theta$, and (iii) the derivative of $\mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},\hat{\boldsymbol{\rho}})] - \mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},{\boldsymbol{\rho}}_0)]$ with respect to $\boldsymbol{\theta}$ is bounded in probability (Assumptions \ref{as:manymarkets} and \ref{as:nonsingular}). As a result, $\mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},\hat{\boldsymbol{\rho}})] - \mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},{\boldsymbol{\rho}}_0)]$ uniformly converges to zero in $\boldsymbol{\theta}$.
This completes the proof of Statement \ref{lemma:uniformconvergence:A}.

For Statement \ref{lemma:uniformconvergence:B}, we first establish pointwise convergence by showing that the variance of $\bar{\mathbf{m}}_M(\boldsymbol{\theta},\hat{\boldsymbol{\rho}})$ vanishes asymptotically. By the law of iterated variances, we have: 
\begingroup
\allowdisplaybreaks
\begin{align}
    &\mathbb V(\bar{\mathbf{m}}_M(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})) = \mathbb V\left\{\mathbb E\big(\bar{\mathbf{m}}_M(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})|\mathbf X, \kappa(\mathcal{A}), \hat{\boldsymbol{\rho}}\big)\right\} + \mathbb E\left\{\mathbb V\big(\bar{\mathbf{m}}_M(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})|\mathbf X, \kappa(\mathcal{A}), \hat{\boldsymbol{\rho}}\big)\right\},\nonumber\\
    &\lim \mathbb V(\bar{\mathbf{m}}_M(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})) = \mathbb V\left\{\plim \mathbb E\big(\bar{\mathbf{m}}_M(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})|\mathbf X, \kappa(\mathcal{A}), \hat{\boldsymbol{\rho}}\big)\right\}~+ \nonumber\\&\quad\quad\quad\quad \mathbb E\left\{\plim \mathbb V\big(\bar{\mathbf{m}}_M(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})|\mathbf X, \kappa(\mathcal{A}), \hat{\boldsymbol{\rho}}\big)\right\},\nonumber\\
    \begin{split}
    &\lim \mathbb V(\bar{\mathbf{m}}_M(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})) = \mathbb V\left\{\plim \mathbb E\big(\bar{\mathbf{m}}_M(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})|\mathbf X, \kappa(\mathcal{A}), \hat{\boldsymbol{\rho}}\big)\right\} ~+ \\&\quad\quad\quad\quad\mathbb E\left\{\plim \dfrac{1}{M^2}\sum_{m = 1}^M\mathbb V\big(\mathbf{m}_m(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})|\mathbf X_m, \mathcal{A}_m, \hat{\boldsymbol{\rho}}\big)\right\}.
    \end{split} \label{eq:Vmbar}
\end{align}
\endgroup
The second equality holds by the dominated convergence theorem.\footnote{Specifically, $\mathbb{E}(\bar{\mathbf{m}}_M(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}}) \mid \mathbf{X}, \kappa(\mathcal{A}), \hat{\boldsymbol{\rho}})$ and $\mathbb{V}(\bar{\mathbf{m}}_M(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}}) \mid \mathbf{X}, \kappa(\mathcal{A}), \hat{\boldsymbol{\rho}})$ are bounded by Assumptions \ref{as:manymarkets} and \ref{as:nonsingular}, as well as by the fact that the conditional variance of $\boldsymbol{\varepsilon}_m$ is uniformly bounded (Assumption \ref{as:finitevariance}). Consequently, we can interchange the expectation and probability limit operators.
} Equation \eqref{eq:Vmbar} holds by the fact that \( \mathbf{m}_m(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}}) \) are independent across \( m \), conditional on \( \mathbf{X}_m, \mathcal{A}_m, \hat{\boldsymbol{\rho}} \). 

From Equation \eqref{eq:Vmbar}, it is thus sufficient to show that \( \plim \mathbb{E}(\bar{\mathbf{m}}_M(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}}) | \mathbf{X}, \kappa(\mathcal{A}), \hat{\boldsymbol{\rho}}) \) is nonstochastic and that \( \plim \dfrac{1}{M^2}\sum_{m = 1}^M \mathbb{V}(\mathbf{m}_m(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}}) | \mathbf{X}_m, \mathcal{A}_m, \hat{\boldsymbol{\rho}}) = \mathbf{0} \).
First, the variance of \( \mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},{\boldsymbol{\rho}}) | \mathbf{X}_m, \kappa(\mathcal{A}_m)] \) vanishes asymptotically by being the variance of an average of independent elements. Therefore, it converges in $\mathcal{L}^2$ and, thus, in probability to its expectation, \( \mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},{\boldsymbol{\rho}})] \), which is nonstochastic. Consequently, \( \plim \mathbb{E}(\bar{\mathbf{m}}_M(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}}) | \mathbf{X}, \kappa(\mathcal{A}), \hat{\boldsymbol{\rho}}) \) is also nonstochastic and, thus,  $\mathbb V\{\plim \mathbb E(\bar{\mathbf{m}}_M(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})|\mathbf X, \kappa(\mathcal{A}), \hat{\boldsymbol{\rho}})\} = \mathbf 0$.

Second,  $\mathbb V(\mathbf{m}_m(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})|\mathbf X_m, \mathcal{A}_m, \hat{\boldsymbol{\rho}}) < \infty$ because $\mathbf{m}_m(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})$ is linear in $\boldsymbol\varepsilon_m$ which has a bounded variance (Assumption \ref{as:finitevariance}). Thus, $\plim \dfrac{1}{M^2}\sum_{m = 1}^M\mathbb V(\mathbf{m}_m(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})|\mathbf X_m, \mathcal{A}_m, \hat{\boldsymbol{\rho}}) = 0$ and $\mathbb E\{\plim \dfrac{1}{M^2}\sum_{m = 1}^M\mathbb V(\mathbf{m}_m(\boldsymbol{\theta}, \hat{\boldsymbol{\rho}})|\mathbf X_m, \mathcal{A}_m, \hat{\boldsymbol{\rho}})\} = \mathbf 0$. 

Consequently, $\bar{\mathbf{m}}_M(\boldsymbol{\theta},\hat{\boldsymbol{\rho}}) - \mathbb{E}[\bar{\mathbf{m}}_M(\boldsymbol{\theta},{\boldsymbol{\rho}}_0)]$ converges in probability to $\mathbf 0$. The convergence is uniform in $\boldsymbol{\theta}$ from Lemma 2.9 of \citeOA{newey1994large} as in Statements \ref{lemma:uniformconvergence:A}. This completes the proof of Statement \ref{lemma:uniformconvergence:B} and, consequently, the lemma, given that Statements \ref{lemma:uniformconvergence:A} and \ref{lemma:uniformconvergence:B} together imply Statement \ref{lemma:uniformconvergence:C}.
\end{proof}

\begin{lemma}\label{sec:stochasticequi}
    The stochastic equicontinuity condition \autoref{cond:sequi} is verified.
\end{lemma}
\begin{proof}
As $\boldsymbol{\theta}_0$ in \autoref{cond:sequi} is fixed, we ignore it in our notations and define $\tilde{\mathbf{m}}_{m}({\boldsymbol{\rho}}) = \mathbf{m}_{m}({\boldsymbol{\theta}}_0,{\boldsymbol{\rho}})$. We follow \citeOA{andrews1994empirical} and define
$$\nu_M({\boldsymbol{\rho}})=\frac{1}{\sqrt{M}}\sum_m [\tilde{\mathbf{m}}_m({\boldsymbol{\rho}})-\mathbb{E}(\tilde{\mathbf{m}}_m({\boldsymbol{\rho}}))],$$
so that conditions \autoref{cond:sequi} is equivalent to $\nu_M(\hat{\boldsymbol{\rho}}) - \nu_M({\boldsymbol{\rho}}_0)=o_p(1)$.
Consider the following pseudo-metric, for any dimension $k$ of the moment function
$$
d_k({\boldsymbol{\rho}}_1,{\boldsymbol{\rho}}_2)=\sup_{m}(\mathbb{E}[\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_1)-\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_2)]^2)^{1/2}.
$$
We say that the process $\nu_M$ is \emph{stochastically equicontinuous} if, $\forall \epsilon>0$, $\exists \delta>0$ such that
$$
\plim\sup_{d_k({\boldsymbol{\rho}}_1,{\boldsymbol{\rho}}_2)<\delta} | \nu_{M,[k]}({\boldsymbol{\rho}}_1)-\nu_{M,[k]}({\boldsymbol{\rho}}_2) |<\epsilon,
$$
for each dimension $[k]$.
To see that stochastic equicontinuity implies \autoref{cond:sequi}, note that, for any $\epsilon > 0$:
\begingroup
\allowdisplaybreaks
\begin{eqnarray*}
&&\lim P(|\nu_{M,[k]}(\hat{\boldsymbol{\rho}})-\nu_{M,[k]}({\boldsymbol{\rho}}_0)|>\epsilon) \\&\leq& \lim P(|\nu_{M,[k]}(\hat{\boldsymbol{\rho}})-\nu_{M,[k]}({\boldsymbol{\rho}}_0)|>\epsilon, d_k(\hat{\boldsymbol{\rho}},{\boldsymbol{\rho}}_0)\leq\delta)  + \lim P( d_k(\hat{\boldsymbol{\rho}},{\boldsymbol{\rho}}_0)>\delta) \\
&\leq& \lim P\left( \sup_{d(\boldsymbol{\rho}_1,\boldsymbol{\rho}_2)<\delta} | \nu_{M,[k]}(\hat{\boldsymbol{\rho}})-\nu_{M,[k]}({\boldsymbol{\rho}}_0) | > \epsilon\right)
\end{eqnarray*}
\endgroup
The last inequality holds because $\lim P( d_k(\hat{\boldsymbol{\rho}},{\boldsymbol{\rho}}_0)>\delta) = 0$ by the consistency of $\hat{\boldsymbol{\rho}}$. Stochastic equicontinuity implies that $\delta$ can be chosen so that $\lim P\Big( \sup_{d(\boldsymbol{\rho}_1,\boldsymbol{\rho}_2)<\delta} | \nu_{M,[k]}(\hat{\boldsymbol{\rho}})-\nu_{M,[k]}({\boldsymbol{\rho}}_0) | > \epsilon\Big)$ is as small as desired. Thus,  
$\lim P(|\nu_{M,[k]}(\hat{\boldsymbol{\rho}})-\nu_{M,[k]}({\boldsymbol{\rho}}_0)|>\epsilon)$  
can also be made arbitrarily small, that is,  
$\nu_M(\hat{\boldsymbol{\rho}}) - \nu_M({\boldsymbol{\rho}}_0) = o_p(1)$,  
which corresponds to our condition \autoref{cond:sequi}. It is thus sufficient to show that $\nu_M$ is stochastically equicontinuous.


Following \citeOA{andrews1994empirical}, Section 5, we say that $\tilde{\mathbf{m}}_m$ is Type $IV(p=2)$ if the parameter space is bounded (Assumption \ref{as:regularity}) and
\begin{equation}\label{eq:IV_cond}
\sup_m\left( \mathbb{E}\Big(\sup_{\boldsymbol{\rho}_1:\Vert {\boldsymbol{\rho}}_1-{\boldsymbol{\rho}}_2\Vert<\delta} (\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_1)-\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_2))^2\Big)\right)^{1/2}\leq C\delta^\psi,
\end{equation}
for all ${\boldsymbol{\rho}}_2$ and all $\delta>0$ in a neighborhood of $0$, for some finite positive constants $C$ and $\psi$, and for all dimensions $[k]$.




We can express $\tilde{\mathbf{m}}_{m,[k]}(\boldsymbol{\rho})$ as a linear function of $\boldsymbol{\varepsilon}_m$ (e.g., see Equation \eqref{eq:m:lineps} in Appendix \ref{sec:proofconsistencySGMM}). Thus, $\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_1)-\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_2) = u_{1,m,[k]}(\boldsymbol{\rho}_1, \boldsymbol{\rho}_2) + \mathbf{u}_{2,m,[k]}(\boldsymbol{\rho}_1, \boldsymbol{\rho}_2)\boldsymbol{\varepsilon}_m$ for some scalar $u_{1,m,[k]}(\boldsymbol{\rho}_1, \boldsymbol{\rho}_2)$ and row vector $\mathbf{u}_{2,m,[k]}(\boldsymbol{\rho}_1, \boldsymbol{\rho}_2)$. Additionally, by Assumptions \ref{as:manymarkets} and \ref{as:nonsingular}, $|u_{1,m,[k]}(\boldsymbol{\rho}_1, \boldsymbol{\rho}_2)|$ and $\lVert \mathbf{u}_{2,m,[k]}(\boldsymbol{\rho}_1, \boldsymbol{\rho}_2) \rVert$ are uniformly bounded by some $\bar{u}_{1,[k]}$ and $\bar{u}_{2,[k]}$, respectively, where $\bar{u}_{1,[k]}$ and $\bar{u}_{2,[k]}$ do not depend on $\boldsymbol{\rho}_1$ and $\boldsymbol{\rho}_2$.  
Therefore, $(\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_1)-\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_2))^2$ is dominated by $(\bar{u}_{1,[k]} + \bar{u}_{2,[k]} \lVert \boldsymbol{\varepsilon}_m \rVert)^2$, for any sub-multiplicative norm $\lVert \cdot \rVert$. 

Since $(\bar{u}_{1} + \bar{u}_{2} \lVert \boldsymbol{\varepsilon}_m \rVert)^2$ is integrable (see Assumption \ref{as:finitevariance}),  
we can apply the dominated convergence theorem and interchange the expectation and the second supremum symbol in \eqref{eq:IV_cond}. A sufficient condition for \eqref{eq:IV_cond} is thus:  
\begin{equation}\label{eq:suffIV}
\sup_m\Big(\sup_{\boldsymbol{\rho}_1:\Vert {\boldsymbol{\rho}}_1-{\boldsymbol{\rho}}_2\Vert<\delta} \mathbb{E} ((\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_1)-\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_2))^2)\Big)^{1/2}\leq C\delta^\psi.
\end{equation}

Now, note that $\mathbb{E} (\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_1)-\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_2))^2$ is continuously differentiable in ${\boldsymbol{\rho}}_1$ with bounded derivatives following the argument in Lemma \ref{lemma:continuity}. See in particular Equation (\ref{eq:EB}).\footnote{The derivative is bounded because the linking probabilities have bounded derivatives (Assumption \ref{as:derivatives_P}), and $\mathbf{X}_m$, $\mathbb{E}(\lVert\boldsymbol{\varepsilon}_m\rVert^2)$, and the entries of the network matrices are bounded (Assumptions \ref{as:manymarkets}, \ref{as:nonsingular}, and \ref{as:finitevariance}).}

Then, by the Mean Value Theorem, we have  
$\mathbb{E} (\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_1)-\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_2))^2 = \mathcal{D}(\boldsymbol{\rho}^+, \boldsymbol{\rho}_2) (\boldsymbol{\rho}_1 - {\boldsymbol{\rho}}_2)$, where $\mathcal{D}(\boldsymbol{\rho}^+, \boldsymbol{\rho}_2)$ is the derivative of $\mathbb{E} (\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_1)-\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_2))^2$ with respect to ${\boldsymbol{\rho}}_1$ at some $\boldsymbol{\rho}^+$ lying between $\boldsymbol{\rho}_1$ and ${\boldsymbol{\rho}}_2$. Thus, $\tilde{\mathbf{m}}_m$ is of Type IV with $p=2$, $\psi = 1/2$, and $C$ as the upper bound of $\mathcal{D}(\boldsymbol{\rho}^+, \boldsymbol{\rho}_2)$. As a result, Condition (\ref{eq:suffIV}), and thus Condition (\ref{eq:IV_cond}), hold.


\begin{comment}
\aristide{An issue with the current proof of (12) is that it is not really mathematically founded. Even if the number of discontinuities is finite, expectations can diverge for example. We did not exploit the fact that our moment function is linear in epsilon. Using this, we can apply the Dominated Convergence Theorem and interchange $\mathbb{E}$ and the second $\sup$. See  page A14.}

Note that from the argument in the proof of Lemma \ref{lemma:continuity}, each dimension $[k]$ of the vector $\tilde{\mathbf{m}}_m({\boldsymbol{\rho}})$ can be written as a function of a finite number of indicator functions (a finite polynomial) of continously differentiable functions in $\boldsymbol{\rho}$, with bounded derivatives, i.e.

$$
\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}})=\phi_k(\mathbbm{1}[\lambda_{m,1}(\boldsymbol{\rho})\geq 0],\mathbbm{1}[\lambda_{m,2}(\boldsymbol{\rho})\geq 0],...),
$$
where each $\lambda_{m,i}$ is continuously differentiable with bounded derivative.


Consider also:
$$
\tilde{\mathbf{m}}^{smooth}_{m,[k]}({\boldsymbol{\rho}})=\phi_k(F[\lambda_{m,1}(\boldsymbol{\rho})/\sigma_\delta],F[\lambda_{m,2}(\boldsymbol{\rho})/\sigma_\delta],...),
$$
where $F$ is continuously differentiable, such that $F(\lambda)\rightarrow 0$ as $\lambda\rightarrow -\infty$, $F(\lambda)\rightarrow 1$ as $\lambda\rightarrow \infty$, and $\sigma_\delta>0$ is such that $\sigma_\delta\rightarrow 0$ as $\delta\rightarrow 0$

We have
\begingroup
\allowdisplaybreaks
\begin{eqnarray*}
&&|\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_1)-\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_2)|\\
&=& |\tilde{\mathbf{m}}^{smooth}_{m,[k]}({\boldsymbol{\rho}}_1) +[\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_1)-\tilde{\mathbf{m}}^{smooth}_{m,[k]}({\boldsymbol{\rho}}_1)] - \tilde{\mathbf{m}}^{smooth}_{m,[k]}({\boldsymbol{\rho}}_2) \\&&+ [\tilde{\mathbf{m}}^{smooth}_{m,[k]}({\boldsymbol{\rho}}_2)-\tilde{\mathbf{m}}_{m,[k]}({\boldsymbol{\rho}}_2)]|\\
&\leq& |\tilde{\mathbf{m}}^{smooth}_{m,[k]}({\boldsymbol{\rho}}_1)-\tilde{\mathbf{m}}^{smooth}_{m,[k]}({\boldsymbol{\rho}}_2)| + error(\boldsymbol{\rho}_1,\boldsymbol{\rho}_2,\delta)
\end{eqnarray*}
\endgroup

First, note that, by the mean value theorem, condition (\ref{eq:IV_cond}) holds for smoothed moments (i.e. the first term on the right hand side). Moreover, whenever $\boldsymbol{\rho}_1$ and $\boldsymbol{\rho}_2$ are not at a discontinuity point, the we can freely select $\sigma_\delta$ such that the approximation error is bounded by $C\delta^\psi$. This is not true, however, if $\boldsymbol{\rho}_1$ or $\boldsymbol{\rho}_2$ is at a discontinuity point, in which case the error is bounded, but not vanishing. However, since this happens with probability zero, Condition \ref{eq:IV_cond} holds.
\end{comment}

By Theorem 4 in \citeOA{andrews1994empirical}, stochastic equicontinuity \autoref{cond:sequi} holds if Ossianders' condition (his condition D) holds, $\lim\frac{1}{M}\sum_m\mathbb{E}\sup_{\boldsymbol{\rho}}|\tilde{\mathbf{m}}_m|^{2+\eta}<\infty$ for some $\eta > 0$ (his condition B), and if groups $m$ are independent (Assumption \ref{as:manymarkets}) implied by his condition C). By Theorem 5 in \citeOA{andrews1994empirical}, Ossianders' condition holds if $\tilde{\mathbf{m}}_m$ is Type $IV(p=2)$, which we just shown. His condition B is  verified because $\mathbb{E}(\lVert\boldsymbol{\varepsilon}_m\rVert^{2 + \eta})$ is bounded for some $\eta > 0$ (Assumption \ref{as:finitevariance}). Thus, as above, we can employ the dominated convergence theorem and interchange the expectation and the second supremum. Since $\mathbb E|\tilde{\mathbf{m}}_m|^{2+\eta}$ is bounded, then condition B follows.
\end{proof}

\subsection{Identification\label{app:ident}}
In this section, we show that Assumption \ref{as:identification} can be expressed as an identification condition on a concentrated objective function.

As \( \mathbf{W}_0 \) is positive definite (Assumption \ref{as:Wm}), Assumption \ref{as:identification} is equivalent to stating that \( Q_0(\boldsymbol{\theta}) \) has a unique minimizer. Since \( Q_0(\boldsymbol{\theta}) \) depends on the true value \( \boldsymbol{\rho}_0 \) and not its estimator, all simulated networks in this section are drawn from the true network distribution. We therefore omit \( \boldsymbol{\rho}_0 \) from the notation for simplicity.


We define: 
\begin{align*}
    \mathbf{B}_m(\alpha)&=\frac{1}{RST}\sum_{rst}\dot{\mathbf{Z}}_m^{(r)\prime}(\mathbf{I}_m-\alpha\ddot{\mathbf{G}}_m^{(s)})(\mathbf{I}_m-\alpha\dddot{\mathbf{G}}_m^{(t)})^{-1}\dddot{\mathbf{V}}_m^{(t)},\\
    \mathbf{D}_m(\alpha)&=\break\frac{1}{RS}\sum_{rs}\dot{\mathbf{Z}}_m^{(r)\prime}(\mathbf{I}_m-\alpha\ddot{\mathbf{G}}_m^{(s)}).
\end{align*}
We have $\textstyle\bar{\mathbf{m}}_M(\boldsymbol{\theta},\boldsymbol{\rho}_0)=\frac{1}{M}\sum_m[\mathbf{D}_m(\alpha)\mathbf{y}_m-\mathbf{B}_m(\alpha)\tilde{\boldsymbol{\theta}}]$. The first-order condition of the minimization of $Q_0 (\boldsymbol{\theta})$ with respect to $\tilde{\boldsymbol{\theta}}$ is: $$
\left[\lim \frac{1}{M}\sum_m\mathbb E\left[\mathbf{B}_m(\alpha)\right]\tilde{\boldsymbol{\theta}}\right]'\mathbf{W}_0\left[\lim \frac{1}{M}\sum_m\big(\mathbb E\left[\mathbf{D}_m(\alpha)\mathbf{y}_m\right]-\mathbb E\left[\mathbf{B}_m(\alpha)\right]\tilde{\boldsymbol{\theta}}\big)\right] = 0.
$$
A sufficient condition for the last equation to have a unique solution in $\tilde{\boldsymbol{\theta}}$ is that $\textstyle\bar{\mathbf{B
}}_0(\alpha):=\lim \frac{1}{M}\sum_m\mathbb E\left[\mathbf{B}_m(\alpha)\right]$ is a full rank matrix for all $\alpha$. Under this condition, the solution $\tilde{\boldsymbol{\theta}}$ can be expressed as:
$$\hat{\tilde{\boldsymbol{\theta}}}(\alpha)=[\bar{\mathbf{B
}}_0'(\alpha)\mathbf{W}_0\bar{\mathbf{B
}}_0]^{-1}\bar{\mathbf{B
}}_0'(\alpha)\mathbf{W}_0\bar{\mathbf F}_0(\alpha),$$
where $\textstyle\bar{\mathbf F}_0(\alpha) = \plim \frac{1}{M}\sum_m\mathbf{D}_m(\alpha)\mathbf{y}_m$. By replacing $\mathbf y_m = (\mathbf I_m - \alpha_0 \mathbf G_m)^{-1}(\mathbf V_m \tilde{\boldsymbol\theta}_0 + \boldsymbol{\varepsilon}_m)$ in the expression of $\textstyle\bar{\mathbf F}_0(\alpha)$, we obtain:
\begin{align*}
    \bar{\mathbf F}_0(\alpha) &= \lim \frac{1}{M}\sum_m\mathbb E\left[\mathbf{F}_m(\alpha)\right], \quad \text{where}\\
    \mathbf{F}_m(\alpha)&=\frac{1}{RS}\sum_{rs}\mathbb E \left(\dot{\mathbf{Z}}_m^{(r)\prime}(\mathbf{I}_m-\alpha\ddot{\mathbf{G}}_m^{(s)})(\mathbf{I}_m-\alpha_0\mathbf{G}_m)^{-1}\mathbf{V}_m\tilde{\boldsymbol\theta}_0\right).
\end{align*}
Since $\bar{\mathbf F}_0(\alpha_0) = \bar{\mathbf{B
}}_0(\alpha_0)\tilde{\boldsymbol\theta}_0$, it follows that $\hat{\tilde{\boldsymbol{\theta}}}(\alpha_0) = \tilde{\boldsymbol\theta}_0$, which means that $\tilde{\boldsymbol\theta}_0$ is identified if $\alpha_0$ is identified; the underlying condition being that $\bar{\mathbf{B
}}_0(\alpha)$ is full rank.

By replacing the solution $\hat{\tilde{\boldsymbol{\theta}}}(\alpha)$ in the objective function, we can concentrate $Q_0(\boldsymbol{\theta})$ around $\alpha$ as
$Q_0^c(\alpha) = \bar{\mathbf Q}^c(\alpha)'\mathbf{W}_0\bar{\mathbf Q}^c(\alpha)$,
Where $$\bar{\mathbf Q}^c(\alpha) = \bar{\mathbf F}_0(\alpha) - \bar{\mathbf{B
}}_0(\alpha)[\bar{\mathbf{B
}}_0'(\alpha)\mathbf{W}_0\bar{\mathbf{B
}}_0]^{-1}\bar{\mathbf{B
}}_0'(\alpha)\mathbf{W}_0\bar{\mathbf F}_0(\alpha).$$

Let $\mathbf{W}_0^{1/2}$ be the positive definite square root of  $\mathbf{W}_0$. We have $\mathbf{W}_0^{1/2}\bar{\mathbf Q}^c(\alpha) = [\mathbf I_{w} - \mathbf P_{\mathbf B}(\alpha)]\mathbf{W}_0^{1/2}\bar{\mathbf F}_0(\alpha)$, where $\mathbf P_{\mathbf B}(\alpha) := \mathbf{W}_0^{1/2}\bar{\mathbf{B
}}_0(\alpha)[\bar{\mathbf{B
}}_0'(\alpha)\mathbf{W}_0\bar{\mathbf{B
}}_0]^{-1}\bar{\mathbf{B
}}_0'(\alpha)\mathbf{W}_0^{1/2}$ is a projection matrix onto the space of the column of $\mathbf{W}_0^{1/2}\bar{\mathbf{B
}}_0(\alpha)$ and $\mathbf I_{w}$ if the identity matrix of the same dimension as $\mathbf{W}_0$. The concentrated objective function can be written as:  
$$Q_0^c(\alpha) = [\mathbf{W}_0^{1/2}\bar{\mathbf F}_0(\alpha)]^{\prime}[\mathbf I_{w} - \mathbf P_{\mathbf B}(\alpha)]\mathbf{W}_0^{1/2}\bar{\mathbf F}_0(\alpha).$$

For Assumption \ref{as:identification} to hold, the equation \( Q_0^c(\alpha) = 0 \) must not have multiple solutions. Unfortunately, simplifying this condition is challenging due to the nonlinearity of $Q_0^c(\alpha)$. A similar issue arises with the maximum likelihood estimator even when the network is fully observed. In this case, the identification condition also leads to a nonlinear equation in the peer effect parameter \citepOA[see][Assumption 9]{lee2004asymptotic}.  

Nevertheless, it is straightforward to sketch the empirical counterpart of \( Q_0^c(\alpha) \) since it is a function of a single variable. In numerous simulation exercises, we observe that \( Q_0^c(\alpha) \) is strictly convex, even when all entries of \( \mathbf{A}_m \) are simulated from an estimated distribution (without setting some entries to observed data). This evidence is encouraging and suggests that the solution to \( Q_0^c(\alpha) = 0 \) is likely unique.


\subsection{Asymptotic variance estimation}\label{sec:varestim}
Estimating the asymptotic variance of $\sqrt{M}(\hat{\boldsymbol{\theta}} - \boldsymbol{\theta}_0)$ can be challenging, as it requires computing the derivative of the expected moment function to estimate $\boldsymbol{\Gamma}_0 = \plim \frac{\partial \bar{\mathbf{m}}^{\ast}_M(\boldsymbol{\theta}_0, \boldsymbol{\rho}^+)}{\partial {\boldsymbol{\rho}^{\prime}}}$ (see Appendix \ref{sec:asymptnorm}). We now present a simple method for estimating this asymptotic variance by adapting \citeOA{houndetoungan2024inference}.

Taking the first derivative of the objective function at the second stage (for finite $R$,$S$,$T$ and conditional on $\hat{\mathbf{\rho}}$) with respect to $\boldsymbol{\theta}$, we have
$$
\left(\frac{\partial\bar{\mathbf{m}}_M(\hat{\boldsymbol{\theta}}, {\boldsymbol{\rho}})}{\partial\boldsymbol{\theta}^{\prime}}\right)^{\prime}\mathbf{W}_M[\bar{\mathbf{m}}_M(\hat{\boldsymbol{\theta}}, {\boldsymbol{\rho}})]=\mathbf{0}.
$$
By applying the mean value theorem to $\bar{\mathbf{m}}_M(\boldsymbol{\theta}, {\boldsymbol{\rho}})$, we have
$$\sqrt{M}(\hat{\boldsymbol{\theta}}-\boldsymbol{\theta}_0)=-\left[\mathbf H_M(\hat{\boldsymbol \theta})^{\prime} \mathbf{W}_M \mathbf H_M({\boldsymbol \theta}^{\ast})\right]^{-1}\mathbf H_M(\hat{\boldsymbol \theta})^{\prime}  \mathbf{W}_M\dfrac{1}{\sqrt{M}}\sum_{m = 1}^M\mathbf{m}_m(\boldsymbol{\theta}_0, \hat{\boldsymbol \rho}),   $$
where $\mathbf H_M(\boldsymbol \theta) = \dfrac{\partial\bar{\mathbf{m}}_M({\boldsymbol{\theta}}, \hat{\boldsymbol{\rho}})}{\partial\boldsymbol{\theta}^{\prime}}$ and $\boldsymbol \theta^{\ast}$ is some point between $\hat{\boldsymbol{\theta}}$ and $\boldsymbol{\theta}_0$.  

Let $\textstyle\boldsymbol{\Omega}_M = \Var(\frac{1}{\sqrt{M}}\sum_{m = 1}^M\mathbf{m}_m(\boldsymbol{\theta}_0, \hat{\boldsymbol \rho}))$. We assume the following:
\begin{assumption}
$\plim \boldsymbol{\Omega}_M = \boldsymbol{\Omega}_0$ and $\plim \mathbf{H}_M({\boldsymbol \theta}_0) = \mathbf{H}_0$ exist and are finite matrices.
\end{assumption}

Under this assumption, the asymptotic variance of $\sqrt{M}(\hat{\boldsymbol{\theta}}-\boldsymbol{\theta}_0)$ is:
$$\mathbb{V}_0(\sqrt{M}(\hat{\boldsymbol{\theta}}-\boldsymbol{\theta}_0)) = (\mathbf H_0^{\prime} \mathbf{W}_0 \mathbf H_0)^{-1}\mathbf H_0^{\prime}  \mathbf{W}_0 \boldsymbol{\Omega}_0 \mathbf{W}_0 \mathbf H_0 (\mathbf H_0^{\prime} \mathbf{W}_0 \mathbf H_0)^{-1}.$$

The expression for the asymptotic variance is similar to the variance of the standard GMM estimator. The key difference is that $\boldsymbol{\Omega}_0$, which is the asymptotic variance of $\frac{1}{\sqrt{M}}\sum_{m = 1}^M\mathbf{m}_m(\boldsymbol{\theta}_0, \hat{\boldsymbol \rho})$, accounts for the uncertainty in $\boldsymbol\varepsilon_m$, the first-stage estimator $\hat{\boldsymbol{\rho}}$, and the finite number of simulated networks from the estimated network distribution.

To estimate $\mathbb{V}_0(\sqrt{M}(\hat{\boldsymbol{\theta}}-\boldsymbol{\theta}_0))$, one can replace $\mathbf{H}_0$ and $\mathbf{W}_0$ with their usual estimators. Specifically, $\mathbf{H}_0$ can be estimated by $\mathbf{H}_M(\hat{\boldsymbol{\theta}})$ and $\mathbf{W}_0$ can be estimated by $\mathbf{W}_M$. Let $\mathcal S$ be the set of simulated networks from the network distribution and the true network. To estimate $\boldsymbol{\Omega}_0$, we rely on the following decomposition.
\begingroup
\allowdisplaybreaks
\begin{align}
    \boldsymbol{\Omega}_M &= \mathbb V \left(\frac{1}{\sqrt{M}}\sum_{m = 1}^M\mathbf{m}_m(\boldsymbol{\theta}_0, \hat{\boldsymbol \rho})\right),\nonumber\\
    \boldsymbol{\Omega}_M &= \mathbb E\left\{\mathbb V \left(\frac{1}{\sqrt{M}}\sum_{m = 1}^M\mathbf{m}_m(\boldsymbol{\theta}_0, \hat{\boldsymbol \rho})| \mathbf X_m, \mathcal S\right)\right\} + \mathbb V\left\{\mathbb E \left(\frac{1}{\sqrt{M}}\sum_{m = 1}^M\mathbf{m}_m(\boldsymbol{\theta}_0, \hat{\boldsymbol \rho})| \mathbf X_m, \mathcal S\right)\right\}, \nonumber\\
    \boldsymbol{\Omega}_M &= \mathbb E\left(\frac{1}{M}\sum_{m = 1}^M\mathbf V_m\right) + \mathbb V\left(\frac{1}{\sqrt{M}}\sum_{m = 1}^M\mathcal E_m\right). \nonumber
\end{align}
\endgroup
where $\mathbf V_m = \mathbb V \left(\mathbf{m}_m(\boldsymbol{\theta}_0, \hat{\boldsymbol \rho})| \mathbf X_m, \hat{\boldsymbol{\rho}}, \kappa(\mathcal{A}_m)\right)$ and $\mathcal E_m = \mathbb E \left(\mathbf{m}_m(\boldsymbol{\theta}_0, \hat{\boldsymbol \rho})| \mathbf X_m, \hat{\boldsymbol{\rho}}, \kappa(\mathcal{A}_m)\right)$.

Note that both $\mathbf{V}_m$ and $\mathcal{E}_m$ can be easily computed and estimated. They represent the conditional variance and the conditional expectation of the moment function, given $\mathcal{S}$. 

Let $\mathbf V_M = \frac{1}{M} \sum_{m = 1}^{M} \mathbf{V}_m$ and $\mathcal{E}_M = \frac{1}{\sqrt{M}} \sum_{m = 1}^{M} \mathcal{E}_m$. It follows that:
$$\boldsymbol{\Omega}_0 = \plim  \mathbf V_M + \lim \mathbb{V} \left(\mathcal E_M\right).$$

The first term is due to the error term of the model $\boldsymbol{\varepsilon}_m$, whereas the second term reflects the uncertainty associated with the estimation of $\hat{\boldsymbol{\rho}}$ and the simulated networks.
In practice, $\plim  \mathbf V_M$ can be estimated by the average of the conditional variance of the moment function without accounting for the uncertainty in the simulated network. To estimate $\lim \mathbb{V} \left(\mathcal E_M\right)$, we repeatedly generate many $\mathcal{S}$, each associated with a new $\boldsymbol{\rho}$ simulated from the estimator of the distribution of $\hat{\boldsymbol{\rho}}$. For each $\mathcal{S}$, we compute the associated $\mathcal E_M$. Finally, the sample variance of the generated values of $\mathcal E_M$ serves as an estimator of $\lim \mathbb{V} \left(\mathcal E_M\right)$.\footnote{Our R package offers tools to compute this variance.}


==> RestatRR1/OA_application_2.tex <==
\section{Application}\label{sec:OAapplication}

\input{appendix_addhealth}

\begin{figure}[!h]
    \centering
    \caption{MCMC Simulations --  Peer Effect Model}
    \label{fig:mcmc:theta}
    \includegraphics[scale = 0.40]{graphs/simutheta.pdf}
\end{figure}

\begin{figure}[!h]
    \centering
    \caption{MCMC Simulations --  Network Formation Model}
    \label{fig:mcmc:rho}
    \includegraphics[scale = 0.55]{graphs/simurho.pdf}
\end{figure}

==> RestatRR1/addhealth.tex <==

\section{Application}\label{sec:addhealth}

In this section, we assume that the econometrician has access to network data but that the data may contain errors due to both \emph{sampling} (links coded with errors) and \emph{censoring}. To show how our method can be used to address these issues, we consider a simple example where we are interested in estimating peer effects on adolescents' academic achievements.

We use the widely used AddHealth database and show that network data errors have a first-order impact on the estimated peer effects. Specifically, we focus on a subset of schools from the Wave I ``In School'' sample that have less than 200 students (33 schools). Table \ref{tab:sumstats} in the Online Appendix \ref{sec:app_tables} presents the summary statistics.

Most papers estimating peer effects that use this particular database have taken the network structure as given. One notable exception is \cite{griffith2019namefriends}, looking at censoring: students can only report up to five male and five female friends. We also allow for censoring but show that censoring is not the most important issue with the Add Health data. To understand why, we discuss the organization of the data.

Each adolescent is assigned a unique identifier. The data includes ten variables for the ten potential friendships (maximum of five male and five female friends). These variables can contain missing values (no friendship was reported), an error code (the named friend could not be found in the database), or an identifier for the reported friends. These data are then used to generate the network's adjacency matrix $\mathbf{A}$.

Of course, error codes cannot be matched to any particular adolescent. Moreover, even in the case where the friendship variable refers to a valid identifier, the referred adolescent may still be absent from the database. A prime example is when the referred adolescent has been removed from the database by the researcher, perhaps because of other missing variables for these particular individuals. These missing links are quantitatively important as they account for roughly 45\% of the total number of links (7,830 missing for 10,163 observed links). Figure \ref{fig:misfr} displays the distribution of the number of ``unmatched named friends.''\footnote{We focus on within-school friendships; thus, nominations outside of school are not treated as ``unmatched friends.'' Note also that these data errors could be viewed as a special case of censoring \citep{griffith2019namefriends} in which researchers know exactly how many links are censored. The attenuation bias is thus expected.}
\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.6]{graphs/Missing.pdf}
    \caption{Frequencies of the number of missing links per adolescent}
    \label{fig:misfr}
\end{figure}

To use the methodology developed in sections \ref{sec:iv} and \ref{sec:genestim}, we first need to estimate a network formation model using the observed network data. In this section, we assume that links are generated using a simple logistic framework, i.e.,
$$
P(a_{ij,m}=1)=\frac{\exp\{\mathbf{w}_{ij,m}\boldsymbol{\rho}\}}{1+\exp\{\mathbf{w}_{ij,m}\boldsymbol{\rho}\}},
$$
where $\mathbf{w}_{ij,m}$ is built to capture homophily on the observed characteristics of $i$ and $j$ (see Tables \ref{tab:appendapplicationB} and \ref{tab:appendapplicationG} in the Online Appendix \ref{sec:app_tables}).

We estimate the network formation model on the set of individuals for which we observe no ``unmatched friends.'' For these students, we know for sure that their friendship data are complete. However, even under a missing at-random assumption, the estimation of $\boldsymbol{\rho}$ on this subsample is affected by a selection bias: individuals with more friends have a higher probability of being censored, or of having a friendship nomination coded with error.\footnote{Note that this is different from the random sampling discussed in our Example \ref{ex:sampled} and closer to the misclassification in Example \ref{ex:misclass}, with only false-negative type of errors.}

We control for this selection bias by weighting the log-likelihood of the network following \cite{manski1977estimation}. The details are presented in the Online Appendix \ref{sec:manski1} and Online Appendix \ref{sec:manski2}. Intuitively, individuals in our restricted sample have fewer links. Therefore, the likelihood of \( a_{i,j} \) when \( i \) is selected in our restricted sample is weighted by the inverse selection probability. When accounting for missing data due to error codes only, we estimate the selection probability for an individual \( i \) who declares \( n_i \) friends as the proportion of individuals without missing network data who declare \( n_i \) friends. 

We use the same approach when controlling for missing data due to both error codes and censoring. However, in this case, the individual's censored number of friends has to be replaced with the (unobserved) true number of friends. We estimate individuals' true number of friends using a censored Poisson regression, where the observed number of friends in the network is used as the censored dependent variable: the variable is censored when individual \( i \) nominates five male friends or five female friends.

We present the estimation results for the SGMM and Bayesian estimator. Figure \ref{fig:ahestimations} summarizes the results for the endogenous peer effect coefficient $\alpha$, whereas the full set of results is presented in the Online Appendix \ref{sec:app_tables}. The first two estimations (\emph{Obsv.Bayes} and \emph{Obsv.SGMM}) assume that the observed network is the true network for both estimators. The third and fourth estimations (\emph{Miss.Bayes} and \emph{Miss.SGMM}) account for missing data due to error codes but not for censoring. The last two estimations (\emph{TopMiss.Bayes} and \emph{TopMiss.SGMM}) account for missing data due to error codes and censoring.


\begin{figure}[h]
    \centering
    \includegraphics[scale=0.8]{graphs/PeerEffects.pdf}
    \caption{Peer effect estimate}
    \label{fig:ahestimations}

      \begin{minipage}{14cm}%
  \vspace{0.3cm}
    \footnotesize{Note: Dots represent estimated values (and posterior mean) of $\alpha$, and bars represent 95\% confidence intervals (and 95\% credibility intervals). Tables \ref{tab:appendapplicationB} and \ref{tab:appendapplicationG} in Online Appendix \ref{sec:app_tables} present the full set of estimated coefficients.}
  \end{minipage}%
\end{figure}

We first see that the SGMM estimator is less efficient than the Bayesian estimator. This should not be surprising since the Bayesian estimator uses more structure (in particularity homoscedastic, normally distributed errors). When we compare the estimations \emph{Obsv.SGMM} and \emph{Miss.SGMM}, the observed differences imply that the efficiency loss is because of the relative inefficiency of the GMM approach, and not of the missing links or specifically of our SGMM estimator.\footnote{Recall that when the network is observed, our SGMM uses the same moment conditions as, for example, those suggested by \cite{bramoulle2009identification}.}

Importantly, we see that the bias due to the assumption that the network is fully observed is quantitatively and qualitatively important. Using either estimator, the estimated endogenous peer effect using the reconstructed network is 1.5 times larger than that estimated assuming the observed network is the true network.\footnote{The difference is ``statistically significant'' for the Bayesian estimator.} Almost all of the bias is produced by the presence of error codes and not because of potential censoring.

This exercise shows that data errors are a first-order concern when using the Add Health database. Not only does the bias in the endogenous peer effect coefficient $\alpha$ have an impact on the social multiplier \citep{glaeser2003social}, but it can also affect the anticipated effect of targeted interventions, i.e., the identity of the key player \citep{ballester2006s}. We include a more detailed discussion in Appendix \ref{sec:keyplayer}.

However, we would like to stress that we do not argue that our estimated coefficients are causal, because the friendship network is likely endogenous \citep[e.g.,][]{goldsmith2013social,hsieh2018smoking,hsieh2019specification}. While previous literature has focused on the impact of network endogeneity, it has done so by assuming that the network is fully observed, despite the fact that roughly 45\% of the links are missing. Above, we showed that errors in the observed network have a first-order impact on the estimated peer effect, even when one assumes that the network is exogenous.








==> RestatRR1/bayesian_2.tex <==

\section{Bayesian  Estimator}\label{sec:genestim}

In this section, we present a likelihood-based estimator. Accordingly, greater structure must be imposed on the errors $\boldsymbol{\varepsilon}_m$. %To clarify the exposition, we will focus on the network adjacency matrix $\mathbf{A}$ rather than the interaction matrix $\mathbf{G}$. Of course, this is without any loss of generality. 
Specifically, given parametric assumptions for $\boldsymbol{\varepsilon}_m$, one can write the log-likelihood of the outcome as:
\begin{equation}\label{eq:likelihood}
\ln \mathcal{P}(\mathbf{y}|\mathbf{A},\mathbf{X},\boldsymbol{\theta})=\sum_m \ln\mathcal{P}(\mathbf{y}_m|\mathbf{A}_m,\mathbf{X}_m;\boldsymbol{\theta}) ,    
\end{equation}
where notation without the index $m$ denotes vectors and matrices at the sample level. We abuse notation by letting $\boldsymbol{\theta}=[\alpha,\boldsymbol{\beta}',\boldsymbol{\gamma}',\boldsymbol{\sigma}']'$, which now includes $\boldsymbol{\sigma}$, additional unknown parameters of the distribution of $\boldsymbol{\varepsilon}_m$. Recall that from Equation (\ref{eq:linearinmean}), we have: $\mathbf{y}_m=(\mathbf{I}_m-\alpha\mathbf{G}_m)^{-1}(c\mathbf{1}_m+\mathbf{X}_m\boldsymbol{\beta}+{\mathbf{G}_m\mathbf{X}_m}\boldsymbol{\gamma}+\boldsymbol{\varepsilon}_m)$ since $(\mathbf{I}_m-\alpha\mathbf{G}_m)^{-1}$ exists under our Assumption \ref{as:alpha}.

If the adjacency matrix $\mathbf{A}_m$ is observed, then $\boldsymbol{\theta}$ could be estimated using a simple maximum likelihood estimator \citep[as in][]{lee2010specification} or using Bayesian inference \cite[as in][]{goldsmith2013social}. See in particular the identification conditions presented in \cite{lee2004asymptotic} and \cite{lee2010specification}. Since $\mathbf{A}_m$ is not observed, but that $\mathcal{A}_m$ is observed, we focus on the following alternative likelihood:
$$
\ln \mathcal{P}(\mathbf{y}|\mathcal{A},\mathbf{X};\boldsymbol{\theta},\boldsymbol{\rho})=\sum_m \ln \sum_{\mathbf{A}_m}\mathcal{P}(\mathbf{y}_m|\mathbf{A}_m,\boldsymbol{\theta}){P}(\mathbf{A}_m|{\boldsymbol{\rho}},\mathbf{X}_m,\mathcal{A}_m).
$$
That is, we integrate the likelihood using posterior distribution obtained from the network formation model in Equation (\ref{eq:gennetfor}) after observing $\mathcal{A}_m$.\footnote{See Equation (\ref{eq:Bayes}). Note also that, conceptually, we could condition on $\kappa(\mathcal{A})$ instead of $\mathcal{A}$ as in Section \ref{sec:iv}. However, this is much less attractive from a Bayesian perspective and thus limit ourselves to this (more efficient) case.}

One particular issue with estimating $\ln \mathcal{P}(\mathbf{y}|\mathcal{A},\mathbf{X};\boldsymbol{\theta},\boldsymbol{\rho})$ is that the summations over the set of all possible network structures $\mathbf{A}_m$, for each group $m$ is not tractable. Indeed, for a group of size $N_m$, the sum is over the set of possible adjacency matrices, which contain $2^{N_m(N_m-1)}$ elements. Then, simply simulating networks from ${P}(\mathbf{A}_m|{\boldsymbol{\rho}},\mathbf{X}_m,\mathcal{A}_m)$ and taking the average likely lead to poor approximations. A classical way to address this issue is to use an EM algorithm \citep{hardy2019estimating}. Although valid, we found that the Bayesian estimator proposed in this section is less restrictive and numerically outperforms its classical counterpart. The Bayesian treatment also has the advantage of being valid in finite samples, allowing for a richer set of network formation models and partially observed network information $\mathcal{A}$.\footnote{For example, models estimated using Aggregated Relational Data, see the Online Appendix \ref{sec:ardsetting}.}

For concreteness, we will assume that $\boldsymbol{\varepsilon}_m\sim\mathcal{N}(0,\sigma^2\mathbf{I}_m)$ for all $m$; however, it should be noted that our approach is valid for several alternative assumptions as long as it yields a computationally tractable likelihood. For each group $m$, and recalling that $\mathbf{G}_m=f(\mathbf{A}_m)$, we have:
\begin{eqnarray*}
\ln \mathcal{P}(\mathbf{y}_m|\mathbf{A}_m,\boldsymbol{\theta})&=&-N_m\ln(\sigma)+\ln|\mathbf{I}_m-\alpha\mathbf{G}_m|-\frac{N_m}{2}\ln(\pi)\\&&-\frac{1}{2\sigma^2}[(\mathbf{I}_m-\alpha\mathbf{G}_m)\mathbf{y}_m-c\mathbf{1}_m-\mathbf{X}_m\boldsymbol{\beta}-\mathbf{G}_m\mathbf{X}_m\boldsymbol{\gamma}]'\cdot\\ &&[(\mathbf{I}_m-\alpha\mathbf{G}_m)\mathbf{y}_m-c\mathbf{1}_m-\mathbf{X}_m\boldsymbol{\beta}-\mathbf{G}_m\mathbf{X}_m\boldsymbol{\gamma}].
\end{eqnarray*}
Because $\mathbf{A}_m$ is not observed, we follow \cite{tanner1987calculation}, and we use data augmentation to evaluate the posterior distribution of $\boldsymbol{\theta}$. That is, instead of focusing on the posterior distribution of $\boldsymbol{\theta}$ (i.e., $P(\boldsymbol{\theta}|\mathbf{y},\mathbf{A},\mathbf{X})$) in the case in which the network was observed, we focus instead on the posterior distribution $P(\boldsymbol{\theta},\mathbf{A}|\mathbf{y},\mathcal{A},\mathbf{X})$, treating $\mathbf{A}$ as another set of unknown parameters.

Since the number of parameters to be estimated is larger than the number of observations,\footnote{Each group contains $N_m$ observations while the dimension of $\mathbf{A}_m$ is $N_m(N_m-1)$.} the identification of the model rests on the a priori information on $\mathbf{A}$. A sensible prior for $\mathbf{A}$ is the consistent estimator of its distribution, i.e., $\Pi_m\hat{P}(\mathbf{A}_m|\hat{\boldsymbol{\rho}},\mathbf{X}_m,\mathcal{A}_m)$. Let $\pi(\boldsymbol{\rho}|\mathbf{X},\mathcal{A})$ be the prior density on $\boldsymbol{\rho}$. How to obtain $\pi(\boldsymbol{\rho}|\mathbf{X},\mathcal{A})$, depending on whether $\hat{\boldsymbol{\rho}}$ is obtained using a Bayesian or classical setting, is discussed in Examples \ref{ex:prior_distr} and \ref{ex:prior_post} of the Online Appendix \ref{sec:appendix_prior}. Given $\pi(\boldsymbol{\rho}|\mathbf{X},\mathcal{A})$, it is possible to obtain draws from the posterior distribution $P(\boldsymbol{\theta},\mathbf{A},\boldsymbol{\rho}|\mathbf{y},\mathcal{A})$ using the following Metropolis-Hastings MCMC:\footnote{As customary, for the rest of this section, we omit the dependence on $\mathbf{X}$ to lighten the notation. The notation with the index $t-1$ in this section refers to the $(t-1)$-th iteration of the MCMC, not the $(t-1)$-th group. Specifically, $\mathbf{A}_{t-1}$ denotes the adjacency matrix at the sample level in iteration $t-1$. Since the MCMC is a Metropolis-Hastings, the detailed balance and ergodicity conditions hold so the MCMC converges to $P(\boldsymbol{\theta},\mathbf{A},\boldsymbol{\rho}|\mathbf{y},\mathcal{A})$. See \cite{cameron2005microeconometrics}, Section 13.5.4 for more details.}

% One may wish, however, to also use the information regarding the sampling uncertainty around this first stage. This is very similar to the inference for two-step estimators in a classical setting (e.g. for our SGMM estimator); estimation uncertainty in the first stage must be accounted for to provide valid inference in the second stage (see Section \ref{sec:iv}). To do this, we must also estimate $\boldsymbol{\rho}$ jointly with $\boldsymbol{\theta}$ (and $\mathbf{A}$).


\begin{algorithm}\label{algo:mcmc} The MCMC goes as follows for $t=1,...,T$, starting from any $\mathbf{A}_0,\boldsymbol{\theta}_0$, and $\boldsymbol{\rho}_0$.
\begin{enumerate}
    \item Draw $\boldsymbol{\rho}^*$ from the proposal distribution $q_\rho(\boldsymbol{\rho}^*|\boldsymbol{\rho}_{t-1})$ and accept $\boldsymbol{\rho}^*$ with probability
    $$
    \min\left\lbrace 1,\frac{P(\mathbf{A}_{t-1}|\boldsymbol{\rho}^*,\mathcal{A})q_\rho(\boldsymbol{\rho}_{t-1}|\boldsymbol{\rho}^*)\pi(\boldsymbol{\rho}^*|\mathcal{A})}
    {P(\mathbf{A}_{t-1}|\boldsymbol{\rho}_{t-1},\mathcal{A})q_\rho(\boldsymbol{\rho}^*|\boldsymbol{\rho}_{t-1})\pi(\boldsymbol{\rho}_{t-1}|\mathcal{A})} \right\rbrace.
    $$
    \item Propose $\mathbf{A}^*$ from the proposal distribution $q_A(\mathbf{A}^*|\mathbf{A}_{t-1})$ and accept $\mathbf{A}^*$ with probability
    $$
    \min\left\lbrace 1,\frac{\mathcal{P}(\mathbf{y}|\boldsymbol{\theta}_{t-1},\mathbf{A}^*)q_A(\mathbf{A}_{t-1}|\mathbf{A}^*)P(\mathbf{A}^*|{\boldsymbol{\rho}_{t-1}},\mathcal{A})}{\mathcal{P}(\mathbf{y}|\boldsymbol{\theta}_{t-1},\mathbf{A}_{t-1})q_A(\mathbf{A}^*|\mathbf{A}_{t-1})P(\mathbf{A}_{t-1}|{\boldsymbol{\rho}_{t-1}},\mathcal{A})} \right\rbrace.
    $$
    \item Draw $\alpha^*$ from the proposal $q_\alpha(\cdot|\alpha_{t-1})$ and accept $\alpha^*$ with probability
    $$
    \min\left\lbrace 1,\frac{\mathcal{P}(\mathbf{y}|\mathbf{A}_{t};\boldsymbol{\beta}_{t-1},\boldsymbol{\gamma}_{t-1},\alpha^*)q_\alpha(\alpha_{t - 1}|\alpha^*)\pi(\alpha^*)}{\mathcal{P}(\mathbf{y}|\mathbf{A}_{t};\boldsymbol{\theta}_{t-1})q_\alpha(\alpha^*|\alpha_{t-1})\pi(\alpha_{t-1})}\right\rbrace.
    $$
    \item Draw $[\boldsymbol{\beta,\gamma},\sigma]$ from their posterior conditional distributions (see Online Appendix \ref{sec:OA_bayesian}).
\end{enumerate}
\end{algorithm}

Step 1 allows to refine the estimation of $\boldsymbol{\rho}$. Indeed, in the first stage, $\boldsymbol{\rho}$ is inferred using the information provided by $\mathcal{A}$. In Step 1, however, $\boldsymbol{\rho}$ is updated conditional on $\mathcal{A}$ \emph{and} $\mathbf{A}_{t-1}$. This provides additional information not available in the first stage since $\mathbf{A}_{t-1}$ uses information provided by the likelihood function (\ref{eq:likelihood}).%\footnote{This is similar to, in a classical setting, the difference between using a sequential estimator, or a joint estimator. In a sequential estimator, the estimation in the first stage does not use the information provided by the objective function of the second stage leading to an efficiency loss.}


%Step 1 shows that the flexibility of the network formation model comes at a cost. For example, \cite{graham2017econometric} and \cite{breza2017using} propose network formation models for which the number of parameters is $O(N_r)$. In turn, this large number of parameters increases the computational cost of Step 1.




Steps 3 and 4 are standard and detailed distributions can be found in the Online Appendix \ref{sec:OA_bayesian}. Step 2, however, requires some discussion. Indeed, the idea is the following: given the prior information $P(\textbf{A}|\boldsymbol{\rho}_{t-1},\mathcal{A})$, one must be able to draw samples from the posterior distribution of $\mathbf{A}$, given $\mathbf{y}$. This is not a trivial task.

In particular, there is no general rule for selecting the network proposal distribution $q_A(\cdot\vert\cdot)$. A natural candidate is a Gibbs sampling algorithm for each link, i.e., change only one link $ij$ at every step $t$ and propose $a_{ij}$ according to its marginal distribution, i.e., $a_{ij}\sim P(\cdot|\mathbf{A}_{-ij},\mathbf{y},\mathcal{A})$, where $\mathbf{A}_{-ij} = \{a_{kl}; k \ne i, l \ne j\}$. In this case, the proposal is always accepted.
%$$
%a_{ij}\sim P(\cdot|\mathbf{A}_{-ij},\mathbf{y},\mathcal{A})=\frac{\mathcal{P}(\mathbf{y}|a_{ij},\mathbf{A}_{-ij})P(a_{ij}|\mathbf{A}_{-ij};\tilde{\boldsymbol{\rho}},\mathcal{A})}{\mathcal{P}(\mathbf{y}|1,\mathbf{A}_{-ij})P(a_{ij}=1|\mathbf{A}_{-ij};\tilde{\boldsymbol{\rho}},\mathcal{A})+\mathcal{P}(\mathbf{y}|0,\mathbf{A}_{-ij})P(a_{ij}=0|\mathbf{A}_{-ij};\tilde{\boldsymbol{\rho}},\mathcal{A})},
%$$

However, it has been argued that Gibbs sampling could lead to slow convergence \citep[e.g.,][]{snijders2002markov,chatterjee2013estimating}, especially when the network is \emph{sparse} or exhibits a high level of \emph{clustering}. For example, \cite{mele2017} and \cite{bhamidi2008mixing} propose different blocking techniques meant to improve convergence.

Here, however, achieving Step 2 involves an additional computational issue because evaluating the likelihood ratio in Step 1 requires comparing the determinants $|\mathbf{I}-\alpha f(\mathbf{A}^*)|$ for each proposed $\mathbf{A}^*$, which is computationally intensive. %In particular, taking $\mathbf{G}^*=f(\mathbf{A}^*)$ to be a row-normalization of $\mathbf{A}^*$, altering a single element of $\mathbf{A}^*$ results in a change in the entire corresponding row of $\mathbf{G}^*$. Still, comparing the determinant of two matrices that differ only in a single row is relatively fast. Moreover, when $\mathbf{G}=\mathbf{A}$, \cite{hsieh2019structural} propose a blocking technique that facilitates the computation of the determinant.

%In any case, note that the computational complexity of Step 2 depends strongly on $P(\textbf{A}|\boldsymbol{\rho}_{t-1},\mathcal{A})$, which is a function of the assumed network formation model (\ref{eq:gennetfor}) and the observed information about the network structure $\mathcal{A}$. For censored network data, for example, most of the network structure is observed (see Example \ref{ex:censored}). This implies that $P(a_{ij}|\boldsymbol{\rho}_{t-1},\mathcal{A})\in\{0,1\}$ for most pairs $ij$. As such, few entries of $\mathbf{A}$ must be updated in Step 2. The opposite is true for ARD (see Example \ref{ex:ard}) for which all entries of $\mathbf{A}$ must be updated.

Then, the appropriate blocking technique depends strongly on $P(\textbf{A}|\boldsymbol{\rho}_{t-1},\mathcal{A})$ and the assumed distribution for $\boldsymbol{\varepsilon}$. For the simulations and estimations presented in this paper, we use the Gibbs sampling algorithm for each link, adapting the strategy proposed by \cite{hsieh2019structural} to our setting (see Proposition \ref{prop:det} in the Online Appendix \ref{sec:networksampling}). This can be viewed as a \emph{worst-case} scenario. Nonetheless, the Gibbs sampler performs reasonably well in practice however, we encourage researchers to try other updating schemes if Gibbs sampling performs poorly in their specific contexts. In particular, we present a blocking technique in the Online Appendix \ref{sec:OA_bayesian} that is also implemented in our R package \texttt{PartialNetwork}.\footnote{The complexity of Step 2 is not limited to our Bayesian approach. Classical estimators, such as GMM estimators, face a similar challenge in requiring the integration over the entire set of networks. The strategy used here is to rely on a Metropolis-Hastings algorithm, a strategy that has also been successfully implemented in the related literature on ERGMs \cite[e.g.,][]{snijders2002markov,mele2017,mele2020does,badev2018nash,hsieh2019structural}.}

Finally, note that for simple network formation models, it is possible to jointly estimate $\boldsymbol{\rho}$ and $\boldsymbol{\theta}$ within the same MCMC instead of using the two-step procedure described above. In this case, Step 1 can simply be replaced by:
\begin{enumerate}
    \item[1'.]  Draw $\boldsymbol{\rho}^*$ from the proposal distribution $q_\rho(\boldsymbol{\rho}^*|\boldsymbol{\rho}_{t-1})$ and accept $\boldsymbol{\rho}^*$ with probability
    $$
    \min\left\lbrace 1,\frac{P(\mathbf{A}_{t-1}|\boldsymbol{\rho}^*,\mathcal{A})P(\mathcal{A}|\boldsymbol{\rho}^*)q_\rho(\boldsymbol{\rho}_{t-1}|\boldsymbol{\rho}^*)\pi(\boldsymbol{\rho}^*)}
    {P(\mathbf{A}_{t-1}|\boldsymbol{\rho}_{t-1},\mathcal{A})P(\mathcal{A}|\boldsymbol{\rho}_{t-1})q_\rho(\boldsymbol{\rho}^*|\boldsymbol{\rho}_{t-1})\pi(\boldsymbol{\rho}_{t-1})} \right\rbrace.
    $$
\end{enumerate}
Here, $P(\mathcal{A}|\boldsymbol{\rho}^*)$ is the likelihood of the network information $\mathcal{A}$ assuming the network formation model in (\ref{eq:gennetfor}). Note that $\pi(\boldsymbol{\rho})$, the prior density on $\boldsymbol{\rho}$, no longer depends on $\mathcal{A}$ and can be chosen arbitrarily (e.g., uniform).

%This approach would work well for simple models, such as the ones discussed in Examples \ref{ex:sampled} and \ref{ex:misclass}. It is impractical, however, for more involved models, such as that proposed by \cite{breza2017using}.


==> RestatRR1/discussion.tex <==


\section{Conclusion}\label{sec:conclusion}
In this paper, we propose two estimators for which peer effects can be estimated without observing the entire network structure. We find, perhaps surprisingly, that even very partial information on network structure is sufficient. By specifying a network formation model, researchers can probabilistically reconstruct the true network and base the estimation of peer effects on this reconstructed network. Importantly, we provide computationally tractable and flexible estimators to do so, all of which are available in our R package \texttt{PartialNetwork}. We apply our methodology to the widely used Add Health data and find that missing links due to noise in the data have first-order effects on the estimated peer effect coefficient.


==> RestatRR1/intro_2.tex <==
\section{Introduction}
There is a large and growing literature on the impact of peer effects in social networks.\footnote{For recent reviews, see \cite{bramoulle2019peer}, and \cite{de2015econometrics}.} However, since eliciting network data is expensive \citep{breza2017using}, relatively few data sets contain comprehensive network information, and existing ones are prone to data errors. Despite some recent contributions, existing methodologies for the estimation of peer effects with incomplete or erroneous network data either focus on a specific kind of sampling or error, or they are highly computationally demanding.

In this paper, we propose a unifying framework that allows for the estimation of peer effects under the widely used linear-in-means model (e.g. \cite{manski1993identification,bramoulle2009identification}) when the researcher does not observe the entire network structure. Our methodology is computationally attractive and sufficiently flexible to cover cases where, for example, network data are sampled \citep{chandrasekhar2011econometrics,liu2013estimation,lewbel2019social}, censored \citep{griffith2019namefriends}, or misclassified \citep{hardy2019estimating}. Our central assumption is that the researcher is able to estimate a network formation model using some partial information about the network structure. Leveraging recent contributions on the estimation of network formation models, we show that this assumption is sufficient to identify and estimate peer effects.

We propose two estimators. First, we present a computationally attractive estimator based on a simulated generalized method of moments (SGMM). The moments are built using draws from the (estimated) network formation model. We study the finite sample properties of our SGMM estimator via Monte Carlo simulations. We show that the estimator performs very well, even when a large fraction of the links are missing or misclassified. Second, we present a flexible likelihood-based (Bayesian) estimator allowing us to exploit the entire structure of the data-generating process. The Bayesian approach is flexible as it allows to cover cases for which the asymptotic framework of our SGMM fails. Although the computational cost is higher than that of the SGMM, we exploit recent computational advances in the literature, e.g. \cite{mele2017,hsieh2019structural}, and show that the estimator can be successfully implemented on common-sized data sets. In particular, we apply our estimator to study peer effects on academic achievement using the widely used Add Health database. We find that data errors have a first-order downward bias on the estimated endogenous effect.

Our SGMM estimator is built as a bias-corrected version of the instrumental strategy proposed by \cite{bramoulle2009identification}. Using a network formation model, we obtain a consistent estimator of the distribution of the true network. We then use this estimated distribution to obtain different draws from the distribution of the network. We show that our moment conditions are asymptotically valid and that the estimator is consistent and asymptotically normal, even with a finite number of draws from the estimated distribution of the network. This property significantly reduces the computational cost of the method compared to methods that rely on integrating the moment conditions \citep[e.g.,][]{chandrasekhar2011econometrics}.

Importantly, our SGMM strategy requires only the (partial) observation of a \emph{single} cross-section, unlike, for example, the approach of \cite{zhang2020spillovers}. The presence of this feature is because of two main properties of the model. First, we can consistently estimate the distribution of the mismeasured variable (i.e., the network) using a single (partial) observation of the variable. Second, in the absence of measurement error, valid instruments for the endogenous peer variable are available \citep{bramoulle2009identification}.

%We explore the finite sample properties of our instrumental variable estimator using Monte Carlo simulations. We consider the case in which a large fraction of the links are unobserved. When there are no unobserved group-level fixed effects, the loss in precision due to missing links is very small, even a very large fraction of links are missing (up to 75\%). With group-level unobservable fixed effects, the loss in precision is larger, but the estimator still performs very well when up to 25\%-50\% of the links are missing.

Our Bayesian estimator is based on the likelihood function and therefore uses more information about the structure of the model, leading to more precise estimates. In the context of this estimator, the estimated distribution for the network acts as a prior distribution, and the inferred network structure is updated through a Markov chain Monte Carlo (MCMC) algorithm. Our approach relies on data augmentation \citep{tanner1987calculation}, which treats the network as an additional set of parameters to be estimated. In particular, our MCMC builds on recent developments from the empirical literature on network formation \citep[e.g.,][]{mele2017,hsieh2019structural}. We show that the computational cost of our estimator is reasonable and that it can easily be applied to standard data sets.

We study the impact of errors in adolescents' friendship network data for the estimation of peer effects in education \citep{calvo2009peer}. We show that the widely used Add Health database features many missing links---around 45\% of the within-school friendship nominations are coded with error---and that these data errors strongly bias the estimated peer effects. Specifically, we estimate a model of peer effects on students' academic achievement. We probabilistically reconstruct the missing links, accounting for the potential censoring, and we obtain a consistent estimator of peer effects using both our estimators. The bias due to data errors is qualitatively important, even assuming that the network is exogenous. Our estimated endogenous peer effect coefficient is 1.5 times larger than that obtained by assuming the data contains no errors.

This paper contributes to the recent literature on the estimation of peer effects when the network is either not entirely observed or observed with noise. In particular, our framework is valid when network data are either sampled, censored, or misclassified.\footnote{For related literature that studies the estimation of peer effects when researchers have no network data, see \cite{manresa2016estimating,de2018recovering,lewbel2019social}.} We unify these strands in the literature and provide a flexible and computationally tractable framework for estimating peer effects with incomplete or erroneous network data.

\emph{Sampled networks and censoring:} \cite{chandrasekhar2011econometrics} show that models estimated using sampled networks are generally biased. They propose an analytical correction as well as a two-step general method of moment (GMM) estimator. \cite{liu2013estimation} shows that when the interaction matrix is not row-normalized, instrumental variable estimators based on an out-degree distribution are valid, even with sampled networks. \cite{hsieh2018non} focus on a regression model that depends on global network statistics. They propose analytical corrections to account for nonrandom sampling of the network \citep[see also][]{chen2013impact}. \cite{thirkettleidentification} also focuses on global network statistics, assuming that the researcher only observes a random sample of links. Using a structural network formation model, he derives bounds on the identified set for both the network formation model and the network statistic of interest.  \cite{lewbel2021social} develop a two-stage least squares estimator for the linear-in-means model when some links are potentially misclassified. They propose valid instruments under some restrictions on the observed and true interactions matrices, or when researchers observe at least two samples of the same true network. Finally, \cite{zhang2020spillovers} studies program evaluation in a context in which networks are sampled locally and where some links might be unobserved. Assuming that the researcher has access to two measurements of the network for each sampled unit, she presents a nonparametric estimator of the treatment and spillover effects.

Relatedly, \cite{griffith2019namefriends} explores the impact of imposing an upper bound to the number of links when eliciting network data, e.g., ``Name your five best friends.'' He presents a bias-correction method and explores the impact of censoring using two empirical applications. He finds that censoring underestimates peer effects. \cite{griffith2023} present a characterization of the analytic bias of censoring for the reduced-form parameters in the linear-in-means and linear-in-sums models under an Expectational Equivalence assumption.

We contribute to this literature by proposing two simple and flexible estimators for the estimation of peer effects based on a linear-in-means model. Our estimators do not require many observations of the sampled network. Similar to \cite{griffith2019namefriends} and \cite{griffith2023}, we find---using the Add Health database---that sampling leads to an underestimation of peer effects, although we find that censoring has a negligible impact, in the context of peer effects, on academic achievement.

Our SGMM estimator does not suffer from the computational cost resulting from integrating the moment conditions \citep[as in][]{chandrasekhar2011econometrics} and can produce precise estimates with as little as three network simulations. While our Bayesian estimator is more computationally demanding, we exploit recent developments from the empirical literature on network formation \cite[e.g.,][]{mele2017,hsieh2019structural} and show that it is computationally tractable. Moreover, the Bayesian estimator is valid in finite samples, which allows in particular to cover cases not covered by the asymptotic framework on which our SGMM relies.

\emph{Misclassification:} \cite{hardy2019estimating} look at the estimation of (discrete) treatment effects when the network is observed noisily. Specifically, they assume that observed links are affected by iid errors and present an expectation maximization (EM) algorithm that allows for a consistent estimator of the treatment effect. \cite{lewbel2023social} show that when the expected number of missing links grows at a rate strictly lower than the number of sampled individuals $n$, the 2SLS estimator in \cite{bramoulle2009identification} is consistent.\footnote{When the growth rate is strictly smaller than $\sqrt{n}$, the inference is also valid.}

Our model allows for the misclassification of all links with positive probability, and we do not impose restrictions on the rate of misclassification. As in \cite{hardy2019estimating}, we use a network formation model to estimate the probability of false positives and false negatives. However, our two-stage strategy---estimating the network formation model and then the peer effect model---allows for greater flexibility. In particular, our network formation model is allowed to flexibly depend on covariates. This is empirically important, as networks typically feature homophily on observed characteristics \cite[e.g.,][]{currarini2010identifying,bramoulle2012homophily}.\footnote{Formally, \cite{hardy2019estimating} do not require the specification of distribution of the network, but only the distribution of the degree sequence, which is assumed not to depend on covariates.}
\begin{comment}
\emph{Aggregate relational data:} \cite{breza2017using} propose to estimate network effects using aggregate relation data (ARD). These are obtained from such survey questions as, ``How many of your friends have trait X?'' They present a network formation model that can be estimated using only ARD. They show the validity of their methodology using two empirical applications in which the outcome of interest depends on the summary statistics of the network. \cite{alidaee2020recovering} present an alternative estimator allowing to recover nonparametrically the linking probability through ARD. Using a low-rank assumption, they present a simple penalized regression.

We show that these recent methodologies can also be applied to the study of peer effects using a linear-in-means model, which significantly expands the scope of the potential applications of these approaches. %In particular, we study the finite sample performance of our SGMM estimator using Monte Carlo simulations and show that we can successfully recover the simulated parameters when combined with the network formation estimators proposed by \cite{breza2017using} and  \cite{alidaee2020recovering}.

A main contribution of this paper is that our estimators can be applied to each of the previously mentioned data issues or to their combination. Our two-step approach---first estimating the network formation and then the peer effects---is flexible and computationally attractive. To reduce the implementation costs, we also present an easy-to-use R package---named \texttt{PartialNetwork}---for applying our estimators. The package allows replicating all simulations and empirical applications in the paper, including the estimator proposed by \cite{breza2017using}. The package is available online at: \url{https://github.com/ahoundetoungan/PartialNetwork}. Additional implementation examples are provided in the Vignette accompanying the package. For example, we show that the implementation of our Bayesian estimator, combined with the estimator for ARD proposed by \cite{breza2017using}, is straightforward and computationally tractable.
\end{comment}

The remainder of the paper is organized as follows. In Section \ref{sec:linearinmean}, we present the econometric model as well as the main assumptions. In Section \ref{sec:iv}, we present our SGMM estimator and study its performance via Monte Carlo simulations. In Section \ref{sec:genestim}, we present our likelihood-based estimation strategy. In Section \ref{sec:addhealth}, we present our application to peer effects on academic achievement. Section \ref{sec:conclusion} concludes the paper.% with a discussion of the main results, limits, and challenges for future research.


==> RestatRR1/iv_2.tex <==
\section{Simulated Generalized Method of Moment Estimators}\label{sec:iv}

In this section, we present an estimator based on a Simulated Generalized Method of Moments (SGMM). Our SGMM is constructed as a de-biased simulated version of the widely used linear GMM in \cite{bramoulle2009identification}. 

Before presenting the estimator, we start with an informal discussion of how the moment function is built. A formal treatment is presented in Appendix \ref{sec:appendix_proofs}. Recall first the linear-in-means model presented in the previous section:
\begin{eqnarray*}
\mathbf{y}_m
&=&\mathbf{V}_m\tilde{\boldsymbol{\theta}} + \alpha\mathbf{G}_m\mathbf{y}_m + \boldsymbol{\varepsilon}_m,
\end{eqnarray*}
where we defined $\mathbf{V}_m=[\mathbf{1}_m,\mathbf{X}_m,\mathbf{G}_m\mathbf{X}_m]$, and $\tilde{\boldsymbol{\theta}} =[c,\boldsymbol{\beta}',\boldsymbol{\gamma}']'$. A valid set of instruments for the endogenous variable $\mathbf{G}_m\mathbf{y}_m$ is: $\mathbf{Z}_m=[\mathbf{1}_m,\mathbf{X}_m,\mathbf{G}_m\mathbf{X}_m,\mathbf{G}_m^2\mathbf{X}_m,\mathbf{G}_m^3\mathbf{X}_m,...]$. \citep{bramoulle2009identification} This defines the following moment function: $\mathbf{m}(\boldsymbol{\theta})=\mathbf{Z}_m'\boldsymbol{\varepsilon}_m$, where $\boldsymbol{\theta}=[\alpha,c,\boldsymbol{\beta}',\boldsymbol{\gamma}']'$, and one can easily show that $\mathbb{E}[\mathbf{m}(\boldsymbol{\theta})|\mathbf{A}_m,\mathbf{X}_m]=\mathbf{0}$ for $\boldsymbol{\theta}=\boldsymbol{\theta}_0$ and that $\boldsymbol{\theta}_0$ is identified under the usual rank condition.\footnote{As standard, we use the subscript $0$ to denote the true value of the parameter. See e.g., \cite{bramoulle2009identification} and \cite{lee2010specification} for identification results when $\mathbf{G}_m$ is observed.}

Unfortunately, this approach is not feasible when $\mathbf{G}_m=f(\mathbf{A}_m)$ is not observed. As discussed, our strategy is to develop a simulated version of this simple linear GMM estimator. Indeed, equipped with a consistent estimator of the distribution of $\mathbf{A}_m$ (see Definition \ref{def:estimator}), we can draw network structures from that same distribution.

To simplify the notation, we denote $\dot{\mathbf{G}}_m=f(\dot{\mathbf{A}}_m)$, $\ddot{\mathbf{G}}_m=f(\ddot{\mathbf{A}}_m)$, and $\dddot{\mathbf{G}}_m=f(\dddot{\mathbf{A}}_m)$ as independent draws from the distribution $\hat{P}(\mathbf{A}_m|\hat{\boldsymbol{\rho}},\mathbf{X}_m,\kappa(\mathcal{A}_m))$. We will also note $\dot{\mathbf{Z}}_m$ and $\dot{\mathbf{V}}_m$, the versions of ${\mathbf{Z}}_m$ and ${\mathbf{V}}_m$ in which $\mathbf{G}_m$ is replaced with $\dot{\mathbf{G}}_m$ (and similarly for $\ddot{\mathbf{G}}_m$ and $\dddot{\mathbf{G}}_m$).

Now, suppose that we replace the unobserved $\mathbf{G}_m$ with $\dot{\mathbf{G}}_m$ everywhere in the expression $\mathbf{Z}_m'\boldsymbol{\varepsilon}_m$. This would lead to a moment function with an expectation given by:
\begin{eqnarray*}
\mathbb{E}(\dot{\mathbf{m}}(\boldsymbol{\theta})|\mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m)&=&\mathbb{E}(\dot{\mathbf{Z}}'_m[(\mathbf I_m - \alpha \dot{\mathbf G}_m )\mathbf{y}_m - \dot{\mathbf{V}}\tilde{\boldsymbol{\theta}}]| \mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m)\\
&=&\mathbb{E}(\dot{\mathbf{Z}}'_m\dot{\boldsymbol{\varepsilon}}|\mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m),
\end{eqnarray*}
where $\mathbf I_m$ is the identity matrix of dimension $N_m$. The expectation of the moment function does not generally equal $\mathbf{0}$ when $\boldsymbol{\theta}=\boldsymbol{\theta}_0$, even asymptotically.\footnote{Recall from Definition \ref{def:estimator} that $\dot{\mathbf{G}}_m$ is drawn from the same distribution as $\mathbf{G}_m$ only as $M\rightarrow\infty$.}

There are two issues with the previous moment function. First, the instruments and the explanatory variables are generated using the same network draw $\dot{\mathbf{G}}_m$, which introduces a correlation between the $\dot{\mathbf{Z}}_m$ and $\dot{\boldsymbol{\varepsilon}}$, conditionally on $\mathbf{A}_m$,  $\mathcal{A}_m$, and $\mathbf X_m$. This can easily be resolved by simply using different draws to construct the instruments and the explanatory variables. This leads to:
\begin{eqnarray*}
\mathbb{E}\left(\ddot{\mathbf{m}}(\boldsymbol{\theta})|\mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m\right)&=&\mathbb{E}(\dot{\mathbf{Z}}'_m\ddot{\boldsymbol{\varepsilon}}|\mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m)\\&=&\mathbb{E}(\dot{\mathbf{Z}}'_m|\mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m)\mathbb{E}(\ddot{\boldsymbol{\varepsilon}}|\mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m),
\end{eqnarray*}
where $\ddot{\boldsymbol{\varepsilon}}_m=(\mathbf I_m - \alpha \ddot{\mathbf G}_m )\mathbf{y}_m - \ddot{\mathbf{V}}\tilde{\boldsymbol{\theta}}$. 
However, in general, $\mathbb{E}(\ddot{\boldsymbol{\varepsilon}}|\mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m)\neq\mathbf{0}$ at $\boldsymbol{\theta}=\boldsymbol{\theta}_0$. 
To see why, note that we can rewrite:
$$
\ddot{\boldsymbol{\varepsilon}}_m=(\mathbf I_m - \alpha \ddot{\mathbf G}_m )(\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}[\mathbf{V}_m\tilde{\boldsymbol{\theta}}_0+\boldsymbol{\varepsilon}_m]-\ddot{\mathbf{V}}_m\tilde{\boldsymbol{\theta}}.
$$
While we can show that $\mathbb{E}(\mathbf I_m - \alpha \ddot{\mathbf G}_m )(\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}{\boldsymbol{\varepsilon}}|\mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m)=\mathbf{0}$ from the law of iterated expectations and Assumption \ref{as:exonet}, we have:
\begin{eqnarray*}
\mathbb{E}[(\mathbf I_m - \alpha \ddot{\mathbf G}_m )(\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}\mathbf{V}_m\tilde{\boldsymbol{\theta}}_0 |\mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m]-\mathbb{E}[\ddot{\mathbf{V}}_m\tilde{\boldsymbol{\theta}}|\mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m]\neq 0,
\end{eqnarray*}
when $\boldsymbol{\theta}=\boldsymbol{\theta}_0$, even asymptotically. This is due to the approximation error in using $\ddot{\mathbf{G}}_m$ instead of $\mathbf{G}_m$. This approximation error does not vanish asymptotically. In particular, because groups have bounded, the product $(\mathbf I_m - \alpha_0 \ddot{\mathbf G}_m )(\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}$ does not converge to the identity matrix. If it did, consistency would follow.

%This implies that \emph{if} $\mathbb{E}(\ddot{\boldsymbol{\varepsilon}}|\mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m)$ did converge to $\mathbf{0}$ at $\boldsymbol{\theta}=\boldsymbol{\theta}_0$, a simple simulated version of the linear GMM proposed by \cite{bramoulle2009identification}, in which different simulated network structures are used to construct the instruments and the explanatory variables, could be used. Since the resulting simulated GMM would also be linear, identification would also follow form the usual rank conditions. Unfortunately, this estimator is not consistent.\footnote{In Proposition \ref{prop:bias_nocontext} of the Online Appendix \ref{sec:appendix_otherresults}, we derive the explicit asymptotic bias for this estimator and show that it is minimized when the weighting matrix for the GMM is the identity matrix.}

Our SGMM presented below offers a bias-corrected version of this estimator. Specifically, consider the following (feasible) approximation of the bias of $\mathbb{E}(\ddot{\boldsymbol{\varepsilon}}|\mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m)$:
$$
\boldsymbol{\delta}_m=(\mathbf I_m - \alpha \ddot{\mathbf G}_m )(\mathbf I_m - \alpha \dddot{\mathbf G}_m )^{-1}\dddot{\mathbf{V}}_m\tilde{\boldsymbol{\theta}}-\ddot{\mathbf{V}}\tilde{\boldsymbol{\theta}}.
$$
We obtain $\ddot{\boldsymbol{\varepsilon}}_m-\boldsymbol{\delta}_m=(\mathbf I_m - \alpha \ddot{\mathbf G}_m )\mathbf{y}_m-(\mathbf I_m - \alpha \ddot{\mathbf G}_m )(\mathbf I_m - \alpha \dddot{\mathbf G}_m )^{-1}\dddot{\mathbf{V}}_m\tilde{\boldsymbol{\theta}}$, and we can show that $\mathbb{E}(\ddot{\boldsymbol{\varepsilon}}_m-\boldsymbol{\delta}_m|\mathbf{A}_m,\mathcal{A}_m,\mathbf{X}_m)=\mathbf{0}$ for $\boldsymbol{\theta}=\boldsymbol{\theta}_0$ as $M\rightarrow\infty$.\footnote{In the bias approximation expression, we use a third independent draw, $\dddot{\mathbf{G}}_m$, as an approximation of $\mathbf{G}_m$ to ensure that it remains independent of $\dot{\mathbf{G}}_m$ and $\ddot{\mathbf{G}}_m$, just as $\mathbf{G}_m$ is.}

The above discussion thus leads to the definition of our SGMM. Let $\lbrace \dot{\mathbf{G}}_m^{(r)}\rbrace_{r=1}^R$, $\lbrace \ddot{\mathbf{G}}^{(s)}_m\rbrace_{s=1}^S$, and $\lbrace \dddot{\mathbf{G}}^{(t)}_m\rbrace_{t=1}^T$ be sequences of independent draws from estimator of the network formation process (see Definition \ref{def:estimator}), we have the following.


\begin{theorem}[SGMM]\label{prop:non_observed} Suppose that Assumptions \ref{as:manymarkets}--\ref{as:partial} and regularity conditions \ref{as:regularity}--\ref{as:Wm} and \ref{as:reg_variance} hold (see Appendix \ref{sec:appendix_proofs}). Suppose also that the identification condition \ref{as:identification} holds (see Appendix \ref{sec:appendix_proofs}). Let $\dot{\mathbf{Z}}^{(r)}_m=[\mathbf{1}_m,\mathbf{X}_m,\dot{\mathbf{G}}^{(r)}_m\mathbf{X}_m,(\dot{\mathbf{G}}^{(r)}_m)^2\mathbf{X}_m,(\dot{\mathbf{G}}_m^{(r)})^3\mathbf{X}_m,...]$ and $\dddot{\mathbf{V}}_m^{(t)}=[\mathbf{1}_m,\mathbf{X}_m,\dddot{\mathbf{G}}_m^{(t)}\mathbf{X}_m]$. Consider also the following (simulated) moment function:
\begin{equation}\label{eq:moment}
\bar{\mathbf{m}}_{M}(\boldsymbol{\theta})=\frac{1}{M}\sum_m\frac{1}{RST}\sum_{rst}\dot{\mathbf{Z}}^{(r)\prime}_m\left[(\mathbf{I}_m-\alpha\ddot{\mathbf{G}}^{(s)}_m)\left(\mathbf{y}_m-(\mathbf{I}_m-\alpha\dddot{\mathbf{G}}_m^{(t)})^{-1}\dddot{\mathbf{V}}_m^{(t)}\tilde{\boldsymbol{\theta}}\right)\right]
\end{equation}

Then, for any positive integers $R$, $S$, and $T$, the (simulated) GMM estimator based on (\ref{eq:moment}) is consistent and asymptotically normally distributed.
\end{theorem}
The identification condition is standard and ensures that the moment condition is uniquely solved at $\boldsymbol{\theta}_0$. We discuss it in more detail below.

Theorem \ref{prop:non_observed} presents conditions for the consistency and asymptotic normality of our two-step estimator. In particular, similar to a standard simulated GMM \citep{gourieroux1996simulation}, consistency holds for a finite number of simulations. Our estimator therefore does not suffer from the curse of dimensionality faced by \cite{chandrasekhar2011econometrics}.\footnote{The unconditional moment condition in \cite{chandrasekhar2011econometrics} is based on the (Monte Carlo) integration of the moment condition $\mathbb{E}(\mathbf{Z}^{(s)\prime}_m\boldsymbol{\varepsilon}_m|\mathbf{G}_m)$ over $\mathbf{G}_m$.}

Here, a few remarks regarding the consistency and asymptotic normality are in order. Note that the simulated moment function is based on network draws that depend on an \emph{estimated} distribution. In particular, we have: $\dot{\mathbf{G}}_m=\dot{\mathbf{G}}_m(\hat{\boldsymbol{\rho}})=f(\{\dot{a}_{m,ij}\}_{ij})=f(\{\mathbbm{1}[\hat{P}(\dot{a}_{m,ij} = 1|\hat{\boldsymbol{\rho}};\mathbf{X}_m, \kappa(\mathcal{A}_m))\geq \dot{u}_{m,ij}]\}_{ij})$, where $\dot{u}_{m,ij}\sim_{iid}U[0,1]$ and independent of $\boldsymbol \varepsilon_m$ (and similarly for $\ddot{\mathbf{G}}_m$ and $\dddot{\mathbf{G}}_m$), and $\mathbbm{1}$ is the indicator function.

This has two implications. First, it implies that our SGMM estimator is a two-stage estimator and therefore that the asymptotic variance-covariance matrix for $\boldsymbol{\theta}$ has to account for the first-stage sampling uncertainty. We show how to estimate the resulting asymptotic variance-covariance in the Online Appendix \ref{sec:varestim}.

Second, the indicator function $\mathbbm{1}[\hat{P}(\dot{a}_{m,ij} = 1|{\boldsymbol{\rho}};\mathbf{X}_m, \kappa(\mathcal{A}_m))\geq \dot{u}_{m,ij}]$ implies that the objective function of the two-stage estimator is not everywhere continuous in ${\boldsymbol{\rho}}$. While this has a limited impact on consistency, it does complicate the proof of the asymptotic normality. Our proof builds on the argument in \cite{andrews1994empirical}, and we show that the stochastic equicontinuity condition holds using a bracketing argument.

Consistency and asymptotic normality also obviously depend on an identification condition. Here, the fact that the approximation of the bias $\boldsymbol{\delta}_m$ is non-linear in $\alpha$ implies that our SGMM is non-linear and that the identification condition cannot be simplified to a simple rank condition.

In Appendix \ref{app:ident}, we show that the objective function of our SGMM can be concentrated around $\alpha$ and that \emph{conditional on $\alpha$}, the identification conditions for $\tilde{\boldsymbol{\theta}}$ reduces to an asymptotic rank condition. Specifically, a sufficient condition for the identification of $\tilde{\boldsymbol{\theta}}$, conditional on $\alpha$, is that the expected value of:
$$
\frac{1}{RST}\sum_{rst}\dot{\mathbf{Z}}_m^{(r)\prime}(\mathbf{I}_m-\alpha\ddot{\mathbf{G}}_m^{(s)})(\mathbf{I}_m-\alpha\dddot{\mathbf{G}}_m^{(t)})^{-1}\dddot{\mathbf{V}}_m^{(t)}
$$
converges in probability, to a full rank matrix for all $\alpha$.\footnote{The identification of $\alpha$ then requires that the concentrated objective function is uniquely minimized.} The last expression makes it clear that the non-linearity in our SGMM is sourced in the approximation of the asymptotic bias $\boldsymbol{\delta}_m=(\mathbf I_m - \alpha \ddot{\mathbf G}_m )(\mathbf I_m - \alpha \dddot{\mathbf G}_m )^{-1}\dddot{\mathbf{V}}_m\tilde{\boldsymbol{\theta}}-\ddot{\mathbf{V}}_m\tilde{\boldsymbol{\theta}}$.

When the matrix $\mathbf{G}_m$ is observed, we have $\dot{\mathbf{G}}_m^{(r)}=\ddot{\mathbf{G}}_m^{(s)}=\dddot{\mathbf{G}}_m^{(t)}={\mathbf{G}}_m$ and the expression reduces to $\mathbf{Z}'_m\mathbf{V}_m$, \citep{bramoulle2009identification} which does not depend on $\alpha$. This shows that the quality of $\hat{P}(\mathbf{A}_m|\hat{\boldsymbol{\rho}},\mathbf{X}_m,\kappa(\mathcal{A}_m))$ has strong implications for identification since the dependence on $\alpha$ is weaker when the correlation between network draws is strong. We study the finite sample properties of our estimator using Monte Carlo simulation in Section \ref{sec:montecarlo}.\footnote{Theorem \ref{prop:non_observed} assumes that the partial observability of $\mathbf{A}_m$ implies that $\mathbf{G}_m\mathbf{X}_m$ and $\mathbf{G}_m\mathbf{y}_m$ are both unobserved. However, in some cases, researchers can separately observe these quantities from survey questions. For example, one could simply obtain ${\mathbf{G}_m\mathbf{y}_m}$ from a question of the type: ``What is the average value of your friends' $y$?'' In these cases, it is possible to improve on our SGMM estimator by using this additional information. The resulting estimators are presented in Corollary \ref{prop:GXobs} and Corollary \ref{prop:Gyobs} of the Online Appendix \ref{sec:appendix_otherresults}.}

\subsection{Monte Carlo Simulations}\label{sec:montecarlo}

In this subsection, we study the performance of our SGMM estimator using Monte Carlo simulations. We consider cases where links are missing at random (see Example \ref{ex:sampled}) and misclassified at random (see Example \ref{ex:misclass}). The simulated individual characteristics (i.e., the matrix $\mathbf X$) include two characteristics similar to "age" and "female" in our empirical application.\footnote{See Section \ref{sec:addhealth}. We simulate those variables from their empirical distributions in our sample. Parameter values are set to the estimates from our application: $(\alpha, \boldsymbol{\beta}, \boldsymbol{\gamma}) = (0.538, 3.806, -0.072, 0.132, 0.086, -0.003)$. {We assume that $\varepsilon$ is iid normally distributed with standard deviation of $\sigma = 0.707$.}}  The network formation process follows a logistic regression model: $$P(a_{ij} = 1|\mathbf X) = \frac{\exp\{\rho_1 + \rho_2 |x_{i1} - x_{j1}| + \rho_3 \mathbbm{1}\{x_{i2} = x_{j2}\}\}}{1 + \exp\{\rho_1 + \rho_2 |x_{i1} - x_{j1}| + \rho_3 \mathbbm{1}\{x_{i2} = x_{j2}\}\}},$$ where $x_{i1}$ represents "age" and $x_{i2}$ represents "female".\footnote{The parameter vector $\boldsymbol{\rho}$ is also set to its empirically estimated values: $\boldsymbol{\rho} = (-2.349, -0.700, 0.404)$.}

% The estimator proposed by \cite{bramoulle2009identification} is inconsistent unless the group size $N_m$ is unbounded and the expected number of missing and misclassified links grows at a rate strictly less than $N_m$ \citep{lewbel2023social}. Nevertheless, the estimator in \cite{bramoulle2009identification} serves as a natural benchmark, as it is a special case of our SGMM estimator when all links are observed.\footnote{When all links are observed, $\dot{\mathbf{G}}^{(r)}_m=\ddot{\mathbf{G}}^{(s)}_m=\dddot{\mathbf{G}}^{(t)}_m=\mathbf{G}^{obs}_m$. See our discussion of the estimator above.} 

We analyze different proportions of randomly missing and misclassified entries in the network matrix. Figure \ref{fig:mc_noFE} presents estimates for the endogenous peer effect coefficient $\alpha$ using our SGMM estimator. The left panel shows the peer effect estimates for the case of missing links, while the right panel displays the estimates for the case of misclassified links.\footnote{Tables \ref{tan:sim:noFE}--\ref{tab:simmclas:FE} in Online Appendix \ref{append:fullsimu} provide the full set of estimated coefficients, including results that control for unobserved group heterogeneity through fixed effects.} Additionally, we report estimates obtained using the standard IV estimator of \cite{bramoulle2009identification}, treating the observed network with missing values or misclassified links as the true network.

\begin{figure}[h]
    \centering
    \includegraphics[scale = 0.9]{graphs/mc_BOTH.pdf}
    \caption{Estimated peer effects under missing links}
    \label{fig:mc_noFE}

   \begin{minipage}{16cm}%
  \vspace{0.3cm}
\footnotesize{Note: Dots represent the average estimated values of $\alpha$, and bars indicate 95\% confidence intervals. Tables \ref{tan:sim:noFE}--\ref{tab:simmclas:FE} in Online Appendix \ref{append:fullsimu} provide the full set of estimated coefficients. The "Classical IV" refers to the standard estimator of \cite{bramoulle2009identification}. We simulate data for 100 groups of 30 individuals each. We assume that $\varepsilon_i$ follows a normal distribution. We estimate $\boldsymbol{\rho}$ using a logit model based on the observed network entries (left panel) and a logit model with misclassification (right panel). The resulting estimates allow us to construct the network distribution (see Definition \ref{def:estimator}) and subsequently compute our SGMM estimator.}
  \end{minipage}%
\end{figure}


For the case of missing links, the estimates are centered around the true value. Although precision decreases as the fraction of missing links increases, our SGMM estimator maintains a reasonable level of accuracy, even when \emph{half} of the links are missing. In contrast, the standard IV estimator significantly underestimates the peer effect coefficient $\alpha$.  

For the case of misclassified links, the estimator performs well when there are false negatives only. Precision is affected when there are false positives, although the estimates remain centered around the true value. With false positives, the estimator for $\boldsymbol{\rho}$ loses precision since the network is simulated to match the one in our application: the density of the network is low.\footnote{This is typical of most network data: two randomly selected individuals are unlikely to be linked, even conditional on observables.} With few links, the finite sample cost of false positives is thus more important.


==> RestatRR1/iv_backup_parts.tex <==

\section{Temporary}
Once the network distribution is estimated, a simple and intuitive (but invalid) approach to estimating peer effects is to replace the true network in the classical moment function of the linear-in-means peer effects model \citep[see][]{bramoulle2009identification} with a simulated network from the estimated distribution. What follows also holds if one simulates many networks and takes the average of corresponding moment functions.

For each group $m$, this approach leads to the moment function:
\[
\dot{\mathbf m}_m (\boldsymbol{\theta}) = \dot{\mathbf Z}_m^{\prime}(\mathbf y_m - \alpha \dot{\mathbf G}_m \mathbf y_m - c\mathbf{1}_m - \mathbf X_m\boldsymbol{\beta} - \dot{\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}),
\]
where $\boldsymbol{\theta} = (\alpha, ~c, ~\boldsymbol{\beta}^{\prime}, ~\boldsymbol{\gamma}^{\prime})^{\prime}$, $\dot{\mathbf G}_m = f(\dot{\mathbf A}_m)$, $\dot{\mathbf A}_m$ is the simulated network from the estimated distribution, and $\mathbf 1_m$ is an $n_m$-dimensional vector of ones. By substituting $\mathbf y_m$ with its specification given in \eqref{eq:linearinmean}, we obtain:
\begin{align}
\begin{split}
    \dot{\mathbf m}_m (\boldsymbol{\theta}) &= \dot{\mathbf Z}_m^{\prime} \big[(\mathbf I_m - \alpha \dot{\mathbf G}_m )(\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}(c_0\mathbf{1}_m + \mathbf X_m\boldsymbol{\beta}_0 + {\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}_0 + \boldsymbol{\varepsilon}_m)\\
    &\hspace{1.5cm} - c\mathbf{1}_m - \mathbf X_m\boldsymbol{\beta} - \dot{\mathbf G}_m\mathbf X_m\boldsymbol{\gamma} \big],
\end{split} \label{eq:dotm}
\end{align}
where the subscript $0$ denotes the true parameter values, and $\mathbf I_m$ is the $n_m \times n_m$ identity matrix. Although $\mathbb{E}[\boldsymbol{\varepsilon}_m|\mathbf{X}_m,\mathcal{A}_m]=\mathbf{0}$ (Assumption \ref{as:exonet}), it is clear that $\mathbb{E}[\dot{\mathbf m}_m (\boldsymbol{\theta}_0)] \neq \mathbf{0}$ in general (even asymptotically), unless $\dot{\mathbf G}_m = \mathbf G_m$ for all $m$. Indeed, $\dot{\mathbf G}_m$ is not a consistent estimator of $\mathbf G_m$. Importantly, this issue is not resolved by simulating multiple $\dot{\mathbf G}_m$ and averaging the corresponding moment functions $\dot{\mathbf m}_m (\boldsymbol{\theta})$.


We denote by \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) the term in square brackets in \eqref{eq:dotm}, so that \( \dot{\mathbf{m}}_m (\boldsymbol{\theta}) = \dot{\mathbf{Z}}_m^{\prime} \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \). The sources of the inconsistency of \( \dot{\mathbf{m}}_m \) are twofold. First, \( \dot{\mathbf{Z}}_m \) and \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}_0) \) are correlated, as they depend on the same simulation \( \dot{\mathbf{G}}_m \). Second, even if \( \dot{\mathbf{Z}}_m \) and \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}_0) \) were independent, \( \mathbb{E}(\dot{\boldsymbol{\varepsilon}}_m | \mathbf{X}_m, \mathcal{A}_m) \neq \mathbf{0} \) (even asymptotically) because \( \dot{\mathbf{G}}_m \) is not a consistent estimator of \( \mathbf{G}_m \). For a moment function of the form \( \dot{\mathbf{Z}}_m^{\prime} \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \), the desired properties are that \( \dot{\mathbf{Z}}_m \) and \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) are independent and that \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) is centered (conditional on the observable exogenous variables).



To address the first issue, it is sufficient to use two different simulations for \( \dot{\mathbf{Z}}_m \) and \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \). We then replace \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) with some \( \ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \), which has the same expression as \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) with the difference that \( \dot{\mathbf{G}}_m \) is replaced with a new simulated network \( \ddot{\mathbf{G}}_m \). This guarantees that \( \dot{\mathbf{Z}}_m \) and \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) are independent conditional on \( \mathbf{X}_m \) and \( \mathcal{A}_m \). We thus have a new moment function, which is \( \ddot{\mathbf{m}}_m (\boldsymbol{\theta}) = \dot{\mathbf{Z}}_m^{\prime} \ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \).


As now \( \mathbb{E} (\ddot{\mathbf{m}}_m (\boldsymbol{\theta})|\mathbf{X}_m, \mathcal{A}_m) = \mathbb{E} (\dot{\mathbf{Z}}_m^{\prime}|\mathbf{X}_m, \mathcal{A}_m) \mathbb{E} [\ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta})|\mathbf{X}_m, \mathcal{A}_m] \), we only need to "force" \( \mathbb{E} (\ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}_0)) \) to be zero to establish consistency. To achieve this, we can replace \( \ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) with the \textit{unfeasible} debiased equivalent \( \ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) - \mathbb{E} [\ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta})|\mathbf{X}_m, \mathcal{A}_m, \ddot{\mathbf{G}}_m, \mathbf{G}_m] \). This debiasing approach is unfeasible since the removed bias is conditional on the unobserved true network matrix \( \mathbf{G}_m \) and the true parameters. We condition on \( \mathbf{G}_m \) only to make the computation of the removed bias easier. The resulting expression then depends on \( \mathbf{G}_m \), which can be approximated using a third simulated network.


From \eqref{eq:dotm}, we have:
\begin{align}
    &\mathbb E [\ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta})|\mathbf{X}_m,\mathcal{A}_m, \ddot{\mathbf G}_m, \mathbf G_m]  = (\mathbf I_m - \alpha \ddot{\mathbf G}_m )(\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}(c_0\mathbf{1}+ \mathbf X_m\boldsymbol{\beta}_0 + {\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}_0) \nonumber\\
    &\hspace{5.5cm}- c\mathbf{1}_m- \mathbf X_m\boldsymbol{\beta} - \ddot{\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}, \nonumber\\
    &\ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) - \mathbb E [\ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta})|\mathbf{X}_m,\mathcal{A}_m, \ddot{\mathbf G}_m, \mathbf G_m] = (\mathbf I_m - \alpha \ddot{\mathbf G}_m)\mathbf y_m -c\mathbf{1}_m- \mathbf X_m\boldsymbol{\beta} - \ddot{\mathbf G}_m\mathbf X_m\boldsymbol{\gamma} \nonumber\\
    & ~- (\mathbf I_m - \alpha \ddot{\mathbf G}_m )(\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}(c_0\mathbf{1}+ \mathbf X_m\boldsymbol{\beta}_0 + {\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}_0) + c\mathbf{1}_m- \mathbf X_m\boldsymbol{\beta} - \ddot{\mathbf G}_m\mathbf X_m\boldsymbol{\gamma},\nonumber \\
    &= (\mathbf I_m - \alpha \ddot{\mathbf G}_m)(\mathbf y_m - (\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}(c_0\mathbf{1}+ \mathbf X_m\boldsymbol{\beta}_0 + {\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}_0) \label{eq:debaisederror}
\end{align}
The feasible equivalent of \eqref{eq:debaisederror} that can lead to similar properties asymptotically is:
$$
    (\mathbf{I}_m - \alpha \ddot{\mathbf{G}}_m)\left(\mathbf{y}_m - (\mathbf{I}_m - \alpha \dddot{\mathbf{G}}_m)^{-1}(c\mathbf{1} + \mathbf{X}_m \boldsymbol{\beta} + \dddot{\mathbf{G}}_m \mathbf{X}_m \boldsymbol{\gamma})\right).
$$
We replace \( \mathbf{G}_m \) with a new independent simulation to preserve the independence between \( \mathbf{G}_m \) and the first two initial simulated networks. Our consistent moment function then becomes:
\begin{equation} \label{eq:moment:3simu}
\dot{\mathbf{Z}}_m^{\prime}(\mathbf{I}_m - \alpha \ddot{\mathbf{G}}_m)\left(\mathbf{y}_m - (\mathbf{I}_m - \alpha \dddot{\mathbf{G}}_m)^{-1}(c\mathbf{1} + \mathbf{X}_m \boldsymbol{\beta} + \dddot{\mathbf{G}}_m \mathbf{X}_m \boldsymbol{\gamma})\right).
\end{equation}


Another approach is to directly correct the bias of the initial function \( \dot{\mathbf{m}}_m (\boldsymbol{\theta}) = \dot{\mathbf{Z}}_m^{\prime} \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \). In this case, an unfeasible debiased moment function can be:
\begin{align}
    &\dot{\mathbf m}_m (\boldsymbol{\theta}) - \mathbb{E}[\dot{\mathbf m}_m (\boldsymbol{\theta})|\mathbf{X}_m, \mathcal{A}_m, \dot{\mathbf{G}}_m, \mathbf{G}_m] = \nonumber\\
    &\dot{\mathbf Z}_m^{\prime}(\mathbf I_m - \alpha \dot{\mathbf G}_m ) \big[\mathbf y_m - (\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}(c_0\mathbf{1}_m + \mathbf X_m\boldsymbol{\beta}_0 + {\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}_0)\big].\nonumber
\end{align}
The feasible equivalent of this moment function is thus:
\begin{equation} \label{eq:moment:2simu}
\dot{\mathbf Z}_m^{\prime}(\mathbf I_m - \alpha \dot{\mathbf G}_m ) \big[\mathbf y_m - (\mathbf I_m - \alpha \ddot{\mathbf G}_m )^{-1}(c\mathbf{1}_m + \mathbf X_m\boldsymbol{\beta} + \ddot{\mathbf G}_m\mathbf X_m\boldsymbol{\gamma})\big].
\end{equation}
While both moment functions \eqref{eq:moment:3simu} and \eqref{eq:moment:2simu} lead to consistent estimators, it can be shown that \eqref{eq:moment:3simu} is more efficient because its variance is lower. The intuition is as follows. Bias correction is generally associated with a loss of efficiency. With \( \dot{\mathbf{m}}_m (\boldsymbol{\theta}) \), we mechanically correct both the bias stemming from the dependence between \( \dot{\mathbf{Z}}_m \) and \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}_0) \), as well as the bias due to the fact that \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}_0) \) is not centered. In contrast, our proposed moment function \eqref{eq:moment:3simu} no longer suffers from the first bias, and we only correct for the second bias mechanically.

Both moment functions have the form \(\dot{\mathbf Z}_m^{\prime}\mathbf u_m\) and \(\dot{\mathbf Z}_m^{\prime}\tilde{\mathbf u}_m\), where \(\mathbf u_m\) and \(\tilde{\mathbf u}_m\) are the terms that post-multiply \(\dot{\mathbf Z}_m^{\prime}\) in \eqref{eq:moment:3simu} and \eqref{eq:moment:2simu}, respectively. Although \(\mathbf u_m\) and \(\tilde{\mathbf u}_m\) have different expressions, they share the same distribution. Indeed, \(\mathbf u_m\) can be written as a function of \(\ddot{\mathbf G}_m\) and \(\dddot{\mathbf G}_m\), whereas \(\tilde{\mathbf u}_m\) can be written as the same function of \(\dot{\mathbf G}_m\) and \(\ddot{\mathbf G}_m\). Since the simulated networks have the same distribution, it follows that \(\mathbf u_m\) and \(\tilde{\mathbf u}_m\) also have the same distribution.

We aim to compare the variance of \(\dot{\mathbf Z}_m^{\prime}\mathbf u_m\) to the variance of \(\dot{\mathbf Z}_m^{\prime}\tilde{\mathbf u}_m\) in a situation where \(\mathbf u_m\) and \(\tilde{\mathbf u}_m\) have the same distribution, \(\tilde{\mathbf u}_m\) is correlated with \(\dot{\mathbf Z}\), and \(\mathbf u_m\) is independent of \(\dot{\mathbf Z}\), conditional on \(\mathbf{X}_m\) and \(\mathcal{A}_m\). Indeed, \(\dot{\mathbf Z}\) and \(\tilde{\mathbf u}_m\) are correlated because they depend on the same simulated network \(\dot{\mathbf G}_m\).

To simplify the comparison of the variances of \(\dot{\mathbf Z}_m^{\prime}\mathbf u_m\) and \(\dot{\mathbf Z}_m^{\prime}\tilde{\mathbf u}_m\), we assume that \(\dot{\mathbf Z}_m\), \(\mathbf u_m\), and \(\tilde{\mathbf u}_m\) are scalars. (It is possible to generalize the result by applying what follows to each entry of the variances, but the notation would become cumbersome.) Let \(\mathbb{V}_1\) and \(\mathbb{V}_2\) be the variances of \(\dot{\mathbf Z}_m^{\prime}\mathbf u_m\) and \(\dot{\mathbf Z}_m^{\prime}\tilde{\mathbf u}_m\), respectively, conditional on \(\mathbf{X}_m\) and \(\mathcal{A}_m\). We have:
\begin{align*}
    \mathbb{V}_2 - \mathbb{V}_1 &= \mathbb{E}(\dot{\mathbf Z}_m^2\tilde{\mathbf u}_m^2|\mathbf{X}_m, \mathcal{A}_m) -  \mathbb{E}(\dot{\mathbf Z}_m^2\mathbf u_m^2|\mathbf{X}_m, \mathcal{A}_m),\\
    \mathbb{V}_2 - \mathbb{V}_1 &= \mathbb{E}(\dot{\mathbf Z}_m^2\tilde{\mathbf u}_m^2|\mathbf{X}_m, \mathcal{A}_m) -  \mathbb{E}(\dot{\mathbf Z}_m^2|\mathbf{X}_m, \mathcal{A}_m)\mathbb{E}(\mathbf u_m^2|\mathbf{X}_m, \mathcal{A}_m),\\
    \mathbb{V}_2 - \mathbb{V}_1 &= \mathbb{E}(\dot{\mathbf Z}_m^2\tilde{\mathbf u}_m^2|\mathbf{X}_m, \mathcal{A}_m) -  \mathbb{E}(\dot{\mathbf Z}_m^2|\mathbf{X}_m, \mathcal{A}_m)\mathbb{E}(\tilde{\mathbf u}_m^2|\mathbf{X}_m, \mathcal{A}_m),\\
    \mathbb{V}_2 - \mathbb{V}_1 &= \operatorname{Cov}(\dot{\mathbf Z}_m^2, ~\tilde{\mathbf u}_m^2|\mathbf{X}_m, \mathcal{A}_m).
\end{align*}
In the third equality, we replace 
\(\mathbb{E}(\mathbf{u}_m^2 \mid \mathbf{X}_m, \mathcal{A}_m)\) 
with 
\(\mathbb{E}(\tilde{\mathbf{u}}_m^2 \mid \mathbf{X}_m, \mathcal{A}_m)\) 
because \(\mathbf{u}_m\) and \(\tilde{\mathbf{u}}_m\) share the same distribution. 
Thus, the moment function with two simulated networks performs better if 
\(\dot{\mathbf{Z}}_m^2\) and \(\tilde{\mathbf{u}}_m^2\) are positively correlated, 
conditional on \(\mathbf{X}_m\) and \(\mathcal{A}_m\). 
This is straightforward to see when there are no contextual effects, 
as both \(\dot{\mathbf{Z}}_m\) and \(\tilde{\mathbf{u}}_m\) are linear in \(\dot{\mathbf{G}}_m\). 
Moreover, \(\dot{\mathbf{Z}}_m^2\) and \(\tilde{\mathbf{u}}_m^2\) remain positively correlated 
regardless of the sign of \(\alpha\).




\section{Simulated Generalized Method of Moment Estimators}\label{sec:iv}


%Note that we can use $\hat{P}(\mathbf{A}_m)$ implicitly defines the analog $\hat{P}(\mathbf{G}_m)$ because $\mathbf{G}_m=f(\mathbf{A}_m)$ for some known function $f$.\footnote{Because $\mathbf{A}_m$ takes a finite number of values (the size of group $m$ is bounded), so does $\mathbf{G}_m$, (thus $\mathbf{A}_m$ and $\mathbf{G}_m$ have multinomial distributions). Then, $P(\mathbf{G}_m)$ is a continuous function of $P(\mathbf{A}_m)$, irrespective of the function $f$ linking $\mathbf{A}_m$ and $\mathbf{G}_m$.}


In this section, we present an estimator based on a Simulated Generalized Method of Moments (SGMM). The key observation underlying our approach is that it is not necessary to observe the complete network structure to observe $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$. For example, one could simply obtain ${\mathbf{Gy}}$ from survey data, ``What is the average value of your friends' $y$?''

However, even observing $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$, the model (\ref{eq:linearinmean}) cannot be simply estimated using simple linear regression. The reason is that ${\mathbf{Gy}}$ is endogenous; thus, a linear regression would produce biased estimates (e.g. \cite{manski1993identification}, \cite{bramoulle2009identification}).

The typical instrumental approach to deal with this endogeneity is to use instruments based on the structural model, i.e. instruments constructed using second-degree peers (e.g. $\mathbf{G}^2\mathbf{X}$, see \cite{bramoulle2009identification}). These are less likely to be found in survey data. Indeed, we could doubt the informativeness of questions such as, ``What is the average value of your friends' average value of their friends' $x$?''

However, the above discussion is encouraging. When researchers observe $[\mathbf{y}, \mathbf{X}]$ and $[{\mathbf{GX}},{\mathbf{Gy}}]$, information about the network is only used as a means to construct a valid instrument, e.g. following \citet{bramoulle2009identification}. Then, if $\mathbf{GX}$ and $\mathbf{Gy}$ are observed, the estimation of peer effects is possible using any exogeneous (strong) predictor of the true network structure, as in \cite{kelejian2014estimation}, \cite{konig2019r}, and \cite{lee2020key}.\footnote{See Proposition \ref{prop:all_observed} of the Online Appendix \ref{sec:appendix_otherresults} for a formal statement. In particular, one needs a predictor of the network such that the resulting instrument is not correlated with $\boldsymbol{\varepsilon}$ and is strongly correlated with $\mathbf{Gy}$.}

The problem is more challenging when $\mathbf{Gy}$ and $\mathbf{GX}$ are not observed.



Finally, for any matrix $\mathbf{B}$, we will use $\mathbf{B}_i$ to denote the $i$th row of $\mathbf{B}$.

Before presenting our estimation strategy, we want to emphasize that we cannot simply proxy $\mathbf{Gy}$ and $\mathbf{GX}$ using draws from $\hat{P}(\mathbf{G})$. To see why, consider the simple case for which $\boldsymbol{\gamma}=\mathbf{0}$, so that the observation of $\mathbf{GX}$ is inconsequential. We have, substituting $\mathbf{Gy}$ with $\ddot{\mathbf{G}}\mathbf{y}$,
$$
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\ddot{\mathbf{G}}\mathbf{y}+[\boldsymbol{\eta}+\boldsymbol{\varepsilon}],
$$
where $\boldsymbol{\eta}=\alpha[\mathbf{G}-\ddot{\mathbf{G}}]\mathbf{y}$ is the error due to the approximation of $\mathbf{Gy}$ by $\ddot{\mathbf{G}}\mathbf{y}$. Importantly, the approximation error does \emph{not} vanish as $N$ grows because individuals belong to bounded groups (see Assumption \ref{as:manymarkets}).\footnote{As opposed to, for example, the context studied by \cite{auerbach2019measuring}.} Moreover, because $\mathbf{y}$ is a function of $\mathbf{G}$ (but not of $\ddot{\mathbf{G}}$), we typically have $\mathbb{E}(\mathbf{Gy})_i|\mathbf{Z}_i\neq\mathbb{E}(\ddot{\mathbf{G}}\mathbf{y})_i|\mathbf{Z}_i$ for some vector of instruments $\mathbf{z}_i$ and all $i$.


In Proposition \ref{prop:bias_nocontext} of the Online Appendix \ref{sec:appendix_otherresults}, we show, using an argument very similar to that of \cite{andrews2017measuring}, that the asymptotic bias induced by $\mathbb{E}\eta_i|\mathbf{z}_i\neq 0$ can be bounded, and simulations show that it can be very small for carefully constructed vectors of instruments, which can be useful in practice.

In any case, in our main result below, we show that we can include the bias directly in the moment function; this provides a consistent estimator of $\boldsymbol{\theta}$.

\subsection{Main Result}
Let $\tilde{\boldsymbol{\theta}}=[c,\boldsymbol{\beta}',\boldsymbol{\gamma}']'$.  We present the following simulated general method of moment estimator. Theorem \ref{prop:non_observed} defines the moment function and shows the consistency of the estimator. Theorem ?? shows the asymptotic normality for a large class of first-stage estimators. 

\begin{theorem}[SGMM - Consistency]\label{prop:non_observed} Suppose that Assumptions \ref{as:alpha}--\ref{as:partial} and regularity conditions \ref{as:regularity}--\ref{as:Wm} hold. Suppose also that the identification condition \ref{as:identification} hold

[Conditions] Let $\dot{\mathbf{Z}}^{(r)}_m=[\mathbf{1},\mathbf{X}_m,\dot{\mathbf{G}}^{(r)}_m\mathbf{X}_m,(\dot{\mathbf{G}}^{(r)}_m)^2\mathbf{X}_m,(\dot{\mathbf{G}}_m^{(r)})^3\mathbf{X}_m,...]$ and $\ddot{\mathbf{V}}_m^{(s)}=[\mathbf{1},\mathbf{X}_m,\ddot{\mathbf{G}}_m^{(s)}\mathbf{X}_m]$. Consider also the following (simulated) moment function:
\begin{equation}\label{eq:moment}
\bar{\mathbf{m}}_{M}(\boldsymbol{\theta})=\frac{1}{M}\sum_m\frac{1}{RST}\sum_{rst}\dot{\mathbf{Z}}^{(r)\prime}_m\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})_m\left(\mathbf{y}_m-(\mathbf{I}-\alpha\ddot{\mathbf{G}}_m^{(s)})^{-1}\ddot{\mathbf{V}}_m^{(s)}\tilde{\boldsymbol{\theta}}\right)\right]
\end{equation}

[Result] For any positive integers $R$, $S$, and $T$, the (simulated) GMM estimator based on (\ref{eq:moment}) is consistent and asymptotically normally distributed.
\end{theorem}



To understand the intuition behind the use of the moment function (\ref{eq:moment}), let us replace $\mathbf{y}=(\mathbf{I}-\alpha\mathbf{G})^{-1}(\mathbf{V}\tilde{\boldsymbol{\theta}}+\boldsymbol{\varepsilon})$ in Equation (\ref{eq:moment}), considering a single group and ignoring the subscript $m$. In doing so, we can rewrite the term inside the triple summation in (\ref{eq:moment}) as a sum of two terms. First, $\dot{\mathbf{Z}}^{(r)\prime}\boldsymbol{\varepsilon}$, which would be the standard moment function if $\mathbf{G}$ was observed (e.g. \cite{bramoulle2009identification}), and second:
\begin{equation}\label{eq:bias_corr}
\dot{\mathbf{Z}}^{(r)\prime}\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})\left((\mathbf{I}-\alpha{\mathbf{G}})^{-1}{\mathbf{V}}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}\ddot{\mathbf{V}}^{(s)}\right)\tilde{\boldsymbol{\theta}}\right].
\end{equation}
That second term can be viewed as the bias-correction term of the moment function.

We show that the expectations of both terms are equal to $0$ as $M$ grows to $\infty$. For the first term, this is true because the simulated network is exogenous. For the second term, this is true because $\mathbf{G}$, $\dot{\mathbf{G}}$, $\ddot{\mathbf{G}}$, and $\dddot{\mathbf{G}}$ are asymptotically drawn from the same distribution.

For the special case in which $\mathbf{G}$ is observed, one could substitute $\dot{\mathbf{G}}^{(r)}=\ddot{\mathbf{G}}^{(s)}=\dddot{\mathbf{G}}^{(t)}=\mathbf{G}$ for all $r,s,t$, and the first term would simply be $\mathbf{Z}'\boldsymbol{\varepsilon}$, whereas the second term would be exactly equal to $\mathbf{0}$.

Note that Theorem \ref{prop:non_observed} is valid whether or not $\mathbf{Gy}$ and $\mathbf{GX}$ are observed because the moment function (\ref{eq:moment}) does not use information on $\mathbf{Gy}$ or $\mathbf{GX}$. It is of course possible to include this additional information if either one is observed.

For example, assume that $\mathbf{GX}$ is observed and replace $\ddot{\mathbf{V}}$ with $\mathbf{V}$ in (\ref{eq:bias_corr}). After some algebra, we obtain: \begin{equation}\label{eq:gxobswrong}
    \dot{\mathbf{Z}}^{(r)\prime}\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}[\alpha(\mathbf{G}-\ddot{\mathbf{G}})\mathbf{y}]\right]
\end{equation}
and a term that is equal to zero in expectation.

We can show that the last term in brackets corresponds to the source of the asymptotic bias because of the approximation error of $\mathbf{Gy}$ by $\ddot{\mathbf{G}}\mathbf{y}$ (see Proposition \ref{prop:bias_nocontext} of the Online Appendix). Whereas Equation (\ref{eq:gxobswrong}) cannot directly be substituted for (\ref{eq:moment}) in Theorem \ref{prop:non_observed}, it is possible to construct moment functions for the particular cases for which $\mathbf{GX}$ or $\mathbf{Gy}$ is observed. These cases can be found in Corollary \ref{prop:GXobs} and \ref{prop:Gyobs} of the Online Appendix.



==> RestatRR1/model.tex <==
\section{The Model}\label{sec:linearinmean}
We assume that the data are partitioned into $M>1$ groups, where group $m$ contains $N_m$ individuals. A sample consists of the following:
$$
\lbrace\mathbf{y}_m,\mathbf{X}_m,\boldsymbol{\varepsilon}_m;\mathcal{A}_m,\mathbf{A}_m \rbrace_{m=1}^M.
$$
For individuals in group $m$, $\mathbf{y}_m$ is a vector of an observed outcome of interest (e.g., academic achievement), $\mathbf{X}_m$ is an observed matrix of individual characteristics (e.g., age and gender), and $\boldsymbol{\varepsilon}_m$ is a vector of \emph{unobserved} individual heterogeneity.

The matrix $\mathbf{A}_m$ is the $N_m\times N_m$ \emph{adjacency matrix} of the network between individuals in group $m$. We assume a directed network:\footnote{All of our results hold for undirected networks.} $a_{ij,m}\in \{0,1\}$, where $a_{ij,m}=1$ if $i$ is linked to $j$. We normalize $a_{ii,m}=0$ for all $i$ and let $n_{i,m}=\sum_j a_{ij,m}$ denote the number of links of $i$ within group $m$.

We assume that $\mathbf{A}_m$ is \emph{not observed} but that researchers observe $\mathcal{A}_m$ instead. Informally, the idea is that $\mathcal{A}_m$ contains some information about the adjacency matrix $\mathbf{A}_m$. Our specific assumptions are presented in Section \ref{sec:partial}. The next assumptions formalize the above discussion.
\begin{assumption}\label{as:manymarkets} The population is partitioned into $M>1$ groups, where the size $N_m$ of each group $m=1,...,M$ is bounded. The sequence $\lbrace\mathbf{y}_m,\mathbf{X}_m,\boldsymbol{\varepsilon}_m;\mathcal{A}_m,\mathbf{A}_m \rbrace$ is independent across $m$. Moreover, $\mathbf{X}_m$ is uniformly bounded in $m$.\footnote{i.e., $\sup_{m \geq 1}\lVert \mathbf X_m \rVert_2 < \infty$, where $\lVert.\rVert_2$ is the Euclidean norm.} 
\end{assumption}
\begin{assumption}\label{as:nosampling} For each group $m$, the variables $\mathbf{y}_m$, $\mathbf{X}_m$ and $\mathcal{A}_m$ are observed. The variables $\boldsymbol{\varepsilon}_m$ and $\mathbf{A}_m$ are not.
\end{assumption}

Assumption \ref{as:manymarkets} implies a ``many markets'' asymptotic framework, meaning that the number of groups $M$ goes to infinity as the number of individuals $N$ goes to infinity. It is a standard assumption in the literature on the econometrics of games and the literature on peer effects.\footnote{See for example \cite{bramoulle2019peer}, \cite{breza2016}, and \cite{de2015econometrics}.} For example, the data could consist of a collection of small villages \citep{banerjee2013diffusion} or schools \citep{calvo2009peer}. Assumption \ref{as:nosampling} implies in particular that the data are composed of group-level censuses for $\mathbf{y}_m$ and $\mathbf{X}_m$.\footnote{Contrary to \cite{liu2017peer} or \cite{wang2013estimation}, for example.} A similar assumption is made by \cite{breza2017using}. 
%(e.g. ) \aristide{(Aguirregabiria and Mira ECMA 2007, Brock Durlauf 2007 JoE with logit model, Tamer papers with airline market? They all need many small markets. Any identification paper would generally need many units that are independent)} \aristide{(Duflo Restud, Changes in Social Network? The paper formally estimates a network formation model but data match what we are saying.) \aristide{Duflo AER 2011 Peer effects, teacher incentives ?}.{\color{red} we need more references} 

%In the next section, we present the \emph{linear-in-means} model, which characterize the relationship between $\mathbf{y}_m$, $\mathbf{X}_m$, $\boldsymbol{\varepsilon}_m$ and $\mathbf{A}_m$.

\subsection{The Linear-in-Means Model}
In this section, we present the linear-in-means model \citep{manski1993identification,bramoulle2009identification}, arguably the most widely used model for studying peer effects in networks \citep[see][for a recent review]{bramoulle2019peer}.

Let $\mathbf{G}_m=f(\mathbf{A}_m)$, the $N_m\times N_m$ \emph{interaction matrix} for some function $f$. Unless otherwise stated, we assume that $\mathbf{G}_m$ is a row-normalization of the adjacency matrix $\mathbf{A}_m$.\footnote{In such a case, $g_{ij,m}=a_{ij,m}/n_{i,m}$ whenever $n_{i,m}>0$, whereas $g_{ij,m}=0$ otherwise.} Most of our results hold for any function $f$.

We focus on the following model:
\begin{equation}\label{eq:linearinmean}
\mathbf{y}_m=c\mathbf{1}_m+\mathbf{X}_m\boldsymbol{\beta}+\alpha\mathbf{G}_m\mathbf{y}_m+{\mathbf{G}_m\mathbf{X}_m}\boldsymbol{\gamma}+\boldsymbol{\varepsilon}_m,
\end{equation}
where $\mathbf{1}_m$ is a $N_m-$dimensional vector of $1$'s.
%where $\mathbf{y}$ is a vector of an outcome of interest (e.g. academic achievement), $c$ is a constant, $\mathbf{1}$ is a vector of ones, $\mathbf{X}$ is a matrix of observable characteristics (e.g. age, gender...), and $\boldsymbol{\varepsilon}$ is a vector of errors.\footnote{Note that \cite{boucher2020binary} show that (\ref{eq:linearinmean}) is valid (coherent, complete, and microfounded), even when $y_i$ is binary.}
The parameter $\alpha$ therefore captures the impact of the average outcome of one's peers on their behavior (the endogenous peer effect). The parameter $\boldsymbol{\beta}$ captures the impact of one's characteristics on their behavior (the individual effects). The parameter $\boldsymbol{\gamma}$ captures the impact of the average characteristics of one's peers on their behavior (the contextual peer effects). For simplicity, we assume that the constant $c$ does not vary across $m$. However, our results hold when considering group-level fixed effects. % $c_m$. %Of course, these cannot be consistently estimated under Assumption \ref{as:manymarkets}, but it is possible to estimate the model in deviation with the group average in order to purge the effect of $c_m$. {\color{red} Footnote and/or references or see appendix for a longer discussion??}

We impose the following assumptions.
\begin{assumption}\label{as:alpha} $|\alpha|<1/\Vert \mathbf{G}_m\Vert$ for some submultiplicative norm $\Vert \cdot\Vert$, and all $m=1,...,M$.
\end{assumption}
\begin{assumption}\label{as:exonet} Exogeneity: $\mathbb{E}[\boldsymbol{\varepsilon}_m|\mathbf{X}_m,\mathbf{A}_m,\mathcal{A}_m]=\mathbf{0}$ for all $m=1,...,M$.
\end{assumption}





Assumption \ref{as:alpha} ensures that the model is coherent and that there exists a unique vector $\mathbf{y}_m$ compatible with (\ref{eq:linearinmean}). When $\mathbf{G}_m$ is row-normalized, $|\alpha|<1$ is sufficient.
Finally, Assumption \ref{as:exonet} implies that individual characteristics and the network structure are exogenous. While the exogeneity of the network is a strong assumption, we consider it as a benchmark and focus on the case in which the network is not perfectly observed. We now describe the network sampling process in more detail.


\subsection{Partial Network Information}\label{sec:partial}

In this paper, we relax the costly assumption that the adjacency matrix $\mathbf{A}_m$ is observed. We assume instead that sufficient information about the network (i.e., $\mathcal{A}_m$) is observed so that a network formation model can be estimated. The discussion below formalizes our assumptions about the relationship between $\mathcal{A}_m$ and $\mathbf{A}_m$. We start by describing the data-generating process for $\mathbf{A}_m$.

%More formally, we let $\mathcal{A}$ denote the observed information about the true network structure. That is, $\mathcal{A}$ is a function of the true network $\mathbf{A}$ and potentially of individuals' characteristics, i.e. there exist functions $\mathcal{F}_m$ such that $\mathcal{A}_m=\mathcal{F}_m(\mathbf{A}_m,\mathbf{X}_m)$. Thus, $\mathcal{A}_M$ in a sample of $M$ groups is drawn from $P(\mathcal{A}_M|\mathbf{A}_M,\mathbf{X}_M).$ We discuss important examples in Examples \ref{ex:sampled}--\ref{ex:ard} below.

We assume that for any group $m$, $P(\mathbf{A}_m|\mathbf{X}_m)=\Pi_{ij}P(a_{ij,m}|\mathbf{X}_m)$, where
\begin{equation}\label{eq:gennetfor}
P(a_{ij,m}|\mathbf{X}_m)=\frac{\exp\{a_{ij,m}Q(\boldsymbol{\rho}_0,\mathbf{w}_{ij,m})\}}{1+\exp\{Q(\boldsymbol{\rho}_0,\mathbf{w}_{ij,m})\}}, 
\end{equation}
and where $Q$ is some known function that is twice continuously differentiable in $\boldsymbol{\rho}$, and $\mathbf{w}_{ij,m}=\mathbf{w}_{ij,m}(\mathbf{X}_m)$ is a vector of observed characteristics for the pair $ij$ in group $m$.\footnote{Throughout, $P$ refers to the probability notation. Note that by construction, links are only defined between individuals of the same group so the probability that individuals from different groups are linked is zero.}

We focus on network formation models that are conditionally independent across links: $P(\mathbf{A}_m|\mathbf{X}_m)=\Pi_{ij}P(a_{ij,m}|\mathbf{X}_m)$. This notably excludes many models of strategic network formation such as the ones in \cite{mele2017} and \cite{de2018identifying}. This is a strong assumption that deserves some discussion. 

As we describe below (see Assumption \ref{as:partial}), our strategy depends on our ability to estimate the network formation model without observing the entire network structure. In models that allow for dependence across links (e.g., Exponential Random Graph Models, henceforth ERGM), the feasibility of this strategy is highly context-dependent. Thus, for simplicity (and clarity) of the analysis in the main text, we restrict our attention to network formation models that are conditionally independent across links. We however note that our methodology can be adapted to more general network formation models.

In Online Appendix \ref{app:specific_netfor}, we further discuss how this can be done for a few specific network formation processes. First, we discuss the model in \cite{graham2017econometric}, which is conditionally independent across links but accounts for unobserved degree heterogeneity. We show that his model can be used, provided that the degree distribution is observed.\footnote{Note that the degree distribution can be obtained from survey questions by simply asking individuals about the number of links they have.} Second, we discuss ERGM. We explain how our setup can be adapted to the model in \cite{boucher2017my}, in which the probability of a link is a function of the individuals' degree. Similarly to \cite{graham2017econometric}, the estimation also requires the observation of the degree distribution. We also discuss the estimation of more general ERGM and their implication for survey design in the Online Appendix \ref{sec:app_ergm}. We now present our main assumption.
\begin{assumption}[Partial Network Information]\label{as:partial} Given $\lbrace \mathcal{A}_m,\mathbf{X}_m\rbrace_{m=1}^M$ and the parametric model (\ref{eq:gennetfor}), there exists an estimator $\hat{\boldsymbol{\rho}}_M$, such that $\sqrt{M}(\hat{\boldsymbol{\rho}}_M-\boldsymbol{\rho}_0)\rightarrow_d N(\boldsymbol{0},\boldsymbol{V}_{\boldsymbol{\rho}})$ as $M\rightarrow\infty$.% Moreover, the derivatives of $P(a_{ij,m}|\boldsymbol{\rho})$ with respect to $\boldsymbol{\rho}$ are bounded uniformly in $i,j$ and $m$. \aristide{This introduces a new notation we didnt define. Maybe be, in \eqref{eq:gennetfor}, write $P(a_{ij,m}|\mathbf{X}_m) = P(a_{ij,m}|\mathbf{X}_m, \boldsymbol{\rho}_0) = ....$. In this case, it would be clear what $P(a_{ij,m}|\mathbf{X}_m, ~\boldsymbol{\rho})$ means here.}{\color{red} I suggest to add another regularity condition in the proof of theorem 1.}
\end{assumption}

Assumption \ref{as:partial} implies that the dependence between $\mathcal{A}_m$ and $\mathbf{A}_m$ is strong enough so that, using (\ref{eq:gennetfor}), the researcher can estimate the data generating process for $\mathbf{A}_m$. We can then use this information in order to obtain an estimator of the conditional distribution of $\mathbf{A}_m$.

\begin{definition}\label{def:estimator}
     A consistent estimator of the distribution of the true network for some function $\kappa$ is a probability distribution $\hat{P}(\mathbf{A}_m|\hat{\boldsymbol{\rho}},\mathbf{X}_m,\kappa(\mathcal{A}_m))$ such that $\sup_m\Vert \hat{P}(\mathbf{A}_m|\hat{\boldsymbol{\rho}},\mathbf{X}_m,\kappa(\mathcal{A}_m))-{P}(\mathbf{A}_m|\mathbf{X}_m,\kappa(\mathcal{A}_m))\Vert\rightarrow_p 0$ as $M\rightarrow\infty$.
\end{definition}

Note that here, the partial information $\mathcal{A}_m$ is used twice. First, in order to estimate $\boldsymbol{\rho}$ (Assumption \ref{as:partial}), and second, to construct a consistent estimator of the distribution of the true network (Definition \ref{def:estimator}). For this second use, we allow the researcher to consider only part of the information in $\mathcal{A}_m$.

Indeed, the function $\kappa$ controls how much information in $\mathcal{A}_m$ is used in order to complement the information obtained by estimating the network formation process in Equation \ref{eq:gennetfor}. Two important polar cases are the identity function $\kappa(\mathcal{A}_m)=\mathcal{A}_m$ implying that all the information in $\mathcal{A}$ is used, and the constant function $\kappa(\mathcal{A}_m)=\kappa_0$ for all $\mathcal{A}_m$ in which no information on $\mathcal{A}$ is used. Although our methodology is valid for any $\kappa$, the choice of $\kappa$ may strongly affect the identification and precision of our estimators.

When $\kappa$ is the identify function, the estimator is obtained from Bayes' rule:
\begin{equation}\label{eq:Bayes}
\hat{P}(\mathbf{A}_m|\hat{\boldsymbol{\rho}},\mathbf{X}_m,\mathcal{A}_m)=\frac{P(\mathcal{A}_m|\mathbf{X}_m,\mathbf{A}_m)P(\mathbf{A}_m|\hat{\boldsymbol{\rho}},\mathbf{X}_m)}{P(\mathcal{A}_m|\mathbf{X}_m)}.
\end{equation}
However, in some contexts, such a quantity may be hard to compute, depending on the nature of the information in $\mathcal{A}_m$. A solution, therefore, could be to disregard the information in $\mathcal{A}$ and use: $$\hat{P}(a_{ij,m}|\hat{\boldsymbol{\rho}},\mathbf{X}_m)=\frac{\exp\{a_{ij,m}Q(\hat{\boldsymbol{\rho}},\mathbf{w}_{ij,m})\}}{1+\exp\{Q(\hat{\boldsymbol{\rho}},\mathbf{w}_{ij,m})\}}.
$$
In that case, the precision of the estimator strongly depends on the network formation process in (\ref{eq:gennetfor}). Thus, the loss in precision is context-dependent. In particular, it depends on the heterogeneity in the probability of link formation implied by (\ref{eq:gennetfor}), and on the specificity about $\mathbf{A}_m$ that is contained in $\mathcal{A}_m$.






%Importantly, it should be noted that even if the econometrician has access to a consistent estimator of the distribution of the true network, it \emph{does not} imply that they could simply proxy $\mathbf{G}_m$ in (\ref{eq:linearinmean}) using a draw $\tilde{\mathbf{G}}_m$ from the distribution $\hat{P}(\mathbf{G}_m)$. The reason is that for any vector $\mathbf{z}_m$, $\tilde{\mathbf{G}}_m\mathbf{z}_m$ generally does not converge to ${\mathbf{G}}_m\mathbf{z}_m$ as the number of individuals $N$ goes to infinity. In other words, knowledge of $\hat{P}(\mathbf{G}_m)$ and $\mathbf{z}_m$ is not sufficient to obtain a consistent estimator of $\mathbf{G}_m\mathbf{z}_m$. To see why, note that $(\mathbf{G}_m\mathbf{z}_m)_i=\sum_{j=1}^{N_m}g_{ij}z_{j,m}$, and, under Assumption \ref{as:manymarkets}, $N_m$ is bounded. %the set of $j$, such that $g_{ij}\neq 0$, is bounded; thus, a consistent estimator of $P(\mathbf{G})$ is not sufficient to obtain a consistent estimator of $\mathbf{GX}$.% This is also true under the alternative assumptions in \cite{lee2004asymptotic} and \cite{de2018identifying},\footnote{\cite{lee2004asymptotic}  requires that $\mathbf{G}$ be bounded in row- and column-sums (in absolute value), whereas \cite{de2018identifying} assume that $\mathbf{A}$ is bounded in row-sums.}, but it contrasts from models based on a large network asymptotic framework (e.g. \cite{auerbach2022identification}).

We specifically discuss three leading examples in which Assumption \ref{as:partial} holds and focus on how $\hat{P}(\mathbf{A}_m|\hat{\boldsymbol{\rho}},\mathbf{X}_m,\kappa(\mathcal{A}_m))$ is constructed: \emph{sampled networks} (Example \ref{ex:sampled}), \emph{censored networks }(Example \ref{ex:censored}), and \emph{misclassified network links} (Example \ref{ex:misclass}). 

However, as discussed, the many-markets asymptotic framework (see Assumption \ref{as:manymarkets}) is restrictive and {does not hold} in some contexts such as when researchers have access to \emph{aggregated relational data} (see the Online Appendix \ref{sec:ardsetting}). In Section \ref{sec:genestim}, we present a Bayesian estimator which uses the same structure as the one presented here but is valid in finite samples.

\begin{example}[Sampled Networks]\label{ex:sampled}
Suppose that we observe the realizations of $a_{ij}$ for a random sample of $m$ pairs \cite[e.g.,][]{chandrasekhar2011econometrics}. Here $\mathcal{A}_m$ is simply a list of sampled pairs: $\mathcal{A}_{m}=\{a_{ij,m}\}_{ij\text{ is sampled}}$ \citep[see e.g.,][for concrete example]{conley2010learning}. Consider the following simple network formation model: $$P(a_{ij,m}=1|\mathbf{X}_m)=\frac{\exp\{\mathbf{w}_{ij,m}\boldsymbol{\rho}\}}{1+\exp\{\mathbf{w}_{ij,m}\boldsymbol{\rho}\}}.$$ In this case, a simple logistic regression on the subset of sampled pairs provides a consistent estimator of $\boldsymbol{\rho}$ since pairs of individuals for which $a_{ij,m}$ is observed is random.

In this simple framework, the linking status of sampled pairs of individuals is known. As such it is natural to define $\kappa$ as the identity map, which leads to the estimator\break $\hat{P}(a_{ij,m}|\hat{\boldsymbol{\rho}},\mathbf{X}_m,\mathcal{A}_m)=a_{ij,m}$ for all sampled pairs $ij$, and
$\hat{P}(a_{ij,m}|\hat{\boldsymbol{\rho}},\mathbf{X}_m, \mathcal{A}_m)={\exp\{\mathbf{w}_{ij,m}\hat{\boldsymbol{\rho}}\}}/\break({1+\exp\{\mathbf{w}_{ij,m}\hat{\boldsymbol{\rho}}\}})$ otherwise. In essence, sampled pairs are used to estimate the network formation model, which is then used in order to predict the probability of a link for pairs that are not sampled.
\end{example}

\begin{example}[Censored Network Data]\label{ex:censored}
As discussed in \cite{griffith2019namefriends}, network data is often censored. This typically arises when surveyed individuals are asked to name only $T>1$ links (among the $N_m$ possible links they may have). Here, $\mathcal{A}_m$ can be represented by an $N_m\times N_m$ binary matrix $\mathbf{A}_m^{obs}$ which takes value $a_{ij,m}=1$ if $i$ nominated $j$, and $0$ otherwise. 
Consider the same simple model as in Example \ref{ex:sampled}:
$$P(a_{ij,m}=1|\mathbf{X}_m)=\frac{\exp\{\mathbf{w}_{ij,m}\boldsymbol{\rho}\}}{1+\exp\{\mathbf{w}_{ij,m}\boldsymbol{\rho}\}}.$$ 
In Section \ref{sec:addhealth} and the Online Appendix \ref{sec:manski2}, we present how to estimate $\boldsymbol{\rho}$ in detail. Here, we discuss how to obtain the estimator $\hat{P}(\mathbf{A}_{m}|\hat{\boldsymbol{\rho}},\mathbf{X}_m,\kappa(\mathcal{A}_m))$ given $\hat{\boldsymbol{\rho}}$. Note that $\hat{P}(a_{ij,m}=1|\hat{\boldsymbol{\rho}},\mathbf{X}_m,a_{ij,m}^{obs}=1)=1$ because observed links necessarily exist. Second, note also that for any individual $i$, such that $n_{i,m}<T$, we have $\hat{P}(a_{ij,m}|\hat{\boldsymbol{\rho}},\mathbf{X}_m,a_{ij,m}^{obs})=a_{ij}^{obs}$ for all $j$, as their network data are not censored.

Thus, the structural model is only used to obtain the probability of links that are not observed for individuals whose links are potentially censored, i.e., $\hat{P}(a_{ij,m}=1|\hat{\boldsymbol{\rho}},\mathbf{X}_m,a_{ij,m}^{obs}=0)={\exp\{\mathbf{w}_{ij,m}\hat{\boldsymbol{\rho}}\}}/({1+\exp\{\mathbf{w}_{ij,m}\hat{\boldsymbol{\rho}}\}})$ for all $ij$, such that $n_i\geq T$.

\end{example}

\begin{example}[Misclassification]\label{ex:misclass}
\cite{hardy2019estimating} study cases in which networks are observed but may include misclassified links (i.e., false positives and false negatives). Here, $\mathcal{A}_m$ can be represented by an $N_m\times N_m$ binary matrix $\mathbf{A}_m^{mis}$. Consider the same simple model as in Example \ref{ex:sampled} and \ref{ex:censored}:
$$P(a_{ij,m}=1|\mathbf{X}_m)=\frac{\exp\{\mathbf{w}_{ij,m}\boldsymbol{\rho}\}}{1+\exp\{\mathbf{w}_{ij,m}\boldsymbol{\rho}\}}.$$ 
The (consistent) estimation $\boldsymbol{\rho}$ in such a context follows directly from the existing literature on misclassification in binary outcome models, e.g., \cite{hausman1998misclassification}. In this context, the simplicity of the sampling scheme allows to consider the identity map $\kappa(\mathcal{A}_m)=\mathcal{A}_m$. The estimator for the distribution of the true network can be obtained using Bayes' rule. We consider this case in our Monte Carlo simulations in Section \ref{sec:montecarlo}. %When $a_{ij,m}^{mis} = 0$, $P(a_{ij,m} = 1|a_{ij,m}^{mis} = 0, \mathbf{X}_m) = \frac{\rho_2P_{ij,m}}{\rho_2P_{ij,m} + (1 - \rho_1)(1 - P_{ij,m})}$, and when $a_{ij,m}^{mis} = 1$, $P(a_{ij,m} = 1|a_{ij,m}^{mis} = 1, \mathbf{X}_m) = \frac{(1 - \rho_2)P_{ij,m}}{(1 - \rho_2)P_{ij,m} + \rho_1(1 - P_{ij,m})}$, where $P_{ij,m} = P(a_{ij,m}=1|\mathbf{X}_m)$.
\end{example}

==> RestatRR1/summary_RR_2.tex <==
\section*{Summary of the changes}

\begin{enumerate}
    \item \textbf{Definitions and implicit assumptions:} We restructured the text in order to formalize definitions and make implicit assumptions explicit and more formal.
    
    In particular, we now state explicitly that all random variables are defined at the group level, and are independent across groups (Assumption 1). We also explicitly state that the network is assumed to be exogenous (Assumption 4). To ensure that there is no confusion regarding the asymptotics, we also index all variables with the group subscript $m$.

    We now formally define the ``estimator of the network formation process'' (Definition 1) and clearly describe that the partial information about the group structure is used for 1) estimating $\boldsymbol{\rho}$ (Assumption 5) and 2) Constructing the estimator of the network formation process (Definition 1).
    
    \item \textbf{Theorem 1:} Following comments from R1 and R2 in particular, Theorem 1 now states that the SGMM estimator is asymptotically normal. To achieve this result, we slightly strenghten our Assumption 5 to ensure that the first stage is normally distributed. This covers all of our examples so the loss is, in our view, minimal.

    We also have completely rewritten the discussion preceding and following the Theorem. (That is, the entire Section 3.) We now clearly describe how the moment condition (that uses three distinct draws) is built as a bias-corrected, simulated, extension of the linear GMM in \cite{bramoulle2009identification}. We also discuss the identification of the estimator in more details.

    We also completely rewrote the proof of the theorem following R1's suggestions. In particular, it is now organized around lematta and regularity conditions are rigorously checked.

    \item \textbf{Aggregated Relational Data (ARD):} We removed all of the analysis based on ARD and moved it to the Online Appendix. 
    
    Given that we had to conform with the 45 pages limit imposed by the journal (see below), we felt that the benefit of including it was not worth it. Estimators based on ARD are complex and take time/space to properly discuss. Moreover, Assumption 5 (specifically the asymptotics) fails for these models since consistency can only be achieved within groups (which we assume are bounded, see Assumption 1).
    
    The argument we used in the previous version of the manuscript was that 1) simulation showed that our SGMM had nonetheless good finite sample properties when applied to ARD, and that 2) The Bayesian estimator (which is valid in finite sample) could we coupled with ARD.

    Given the comments from all three referees, we realized that this was not clearly exposed and that the discussions around ARD created confusion, and were distracting from the main message of the paper.

    \item \textbf{Formatting:} Given the 45 pages limit (using the formatting guideline), we restructured the manuscript as follows:
    \begin{enumerate}
        \item As mentioned, the ARD analysis is now moved to the Online Appendix.
        \item The proof of the lematta on which Theorem 1 depends are presented in the Online Appendix since they mostly show technical steps of the proof (such as uniform convergence and stochastic equicontinuity) and are not the main contribution of this paper. Lemmatta are nonetheless formally stated in the proof of Theorem 1 in the (regular) Appendix.

        One exception is Lemma 1, for which the proof is presented in the (regular) Appendix. This lemma is central as is shows that the moment condition implied by the empirical moment function in Theorem 1 is valid.

        \item The discussion related to cases for which $\mathbf{Gy}$ and/or $\mathbf{GX}$ are observed is now only presented in the Online Appendix. In particular, we now focus our simulations (in the main text) around the distinction between false positive and false negative errors to the network structure in the context of Theorem 1. Moreover, we believe that the way we rewrote the proof of Theorem 1, as well as our discussion in Section 3, clarifies why results of Theorem 1 extend directly to cases for which $\mathbf{Gy}$ and/or $\mathbf{GX}$ are observed.
        
        \item Detailed simulation results are now presented in the Online Appendix.
        \item Discussions of alternative network formation models (in particular the ones in \cite{graham2017econometric} and \cite{boucher2017my} are also presented in the Online Appendix. Similarly to the argument for ARD, these models take time/space to be properly discussed and distract from the main messages of the paper.
        \item Technical details relating to our MCMC are presented in the Online Appendix. We made sure, in the text, to clarify that our MCMC is a Metropolis-Hastings and to explain which parts are standard, and which parts are not.
        \item Details of the Application, including summary statistics, complete estimation results as well as counterfactual simulation for the key player analysis are now presented in the Online Appendix.
    \end{enumerate}
\end{enumerate}

==> archives/bkp/iv-bkp.tex <==
\section{Simulated Generalized Method of Moment Estimators}\label{sec:iv}

In this section, we present estimator based on a Simulated Generalized Method of Moments. The key observation underlying our approach is that it is not necessary to observe the complete network structure to observe $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$. For example, one could simply obtain ${\mathbf{Gy}}$ from survey data, ``What is the average value of your friends' $y$?''

However, even observing $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$, the model (\ref{eq:linearinmean}) cannot be simply estimated using simple linear regression. The reason is that ${\mathbf{Gy}}$ is endogenous; thus, a linear regression would produce biased estimates (e.g. \cite{manski1993identification}, \cite{bramoulle2009identification}).

The typical instrumental approach to deal with this endogeneity is to use instruments based on the structural model, i.e. instruments constructed using second-degree peers (e.g. $\mathbf{G}^2\mathbf{X}$, see \cite{bramoulle2009identification}). These are less likely to be found in survey data. Indeed, we could doubt the informativeness of questions such as, ``What is the average value of your friends' average value of their friends' $x$?''

However, the above discussion is encouraging. When researchers observe $[\mathbf{y}, \mathbf{X}]$ as well as $[{\mathbf{GX}},{\mathbf{Gy}}]$, information about the network is only used as a mean to construct a valid instrument, e.g. following \citet{bramoulle2009identification}. Then, if $\mathbf{GX}$ and $\mathbf{Gy}$ are observed, the estimation of peer effects is possible using any exogeneous predictor of the true network structure, as in \cite{kelejian2014estimation}, \cite{konig2019r} and \cite{lee2020key}.\footnote{See Proposition \ref{prop:all_observed} of the Online Appendix \ref{sec:appendix_otherresults} for a formal statement}

The problem is more challenging when $\mathbf{Gy}$ and $\mathbf{GX}$ are not observed. To simplify the notation, for the remainder of this section, we define $\lbrace \dot{\mathbf{G}}^{(r)}\rbrace_{r=1}^R$, $\lbrace \ddot{\mathbf{G}}^{(s)}\rbrace_{s=1}^S$ and $\lbrace \dddot{\mathbf{G}}^{(t)}\rbrace_{t=1}^T$ as sequences of independent draws from $\hat{P}(\mathbf{G})$. We will also let $\dot{\mathbf{G}}$, $\ddot{\mathbf{G}}$, and $\dddot{\mathbf{G}}$ be single independent draws from $\hat{P}(\mathbf{G})$.

Before presenting our estimation strategy, we want to emphasize that we cannot simply proxy $\mathbf{Gy}$ and $\mathbf{GX}$ using draws form $\hat{P}(\mathbf{G})$. To see why, consider the simple case for which $\boldsymbol{\gamma}=\mathbf{0}$, so the observation of $\mathbf{GX}$ is inconsequential. We have, substituting $\mathbf{Gy}$ with $\ddot{\mathbf{G}}\mathbf{y}$:
$$
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\ddot{\mathbf{G}}\mathbf{y}+[\boldsymbol{\eta}+\boldsymbol{\varepsilon}],
$$
where $\boldsymbol{\eta}=\alpha[\mathbf{G}-\ddot{\mathbf{G}}]\mathbf{y}$ is the error due to the approximation of $\mathbf{Gy}$ by $\ddot{\mathbf{G}}\mathbf{y}$. Importantly, the approximation error does \emph{not} vanish as $N$ grows, due to the fact that individuals belong to bounded groups (see Assumption \ref{as:manymarkets}).\footnote{As opposed, for example, to the context studied by \cite{auerbach2019measuring}.} Moreover, since $\mathbf{y}$ is a function of $\mathbf{G}$ (but not of $\ddot{\mathbf{G}}$), we typically have $\mathbb{E}(\mathbf{Gy})_i|\mathbf{z}_i\neq\mathbb{E}(\ddot{\mathbf{G}}\mathbf{y})_i|\mathbf{z}_i$ for some vector of instruments $\mathbf{z}_i$ and all $i$.


In Proposition \ref{prop:bias_nocontext} of the Online Appendix \ref{sec:appendix_otherresults}, we show, using an argument very similar to \cite{andrews2017measuring}, that the asymptotic bias induced by $\mathbb{E}\eta_i|\mathbf{z}_i\neq 0$ can be bounded, and simulations show that it can be very small for carefully constructed vectors of instruments, which can be useful in practice.

In any case, in our main result below, we show that we can include the bias directly in the moment function, which provides a consistent estimator of $\boldsymbol{\theta}$.

\subsection{Main Result}
Let $\tilde{\boldsymbol{\theta}}=[c,\boldsymbol{\beta}',\boldsymbol{\gamma}']'$. We maintain Assumptions \ref{as:alpha}--\ref{as:partial} and impose the regularity Assumptions \ref{as:regularity} and \ref{as:nonsingular}, as well as the identification Assumptions \ref{as:convex} and \ref{as:globalmin} presented in Appendix.

\begin{theorem}[SGMM]\label{prop:non_observed} $ $

[Conditions] Let $\dot{\mathbf{Z}}^{(r)}=[\mathbf{1},\mathbf{X},\dot{\mathbf{G}}^{(r)}\mathbf{X},(\dot{\mathbf{G}}^{(r)})^2\mathbf{X},(\dot{\mathbf{G}}^{(r)})^3\mathbf{X},...]$ and $\ddot{\mathbf{V}}^{(s)}=[\mathbf{1},\mathbf{X},\ddot{\mathbf{G}}^{(s)}\mathbf{X}]$. Consider also the following (simulated) moment function:
\begin{equation}\label{eq:moment}
\frac{1}{RST}\sum_{r=1}^R\sum_{s=1}^S\sum_{t=1}^T\dot{\mathbf{Z}}^{(r)\prime}_i\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})_i\left(\mathbf{y}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}\ddot{\mathbf{V}}^{(s)}\tilde{\boldsymbol{\theta}}\right)\right]
\end{equation}

[Result] For any positive integers $R$, $S$ and $T$, the (simulated) GMM estimator based on (\ref{eq:moment}) is consistent. Moreover, if the network formation model (\ref{eq:gennetfor}) is estimated using a m-estimator, the GMM estimator based on (\ref{eq:moment}) is asymptotically normal for $R,S,T\rightarrow\infty$, i.e.  $\sqrt{N}(\hat{\boldsymbol{\theta}}-\boldsymbol{\theta}_0)\overset{d}{\to}N(\mathbf{0},\mathbf{V})$, where $\mathbf{V}$ is of the usual sandwish form, clustered at the group level and formally defined in the Appendix.
\end{theorem}

Theorem \ref{prop:non_observed} presents conditions for the consistency and asymptotic normality of our two-steps estimator. In particular, our estimator is somewhat half way between standard simulated GMM and simulated MLE \citep{gourieroux1996simulation} in the sense that consistency holds for a finite number of simulations, while asymptotic normality only holds as the number of simulations goes to infinity. We discuss consistency and asymptotic normality in detail below.

\subsubsection{Consistency}

%The term $\Delta\boldsymbol{\theta}^*$ is introduced due to the fact the our moment condition is equal to zero only asymptotically, and it therefore allows to center the distribution of $\hat{\boldsymbol{\theta}}$ for finite $N$. Similar corrections can be found for penalized likelihood models (e.g. \cite{fan2001variable}, \cite{fan2004nonconcave}, \cite{dzemski2019empirical})

Similar to standard methods of simulated moments (e.g. \cite{gourieroux1993simulation}), the estimation is consistent even for a finite number of simulations (i.e. $R$, $S$, and $T$ are finite). Our estimator therefore does not suffer from the curse of dimensionality faced by \cite{chandrasekhar2011econometrics}.\footnote{The unconditional moment condition in \cite{chandrasekhar2011econometrics} is based on the (Monte Carlo) integration of the moment condition $\mathbb{E}(\mathbf{Z}^{(s)\prime}\boldsymbol{\varepsilon}|\mathbf{G})$ over $\mathbf{G}$. Suppose that there are $m$ pairs of individuals with unknown link status, there would be $2^m$ network structures to integrate from.}

To understand the intuition behind the use of the moment function (\ref{eq:moment}), let us replace $\mathbf{y}=(\mathbf{I}-\alpha\mathbf{G})^{-1}(\mathbf{V}\tilde{\boldsymbol{\theta}}+\boldsymbol{\varepsilon})$ in equation (\ref{eq:moment}). In doing so, we can rewrite the term inside the triple summation in (\ref{eq:moment}) as a sum of two terms. First, $\dot{\mathbf{Z}}^{(r)\prime}_i\boldsymbol{\varepsilon}_i$, which would be the standard moment function if $\mathbf{G}$ was observed (e.g. \cite{bramoulle2009identification}), and second:
\begin{equation}\label{eq:bias_corr}
\dot{\mathbf{Z}}^{(r)\prime}_i\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})_i\left((\mathbf{I}-\alpha{\mathbf{G}})^{-1}{\mathbf{V}}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}\ddot{\mathbf{V}}^{(s)}\right)\tilde{\boldsymbol{\theta}}\right].
\end{equation}
That second term can be viewed as the bias-correction term of the moment function.

We show that the expectation both terms are equal to $0$ as $N$ grows to $\infty$. For the first term, this is true since the simulated network is exogenous. For the second term, this is true because $\mathbf{G}$, $\dot{\mathbf{G}}$, $\ddot{\mathbf{G}}$ and $\dddot{\mathbf{G}}$ are asymptotically drawn from the same distribution.

For the special case in which $\mathbf{G}$ is observed, one could substitute $\dot{\mathbf{G}}^{(r)}=\ddot{\mathbf{G}}^{(s)}=\dddot{\mathbf{G}}^{(t)}=\mathbf{G}$ for all $r,s,t$ and the first term would simply be $\mathbf{Z}'_i\boldsymbol{\varepsilon}_i$, while the second term would be exactly equal to $\mathbf{0}$.

Note that Theorem \ref{prop:non_observed} is valid whether or not $\mathbf{Gy}$ and $\mathbf{GX}$ are observed since the moment function (\ref{eq:moment}) does not use information on $\mathbf{Gy}$ or $\mathbf{GX}$. It is of course possible to include this additional information, if either one is observed.

For example, assume that $\mathbf{GX}$ is observed, and replace $\ddot{\mathbf{V}}$ with $\mathbf{V}$ in (\ref{eq:bias_corr}). After some algebra, we obtain: \begin{equation}\label{eq:gxobswrong}
    \dot{\mathbf{Z}}^{(r)\prime}_i\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})_i(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}[\alpha(\mathbf{G}-\ddot{\mathbf{G}})\mathbf{y}]\right],
\end{equation}
plus a term that is equal to zero in expectation.

We can show that the last term in bracket corresponds to the source of the asymptotic bias due to the approximation error of $\mathbf{Gy}$ by $\ddot{\mathbf{G}}\mathbf{y}$ (see Proposition \ref{prop:bias_nocontext} of the Online Appendix). While Equation (\ref{eq:gxobswrong}) cannot directly be substituted for (\ref{eq:moment}) in Theorem \ref{prop:non_observed}, it is possible to construct moment functions for the particular cases for which $\mathbf{GX}$ or $\mathbf{Gy}$ are observed. These can be found in Corollary \ref{prop:GXobs} and \ref{prop:Gyobs} of the Online Appendix.

\subsubsection{Asymptotic Normality}
The asymptotic variance $\mathbf{V}$ in Theorem \ref{prop:non_observed} includes the sampling uncertainty, the estimating uncertainty of $\hat{\boldsymbol{\rho}}$, as well as the simulating uncertainty (which decreases as $R$, $S$ and $T$ grow). The equation for the asymptotic variance is also valid if the network formation model is not estimated using a m-estimator, but in that case, we can no longer guarantee the asymptotic normality of the estimator.

Indeed, recall that Assumption \ref{as:partial} only imposes the consistency of $\hat{\boldsymbol{\rho}}$ and does not discuss the convergence rate or asymptotic framework in details. Many network formation models, such as the ones described in Examples \ref{ex:sampled}, \ref{ex:censored} and \ref{ex:misclass}, can be written as m-estimators, and as such, asymptotic normality follows under classical assumptions (see e.g. \cite{cameron2005microeconometrics} Section 6.6).

However, researchers may also be interested in network formation model for which the asymptotic properties are less well understood. This is the case for latent space models based on ARD (see Example \ref{ex:ard}). As discussed in Section \ref{sec:ard}, \cite{alidaee2020recovering} propose a penalized regression, while \cite{breza2017using} propose a Bayesian estimator. Neither estimator can directly be written as a m-estimator and the convergence rates in a many-networks asymptotic framework (see our Assumption \ref{as:manymarkets}) as still not well understood.

That said, one can always use a bootstrap procedure to characterize sampling uncertainty, which in the case of ARD is computationally feasible thanks to the estimator proposed by \cite{alidaee2020recovering}, which we discuss in Section \ref{sec:ard}. Alternatively, the Bayesian estimator proposed by \cite{breza2017using} produces draws from the posterior distribution of $\boldsymbol{\rho}$ which can be used to characterize the sampling uncertainty of the first stage even if the asymptotic normality of the second stage cannot be guaranteed.

The results of this Section show that the estimation of (\ref{eq:linearinmean}) is possible, even with very limited information about the network structure. In Section \ref{sec:ard}, we study the finite sample properties of our approach using network formation models estimated on aggregated relational data.

\subsection{Finite Sample Performance Using ARD}\label{sec:ard}
In this section, we study the small sample performance of the estimator presented in Section \ref{sec:iv} when the researcher only has access to ARD (as in Example \ref{ex:ard}). First, we simulate network data using the model proposed by \cite{breza2017using} and simulate outcomes using the linear in means model (\ref{eq:linearinmean}) conditional on the simulated networks. Second, we estimate the network formation model using the Bayesian estimator proposed by \cite{breza2017using} (yielding $\hat{\boldsymbol{\rho}}_B$), as well as using the classical estimator proposed by \cite{alidaee2020recovering} (yielding $\hat{\boldsymbol{\rho}}_A$). Third, we estimate the linear-in-means model, using our the estimators presented in Proposition \ref{prop:bias_nocontext} and Theorem \ref{prop:non_observed}, based on $\hat{\boldsymbol{\rho}}_A$ and $\hat{\boldsymbol{\rho}}_B$.

Recall that
\begin{equation}\label{eq:ard}
P(a_{ij}=1)\propto\exp\{\nu_i+\nu_j+\zeta \mathbf{z}_i'\mathbf{z}_j\},    
\end{equation}
where $\nu_i$, $\nu_j$, $\zeta$, $\mathbf{z}_i$, and $\mathbf{z}_j$ are not observed by the econometrician but follow parametric distributions. We refer the interested reader to \cite{mccormick2015latent}, \cite{breza2017using}, and \cite{breza2019consistently} for a formal discussion of the model, including its identification and consistent estimation. %Here, we discuss the intuition using a simple analogy.

%Suppose that individuals are located according to their geographical position on Earth. Suppose also that there are a fixed number of cities on Earth in which individuals can live. The econometrician does not know the individuals' locations on Earth nor do they know the location of the cities. In model (\ref{eq:ard}), $\mathbf{z}_i$ represent $i$'s position on Earth. However, the econometrician has access to ARD for a subset of the population, i.e. answers to questions such as, ``How many of your friends live in city $A$?''

%To understand the intuition behind the identification of the model, consider the following example: suppose that individual $i$ has many friends living in city $A$. Then, city $A$ is likely located close to $i$'s location. Similarly, if many individuals have many friends living in city $A$, then city $A$ is likely a large city. Finally, if $i$ has many friends from many cities, $i$ likely has a large $\nu_i$.

To study the finite sample performance of our instrumental strategy in this context, we simulate 20 groups of 250 individuals each. Within each subpopulation, we simulate the ARD responses as well as a series of observable characteristics. The details of the Monte Carlo simulations can be found in the Online Appendix.

Importantly, the model in (\ref{eq:ard}) is based on a single population framework. Thus, the network formation model must be estimated separately for each of the 20 groups. With only 250 individuals in each group, we therefore expect significant small-sample bias.

We contrast the estimator proposed by \cite{breza2017using} with the one proposed by \cite{alidaee2020recovering}. Whereas \cite{breza2017using} present a parametric Bayesian estimator, \cite{alidaee2020recovering} propose a (nonparametric) penalized regression based on a low-rank assumption. One main advantage of their estimator is that it allows for a wider class of model and ensures that the estimation is fast and easily implementable.\footnote{The authors developed user-friendly packages in R and Python. See their paper for links and details.} Note, however, that their method only yields a consistent estimator of $\hat{P}(\mathbf{A})$ if the true network is effectively low rank.

Very intuitively, the low-rank assumption implies that linking probabilities were generated from a small number of parameters.%; for example, in the example above, knowing individuals' gregariousness parameters $\nu_i$ and city in which they live would allow a prediction of the linking probabilities.
Importantly, the model (\ref{eq:ard}) is not necessarily low rank; for example, if the individuals' locations on Earth (i.e. the $\mathbf{z}_i$'s) are uniformly distributed and there are only very few  large cities, then the model produced is not low rank and the method proposed by \cite{alidaee2020recovering} performs poorly. Intuitively, in such a case, the fact that individual $i$ lives in city $A$ poorly explains the linking probabilities. 

We compare the performance of both estimators as we vary the concentration parameter (that is, $\kappa$, see the Online Appendix for details). This has the effect of changing the \emph{effective rank} of the linking probabilities: increasing $\kappa$ decreases the effective rank.\footnote{We refer the interested reader to \cite{alidaee2020recovering} for a formal discussion of the effective rank and of its importance for their estimator.} We therefore expect the estimator proposed by \cite{alidaee2020recovering} to perform better for larger values of $\kappa$.

A summary of the results is presented in Tables \ref{tab:gx:obs:short} and \ref{tab:gx:unobs:short}. The complete results can be found in Tables \ref{tab:gx:obs:full} and \ref{tab:gx:unobs:full} of the Online Appendix. Table \ref{tab:gx:obs:short} presents the results for the special case where $\mathbf{GX}$ are observed in the data. The table displays the performance of the simple (biased) estimator in Proposition \ref{prop:bias_nocontext} and that of our simulated GMM (see Corollary \ref{prop:GXobs}) when the network formation model is estimated by \cite{breza2017using} and \cite{alidaee2020recovering}. 

When $\kappa=0$, the network formation is not low-rank. This disproportionately affects the estimator of \cite{alidaee2020recovering}. Although asymptotically biased, the performance of the IV in Proposition \ref{prop:bias_nocontext} is very good and even seems to outperform our SGMM when using the estimator proposed by \cite{alidaee2020recovering}. Moreover, the overidentification test points (on average) to a violation of the exclusion restriction.

When $\kappa=15$ the estimators proposed by \cite{breza2017using} and \cite{alidaee2020recovering} perform similarly and so do our estimators. Both the IV and SGMM estimators recover the true value of $\alpha$.

We now turn to the more general case where $\mathbf{GX}$ are not observed. Note that in that case, Proposition \ref{prop:bias_nocontext} does not apply. Table \ref{tab:gx:unobs:short} presents the performance of our SGMM estimator (Theorem \ref{prop:non_observed}) when the network formation process is estimated using the estimators proposed by \cite{breza2017using} and \cite{alidaee2020recovering}, as well as when we assume that the researcher knows the true distribution of the network.

We see that the performance of our estimator, is strongly affected by the quality of the first-stage network formation estimator. When based on either the estimator proposed by \cite{breza2017using} or \cite{alidaee2020recovering}, for $\kappa=0$ or $\kappa=15$, our SGMM estimator performs poorly.

This poor performance of our SGMM estimator in a context where both $\mathbf{Gy}$ and $\mathbf{GX}$ are unobserved was anticipated. This is due to two main reasons. \emph{First}, the consistency of the network formation estimator in \cite{breza2019consistently} holds as the size of each sub-population goes to infinity, while the consistency of our estimator holds as the number of (bounded) sub-populations goes to infinity. This should affect the performance of our estimator, when based on \emph{estimated} network formation models, but when based on the true distribution of the network.

\emph{Second}, as discussed in Example \ref{ex:ard}, ARD provides very little information about the realized network structure in the data (as opposed, for example, as for censoring issues, see Example \ref{ex:censored}). Then, if the true distribution is vague in the sense that most predicted probabilities are away from $0$ or $1$, we expect the estimation to be imprecise. This is what happens when $\kappa=15$, where our estimation based on the true distribution of the network is very imprecise, in a context where the network affects the outcome through both $\mathbf{Gy}$ and $\mathbf{GX}$.

In the next section, we present a likelihood based estimator, which uses more information on the data generating process of the outcome, in order to improve the precision of the estimation.


\renewcommand{\arraystretch}{.95}
\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD and observed $\bG\bX$} 
\label{tab:gx:obs:short}
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}ld{4}c}
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Parameter              & \multicolumn{2}{c}{Breza et al.} & \multicolumn{2}{c}{Alidaee et al.} \\
                       & \multicolumn{1}{c}{Mean}           & \multicolumn{1}{c}{Std. Dev}        & \multicolumn{1}{c}{Mean}            & \multicolumn{1}{c}{Std. Dev}         \\
 
\hline\\[-1.8ex] 
                      \multicolumn{5}{c}{$\kappa=0$}       \\\hline 
                       \hline\\[-1.8ex] 
                       
                        \multicolumn{5}{c}{IV (Proposition \ref{prop:bias_nocontext})}    \\
                       \\[-1.8ex] 
$\alpha = 0.4$         & 0.392              & (0.009)              & 0.372               & (0.027)               \\
\\[-1.8ex]
Sargan test            & 1.217              & (1.761)              & 7.779               & (10.386)              \\
F-test (Weak inst.)    & 4259.622           & (1140.825)           & 597.055             & (251.886)             \\\hline\\[-1.8ex] 

                       \multicolumn{5}{c}{SGMM (Corollary \ref{prop:GXobs})}                      \\
                       \\[-1.8ex]
                       
   $\alpha = 0.4$         & 0.392              & (0.010)               & 0.492               & (0.057)               \\                    
                       
                       
                       \hline\\
                                        \multicolumn{5}{c}{$\kappa=15$}      \\\hline 
                       \hline\\[-1.8ex] 
                       
                        \multicolumn{5}{c}{IV (Proposition \ref{prop:bias_nocontext})}    \\
                       \\[-1.8ex] 
$\alpha = 0.4$         & 0.400              & (0.007)              & 0.399               & (0.007)               \\
\\[-1.8ex]
Sargan test            & 1.063              & (1.496)              & 2.608               & (1.496)               \\
F-test (Weak inst.)    & 5306.551           & (1519.394)           & 1767.274            & (1519.394)            \\\hline\\[-1.8ex] 
                                        \multicolumn{5}{c}{SGMM (Corollary \ref{prop:GXobs})}                   \\                  \\[-1.8ex]                              $\alpha = 0.4$         & 0.400              & (0.009)              & 0.428               & (0.009)               \\
 
\bottomrule     
\end{tabular}
\begin{tablenotes}[para,flushleft]
\footnotesize Note: For each case, we generated 20 independent subnetworks of 250 individuals each. In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with a location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in the Online Appendix \ref{sec:ardsetting}. Predicted probabilities are computed using the mean of the posterior distribution. Sargan test is the statistic of the overidentification test. F-test is the Fisher-statistic of the Weak instruments test. We chose the weight associated with the nuclear norm penalty to minimize the RMSE through cross-validation. This value of $\lambda=600$ is smaller than the recommended value in \cite{alidaee2020recovering}. See Table \ref{tab:gx:obs:full} for the estimated values of the other parameters. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.
\end{tablenotes}
\end{threeparttable}
\end{table}




\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD and unobserved $\bG\bX$ (SGMM, Theorem \ref{prop:non_observed}) }
\label{tab:gx:unobs:short}
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}ld{4}cd{4}c}
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Parameter       & \multicolumn{2}{l}{Breza et al.} & \multicolumn{2}{l}{Alidaee et al.} & \multicolumn{2}{l}{True distribution} \\
                       & \multicolumn{1}{c}{Mean}           & \multicolumn{1}{c}{Std. Dev}        & \multicolumn{1}{c}{Mean}            & \multicolumn{1}{c}{Std. Dev}        & \multicolumn{1}{c}{Mean}            & \multicolumn{1}{c}{Std. Dev}       \\\hline\\[-1.8ex] 
                \multicolumn{7}{c}{$\kappa = 0$}                                                    \\
                \\[-1.8ex]
$\alpha = 0.4$  & 0.717          & (0.463)         & 0.700           & (0.268)          & 0.400            & (0.056)            
\\\hline\\
                 \multicolumn{7}{c}{$\kappa = 15$}                                                   \\
                 \\[-1.8ex]
$\alpha = 0.4$  & 0.603          & (0.069)         & 0.870           & (0.202)          & 0.434            & (0.394)            \\

\bottomrule     
\end{tabular}
\begin{tablenotes}[para,flushleft]
\footnotesize Note: For each case, we generated 20 independent subnetworks of 250 individuals each. In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with a location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in the Online Appendix. Predicted probabilities are computed using the mean of the posterior distribution. Sargan test is the statistic of the overidentification test. F-test is the Fisher-statistic of the Weak instruments test.  See Table \ref{tab:gx:unobs:full} for the estimated values of the other parameters. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.
\end{tablenotes}
\end{threeparttable}
\end{table}
\renewcommand{\arraystretch}{1}


==> archives/bkp/iv_old__1_.tex <==


\section{Estimation Using Instrumental Variables}\label{sec:iv}

We now present our instrumental variable strategy. To understand the underlying intuition, note that it is not necessary to observe the complete network structure to observe $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$. For example, one could simply obtain ${\mathbf{Gy}}$ from survey data, ``What is the average value of your friends' $y$?''

However, even observing $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$, the model (\ref{eq:linearinmean}) cannot be simply estimated using simple linear regression. The reason is that ${\mathbf{Gy}}$ is endogenous; thus, a linear regression would produce biased estimates (e.g. \cite{manski1993identification}, \cite{bramoulle2009identification}).

The typical instrumental approach to deal with this endogeneity is to use instruments based on the structural model, i.e. instruments constructed using second-degree peers (e.g. $\mathbf{G}^2\mathbf{X}$, see \cite{bramoulle2009identification}). These are less likely to be found in survey data. Indeed, we could doubt the informativeness of questions such as, ``What is the average value of your friends' average value of their friends' $x$?''

However, the above discussion is encouraging. When researchers observe $[\mathbf{y}, \mathbf{X}, {\mathbf{GX}},{\mathbf{Gy}}]$, information about the network is only used as a mean to construct a valid instrument, e.g. following \citet{bramoulle2009identification}. We propose one simple way to construct such an instrument in Proposition \ref{prop:all_observed} below.

\begin{proposition}\label{prop:all_observed}
[Conditions] Suppose that $\mathbf{GX}$ and $\mathbf{Gy}$ are observed and define the matrix $\mathbf{Z}=[\mathbf{1},\mathbf{X},\mathbf{GX},\mathbf{H}^2\mathbf{X},\mathbf{H}^3\mathbf{X}...]$. Let $\boldsymbol{H}$ be a matrix such that: (1) at least one column of $\mathbf{H}^k\mathbf{X}$ is correlated with $\mathbf{G}\mathbf{y}$, conditional on $[\mathbf{1},\mathbf{X},\mathbf{GX}]$ for $k\geq 2$, and (2) $\mathbb{E}[\boldsymbol{\varepsilon}|\mathbf{X},\mathbf{H}]=\mathbf{0}$.

[Results] Then, under classical assumptions (e.g. \cite{cameron2005microeconometrics}, Proposition 6.1), the (linear) GMM estimator based on the moment function $\frac{1}{N}\sum_i\mathbf{Z}_i'\boldsymbol{\varepsilon}_i=\mathbf{0}$ is consistent and asymptotically normally distributed with the usual asymptotic variance-covariance matrix.
\end{proposition}

Condition (1) is the relevancy condition, while condition (2) is the exogeneity condition. While Proposition \ref{prop:all_observed} holds for any matrix $\mathbf{H}$ such that conditions (1) and (2), the most sensible example is when $\mathbf{H}$ is constructed using a draw from $\hat{P}(\mathbf{G})$. A similar strategy is used by \cite{kelejian2014estimation}, \cite{konig2019r} and \cite{lee2020key} in a different context.

Importantly, the moment conditions remain valid even when the researcher uses a \emph{mispecified} estimator of the distribution ${P}(\mathbf{G})$, as long as the specification error on $P(\mathbf{G})$ does not induce a correlation with $\boldsymbol{\varepsilon}$.\footnote{We would like to thank Chih-Sheng Hsieh and Arthur Lewbel for discussions on this important point.} This could be of great practical importance, especially if the estimation of $\hat{P}(\mathbf{G})$ suffers from small sample bias. We provide an example in Section \ref{sec:ard} below.

We now turn to the more general case where $\mathbf{Gy}$ and $\mathbf{GX}$ are not observed. To simplify the notation, for the remainder of this section, we define $\lbrace \dot{\mathbf{G}}^{(s)}\rbrace_{s=1}^S$ and $\lbrace \ddot{\mathbf{G}}^{(t)}\rbrace_{t=1}^T$ be two sequences of independent draws from $\hat{P}(\mathbf{G})$. We will also let $\dot{\mathbf{G}}$ and $\ddot{\mathbf{G}}$ be single draws from $\hat{P}(\mathbf{G})$.

To understand why we cannot simply proxy $\mathbf{Gy}$ and $\mathbf{GX}$ using draws form $\hat{P}(\mathbf{G})$, consider the simple case for which $\boldsymbol{\gamma}=\mathbf{0}$, so the observation of $\mathbf{GX}$ is inconsequential. We have:
$$
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\ddot{\mathbf{G}}\mathbf{y}+[\boldsymbol{\eta}+\boldsymbol{\varepsilon}],
$$
where $\ddot{\mathbf{G}}$ is drawn from $\hat{P}(\mathbf{G})$, and $\boldsymbol{\eta}=\alpha[\mathbf{G}-\ddot{\mathbf{G}}]\mathbf{y}$ is the error due to the approximation of $\mathbf{Gy}$ by $\ddot{\mathbf{G}}\mathbf{y}$. Importantly, the approximation error does \emph{not} vanish as $n$ grows, due to the fact that individuals belong to bounded groups (see Assumption \ref{as:manymarkets}).\footnote{CITE Eric's paper.}

Our moment condition exploit the fact, however, that as $n$ grows, $\ddot{\mathbf{G}}$ and $ {\mathbf{G}}$ are drawn from the same distribution. Then, we can construct an instrument using \emph{another} draw  $\dot{\mathbf{G}}$ from $\hat{P}(\mathbf{G})$, say $\dot{\mathbf{G}}\mathbf{X}$. The intuition is that, as $n$ grows, the dependence between  $\dot{\mathbf{G}}$ and $ \ddot{\mathbf{G}}$ is the same as the dependence between  $\dot{\mathbf{G}}$ and  ${\mathbf{G}}$. This observation however, does not directly implies that $\dot{\mathbf{G}}\mathbf{X}$ is a valid instrument for $\ddot{\mathbf{G}}\mathbf{y}$ because $\dot{\mathbf{G}}\mathbf{X}$ is correlated with $\boldsymbol{\eta}$. This is due to the fact that $\mathbf{y}$ is a function of the true network $\mathbf{G}$, and as such, the correlation between columns of $\dot{\mathbf{G}}\mathbf{X}$ and $\mathbf{Gy}$ is not the same as the correlation between columns of $\dot{\mathbf{G}}\mathbf{X}$ and $\ddot{\mathbf{G}}\mathbf{y}$.\footnote{In an earlier version of this paper, we suggested such an approach. Although inconsistent, the bias in practice is very small. We discuss this point in Appendix.}

That being said we can bound the asymptotic bias, similarly to what is done in \cite{andrews2017measuring}. Proposition \ref{prop:bias_nocontext} formalizes.
\begin{proposition}\label{prop:bias_nocontext}
[Conditions] Assume that $\boldsymbol{\gamma}=\mathbf{0}$. Let $\ddot{\mathbf{S}}=[\mathbf{1},\mathbf{X},\ddot{\mathbf{G}}\mathbf{y}]$ and $\dot{\mathbf{Z}}=[\mathbf{1},\mathbf{X},\dot{\mathbf{G}}\mathbf{X},\dot{\mathbf{G}}^2\mathbf{X},...]$. Denote by $\hat{\boldsymbol{\theta}}$ the linear GMM estimator based on the (pseudo) moment function $\frac{1}{N}\sum_i \dot{\mathbf{Z}}_i[\boldsymbol{\eta}_i+\boldsymbol{\varepsilon}_i]$, and define the sensitivity matrix ${\mathbf{M}}=[\ddot{\mathbf{S}}'\dot{\mathbf{Z}}\mathbf{W}\dot{\mathbf{Z}}'\ddot{\mathbf{S}}]^{-1}\ddot{\mathbf{S}}'\dot{\mathbf{Z}}\mathbf{W}$.

[Result] Then, under classical assumptions (see proof), the asymptotic bias of $\hat{\boldsymbol{\theta}}_k$ is at most $Plim\sum_l |{\mathbf{M}}_{k,l}|b_l$, for all $k$, and where $b_l=|\alpha|^3(2Var_i(\sum_j\dot{\mathbf{Z}}_{jl}\ddot{\mathbf{G}}_{ji}))^{1/2}\max_i|y_i|$. Moreover, letting $\mathbf{W}=\mathbf{I}$ reduces the overall bias in the sense of minimizing the Froenius norm of ${\mathbf{M}}$.
\end{proposition}
Note that $Var_i(\sum_j\dot{\mathbf{Z}}_{jl}\ddot{\mathbf{G}}_{ji})$ decreases as the size $N_r$ of each group $r$ grows. We therefore expect the bias to be small for groups of medium sizes (such as small villages, see REF). The argument is very similar to the one in \cite{andrews2017measuring}, although here perturbation with respect to the true model is not \textit{local}.\footnote{See page 1562 in \cite{andrews2017measuring}.} We also show that we expect $\mathbf{W}=\mathbf{I}$ to minimize the overall bias. Our result therefore provides a theoretical justification for the simulations in \cite{onishi2021sample} who show that the using the identity matrix to weight the moments greatly reduce the bias in the context studied by \cite{andrews2017measuring}.

A similar result holds when we do not impose $\boldsymbol{\gamma}=\mathbf{0}$, although only when $\mathbf{GX}$ is observed.

\begin{corollary}\label{cor:bias}
Assume that $\mathbf{GX}$ is observed, then the results of Proposition \ref{prop:bias_nocontext} hold, with $b_l=|\alpha|^2(2Var_i(\sum_j\dot{\mathbf{Z}}_{jl}\ddot{\mathbf{G}}_{ji}))^{1/2}\max_i|y_i|$ for $\ddot{\mathbf{S}}=[\mathbf{1},\mathbf{X},\mathbf{GX},\ddot{\mathbf{G}}\mathbf{y}]$ and $\dot{\mathbf{Z}}=[\mathbf{1},\mathbf{X},\mathbf{GX},\ddot{\mathbf{G}}\mathbf{X},\dot{\mathbf{G}}^2\mathbf{X},\dot{\mathbf{G}}^3\mathbf{X},...]$.
\end{corollary}
Note that the instrument $\ddot{\mathbf{Z}}$ now includes the term $\ddot{\mathbf{G}}\mathbf{X}$, which is constructed using the same draw that is used to contruct the proxy variable $\ddot{\mathbf{G}}\mathbf{y}$. This is done to ensure that the columns of $\ddot{\mathbf{Z}}'\mathbf{G}$ and the columns of $\ddot{\mathbf{Z}}'\ddot{\mathbf{G}}$ have the same asymptotic distribution.\footnote{This also explains why the observation of $\mathbf{GX}$ is required.}

Following Proposition \ref{prop:bias_nocontext} and Corollary \ref{cor:bias}, if the maximal bias is small in practice, researchers may choose to use the pseudo GMM estimators and to report the maximal bias. However, if the maximal bias is large, we show that we can include the bias directly in the moment function, which provides a consistent estimator of $\boldsymbol{\theta}$. Let $\tilde{\boldsymbol{\theta}}=[c,\boldsymbol{\beta}',\boldsymbol{\gamma}']'$.

\begin{theorem}\label{prop:non_observed} [Conditions] Let $\dot{\mathbf{Z}}^{(s)}=[\mathbf{1},\mathbf{X},\dot{\mathbf{G}}^{(s)}\mathbf{X},(\dot{\mathbf{G}}^{(s)})^2\mathbf{X},(\dot{\mathbf{G}}^{(s)})^3\mathbf{X},...]$ and $\ddot{\mathbf{V}}^{(t)}=[\mathbf{1},\mathbf{X},\ddot{\mathbf{G}}^{(t)}\mathbf{X}]$. Consider also the following (simulated) moment function:
\begin{equation}\label{eq:moment}
\mathbb{E}(\frac{1}{ST}\sum_{t=1}^T\sum_{s=1}^S\dot{\mathbf{Z}}^{(s)\prime}_i(\mathbf{I}-\alpha\dot{\mathbf{G}}^{(s)})_i\left(\mathbf{y}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(t)})^{-1}\ddot{\mathbf{V}}^{(t)}\tilde{\boldsymbol{\theta}}\right))=\mathbf{0}
\end{equation}

[Result] For any $S$ and $T$, the (simulated) GMM estimator based on (\ref{eq:moment}) is consistent and asymptotically normal, i.e.  $\sqrt{N}(\hat{\boldsymbol{\theta}}-\boldsymbol{\theta}_0+\Delta\boldsymbol{\theta}^*)\overset{d}{\to}N(\mathbf{0},\mathbf{V})$, where $\Delta\boldsymbol{\theta}^*$ and $\mathbf{V}$ are defined in (\ref{eq:thetastar}) and (\ref{var:gmm}) in Appendix and where $\Delta\boldsymbol{\theta}^*\rightarrow 0$ as $N\rightarrow\infty$.
\end{theorem}
Here the asymptotic variance $\mathbf{V}$ includes the sampling uncertainty, the estimating uncertainty of $\hat{\boldsymbol{\rho}}$, as well as the simulating uncertainty (which decreases as $S$ and $T$ grow). The term $\Delta\boldsymbol{\theta}^*$ allows to center the distribution of $\hat{\boldsymbol{\theta}}$ for finite $N$, much like for the asymptotic distribution of penalized likelihood models (e.g. \cite{fan2001variable} or \cite{fan2004nonconcave}).

Importantly, and similar to standard methods of simulated moments (e.g. \cite{gourieroux1993simulation}), the estimation is consistent even for a finite number of simulations (i.e. $S$ and $T$ are finite). Our estimator therefore does not suffer from the curse of dimensionality faced by \cite{chandrasekhar2011econometrics}.\footnote{The unconditional moment condition in \cite{chandrasekhar2011econometrics} is based on the integration of the moment condition $\mathbb{E}(\mathbf{Z}^{(s)\prime}\boldsymbol{\varepsilon}|\mathbf{G})$ over $\mathbf{G}$. See our discussion in REFERENCES"}

To understand the intuition behind the use of the moment function (\ref{eq:moment}), let us replace $\mathbf{y}=(\mathbf{I}-\alpha\mathbf{G})^{-1}(\mathbf{V}\tilde{\boldsymbol{\theta}}+\boldsymbol{\varepsilon})$ in equation (\ref{eq:moment}). In doing so, we can rewrite the term inside the double summation in (\ref{eq:moment}) as a sum of two terms.\footnote{The double summation in (\ref{eq:moment}) is not essential and (\ref{eq:moment}) could be replaced by $\mathbb{E}\frac{1}{S}\sum_{t=1}^T\dot{\mathbf{Z}}^{(s)\prime}(\mathbf{I}-\alpha\dot{\mathbf{G}}^{(s)})\left(\mathbf{y}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}\ddot{\mathbf{V}}^{(s)}\tilde{\boldsymbol{\theta}}\right)=\mathbf{0}$. The efficiency loss in practice could however be important.} First, $\dot{\mathbf{Z}}^{(s)\prime}\boldsymbol{\varepsilon}$, which would be the standard moment condition if $\mathbf{G}$ was observed (e.g. \cite{bramoulle2009identification}), and second: $$ \dot{\mathbf{Z}}^{(s)\prime}(\mathbf{I}-\alpha\dot{\mathbf{G}}^{(s)})\left((\mathbf{I}-\alpha{\mathbf{G}})^{-1}{\mathbf{V}}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}\ddot{\mathbf{V}}^{(t)}\right)\tilde{\boldsymbol{\theta}}.$$
We show that both terms are equal to $0$ in expectation as $N$ grows to $\infty$. For the first term, this is true since the simulated network is exogenous. For the second term, this is true because $\mathbf{G}$, $\dot{\mathbf{G}}$ and $\ddot{\mathbf{G}}$ are asymptotically drawn from the same distribution.

For the special case in which $\mathbf{G}$ is observed, one could substitute $\dot{\mathbf{G}}^{(s)}=\mathbf{G}$ and $\ddot{\mathbf{G}}^{(t)}=\mathbf{G}$ for all $s,t$ and the first term would simply be $\mathbf{Z}'\boldsymbol{\varepsilon}$, while the second term would be exactly equal to $\mathbf{0}$.

Note that Theorem \ref{prop:non_observed} is valid whether or not $\mathbf{Gy}$ and $\mathbf{GX}$ are observed since the moment function (\ref{eq:moment}) does not use information on $\mathbf{Gy}$ or $\mathbf{GX}$. Proposition \ref{prop:GXobs} and Proposition \ref{prop:Gyobs} below present specific moment function that use $\mathbf{Gy}$ or $\mathbf{GX}$, if they are observed.

\begin{proposition}\label{prop:GXobs}
Assume that $\mathbf{GX}$ is observed, but that $\mathbf{Gy}$ is not observed. Let $\lbrace \dot{\mathbf{G}}^{(s)}\rbrace_{s=1}^S$ and $\lbrace \ddot{\mathbf{G}}^{(t)}\rbrace_{t=1}^T$ be two sequences of independent draws from $\hat{P}(\mathbf{G})$. Let $\dot{\mathbf{Z}}^{(s)}=[\mathbf{1},\mathbf{X},{\mathbf{G}}\mathbf{X},\dot{\mathbf{G}}^{s}{\mathbf{G}}\mathbf{X},(\dot{\mathbf{G}}^{(s)})^2{\mathbf{G}}\mathbf{X},...]$,
$\ddot{\mathbf{Z}}^{(s,t)}=[\mathbf{1},\mathbf{X},\ddot{\mathbf{G}}^{(t)}\mathbf{X},\dot{\mathbf{G}}^{s}\ddot{\mathbf{G}}^{(t)}\mathbf{X},(\dot{\mathbf{G}}^{(s)})^2\ddot{\mathbf{G}}^{(t)}\mathbf{X},...]$, $\mathbf{V}=[\mathbf{1},\mathbf{X},\mathbf{G}\mathbf{X}]$, and $\ddot{\mathbf{V}}^{(t)}=[\mathbf{1},\mathbf{X},\ddot{\mathbf{G}}^{(t)}\mathbf{X}]$. Then, the simulated GMM estimator based on
\begin{eqnarray}\label{eq:Gyobs}
\mathbb{E}(\frac{1}{S}\sum_{s=1}^S\dot{\mathbf{Z}}_i^{(s)\prime}(\mathbf{I}-\alpha\dot{\mathbf{G}}^{(s)})_i\mathbf{y} -
\frac{1}{ST}\sum_{t=1}^T\sum_{s=1}^S (\dot{\mathbf{Z}}^{(s)\prime}\mathbf{V}-\ddot{\mathbf{Z}}^{(s,t)\prime}\ddot{\mathbf{V}}^{(t)})_i\tilde{\boldsymbol{\theta}}\nonumber\\ -\frac{1}{ST}\sum_{t=1}^T\sum_{s=1}^S  \ddot{\mathbf{Z}}^{(s,t)\prime}_i(\mathbf{I}-\alpha\dot{\mathbf{G}}^{(s)})_i(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(t)})^{-1}\ddot{\mathbf{V}}^{(t)}\tilde{\boldsymbol{\theta}}) =\mathbf{0}
\end{eqnarray}
is consistent and asymptotically normally distributed with asymptotic variance-covariance matrix defined in ????.
\end{proposition}

\begin{proposition}\label{prop:Gyobs}
Assume that $\mathbf{Gy}$ is observed, but that $\mathbf{GX}$ is not observed. Let $\lbrace \dot{\mathbf{G}}^{(s)}\rbrace_{s=1}^S$ and $\lbrace \ddot{\mathbf{G}}^{(t)}\rbrace_{t=1}^T$ be two sequences of independent draws from $\hat{P}(\mathbf{G})$. Let $\dot{\mathbf{Z}}^{(s)}=[\mathbf{1},\mathbf{X},\dot{\mathbf{G}}^{(s)}\mathbf{X},(\dot{\mathbf{G}}^{(s)})^2\mathbf{X},...]$, and $\ddot{\mathbf{V}}^{(t)}=[\mathbf{1},\mathbf{X},\ddot{\mathbf{G}}^{(t)}\mathbf{X}]$. Then, the simulated GMM estimator based on
\begin{eqnarray}\label{eq:GXobs}
\mathbb{E}(\frac{1}{S}\sum_{s=1}^S\dot{\mathbf{Z}}_i^{(s)\prime}(\mathbf{I}-\alpha\mathbf{G})_i\mathbf{y} -
\frac{1}{ST}\sum_{t=1}^T\sum_{s=1}^S \dot{\mathbf{Z}}^{(s)\prime}_i\ddot{\mathbf{V}}^{(t)}_i\tilde{\boldsymbol{\theta}})=\mathbf{0}
\end{eqnarray}
is consistent and asymptotically normally distributed with asymptotic variance-covariance matrix defined in ????.
\end{proposition}

The logic behind Proposition \ref{prop:GXobs} is exactly the same as the one for Proposition \ref{prop:non_observed}. The objective is to use $\lbrace\dot{\mathbf{G}}^{(s)}\rbrace_{s=1}^S$ and $\lbrace \ddot{\mathbf{G}}^{(t)}\rbrace_{t=1}^T$ in order to write the moment condition as a sum of random variables with the same expected value. As for \ref{prop:non_observed}, if $\mathbf{G}$ was observed, we could substitute $\dot{\mathbf{G}}^{(s)}=\mathbf{G}$ and $\ddot{\mathbf{G}}^{(t)}=\mathbf{G}$ for all $s,t$, and the first summation in the moment condition (\ref{eq:GXobs}) would simply reduce to $\mathbb{E}\mathbf{Z}'\boldsymbol{\varepsilon}$, while the other remaining summations would be exactly $0$.


Proposition \ref{prop:all_observed}, Proposition \ref{prop:non_observed} and \ref{prop:GXobs} therefore show that the estimation of (\ref{eq:linearinmean}) is possible, even with very limited information about the network structure. In Section \ref{sec:ard}, we study the finite sample properties of our approach using network formation models estimated on aggregated relational data (\cite{breza2017using}; see Example \ref{ex:ard}). Before, however, we briefly discuss how one can adapt this estimation strategy while allowing for group-level unobservables.

Indeed, a common assumption is that each group in the population is affected by a common shock, unobserved by the econometrician (e.g. \cite{bramoulle2009identification}). As such, for each group $r=1,...,M$, we have: $\mathbf{y}_r=c_r\mathbf{1}_r+\mathbf{X}_r\boldsymbol{\beta}+\alpha\mathbf{G}_r\mathbf{y}_r+{\mathbf{G}_r\mathbf{X}_r}\boldsymbol{\gamma}+\boldsymbol{\varepsilon}_r$, where $c_r$ is not observed, $\mathbf{1}_r$ is an $N_r$-dimensional vector of ones, $N_r$ is the size of the group r, $\bG_r$ is the subinteraction matrix in the group r, and $\bepsilon_r$ is the vector of error terms in the group r.

Under Assumption \ref{as:manymarkets}, it is not possible to obtain a consistent estimator of $\{c_r\}_{r=1}^m$ because the number of observations used to estimate each $c_r$ is bounded. This is known as the \emph{incidental parameter problem}.\footnote{See \cite{lancaster2000incidental} for a review.} A common strategy is to use deviations from the group average and estimate the model in deviations (e.g. \cite{bramoulle2009identification}).

Let $\mathbf{J}=diag\{\mathbf{I}_{N_r}-\frac{1}{N_r}\mathbf{1}_r\mathbf{1}'_r\}$ be the group-differentiating matrix, where $\mathbf{I}_{N_r}$ is the identified matrix of dimension $N_r$. The operator \emph{diag} generates a blog-diagonal matrix in which each group is a block.\footnote{Then, $\mathbf{Jw}$ gives $\mathbf{w}$ minus the group average of $\mathbf{w}$.} We can rewrite: $\mathbf{Jy}=\mathbf{JX}\boldsymbol{\beta}+\alpha{\mathbf{JG}\mathbf{y}}+{\mathbf{JGX}}\boldsymbol{\gamma}+\boldsymbol{J\varepsilon}$. Note that the results of Propositions \ref{prop:all_observed}--\ref{prop:GXobs} extend directly, using instruments in deviation with the group average.

\subsection{Finite Sample Performance Using ARD}\label{sec:ard}
In this section, we study the small sample performance of the estimator presented in Section \ref{sec:iv} when the researcher only has access to ARD (as in Example \ref{ex:ard}). First, we simulate network data using the model proposed by \cite{breza2017using} and simulate outcomes using the linear in means model (\ref{eq:linearinmean}) conditional on the simulated networks. Second, we estimate the network formation model using the Bayesian estimator proposed by \cite{breza2017using} (yielding $\hat{\boldsymbol{\rho}}_B$), as well as using the classical estimator proposed by \cite{alidaee2020recovering} (yielding $\hat{\boldsymbol{\rho}}_A$). Third, we estimate the linear-in-means model, using our IV estimator based on $\hat{\boldsymbol{\rho}}_A$ and $\hat{\boldsymbol{\rho}}_B$.

Recall that
\begin{equation}\label{eq:ard}
P(a_{ij}=1)\propto\exp\{\nu_i+\nu_j+\zeta \mathbf{z}_i'\mathbf{z}_j\},    
\end{equation}
where $\nu_i$, $\nu_j$, $\zeta$, $\mathbf{z}_i$, and $\mathbf{z}_j$ are not observed by the econometrician but follow parametric distributions. We refer the interested reader to \cite{mccormick2015latent}, \cite{breza2017using}, and \cite{breza2019consistently} for a formal discussion of the model, including its identification and consistent estimation. Here, we discuss the intuition using a simple analogy.

Suppose that individuals are located according to their geographical position on Earth. Suppose also that there are a fixed number of cities on Earth in which individuals can live. The econometrician does not know the individuals' locations on Earth nor do they know the location of the cities. In model (\ref{eq:ard}), $\mathbf{z}_i$ represent $i$'s position on Earth. However, the econometrician has access to ARD for a subset of the population, i.e. answers to questions such as, ``How many of your friends live in city $A$?''

To understand the intuition behind the identification of the model, consider the following example: suppose that individual $i$ has many friends living in city $A$. Then, city $A$ is likely located close to $i$'s location. Similarly, if many individuals have many friends living in city $A$, then city $A$ is likely a large city. Finally, if $i$ has many friends from many cities, $i$ likely has a large $\nu_i$.

To study the finite sample performance of our instrumental strategy in this context, we simulate 20 groups of 250 individuals each. Within each subpopulation, we simulate the ARD responses as well as a series of observable characteristics (e.g. cities). The details of the Monte Carlo simulations can be found in Appendix \ref{sec:ardsetting}.

Importantly, the model in (\ref{eq:ard}) is based on a single population framework. Thus, the network formation model must be estimated separately for each of the 20 groups. With only 250 individuals in each group, we therefore expect significant small-sample bias.

We contrast the estimator proposed by \cite{breza2017using} with the one proposed by \cite{alidaee2020recovering}. Whereas \cite{breza2017using} present a parametric Bayesian estimator, \cite{alidaee2020recovering} propose a (nonparametric) penalized regression based on a low-rank assumption. One main advantage of their estimator is that it allows for a wider class of model and ensures that the estimation is fast and easily implementable.\footnote{The authors developed user-friendly packages in R and Python. See their paper for links and details.} Note, however, that their method only yields a consistent estimator of $\hat{P}(\mathbf{A})$ if the true network is effectively low rank.

Very intuitively, the low-rank assumption implies that linking probabilities were generated from a small number of parameters; for example, in the example above, knowing individuals' gregariousness parameters $\nu_i$ and city in which they live would allow a prediction of the linking probabilities.

Importantly, the model (\ref{eq:ard}) is not necessarily low rank; for example, if the individuals' locations on Earth (i.e. the $\mathbf{z}_i$'s) are uniformly distributed and there are only very few  large cities, then the model produced is not low rank and the method proposed by \cite{alidaee2020recovering} performs poorly. Intuitively, in such a case, the fact that individual $i$ lives in city $A$ poorly explains the linking probabilities. 

We compare the performance of both estimators as we vary the concentration parameter for the individuals' locations on Earth (that is, $\kappa$, see Appendix \ref{sec:ardsetting} for details). This has the effect of changing the \emph{effective rank} of the linking probabilities: increasing $\kappa$ decreases the effective rank.\footnote{We refer the interested reader to \cite{alidaee2020recovering} for a formal discussion of the effective rank and of its importance for their estimator.} We therefore expect the estimator proposed by \cite{alidaee2020recovering} to perform better for larger values of $\kappa$.

Results are presented in Tables \ref{tab:breza} and \ref{tab:alidaee}. When $\mathbf{Gy}$ is observed, both estimators perform extremely well. In light of Propositions \ref{prop:gamma0} and \ref{prop:gammanot0}, this is expected, as the IV estimator is valid even under misspecification. When $\mathbf{Gy}$ is not observed, results are more nuanced. First, note that for all specifications, the introduction of the non-pertinent variables $\ddot{\mathbf{G}}\mathbf{X}$ contaminates the estimation of $\boldsymbol{\gamma}$. This occurs because ${\mathbf{G}}\mathbf{X}$ and $\ddot{\mathbf{G}}\mathbf{X}$ are highly correlated.\footnote{This is a small sample issue which is not due to the assumed network formation model and would arise even if the linking probabilities were known (instead of being estimated).} Note, however, that the estimated values for $\boldsymbol{\gamma}+\check{\boldsymbol{\gamma}}$ are centered on the true value. Second, the bias of the estimated endogenous peer effect (i.e. $\alpha$) goes to zero when the linking probabilities are of lower rank, with an advantage for the estimator proposed by  \cite{breza2017using}. This is expected because the model is correctly specified and the estimator is parametric. 

Overall, our IV estimator can be successfully implemented in small samples, using either the estimator proposed by \cite{breza2017using} or by \cite{alidaee2020recovering}, both of which only rely on the observation of ARD.

\renewcommand{\arraystretch}{.9}
\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD - network distribution estimated following \cite{breza2017using} } 
\label{tab:breza}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}d{4}d{4}d{4}d{4}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 0$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1ex]                                             
$\alpha=0.4$    & 0.400  & 0.007 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$                & 5.000  & 0.021 & 4.986   & 5.000  & 5.014   \\
$\gamma_2=-3$              & -3.001 & 0.031 & -3.021  & -3.000 & -2.980  \\  
F-test (Weak inst.) & 3144.574&	874.400&	2492.881&	3075.955&	3672.449 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                                          
$\alpha=0.4$ & 0.371  & 0.013 & 0.363   & 0.372  & 0.380   \\
$\gamma_1=5$            & 5.396  & 0.021 & 5.383   & 5.397  & 5.410   \\
$\gamma_2=-3$          & -2.400 & 0.041 & -2.428  & -2.400 & -2.371  \\
$\hat{\gamma}_1=0$          & -0.380 & 0.028 & -0.400  & -0.382 & -0.362  \\
$\hat{\gamma}_2=0$           & -0.553 & 0.044 & -0.584  & -0.551 & -0.525  \\
F-test (Weak inst.) & 3193.940&	760.793&	2642.815&	3153.048&	3666.220 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 10$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                                              
$\alpha=0.4$   & 0.400  & 0.006 & 0.396   & 0.400  & 0.404   \\
$\gamma_1=5$                & 5.001  & 0.019 & 4.988   & 5.001  & 5.014   \\
$\gamma_2=-3$             & -3.000 & 0.031 & -3.020  & -3.000 & -2.978  \\
F-test (Weak inst.) & 5905.596&	1876.836&	4519.460&	5766.601&	7158.739 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                                          
$\alpha=0.4$ & 0.400  & 0.007 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$            & 5.392  & 0.019 & 5.379   & 5.393  & 5.405   \\
$\gamma_2=-3$          & -2.397 & 0.037 & -2.421  & -2.398 & -2.373  \\
$\hat{\gamma}_1=0$           & -0.391 & 0.022 & -0.405  & -0.390 & -0.375  \\
$\hat{\gamma}_2=0$          & -0.604 & 0.038 & -0.630  & -0.605 & -0.579  \\
F-test (Weak inst.) & 5176.649&	1507.532&	4058.393&	5087.275&	6243.500 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 20$, $N=250$, $M=20$}                                                            \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                                             
$\alpha=0.4$    & 0.400  & 0.006 & 0.396   & 0.400  & 0.404   \\
$\gamma_1=5$                & 5.000  & 0.020 & 4.986   & 4.999  & 5.013   \\
$\gamma_2=-3$            & -3.001 & 0.031 & -3.021  & -3.001 & -2.981  \\
F-test (Weak inst.) &6104.999&	1927.633&	4734.460&	5937.815&	7246.355 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]   
$\alpha=0.4$ & 0.400  & 0.007 & 0.396   & 0.400  & 0.405   \\
$\gamma_1=5$            & 5.390  & 0.019 & 5.377   & 5.390  & 5.403   \\
$\gamma_2=-3$          & -2.398 & 0.036 & -2.422  & -2.398 & -2.375  \\
$\hat{\gamma}_1=0$           & -0.390 & 0.022 & -0.405  & -0.390 & -0.376  \\
$\hat{\gamma}_2=0$          & -0.604 & 0.036 & -0.628  & -0.604 & -0.579 \\ 
F-test (Weak inst.) & 5321.702&	1524.973&	4272.790&	5199.232&	6235.250 \\ 
\hline \\[-1.8ex] 


\multicolumn{6}{l}{%
  \begin{minipage}{15cm}%
    \footnotesize{Note: In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with a location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in Appendix \ref{sec:ardsetting}. Predicted probabilities are computed using the mean of the posterior distribution. F-test is the Fisher-statistic of the Weak instruments test. We do not report the estimated values for $c$ and $\boldsymbol{\beta}$ to keep the table readable, but they are available upon request. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.}
  \end{minipage}%
}\end{tabular}
\end{table}

\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD - network distribution estimated following \cite{alidaee2020recovering} } 
\label{tab:alidaee}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}d{4}d{4}d{4}d{4}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 0$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1ex]                                
$\alpha=0.4$     & 0.400  & 0.012 & 0.393   & 0.400  & 0.407   \\
$\gamma_1=5$             & 5.000  & 0.029 & 4.980   & 4.999  & 5.019   \\
$\gamma_2=-3$             & -3.000 & 0.032 & -3.021  & -3.000 & -2.978  \\
F-test (Weak inst.) & 798.971&	340.558&	560.817&	749.132&	990.407\\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                          
$\alpha=0.4$ & 0.371  & 0.024 & 0.357   & 0.373  & 0.387   \\
$\gamma_1=5$              & 5.504  & 0.036 & 5.479   & 5.503  & 5.528   \\
$\gamma_2=-3$            & -2.480 & 0.057 & -2.517  & -2.480 & -2.441  \\
$\hat{\gamma}_1=0$           & -0.364 & 0.031 & -0.385  & -0.363 & -0.344  \\
$\hat{\gamma}_2=0$          & -0.302 & 0.070 & -0.349  & -0.304 & -0.254  \\
F-test (Weak inst.) & 590.248&	253.853&	409.497&	572.210&	721.788 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 10$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                              
$\alpha=0.4$    & 0.400  & 0.009 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$         & 4.999  & 0.022 & 4.985   & 4.999  & 5.014   \\
$\gamma_2=-3$                & -3.000 & 0.032 & -3.022  & -3.001 & -2.978 \\
F-test (Weak inst.) & 1697.514&	741.478&	1179.079&	1593.284&	2127.582\\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                          
$\alpha=0.4$  & 0.395  & 0.021 & 0.388   & 0.397  & 0.405   \\
$\gamma_1=5$            & 5.396  & 0.027 & 5.378   & 5.394  & 5.412   \\
$\gamma_2=-3$            & -2.412 & 0.045 & -2.439  & -2.410 & -2.383  \\
$\hat{\gamma}_1=0$          & -0.385 & 0.032 & -0.404  & -0.387 & -0.370  \\
$\hat{\gamma}_2=0$           & -0.462 & 0.117 & -0.534  & -0.483 & -0.414  \\
F-test (Weak inst.) &1303.291&	586.429&	895.070&	1227.426&	1652.148\\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 20$, $N=250$, $M=20$}                                                            \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                              
$\alpha=0.4$     & 0.400  & 0.008 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$                & 5.000  & 0.021 & 4.985   & 5.000  & 5.013   \\
$\gamma_2=-3$             & -2.999 & 0.032 & -3.020  & -2.999 & -2.979   \\
F-test (Weak inst.) & 2685.354&	978.512&	1998.396&	2601.996&	3268.714 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]   
$\alpha=0.4$ & 0.399  & 0.010 & 0.393   & 0.400  & 0.406   \\
$\gamma_1=5$        & 5.391  & 0.020 & 5.378   & 5.391  & 5.404   \\
$\gamma_2=-3$             & -2.400 & 0.039 & -2.425  & -2.400 & -2.374  \\
$\hat{\gamma}_1=0$           & -0.391 & 0.022 & -0.406  & -0.391 & -0.376  \\
$\hat{\gamma}_2=0$          & -0.573 & 0.047 & -0.605  & -0.575 & -0.544 \\ 
F-test (Weak inst.) & 2191.313&	774.366&	1656.355&	2130.681&	2668.781\\ 
\hline \\[-1.8ex] 



\multicolumn{6}{l}{%
  \begin{minipage}{15cm}%
    \footnotesize{Note: In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in Appendix \ref{sec:ardsetting}. We chose the weight associated with the nuclear norm penalty to minimize the RMSE through cross-validation. This value of $\lambda=600$ is smaller than the recommended value in \cite{alidaee2020recovering}. F-test is the Fisher-statistic of the Weak instruments test. We do not report the estimated values for $c$ and $\boldsymbol{\beta}$ to keep the table readable, but they are available upon request. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.}
  \end{minipage}%
}\end{tabular}
\end{table}
\renewcommand{\arraystretch}{1}

==> archives/bkp/iv_old_last.tex <==


\section{Estimation Using Instrumental Variables}\label{sec:iv}

We now present our instrumental variable strategy. To understand the underlying intuition, note that it is not necessary to observe the complete network structure to observe $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$. For example, one could simply obtain ${\mathbf{Gy}}$ from survey data, ``What is the average value of your friends' $y$?''

However, even observing $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$, the model (\ref{eq:linearinmean}) cannot be simply estimated using simple linear regression. The reason is that ${\mathbf{Gy}}$ is endogenous; thus, a linear regression would produce biased estimates (e.g. \cite{manski1993identification}, \cite{bramoulle2009identification}).

The typical instrumental approach to deal with this endogeneity is to use instruments based on the structural model, i.e. instruments constructed using second-degree peers (e.g. $\mathbf{G}^2\mathbf{X}$, see \cite{bramoulle2009identification}). These are less likely to be found in survey data. Indeed, we could doubt the informativeness of questions such as, ``What is the average value of your friends' average value of their friends' $x$?''

Propositions \ref{prop:gamma0} and \ref{prop:gammanot0} describe how to construct valid instruments when the researcher observes  $\mathbf{y}$, $\mathbf{X}$, and ${\mathbf{GX}}$. To clearly expose the argument, we first start by discussing the special case where there are no contextual effects: $\boldsymbol{\gamma}=\mathbf{0}$. The model in (\ref{eq:linearinmean}) can therefore be rewritten as: 
$$
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\mathbf{Gy}+\boldsymbol{\varepsilon}.
$$
The following proposition holds.\footnote{Proofs of Propositions \ref{prop:gamma0} and \ref{prop:gammanot0} can be found in Appendix \ref{sec:appendix_proofs}.}
\begin{proposition}\label{prop:gamma0}
Assume that $\boldsymbol{\gamma}=\mathbf{0}$. There are two cases:\begin{enumerate}
\item Suppose that $\mathbf{Gy}$ is observed and let $\boldsymbol{H}$ be an interaction matrix, correlated with $\mathbf{G}$, and such that $\mathbb{E}[\boldsymbol{\varepsilon}|\mathbf{X},\mathbf{H}]=\mathbf{0}$. Then, $\mathbf{H}\mathbf{X}$, $\mathbf{H}^2\mathbf{X}$,... are valid instruments.
\item Suppose that $\mathbf{Gy}$ \emph{is not} observed and let $\dot{\mathbf{G}}$ and $\ddot{\mathbf{G}}$ be two independent draws from the distribution $\hat{P}(\mathbf{G})$. Then, $\dot{\mathbf{G}}\mathbf{X}$, $\dot{\mathbf{G}}^2\mathbf{X}$,... are valid instruments when $\ddot{\mathbf{G}}\mathbf{y}$ is used as a proxy for $\mathbf{Gy}$, as $N\rightarrow\infty$.
\end{enumerate}
\end{proposition}

First, suppose that $\mathbf{Gy}$ is observed directly from the data. Then, any instrument correlated with the usual instruments $\mathbf{GX},\mathbf{G}^2\mathbf{X}$,..., while being exogenous, are valid. Note that a special case of the first part of Proposition \ref{prop:gamma0} is when $\mathbf{H}$ is drawn from $\hat{P}(\mathbf{G})$. However, the instrument remains valid if the researcher uses a \emph{mispecified} estimator of the distribution ${P}(\mathbf{G})$.\footnote{We would like to thank Chih-Sheng Hsieh and Arthur Lewbel for discussions on this important point.} A similar strategy is used by \cite{kelejian2014estimation} and \cite{lee2020key} in a different context. Of course, the specification error on $P(\mathbf{G})$ must be independent of $\boldsymbol{\varepsilon}$. In Section \ref{sec:ard}, we discuss the importance of this robustness feature in a context in which the network formation process could be misspecified or subject to small sample biases.\footnote{Note, however, that if the specification error is too large, the correlation between $\mathbf{Gy}$ and $\mathbf{H}\mathbf{X}$ will likely be small, leading to a problem of weak instruments. It is also worth noting that the first part of Proposition \ref{prop:gamma0} does not depend on the assumption that groups are entirely sampled (i.e. Assumption \ref{as:nosampling}).}

When $\mathbf{Gy}$ is \emph{not} observed directly, however, specification errors typically produce invalid instruments. As stated in Part 2 of Proposition \ref{prop:gamma0}, the estimation also requires two independent draws from $\hat{P}(\mathbf{G})$ instead of just one. To see why, let us rewrite the model as:
$$
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\ddot{\mathbf{G}}\mathbf{y}+[\boldsymbol{\eta}+\boldsymbol{\varepsilon}],
$$
where $\boldsymbol{\eta}=\alpha[\mathbf{G}\mathbf{y}-\ddot{\mathbf{G}}\mathbf{y}]$ is the error due to the approximation of $\mathbf{Gy}$. Suppose also that $\dot{\mathbf{G}}\mathbf{X}$ is used as an instrument for $\mathbf{Gy}$.

The validity of the instrument therefore requires $\mathbb{E}[\boldsymbol{\eta}+\boldsymbol{\varepsilon}|\mathbf{X},\dot{\mathbf{G}}\mathbf{X}]=0$, and in particular: $$\mathbb{E}[\mathbf{G}\mathbf{y}|\mathbf{X},\dot{\mathbf{G}}\mathbf{X}]=\mathbb{E}[\ddot{\mathbf{G}}\mathbf{y}|\mathbf{X},\dot{\mathbf{G}}\mathbf{X}],$$
which is true since $\mathbf{G}$ and $\ddot{\mathbf{G}}$ have the same asymptotic distribution.

Of course, Proposition \ref{prop:gamma0} assumes that there are no contextual effects. We show that a similar result holds when $\boldsymbol{\gamma}\neq \mathbf{0}$. To estimate (\ref{eq:linearinmean}) using an instrumental variable approach, however, we must assume that ${\mathbf{GX}}$ are \emph{observed}. The reason is that there are no natural, strong instruments for ${\mathbf{GX}}$.\footnote{Indeed, the strengths of the instruments in Proposition \ref{prop:gamma0} come from the fact that $\mathbf{GX}$ are strong instruments for $\mathbf{Gy}$ when $\mathbf{G}$ is observed. Proxying $\mathbf{GX}$ with $\ddot{\mathbf{G}}\mathbf{X}$ and instrumenting with $\dot{\mathbf{G}}\mathbf{X}$ would be valid. However, the explanatory power of $\dot{\mathbf{G}}\mathbf{X}$, conditional on $\ddot{\mathbf{G}}\mathbf{X}$, would be much too weak to be of any practical use.} In Section \ref{sec:genestim}, we present an alternative estimation strategy that does not require the observation of $\mathbf{GX}$.

\begin{proposition}\label{prop:gammanot0}
Assume that $\mathbf{GX}$ are observed. There are two cases:\begin{enumerate}
\item Suppose that $\mathbf{Gy}$ is observed and let $\boldsymbol{H}$ be an interaction matrix, correlated with $\mathbf{G}$, and such that $\mathbb{E}[\boldsymbol{\varepsilon}|\mathbf{X},\mathbf{H}]=\mathbf{0}$. Then, $\mathbf{H}^2\mathbf{X}$, $\mathbf{H}^3\mathbf{X}$,... are valid instruments.
\item Suppose that $\mathbf{Gy}$ \emph{is not} observed and let $\dot{\mathbf{G}}$ and $\ddot{\mathbf{G}}$ be two independent draws from the distribution $\hat{P}(\mathbf{G})$. Then, $\dot{\mathbf{G}}^2\mathbf{X}$, $\dot{\mathbf{G}}^3\mathbf{X}$,... are valid instruments when $\ddot{\mathbf{G}}\mathbf{y}$ is used as a proxy for $\mathbf{Gy}$, if $\ddot{\mathbf{G}}\mathbf{X}$ are added as additional explanatory variables and as $N\rightarrow\infty$.
\end{enumerate}
\end{proposition}
The first part of Proposition \ref{prop:gammanot0} is a simple extension of the first part of Proposition \ref{prop:gamma0}. The second part of Proposition \ref{prop:gammanot0} requires more discussion. Essentially, it states that $\dot{\mathbf{G}}^2\mathbf{X}$, $\dot{\mathbf{G}}^3\mathbf{X}$, ... are valid instruments when the following \emph{expanded model} is estimated:
\begin{equation}\label{eq:expanded}
    \mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha{\ddot{\mathbf{G}}\mathbf{y}}+{\mathbf{GX}}\boldsymbol{\gamma}+\ddot{\mathbf{G}}\mathbf{X}\check{\boldsymbol{\gamma}}+\boldsymbol{\eta}+\boldsymbol{\varepsilon},
\end{equation}
where the true value of $\check{\boldsymbol{\gamma}}$ is $\mathbf{0}$.

To understand why the introduction of $\ddpt{\mathbf{G}}\mathbf{X}\check{\boldsymbol{\gamma}}$ is needed, recall that the constructed instrument must be uncorrelated with the approximation error $\boldsymbol{\eta}$. This correlation is conditional on the explanatory variables, which contain $\mathbf{G}$. In particular, it implies that generically, $$\mathbb{E}[\mathbf{G}\mathbf{y}|\mathbf{X},\mathbf{GX},\dot{\mathbf{G}}^2\mathbf{X}]\neq\mathbb{E}[\ddot{\mathbf{G}}\mathbf{y}|\mathbf{X},\mathbf{GX},\dot{\mathbf{G}}^2\mathbf{X}].$$

However, adding the auxiliary variable $\ddot{\mathbf{G}}\mathbf{X}$ as a covariate is sufficient to restore the result, i.e. as $N\rightarrow\infty$: $$\mathbb{E}[\mathbf{G}\mathbf{y}|\mathbf{X},\mathbf{GX},\dot{\mathbf{G}}^2\mathbf{X}, \ddot{\mathbf{G}}\mathbf{X}]=\mathbb{E}[\ddot{\mathbf{G}}\mathbf{y}|\mathbf{X},\mathbf{GX},\dot{\mathbf{G}}^2\mathbf{X}, \ddot{\mathbf{G}}\mathbf{X}].$$


Proposition \ref{prop:gamma0} and Proposition \ref{prop:gammanot0} therefore show that the estimation of (\ref{eq:linearinmean}) is possible, even with very limited information about the network structure. Note, however, that the validity of the constructed instruments only holds asymptotically. In Section \ref{sec:ard}, we study the finite sample properties of our approach using network formation models estimated on aggregated relational data (\cite{breza2017using}; see Example \ref{ex:ard}). Before, however, we briefly discuss how one can adapt this estimation strategy while allowing for group-level unobservables.

Indeed, a common assumption is that each group in the population is affected by a common shock, unobserved by the econometrician (e.g. \cite{bramoulle2009identification}). As such, for each group $r=1,...,M$, we have: $\mathbf{y}_r=c_r\mathbf{1}_r+\mathbf{X}_r\boldsymbol{\beta}+\alpha\mathbf{G}_r\mathbf{y}_r+{\mathbf{G}_r\mathbf{X}_r}\boldsymbol{\gamma}+\boldsymbol{\varepsilon}_r$, where $c_r$ is not observed, $\mathbf{1}_r$ is an $N_r$-dimensional vector of ones, $N_r$ is the size of the group r, $\bG_r$ is the subinteraction matrix in the group r, and $\bepsilon_r$ is the vector of error terms in the group r.

Under Assumption \ref{as:manymarkets}, it is not possible to obtain a consistent estimator of $\{c_r\}_{r=1}^m$ because the number of observations used to estimate each $c_r$ is bounded. This is known as the \emph{incidental parameter problem}.\footnote{See \cite{lancaster2000incidental} for a review.} A common strategy is to use deviations from the group average and estimate the model in deviations (e.g. \cite{bramoulle2009identification}).

Let $\mathbf{J}=diag\{\mathbf{I}_{N_r}-\frac{1}{N_r}\mathbf{1}_r\mathbf{1}'_r\}$ be the group-differentiating matrix, where $\mathbf{I}_{N_r}$ is the identified matrix of dimension $N_r$. The operator \emph{diag} generates a blog-diagonal matrix in which each group is a block.\footnote{Then, $\mathbf{Jw}$ gives $\mathbf{w}$ minus the group average of $\mathbf{w}$.} We can rewrite: $\mathbf{Jy}=\mathbf{JX}\boldsymbol{\beta}+\alpha{\mathbf{JG}\mathbf{y}}+{\mathbf{JGX}}\boldsymbol{\gamma}+\boldsymbol{J\varepsilon}$. Note that the results of Propositions \ref{prop:gamma0} and \ref{prop:gammanot0} extend directly, using instruments in deviation with the group average.

\subsection{Finite Sample Performance Using ARD}\label{sec:ard}
In this section, we study the small sample performance of the estimator presented in Section \ref{sec:iv} when the researcher only has access to ARD (as in Example \ref{ex:ard}). First, we simulate network data using the model proposed by \cite{breza2017using} and simulate outcomes using the linear in means model (\ref{eq:linearinmean}) conditional on the simulated networks. Second, we estimate the network formation model using the Bayesian estimator proposed by \cite{breza2017using} (yielding $\hat{\boldsymbol{\rho}}_B$), as well as using the classical estimator proposed by \cite{alidaee2020recovering} (yielding $\hat{\boldsymbol{\rho}}_A$). Third, we estimate the linear-in-means model, using our IV estimator based on $\hat{\boldsymbol{\rho}}_A$ and $\hat{\boldsymbol{\rho}}_B$.

Recall that
\begin{equation}\label{eq:ard}
P(a_{ij}=1)\propto\exp\{\nu_i+\nu_j+\zeta \mathbf{z}_i'\mathbf{z}_j\},    
\end{equation}
where $\nu_i$, $\nu_j$, $\zeta$, $\mathbf{z}_i$, and $\mathbf{z}_j$ are not observed by the econometrician but follow parametric distributions. We refer the interested reader to \cite{mccormick2015latent}, \cite{breza2017using}, and \cite{breza2019consistently} for a formal discussion of the model, including its identification and consistent estimation. Here, we discuss the intuition using a simple analogy.

Suppose that individuals are located according to their geographical position on Earth. Suppose also that there are a fixed number of cities on Earth in which individuals can live. The econometrician does not know the individuals' locations on Earth nor do they know the location of the cities. In model (\ref{eq:ard}), $\mathbf{z}_i$ represent $i$'s position on Earth. However, the econometrician has access to ARD for a subset of the population, i.e. answers to questions such as, ``How many of your friends live in city $A$?''

To understand the intuition behind the identification of the model, consider the following example: suppose that individual $i$ has many friends living in city $A$. Then, city $A$ is likely located close to $i$'s location. Similarly, if many individuals have many friends living in city $A$, then city $A$ is likely a large city. Finally, if $i$ has many friends from many cities, $i$ likely has a large $\nu_i$.

To study the finite sample performance of our instrumental strategy in this context, we simulate 20 groups of 250 individuals each. Within each subpopulation, we simulate the ARD responses as well as a series of observable characteristics (e.g. cities). The details of the Monte Carlo simulations can be found in Appendix \ref{sec:ardsetting}.

Importantly, the model in (\ref{eq:ard}) is based on a single population framework. Thus, the network formation model must be estimated separately for each of the 20 groups. With only 250 individuals in each group, we therefore expect significant small-sample bias.

We contrast the estimator proposed by \cite{breza2017using} with the one proposed by \cite{alidaee2020recovering}. Whereas \cite{breza2017using} present a parametric Bayesian estimator, \cite{alidaee2020recovering} propose a (nonparametric) penalized regression based on a low-rank assumption. One main advantage of their estimator is that it allows for a wider class of model and ensures that the estimation is fast and easily implementable.\footnote{The authors developed user-friendly packages in R and Python. See their paper for links and details.} Note, however, that their method only yields a consistent estimator of $\hat{P}(\mathbf{A})$ if the true network is effectively low rank.

Very intuitively, the low-rank assumption implies that linking probabilities were generated from a small number of parameters; for example, in the example above, knowing individuals' gregariousness parameters $\nu_i$ and city in which they live would allow a prediction of the linking probabilities.

Importantly, the model (\ref{eq:ard}) is not necessarily low rank; for example, if the individuals' locations on Earth (i.e. the $\mathbf{z}_i$'s) are uniformly distributed and there are only very few  large cities, then the model produced is not low rank and the method proposed by \cite{alidaee2020recovering} performs poorly. Intuitively, in such a case, the fact that individual $i$ lives in city $A$ poorly explains the linking probabilities. 

We compare the performance of both estimators as we vary the concentration parameter for the individuals' locations on Earth (that is, $\kappa$, see Appendix \ref{sec:ardsetting} for details). This has the effect of changing the \emph{effective rank} of the linking probabilities: increasing $\kappa$ decreases the effective rank.\footnote{We refer the interested reader to \cite{alidaee2020recovering} for a formal discussion of the effective rank and of its importance for their estimator.} We therefore expect the estimator proposed by \cite{alidaee2020recovering} to perform better for larger values of $\kappa$.

Results are presented in Tables \ref{tab:breza} and \ref{tab:alidaee}. When $\mathbf{Gy}$ is observed, both estimators perform extremely well. In light of Propositions \ref{prop:gamma0} and \ref{prop:gammanot0}, this is expected, as the IV estimator is valid even under misspecification. When $\mathbf{Gy}$ is not observed, results are more nuanced. First, note that for all specifications, the introduction of the non-pertinent variables $\ddot{\mathbf{G}}\mathbf{X}$ contaminates the estimation of $\boldsymbol{\gamma}$. This occurs because ${\mathbf{G}}\mathbf{X}$ and $\ddot{\mathbf{G}}\mathbf{X}$ are highly correlated.\footnote{This is a small sample issue which is not due to the assumed network formation model and would arise even if the linking probabilities were known (instead of being estimated).} Note, however, that the estimated values for $\boldsymbol{\gamma}+\check{\boldsymbol{\gamma}}$ are centered on the true value. Second, the bias of the estimated endogenous peer effect (i.e. $\alpha$) goes to zero when the linking probabilities are of lower rank, with an advantage for the estimator proposed by  \cite{breza2017using}. This is expected because the model is correctly specified and the estimator is parametric. 

Overall, our IV estimator can be successfully implemented in small samples, using either the estimator proposed by \cite{breza2017using} or by \cite{alidaee2020recovering}, both of which only rely on the observation of ARD.

\renewcommand{\arraystretch}{.9}
\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD - network distribution estimated following \cite{breza2017using} } 
\label{tab:breza}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}d{4}d{4}d{4}d{4}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 0$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1ex]                                             
$\alpha=0.4$    & 0.400  & 0.007 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$                & 5.000  & 0.021 & 4.986   & 5.000  & 5.014   \\
$\gamma_2=-3$              & -3.001 & 0.031 & -3.021  & -3.000 & -2.980  \\  
F-test (Weak inst.) & 3144.574&	874.400&	2492.881&	3075.955&	3672.449 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                                          
$\alpha=0.4$ & 0.371  & 0.013 & 0.363   & 0.372  & 0.380   \\
$\gamma_1=5$            & 5.396  & 0.021 & 5.383   & 5.397  & 5.410   \\
$\gamma_2=-3$          & -2.400 & 0.041 & -2.428  & -2.400 & -2.371  \\
$\hat{\gamma}_1=0$          & -0.380 & 0.028 & -0.400  & -0.382 & -0.362  \\
$\hat{\gamma}_2=0$           & -0.553 & 0.044 & -0.584  & -0.551 & -0.525  \\
F-test (Weak inst.) & 3193.940&	760.793&	2642.815&	3153.048&	3666.220 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 10$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                                              
$\alpha=0.4$   & 0.400  & 0.006 & 0.396   & 0.400  & 0.404   \\
$\gamma_1=5$                & 5.001  & 0.019 & 4.988   & 5.001  & 5.014   \\
$\gamma_2=-3$             & -3.000 & 0.031 & -3.020  & -3.000 & -2.978  \\
F-test (Weak inst.) & 5905.596&	1876.836&	4519.460&	5766.601&	7158.739 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                                          
$\alpha=0.4$ & 0.400  & 0.007 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$            & 5.392  & 0.019 & 5.379   & 5.393  & 5.405   \\
$\gamma_2=-3$          & -2.397 & 0.037 & -2.421  & -2.398 & -2.373  \\
$\hat{\gamma}_1=0$           & -0.391 & 0.022 & -0.405  & -0.390 & -0.375  \\
$\hat{\gamma}_2=0$          & -0.604 & 0.038 & -0.630  & -0.605 & -0.579  \\
F-test (Weak inst.) & 5176.649&	1507.532&	4058.393&	5087.275&	6243.500 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 20$, $N=250$, $M=20$}                                                            \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                                             
$\alpha=0.4$    & 0.400  & 0.006 & 0.396   & 0.400  & 0.404   \\
$\gamma_1=5$                & 5.000  & 0.020 & 4.986   & 4.999  & 5.013   \\
$\gamma_2=-3$            & -3.001 & 0.031 & -3.021  & -3.001 & -2.981  \\
F-test (Weak inst.) &6104.999&	1927.633&	4734.460&	5937.815&	7246.355 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]   
$\alpha=0.4$ & 0.400  & 0.007 & 0.396   & 0.400  & 0.405   \\
$\gamma_1=5$            & 5.390  & 0.019 & 5.377   & 5.390  & 5.403   \\
$\gamma_2=-3$          & -2.398 & 0.036 & -2.422  & -2.398 & -2.375  \\
$\hat{\gamma}_1=0$           & -0.390 & 0.022 & -0.405  & -0.390 & -0.376  \\
$\hat{\gamma}_2=0$          & -0.604 & 0.036 & -0.628  & -0.604 & -0.579 \\ 
F-test (Weak inst.) & 5321.702&	1524.973&	4272.790&	5199.232&	6235.250 \\ 
\hline \\[-1.8ex] 


\multicolumn{6}{l}{%
  \begin{minipage}{15cm}%
    \footnotesize{Note: In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with a location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in Appendix \ref{sec:ardsetting}. Predicted probabilities are computed using the mean of the posterior distribution. F-test is the Fisher-statistic of the Weak instruments test. We do not report the estimated values for $c$ and $\boldsymbol{\beta}$ to keep the table readable, but they are available upon request. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.}
  \end{minipage}%
}\end{tabular}
\end{table}

\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD - network distribution estimated following \cite{alidaee2020recovering} } 
\label{tab:alidaee}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}d{4}d{4}d{4}d{4}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 0$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1ex]                                
$\alpha=0.4$     & 0.400  & 0.012 & 0.393   & 0.400  & 0.407   \\
$\gamma_1=5$             & 5.000  & 0.029 & 4.980   & 4.999  & 5.019   \\
$\gamma_2=-3$             & -3.000 & 0.032 & -3.021  & -3.000 & -2.978  \\
F-test (Weak inst.) & 798.971&	340.558&	560.817&	749.132&	990.407\\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                          
$\alpha=0.4$ & 0.371  & 0.024 & 0.357   & 0.373  & 0.387   \\
$\gamma_1=5$              & 5.504  & 0.036 & 5.479   & 5.503  & 5.528   \\
$\gamma_2=-3$            & -2.480 & 0.057 & -2.517  & -2.480 & -2.441  \\
$\hat{\gamma}_1=0$           & -0.364 & 0.031 & -0.385  & -0.363 & -0.344  \\
$\hat{\gamma}_2=0$          & -0.302 & 0.070 & -0.349  & -0.304 & -0.254  \\
F-test (Weak inst.) & 590.248&	253.853&	409.497&	572.210&	721.788 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 10$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                              
$\alpha=0.4$    & 0.400  & 0.009 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$         & 4.999  & 0.022 & 4.985   & 4.999  & 5.014   \\
$\gamma_2=-3$                & -3.000 & 0.032 & -3.022  & -3.001 & -2.978 \\
F-test (Weak inst.) & 1697.514&	741.478&	1179.079&	1593.284&	2127.582\\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                          
$\alpha=0.4$  & 0.395  & 0.021 & 0.388   & 0.397  & 0.405   \\
$\gamma_1=5$            & 5.396  & 0.027 & 5.378   & 5.394  & 5.412   \\
$\gamma_2=-3$            & -2.412 & 0.045 & -2.439  & -2.410 & -2.383  \\
$\hat{\gamma}_1=0$          & -0.385 & 0.032 & -0.404  & -0.387 & -0.370  \\
$\hat{\gamma}_2=0$           & -0.462 & 0.117 & -0.534  & -0.483 & -0.414  \\
F-test (Weak inst.) &1303.291&	586.429&	895.070&	1227.426&	1652.148\\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 20$, $N=250$, $M=20$}                                                            \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                              
$\alpha=0.4$     & 0.400  & 0.008 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$                & 5.000  & 0.021 & 4.985   & 5.000  & 5.013   \\
$\gamma_2=-3$             & -2.999 & 0.032 & -3.020  & -2.999 & -2.979   \\
F-test (Weak inst.) & 2685.354&	978.512&	1998.396&	2601.996&	3268.714 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]   
$\alpha=0.4$ & 0.399  & 0.010 & 0.393   & 0.400  & 0.406   \\
$\gamma_1=5$        & 5.391  & 0.020 & 5.378   & 5.391  & 5.404   \\
$\gamma_2=-3$             & -2.400 & 0.039 & -2.425  & -2.400 & -2.374  \\
$\hat{\gamma}_1=0$           & -0.391 & 0.022 & -0.406  & -0.391 & -0.376  \\
$\hat{\gamma}_2=0$          & -0.573 & 0.047 & -0.605  & -0.575 & -0.544 \\ 
F-test (Weak inst.) & 2191.313&	774.366&	1656.355&	2130.681&	2668.781\\ 
\hline \\[-1.8ex] 



\multicolumn{6}{l}{%
  \begin{minipage}{15cm}%
    \footnotesize{Note: In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in Appendix \ref{sec:ardsetting}. We chose the weight associated with the nuclear norm penalty to minimize the RMSE through cross-validation. This value of $\lambda=600$ is smaller than the recommended value in \cite{alidaee2020recovering}. F-test is the Fisher-statistic of the Weak instruments test. We do not report the estimated values for $c$ and $\boldsymbol{\beta}$ to keep the table readable, but they are available upon request. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.}
  \end{minipage}%
}\end{tabular}
\end{table}
\renewcommand{\arraystretch}{1}

==> archives/forQE/addhealth.tex <==

\section{Imperfectly Measured Networks}\label{sec:addhealth}

In this section, we assume that the econometrician has access to network data but that the data may contain errors. To show how our method can be used to address these issues, we consider a simple example where we are interested in estimating peer effects on adolescents' academic achievements.

We use the widely used AddHealth database and show that network data errors have a first-order impact on the estimated peer effects. Specifically, we focus on a subset of schools from the ``In School'' sample that each have less than 200 students. Table \ref{tab:sumstats} displays the summary statistics.

\begin{table}[!htbp] 
   \centering 
  \caption{Summary statistics} 
  \label{tab:sumstats} 
\begin{tabular}{@{\extracolsep{5pt}} lld{3}ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
\multicolumn{2}{l}{Statistic} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline \\[-1.8ex] 
\multicolumn{2}{l}{Female} & 0.540 & 0.498 & 0 & 1 \\ 
\multicolumn{2}{l}{Hispanic}  & 0.157 & 0.364 & 0 & 0 \\ 
\multicolumn{2}{l}{Race} &  &  &  &  \\ 
 & White & 0.612 & 0.487 & 0 & 1 \\ 
 & Black & 0.246 & 0.431 & 0 & 0 \\ 
 & Asian & 0.022 & 0.147 & 0 & 0 \\ 
 & Other & 0.088 & 0.283 & 0 & 0 \\ 
\multicolumn{2}{l}{Mother's education}  &  &  &  &  \\ 
 & High & 0.310 & 0.462 & 0 & 1 \\ 
 & <High & 0.193 & 0.395 & 0 & 0 \\ 
 & >High & 0.358 & 0.480 & 0 & 1 \\ 
 & Missing & 0.139 & 0.346 & 0 & 0 \\ 
\multicolumn{2}{l}{Mother's job}  &  &  &  &  \\ 
 & Stay-at-home & 0.225 & 0.417 & 0 & 0 \\ 
 & Professional & 0.175 & 0.380 & 0 & 0 \\ 
 & Other & 0.401 & 0.490 & 0 & 1 \\ 
 & Missing & 0.199 & 0.399 & 0 & 0 \\ 
\multicolumn{2}{l}{Age}  & 13.620 & 1.526 & 13 & 14 \\ 
\multicolumn{2}{l}{GPA}  & 2.912    &0.794    &2.333      &3.5\\ 
\hline \\[-1.8ex] 
\multicolumn{6}{l}{%
  \begin{minipage}{11.6cm}%
    \footnotesize{Note: We only keep the 33 schools having less than 200 students from the In-School sample. The variable GPA is computed by taking the average grade for English, Mathematics, History, and Science, letting $A=4$, $B=3$, $C=2$, and $D=1$. Thus, higher scores indicate better academic achievement.}
  \end{minipage}%
  }
\end{tabular} 

\end{table} 

Most papers estimating peer effects that use this particular database have taken the network structure as given. One notable exception is \cite{griffith2019namefriends}, looking at censoring: students can only report up to five male and five female friends. We also allow for censoring but show that censoring is not the most important issue with the Add Health data. To understand why, we discuss the organization of the data.

Each adolescent is assigned a unique identifier. The data includes ten variables for the ten potential friendships (maximum of five male and five female friends). These variables can contain missing values (no friendship was reported), an error code (the named friend could not be found in the database), or an identifier for the reported friends. This data is then used to generate the network's adjacency matrix $\mathbf{A}$.

Of course, error codes cannot be matched to any particular adolescent. Moreover, even in the case where the friendship variable refers to a valid identifier, the referred adolescent may still be absent from the database. A prime example is when the referred adolescent has been removed from the database by the researcher, perhaps because of other missing variables for these particular individuals. These missing links are quantitatively important as they account for roughly 30\% of the total number of links (7,830 missing for 17,993 observed links). Figure \ref{fig:misfr} displays the distribution of the number of ``unmatched named friends.''\footnote{We focus on within-school friendships; thus, nominations outside of school are not treated as ``unmatched friends.''}
\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.6]{graphs/Missing.pdf}
    \caption{Frequencies of the number of missing links per adolescent}
    \label{fig:misfr}
\end{figure}

To use the methodology developed in Section \ref{sec:genestim}, we first need to estimate a network formation model using the observed network data. In this section, we assume that links are generated using a simple logistic framework, i.e.
$$
P(a_{ij}=1)\propto\exp\{\mathbf{w}_{ij}\boldsymbol{\rho}\},
$$
where $\mathbf{w}_{ij}$ is built to capture homophily on the observed characteristics of $i$ and $j$ (see Tables \ref{tab:appendapplicationB} and \ref{tab:appendapplicationG} in Appendix \ref{sec:addhealth_appendix}). We estimate the network formation model on the set of individuals for which we observe no ``unmatched friends.'' For these students, we know for sure that their friendship data is complete. Under a missing at-random assumption, the estimation of the explanatory variables is consistent, but the intercept is affected by a selection bias. We control for this by weighting the log-likelihood of the network following \cite{manski1977estimation}. The details are presented in Appendix \ref{sec:addhealth_appendix}.

We present the estimation results for the SGMM and for the Bayesian estimator. Figure \ref{fig:ahestimations} summarizes the results for the endogenous peer effect coefficient $\alpha$, whereas the full set of results is presented in Appendix \ref{sec:addhealth_appendix}. The first two estimations (\emph{Obsv.Bayes} and \emph{Obsv.SGMM}) assume that the observed network is the true network for both estimators. The third and fourth estimations (\emph{Miss.Bayes} and \emph{Miss.SGMM}) account for missing data due to error codes but not for censoring. The last two estimations (\emph{TopMiss.Bayes} and \emph{TopMiss.SGMM}) account for missing data due to error codes or censoring.


\begin{figure}[h]
    \centering
    \includegraphics[scale=0.8]{graphs/PeerEffects.pdf}
    \caption{Peer effect estimate}
    \label{fig:ahestimations}

      \begin{minipage}{14cm}%
  \vspace{0.3cm}
    \footnotesize{Note: Dots represent estimated values (and posterior mean) of $\alpha$, and bars represent 95\% confidence intervals (and 95\% credibility intervals). Tables \ref{tab:appendapplicationB} and \ref{tab:appendapplicationG} in Appendix \ref{sec:addhealth_appendix} present the full set of estimated coefficients.}
  \end{minipage}%
\end{figure}

We first see that the SGMM is less efficient than the Bayesian. This should not be surprising since the Bayesian estimator uses more structure (in particularity homoscedastic, normally distributed errors). When we compare the estimations \emph{Obsv.SGMM} and \emph{Miss.SGMM}, the observed differences imply that the efficiency loss is because of the properties of the estimator and not the missing links.\footnote{Recall that when the network is observed, our SGMM uses the same moment conditions as, for example, those suggested by \cite{bramoulle2009identification}.}

Importantly, we see that the bias due to the assumption that the network is fully observed is quantitatively and qualitatively important. Using either estimator, the estimated endogenous peer effect using the reconstructed network is 1.5 times larger than thatestimated assuming the observed network is the true network.\footnote{The difference is ``statistically significant'' for the Bayesian estimator.} Almost all of the bias is produced by the presence of error codes and not because of potential censoring.

This exercise shows that data errors are a first-order concern when using the Add Health database.\footnote{We do not argue, however, that our estimated coefficients are necessarily causal because the friendship network is likely endogenous (e.g. \cite{goldsmith2013social,hsieh2018smoking,hsieh2019specification}). The estimation of peer effects with partial endogenous network data is left for future research.} Not only does the bias in the endogenous peer effect coefficient $\alpha$ have an impact on the social multiplier \citep{glaeser2003social}, but it can also affect the anticipated effect of targeted interventions, i.e. the identity of the key player \citep{ballester2006s}.

Indeed, Figure \ref{fig:centrality} shows a scatter plot of the vector of centralities in the observed and reconstructed networks. The figure illustrates the effects of missing network data. First, because the reconstructed network has more links, centrality is higher on average. This is essentially the social multiplier effect. Not accounting for missing links leads to an underestimation of spillover effects.
Second, some individuals, in particular those having very few links in the observed network, are in reality highly central. Therefore, targeting a policy at individuals having a high centrality in the observed network would be inefficient. In particular, Figure \ref{fig:centrality2} shows that even isolated individuals and individuals interacting in isolated pairs in the observed network (having centralities of $1$ and $1.35$ respectively) can be, in reality, highly central. Thus, a policy based on the evaluation of an observed network, coupled with the associated endogenous peer effect coefficient $\alpha$, would not only underestimate the social multiplier but would also target the wrong individuals.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.7]{graphs/centralityscatter.pdf}
    \caption{Centrality}
    \label{fig:centrality}
    
      \begin{minipage}{14cm}%
  \vspace{0.3cm}
    \footnotesize{Note: The centrality vector is given by $(\mathbf{I}-\hat{\alpha}\mathbf{G})^{-1}\mathbf{1}$. To compute centrality based on the observed network, we use the observed network $\mathbf{G}$ and the $\hat{\alpha}$ estimated using specification \emph{Obsv.Bayes}. To compute centrality based on the reconstructed network, we use $\hat{\alpha}$ and $\mathbf{G}$ estimated using the specification \emph{TopMiss.Bayes}. For both centrality vectors, we use the average vector centrality across 10 000 draws from their respective posterior distributions.}
  \end{minipage}%
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[scale=0.7]{graphs/centrality.pdf}
    \caption{Centrality}
    \label{fig:centrality2}
    \begin{minipage}{14cm}%
  \vspace{0.3cm}
    \footnotesize{Note: See note of Figure \ref{fig:centrality}.}
  \end{minipage}%
\end{figure}




==> archives/forQE/bayesian.tex <==

\section{Estimation Using Bayesian Inference}\label{sec:genestim}

In the previous section, we showed that in a context in which $\mathbf{Gy}$ and $\mathbf{GX}$ are unobserved and the distribution of the network is imprecise, the SGMM estimator can be imprecise. In this section, we therefore present a likelihood-based estimator. Accordingly, greater structure must be imposed on the errors $\boldsymbol{\varepsilon}$.\footnote{One could also use our estimator to solve a classical estimator, for example a GMM estimator such as that proposed by \cite{chandrasekhar2011econometrics}, using either the approach proposed by \cite{chernozhukov2003mcmc}, or the Bayesian empirical likelihood approach of \cite{chib2018bayesian}.}

To clarify the exposition, we will focus on the network adjacency matrix $\mathbf{A}$ rather than the interaction matrix $\mathbf{G}$. Of course, this is without any loss of generality. Given parametric assumptions for $\boldsymbol{\varepsilon}$, one can write the log-likelihood of the outcome as \footnote{Note that under Assumption \ref{as:manymarkets}, the likelihood can be factorized across groups.}
\begin{equation}\label{eq:likelihood}
\ln \mathcal{P}(\mathbf{y}|\mathbf{A},\boldsymbol{\theta}),    
\end{equation}
where $\boldsymbol{\theta}=[\alpha,\boldsymbol{\beta}',\boldsymbol{\gamma}',\boldsymbol{\sigma}']'$, and $\boldsymbol{\sigma}$ are unknown parameters from the distribution of $\boldsymbol{\varepsilon}$. Note that $\mathbf{y}=(\mathbf{I}_N-\alpha\mathbf{G})^{-1}(c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+{\mathbf{GX}}\boldsymbol{\gamma}+\boldsymbol{\varepsilon})$ and $(\mathbf{I}_N-\alpha\mathbf{G})^{-1}$ exists under our Assumption \ref{as:alpha}.

If the adjacency matrix $\mathbf{A}$ is observed, then $\boldsymbol{\theta}$ could be estimated using a simple maximum likelihood estimator (as in \cite{lee2010specification}) or using Bayesian inference (as in \cite{goldsmith2013social}).

Since $\mathbf{A}$ is not observed, an alternative would be to focus on the unconditional likelihood, i.e.
$$
\ln \mathcal{P}(\mathbf{y}|\boldsymbol{\theta})=\ln \sum_\mathbf{A}\mathcal{P}(\mathbf{y}|\mathbf{A},\boldsymbol{\theta})P(\mathbf{A}).
$$
A similar strategy is proposed by \cite{chandrasekhar2011econometrics} using a GMM estimator.

One particular issue with estimating $\ln \mathcal{P}(\mathbf{y}|\boldsymbol{\theta})$ is that the summation is not tractable. Indeed, the sum is over the set of possible adjacency matrices, which contain $2^{N(N-1)}$ elements. Then, simply simulating networks from $P(\mathbf{A})$ (or rather from $\hat{P}(\mathbf{A})$) and taking the average likely lead to poor approximations. A classical way to address this issue is to use an EM algorithm \citep{dempster1977maximum}. Although valid, we found that the Bayesian estimator proposed in this section is less restrictive and numerically outperforms its classical counterpart.

For concreteness, we will assume that $\boldsymbol{\varepsilon}\sim\mathcal{N}(0,\sigma^2\mathbf{I}_N)$; however, it should be noted that our approach is valid for a number of alternative assumptions as long as it yields a computationally tractable likelihood. We have, for $\mathbf{G}=f(\mathbf{A})$,
\begin{eqnarray*}
\ln \mathcal{P}(\mathbf{y}|\mathbf{A},\boldsymbol{\theta})&=&-N\ln(\sigma)+\ln|\mathbf{I}_N-\alpha\mathbf{G}|-\frac{N}{2}\ln(\pi)\\&&-\frac{1}{2\sigma^2}[(\mathbf{I}_N-\alpha\mathbf{G})\mathbf{y}-c\mathbf{1}_N-\mathbf{X}\boldsymbol{\beta}-\mathbf{GX}\boldsymbol{\gamma}]'\cdot\\ &&[(\mathbf{I}_N-\alpha\mathbf{G})\mathbf{y}-c\mathbf{1}_N-\mathbf{X}\boldsymbol{\beta}-\mathbf{GX}\boldsymbol{\gamma}].
\end{eqnarray*}
Because $\mathbf{A}$ is not observed, we follow \cite{tanner1987calculation} and \cite{albert1993bayesian}, and we use data augmentation to evaluate the posterior distribution of $\boldsymbol{\theta}$. That is, instead of focusing on the posterior $p(\boldsymbol{\theta}|\mathbf{y},\mathbf{A})$, we focus on the posterior $p(\boldsymbol{\theta},\mathbf{A}|\mathbf{y},\mathcal{A})$, treating $\mathbf{A}$ as another set of unknown parameters. Note that we now make  the dependence on $\mathcal{A}$ explicit for clarity.

Indeed, the identification of the model rests on the a priori information of $\mathbf{A}$. A sensible prior for $\mathbf{A}$ is the consistent estimator of its distribution, i.e. $\hat{P}(\mathbf{A}|\mathcal{A})\equiv P(\mathbf{A}|\hat{\boldsymbol{\rho}},\mathcal{A})$. One may wish, however, to also use the information regarding the sampling uncertainty around $\hat{P}(\mathbf{A}|\mathcal{A})$. This is very similar to the inference for two-step estimators in a classical setting (e.g. for our SGMM estimator); estimation uncertainty in the first stage must be accounted for to provide valid inference in the second stage (see Section \ref{sec:iv}).

Let $\pi(\boldsymbol{\rho}|\mathcal{A})$ be the prior density on $\boldsymbol{\rho}$. How to obtain $\pi(\boldsymbol{\rho}|\mathcal{A})$, depending on whether $\hat{\boldsymbol{\rho}}$ is obtained using a Bayesian or classical setting, is discussed in Examples \ref{ex:prior_distr} and \ref{ex:prior_post} below. Given $\pi(\boldsymbol{\rho}|\mathcal{A})$, it is possible to obtain draws from the posterior distribution $p(\boldsymbol{\rho},\mathbf{A}|\mathbf{y},\mathcal{A})$ using the following MCMC:
\begin{algorithm}\label{algo:mcmc} The MCMC goes as follows for $t=1,...,T$, starting from any $\mathbf{A}_0,\boldsymbol{\theta}_0$, and $\boldsymbol{\rho}_0$.
\begin{enumerate}
    \item Draw $\boldsymbol{\rho}^*$ from the proposal distribution $q_\rho(\boldsymbol{\rho}^*|\boldsymbol{\rho}_{t-1})$ and accept $\boldsymbol{\rho}^*$ with probability
    $$
    \min\left\lbrace 1,\frac{P(\mathbf{A}_{t-1}|\boldsymbol{\rho}^*,\mathcal{A})q_\rho(\boldsymbol{\rho}_{t-1}|\boldsymbol{\rho}^*)\pi(\boldsymbol{\rho}^*|\mathcal{A})}
    {P(\mathbf{A}_{t-1}|\boldsymbol{\rho}_{t-1},\mathcal{A})q_\rho(\boldsymbol{\rho}^*|\boldsymbol{\rho}_{t-1})\pi(\boldsymbol{\rho}_{t-1}|\mathcal{A})} \right\rbrace.
    $$
    \item Propose $\mathbf{A}^*$ from the proposal distribution $q_A(\mathbf{A}^*|\mathbf{A}_{t-1})$ and accept $\mathbf{A}^*$ with probability
    $$
    \min\left\lbrace 1,\frac{\mathcal{P}(\mathbf{y}|\boldsymbol{\theta}_{t-1},\mathbf{A}^*)q_A(\mathbf{A}_{t-1}|\mathbf{A}^*)P(\mathbf{A}^*|{\boldsymbol{\rho}_{t-1}},\mathcal{A})}{\mathcal{P}(\mathbf{y}|\boldsymbol{\theta}_{t-1},\mathbf{A}_{t-1})q_A(\mathbf{A}^*|\mathbf{A}_{t-1})P(\mathbf{A}_{t-1}|{\boldsymbol{\rho}_{t-1}},\mathcal{A})} \right\rbrace.
    $$
    \item Draw $\alpha^*$ from the proposal $q_\alpha(\cdot|\alpha_{t-1})$ and accept $\alpha^*$ with probability
    $$
    \min\left\lbrace 1,\frac{\mathcal{P}(\mathbf{y}|\mathbf{A}_{t};\boldsymbol{\beta}_{t-1},\boldsymbol{\gamma}_{t-1},\alpha^*)q_\alpha(\alpha_{t - 1}|\alpha^*)\pi(\alpha^*)}{\mathcal{P}(\mathbf{y}|\mathbf{A}_{t};\boldsymbol{\theta}_{t-1})q_\alpha(\alpha^*|\alpha_{t-1})\pi(\alpha_{t-1})}\right\rbrace.
    $$
    \item Draw $[\boldsymbol{\beta,\gamma},\sigma]$ from their conditional distributions.
\end{enumerate}
\end{algorithm}

As discussed, Step 1 accounts for the sampling uncertainty around the true value of $\boldsymbol{\rho}$. If the true value of $\boldsymbol{\rho}$ was known (instead of being estimated), Step 1 would not be required. Step 1 shows that the flexibility of the network formation model comes at a cost. For example, \cite{graham2017econometric} and \cite{breza2017using} propose network formation models for which the number of parameters is $O(N_r)$. In turn, this large number of parameters increases the computational cost of Step 1.


\begin{example}[Priors from the Asymptotic Distribution of $\boldsymbol{\rho}$]\label{ex:prior_distr}
In a classical setting, and under the usual assumptions, the estimation of (\ref{eq:gennetfor}) produces an estimator $\hat{\boldsymbol{\rho}}$ of $\boldsymbol{\rho}_0$ and an estimator of the asymptotic variance of $\hat{\boldsymbol{\rho}}$, i.e. $\hat{\mathbf{V}}(\hat{\boldsymbol{\rho}})$. In this case, we define the prior density $\pi(\boldsymbol{\rho})$ as the density of a multivariate normal distribution with mean $\hat{\boldsymbol{\rho}}$ and variance--covariance matrix $\hat{\mathbf{V}}(\hat{\boldsymbol{\rho}})$.
\end{example}

\begin{example}[Priors from the Posterior Distribution of $\boldsymbol{\rho}$]\label{ex:prior_post}
In a Bayesian setting, the estimation of $\boldsymbol{\rho}$ from the network formation model (\ref{eq:gennetfor}) results in draws from the posterior distribution of $\boldsymbol{\rho}$. It is therefore natural to use such a posterior distribution as the prior distribution of $\mathbf{A}$ for the estimation based on (\ref{eq:likelihood}). Performing such a sequential Bayesian updating approach comes with a well-known numerical issue.\footnote{See \cite{thijssen2020approximating} for a recent discussion.}

Indeed, the evaluation of the acceptance ratio in Step 1 of Algorithm \ref{algo:mcmc} below requires the evaluation of the density of $\boldsymbol{\rho}$ at different values. Ideally, one would use the draws from the posterior distribution of $\boldsymbol{\rho}$ from the first step (network formation model) and perform a nonparametric kernel density estimation of the posterior distribution. However, when the dimension of $\boldsymbol{\rho}$ is large, the kernel density estimation may be infeasible in practice.

This is especially true for very flexible network formation models, such as that proposed by \cite{breza2017using} for which the number of parameters to estimate is $O(N_r)$. In such a case, it might be more reasonable to use a more parametric approach or to impose additional restrictions on the dependence structure of $\boldsymbol{\rho}$ across dimensions.\footnote{For example, if we assume that the posterior distribution of $\boldsymbol{\rho}$ is jointly normal, the estimation of the mean and variance--covariance matrix is straightforward, even in a high-dimensional setting. Simulations suggest that this approach performs well in practice. See the Vignette accompagning our R package.}
\end{example}


Detailed distributions for Steps 3 and 4 can be found in the Online Appendix. Step 2, however, requires some discussion. Indeed, the idea is the following: given the prior information $P(\textbf{A}|\boldsymbol{\rho}_{t-1},\mathcal{A})$, one must be able to draw samples from the posterior distribution of $\mathbf{A}$, given $\mathbf{y}$. This is not a trivial task.

In particular, there is no general rule for selecting the network proposal distribution $q_A(\cdot\vert\cdot)$. A natural candidate is a Gibbs sampling algorithm for each link, i.e. change only one link $ij$ at every step $t$ and propose $a_{ij}$ according to its marginal distribution, i.e. $a_{ij}\sim P(\cdot|\mathbf{A}_{-ij},\mathbf{y},\mathcal{A})$, where $\mathbf{A}_{-ij} = \{a_{kl}; k \ne i, l \ne j\}$. In this case, the proposal is always accepted.
%$$
%a_{ij}\sim P(\cdot|\mathbf{A}_{-ij},\mathbf{y},\mathcal{A})=\frac{\mathcal{P}(\mathbf{y}|a_{ij},\mathbf{A}_{-ij})P(a_{ij}|\mathbf{A}_{-ij};\tilde{\boldsymbol{\rho}},\mathcal{A})}{\mathcal{P}(\mathbf{y}|1,\mathbf{A}_{-ij})P(a_{ij}=1|\mathbf{A}_{-ij};\tilde{\boldsymbol{\rho}},\mathcal{A})+\mathcal{P}(\mathbf{y}|0,\mathbf{A}_{-ij})P(a_{ij}=0|\mathbf{A}_{-ij};\tilde{\boldsymbol{\rho}},\mathcal{A})},
%$$

However, it has been argued that Gibbs sampling could lead to slow convergence (e.g. \cite{snijders2002markov}, \cite{chatterjee2013estimating}), especially when the network is \emph{sparse} or exhibits a high level of \emph{clustering}. For example, \cite{mele2017} and \cite{bhamidi2008mixing} propose different blocking techniques meant to improve convergence.

Here, however, achieving Step 2 involves an additional computational issue because evaluating the likelihood ratio in Step 1 requires comparing the determinants $|\mathbf{I}-\alpha f(\mathbf{A}^*)|$ for each proposed $\mathbf{A}^*$, which is computationally intensive. In particular, taking $\mathbf{G}^*=f(\mathbf{A}^*)$ to be a row-normalization of $\mathbf{A}^*$, altering a single element of $\mathbf{A}^*$ results in a change in the entire corresponding row of $\mathbf{G}^*$. Still, comparing the determinant of two matrices that differ only in a single row is relatively fast. Moreover, when $\mathbf{G}=\mathbf{A}$, \cite{hsieh2019structural} propose a blocking technique that facilitates the computation of the determinant.

In any case, note that the computational complexity of Step 2 depends strongly on $P(\textbf{A}|\boldsymbol{\rho}_{t-1},\mathcal{A})$, which is a function of the assumed network formation model (\ref{eq:gennetfor}) and the observed information about the network structure $\mathcal{A}$. For censored network data, for example, most of the network structure is observed (see Example \ref{ex:censored}). This implies that $P(a_{ij}|\boldsymbol{\rho}_{t-1},\mathcal{A})\in\{0,1\}$ for most pairs $ij$. As such, few entries of $\mathbf{A}$ must be updated in Step 2. The opposite is true for ARD (see Example \ref{ex:ard}) for which all entries of $\mathbf{A}$ must be updated.

Then, the appropriate blocking technique depends strongly on $P(\textbf{A}|\boldsymbol{\rho}_{t-1},\mathcal{A})$ and the assumed distribution for $\boldsymbol{\varepsilon}$. For the simulations and estimations presented in this paper, we use the Gibbs sampling algorithm for each link, adapting the strategy proposed by \cite{hsieh2019structural} to our setting (see Proposition \ref{prop:det} in the Online Appendix). This can be viewed as a \emph{worst-case} scenario. Nonetheless, the Gibbs sampler performs reasonably well in practice, even for ARD;\footnote{Simulations available upon request.} however, we encourage researchers to try other updating schemes if Gibbs sampling performs poorly in their specific contexts. In particular, we present a blocking technique in the Online Appendix \ref{sec:appendix_bayesian} that is also implemented in our R package \texttt{PartialNetwork}.\footnote{Available at: \url{https://github.com/ahoundetoungan/PartialNetwork}}

It is important to note that the complexity of Step 2 is not limited to our Bayesian approach. Classical estimators, such as GMM estimators, face a similar challenge in requiring the integration over the entire set of networks. The strategy used here is to rely on a Metropolis--Hastings algorithm, a strategy that has also been successfully implemented in the related literature on ERGMs (e.g. \cite{snijders2002markov,mele2017,mele2020does,badev2018nash,hsieh2019structural,hsieh2019specification}).

Finally, note that for simple network formation models, it is possible to jointly estimate $\boldsymbol{\rho}$ and $\boldsymbol{\theta}$ within the same MCMC instead of using the two-step procedure described above. In this case, Step 1 can simply be replaced by:
\begin{enumerate}
    \item[1'.]  Draw $\boldsymbol{\rho}^*$ from the proposal distribution $q_\rho(\boldsymbol{\rho}^*|\boldsymbol{\rho}_{t-1})$ and accept $\boldsymbol{\rho}^*$ with probability
    $$
    \min\left\lbrace 1,\frac{P(\mathbf{A}_{t-1}|\boldsymbol{\rho}^*,\mathcal{A})P(\mathcal{A}|\boldsymbol{\rho}^*)q_\rho(\boldsymbol{\rho}_{t-1}|\boldsymbol{\rho}^*)\pi(\boldsymbol{\rho}^*)}
    {P(\mathbf{A}_{t-1}|\boldsymbol{\rho}_{t-1},\mathcal{A})P(\mathcal{A}|\boldsymbol{\rho}_{t-1})q_\rho(\boldsymbol{\rho}^*|\boldsymbol{\rho}_{t-1})\pi(\boldsymbol{\rho}_{t-1})} \right\rbrace.
    $$
\end{enumerate}
Here, $P(\mathcal{A}|\boldsymbol{\rho}^*)$ is the likelihood of the network information $\mathcal{A}$ assuming the network formation model in (\ref{eq:gennetfor}). Note that $\pi(\boldsymbol{\rho})$, the prior density on $\boldsymbol{\rho}$, no longer depends on $\mathcal{A}$ and can be chosen arbitrarily (e.g. uniform).

This approach would work well for simple models, such as the ones discussed in Examples \ref{ex:sampled} and \ref{ex:misclass}. It is impractical, however, for more involved models, such as that proposed by \cite{breza2017using}.


==> archives/forQE/discussion.tex <==


\section{Conclusion} In this paper, we proposed two estimators where peer effects can be estimated without having knowledge of the entire network structure. We found, perhaps surprisingly, that even very partial information on network structure is sufficient. By specifying a network formation model, researchers can probabilistically reconstruct the true network and base the estimation of peer effects on this reconstructed network. Importantly, we provide computationally tractable and flexible estimators to do so, all of which are available in our R package \texttt{PartialNetwork}. We apply our methodology to the widely used AddHealth data and find that missing links due to noise in the data have first-order effects on the estimated peer effect coefficient. This leads to an underestimation of the social multiplier and the incorrect identification of the key players.


==> archives/forQE/intro.tex <==
\section{Introduction}
There is a large and growing literature on the impact of peer effects in social networks.\footnote{For recent reviews, see \cite{boucher2015some}, \cite{bramoulle2019peer}, \cite{breza2016}, and \cite{de2015econometrics}.} However, since eliciting network data is expensive \citep{breza2017using}, relatively few data sets contain comprehensive network information, and existing ones are prone to data errors. Despite some recent contributions, existing methodologies for the estimation of peer effects with incomplete or erroneous network data either focus on a specific kind of sampling or errors or they are highly computationally demanding.

In this paper, we propose a unifying framework that allows for the estimation of peer effects under the widely used linear-in-means model (e.g. \cite{manski1993identification,bramoulle2009identification}) when the researcher does not observe the entire network structure. Our methodology is computationally attractive and flexible enough to cover cases in which, for example, network data are sampled \citep{chandrasekhar2011econometrics,liu2013estimation,lewbel2019social}, censored \citep{griffith2019namefriends}, missclassified \citep{hardy2019estimating}, or summarized by aggregated relational data (ARD; \cite{breza2017using,alidaee2020recovering}). Our central assumption is that the researcher is able to estimate a network formation model using some partial information about the network structure. Leveraging recent contributions on the estimation of network formation models, we show that this assumption is sufficient to identify and estimate peer effects.

We propose two estimators. First, we present a computationally attractive estimator based on a simulated generalized method of moment (SGMM). The moments are built using draws from the (estimated) network formation model. We study the finite sample properties of our SGMM estimator in the context of ARD using Monte Carlo simulations. We show that the estimator performs very well when the distribution of the true network is relatively informative about the realized network structure in the data. Second, we present a flexible Bayesian estimator allowing us to exploit the entire structure of the data-generating process. Although the computational cost is greater, we exploit recent computational advances in the literature, e.g. \cite{mele2017,hsieh2019structural}, and show that the estimator can be successfully implemented on common-sized data sets. In particular, we apply our estimator to study peer effects on academic achievement using the widely used Add Health database. We find that data errors have first-order downward bias on the estimated endogenous effect.

Our SGMM estimator is inspired by the literature on error-in-variable models with repeated observations.\footnote{See \cite{bound2001measurement} for a review and \cite{chen2011nonlinear} for a review focused on nonlinear models.} Using a network formation model, we obtain a consistent estimator of the distribution of the true network. We then use this estimated distribution to obtain different draws from the distribution of the network.
Our moment condition can be seen as a biased-corrected version of the instrumental strategy proposed by \cite{bramoulle2009identification}, in which we substitute the true network with the draws from the estimated distribution. We show that our moment conditions are asymptotically valid and that the estimator is consistent for a finite number of draws from the estimated distribution of the network. This property implies a significant reduction in the computational cost of the method relative to methods based on the integration of the moment conditions (e.g. \cite{chandrasekhar2011econometrics}).

Importantly, our SGMM strategy requires only the (partial) observation of a \emph{single} cross-section, as opposed to, for example, the approach of \cite{zhang2020spillovers}. The presence of this feature is because of two main properties of the model. First, we can consistently estimate the distribution of the mismeasured variable (i.e. the network) using a single (partial) observation of the variable. Second, in the absence of measurement error, valid instruments for the endogenous peer variable are available \citep{bramoulle2009identification}.

We explore the finite sample properties of our instrumental variable estimator using Monte Carlo simulations. We consider the case in which the researcher only has access to aggregated relational data (ARD). In particular, we show that our SGMM estimator can be successfully combined with the network formation estimators proposed by \cite{breza2017using} and \cite{alidaee2020recovering}. As long as ARD are sufficiently informative in regard to the linking probabilities, our SGMM estimator successfully recovers the model's parameters.

Our Bayesian estimator is based on likelihood and therefore uses more information about the structure of the model, leading to more precise estimates. In the context of this estimator, the estimated distribution for the network acts as a prior distribution, and the inferred network structure is updated through a Markov chain Monte Carlo (MCMC) algorithm. Our approach relies on data augmentation \citep{tanner1987calculation}, which treats the network as an additional set of parameters to be estimated. This approach saves us from integrating over the $2^{N(N-1)}$ potential networks compatible with the data, which would create a serious computational issue. In particular, our MCMC builds on recent developments from the empirical literature on network formation (e.g. \cite{mele2017,hsieh2019structural,hsieh2019specification}). We show that the computational cost of our estimator is reasonable and that it can easily be applied to standard data sets.

We study the impact of errors in adolescents' friendship network data for the estimation of peer effects in education \citep{calvo2009peer}. We show that the widely used Add Health database features many missing links---around 30\% of the within-school friendship nominations are coded with error---and that these data errors strongly bias the estimated peer effects. Specifically, we estimate a model of peer effects on students' academic achievement. Our Bayesian estimator probabilistically reconstructs the missing links, and we obtain a consistent estimator of peer effects. The bias due to data errors is qualitatively important. Our estimated endogenous peer effect coefficient is 1.5 times larger than that obtained by assuming the data contains no errors.

This paper contributes to the recent literature on the estimation of peer effects when the network is either not entirely observed or observed with noise. In particular, our framework is valid when network data are either sampled, censored, misclassified, or consist of aggregate relational data.\footnote{For related literature that studies the estimation of peer effects when researchers have no network data, see \cite{manresa2016estimating,de2018recovering,souza2014estimating,lewbel2019social}.} We unify these strands in the literature and provide a flexible and computationally tractable framework for estimating peer effects with incomplete or erroneous network data.

\emph{Sampled networks and censoring:} \cite{chandrasekhar2011econometrics} show that models estimated using sampled networks are generally biased. They propose an analytical correction as well as a two-step general method of moment (GMM) estimator. \cite{liu2013estimation} shows that when the interaction matrix is not row-normalized, instrumental variable estimators based on an out-degree distribution are valid, even with sampled networks. \cite{hsieh2018non} focus on a regression model that depends on global network statistics. They propose analytical corrections to account for nonrandom sampling of the network (see also \cite{chen2013impact}). \cite{thirkettleidentification} also focuses on global network statistics, assuming that the researcher only observes a random sample of links. Using a structural network formation model, he derives bounds on the identified set for both the network formation model and the network statistic of interest.  \cite{lewbel2021social} develop a two-stage least square estimator for the linear in means model when some links are potentially missing. They propose valid instruments under some restrictions on the observed and true interactions matrices, or when researchers observe at least two samples of the same true network. Finally, \cite{zhang2020spillovers} studies program evaluation in a context in which networks are sampled locally and affected by a single type measurement error (either false positives or false negatives, but not both). Assuming that the researcher has access to two measurements of the network for each sampled unit, she presents a nonparametric estimator of the treatment and spillover effects.

Relatedly, \cite{griffith2019namefriends} explores the impact of imposing an upper bound to the number of links when eliciting network data, e.g. ``Name your five best friends.'' He shows, analytically and through simulations, that these bounds may bias the estimates significantly. He presents a bias-correction method and explores the impact of censoring using two empirical applications. He finds that censoring underestimates peer effects.

We contribute to this literature by proposing two simple and flexible estimators for the estimation of peer effects based on a linear-in-means model (as opposed to network statistics as in \cite{hsieh2016social} and \cite{thirkettleidentification}). Our estimators do not require many observations of the sampled network (contrary to \cite{zhang2020spillovers} and \cite{lewbel2019social}). Similar to \cite{griffith2019namefriends}, we find---using the Add Health database---that sampling leads to an underestimation of peer effects, although we find that censoring has a negligible impact, in the context of peer effects, on academic achievement.

Our Bayesian estimator is similar in spirit to the two-stage GMM estimator proposed by \cite{chandrasekhar2011econometrics}, but it is computationally advantageous. Indeed, their GMM estimator is based on an unconditional moment condition, which requires integrating over the entire set of networks that are compatible in the data. In \cite{chandrasekhar2011econometrics}, there are $2^{N(N-1)-M}$ such networks, where $M$ is the number of sampled pairs of individuals. Even for small networks, the computational cost is substantial whenever sampling is nontrivial. Our SGMM estimator does not suffer from this computational cost and can produce precise estimates with as little as three network simulations. While our Bayesian estimator is more computationally demanding, we exploit recent developments from the empirical literature on network formation (e.g. \cite{mele2017,hsieh2019structural}) and show that it is computationally tractable, even when no link is sampled (e.g. with aggregated relational data (ARD)), which would otherwise require integrating over the $2^{N(N-1)}$ networks compatible with the data.

\emph{Misclassification:} \cite{hardy2019estimating} look at the estimation of (discrete) treatment effects when the network is observed noisily. Specifically, they assume that observed links are affected by iid errors and present an expectation maximization (EM) algorithm that allows for a consistent estimator of the treatment effect.

Our model allows for the misclassification of all links with positive probability. As in \cite{hardy2019estimating}, we use a network formation model to estimate the probability of false positives and false negatives. However, our two-stage strategy---estimating the network formation model and then the peer effect model---allows for greater flexibility. In particular, our network formation model is allowed to flexibly depend on covariates. This is empirically important, as networks typically feature homophily on observed characteristics (e.g. \cite{currarini2010identifying,bramoulle2012homophily}).

\emph{Aggregate relational data:} \cite{breza2017using} propose to estimate network effects using aggregate relation data (ARD). These are obtained from such survey questions as, ``How many of your friends have trait X?'' They present a network formation model that can be estimated using only ARD. They show the validity of their methodology using two empirical applications in which the outcome of interest depends on the summary statistics of the network. \cite{alidaee2020recovering} present an alternative estimator allowing to recover nonparametrically the linking probability through ARD. Using a low-rank assumption, they present a simple penalized regression.

We show that these recent methodologies can also be applied to the study of peer effects using a linear-in-means model, which significantly expands the scope of the potential applications of these approaches. In particular, we study the finite sample performance of our SGMM estimator using Monte Carlo simulations and show that we can successfully recover the simulated parameters when combined with the network formation estimators proposed by \cite{breza2017using} and  \cite{alidaee2020recovering}.

A main contribution of this paper is that our estimators can be applied to each of the previously mentioned data issues or to their combination. Our two-step approach---first estimating the network formation and then the peer effects---is flexible and computationally attractive. To reduce the implementation costs, we also present an easy-to-use R package---named \texttt{PartialNetwork}---for applying our estimators. The package allows replicating all simulations and empirical applications in the paper, including the estimator proposed by \cite{breza2017using}. The package is available online at: \url{https://github.com/ahoundetoungan/PartialNetwork}. Additional implementation examples are provided in the Vignette accompanying the package. For example, we show that the implementation of our Bayesian estimator, combined with the estimator for ARD proposed by \cite{breza2017using}, is straightforward and computationally tractable.

The remainder of the paper is organized as follows. In Section 2, we present the econometric model as well as the main assumptions. In Section 3, we present our SGMM estimator and study its performance when combined with the estimators for ARD proposed by \cite{breza2017using} and \cite{alidaee2020recovering}. In Section 4, we present our Bayesian estimation strategy. In Section 5, we present our application to peer effects on academic achievement. Section 6 concludes the paper.% with a discussion of the main results, limits, and challenges for future research.


==> archives/forQE/iv.tex <==
\section{Simulated Generalized Method of Moment Estimators}\label{sec:iv}

In this section, we present an estimator based on a Simulated Generalized Method of Moments (SGMM). The key observation underlying our approach is that it is not necessary to observe the complete network structure to observe $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$. For example, one could simply obtain ${\mathbf{Gy}}$ from survey data, ``What is the average value of your friends' $y$?''

However, even observing $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$, the model (\ref{eq:linearinmean}) cannot be simply estimated using simple linear regression. The reason is that ${\mathbf{Gy}}$ is endogenous; thus, a linear regression would produce biased estimates (e.g. \cite{manski1993identification}, \cite{bramoulle2009identification}).

The typical instrumental approach to deal with this endogeneity is to use instruments based on the structural model, i.e. instruments constructed using second-degree peers (e.g. $\mathbf{G}^2\mathbf{X}$, see \cite{bramoulle2009identification}). These are less likely to be found in survey data. Indeed, we could doubt the informativeness of questions such as, ``What is the average value of your friends' average value of their friends' $x$?''

However, the above discussion is encouraging. When researchers observe $[\mathbf{y}, \mathbf{X}]$ and $[{\mathbf{GX}},{\mathbf{Gy}}]$, information about the network is only used as a means to construct a valid instrument, e.g. following \citet{bramoulle2009identification}. Then, if $\mathbf{GX}$ and $\mathbf{Gy}$ are observed, the estimation of peer effects is possible using any exogeneous (strong) predictor of the true network structure, as in \cite{kelejian2014estimation}, \cite{konig2019r}, and \cite{lee2020key}.\footnote{See Proposition \ref{prop:all_observed} of the Online Appendix \ref{sec:appendix_otherresults} for a formal statement. In particular, one needs a predictor of the network such that the resulting instrument is not correlated with $\boldsymbol{\varepsilon}$ and is strongly correlated with $\mathbf{Gy}$.}

The problem is more challenging when $\mathbf{Gy}$ and $\mathbf{GX}$ are not observed. To simplify the notation, for the remainder of this section we define $\lbrace \dot{\mathbf{G}}^{(r)}\rbrace_{r=1}^R$, $\lbrace \ddot{\mathbf{G}}^{(s)}\rbrace_{s=1}^S$, and $\lbrace \dddot{\mathbf{G}}^{(t)}\rbrace_{t=1}^T$ as sequences of independent draws from $\hat{P}(\mathbf{G})$. We will also let $\dot{\mathbf{G}}$, $\ddot{\mathbf{G}}$, and $\dddot{\mathbf{G}}$ be single independent draws from $\hat{P}(\mathbf{G})$. Finally, for any matrix $\mathbf{B}$, we will use $\mathbf{B}_i$ to denote the $i$th row of $\mathbf{B}$.

Before presenting our estimation strategy, we want to emphasize that we cannot simply proxy $\mathbf{Gy}$ and $\mathbf{GX}$ using draws from $\hat{P}(\mathbf{G})$. To see why, consider the simple case for which $\boldsymbol{\gamma}=\mathbf{0}$, so that the observation of $\mathbf{GX}$ is inconsequential. We have, substituting $\mathbf{Gy}$ with $\ddot{\mathbf{G}}\mathbf{y}$,
$$
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\ddot{\mathbf{G}}\mathbf{y}+[\boldsymbol{\eta}+\boldsymbol{\varepsilon}],
$$
where $\boldsymbol{\eta}=\alpha[\mathbf{G}-\ddot{\mathbf{G}}]\mathbf{y}$ is the error due to the approximation of $\mathbf{Gy}$ by $\ddot{\mathbf{G}}\mathbf{y}$. Importantly, the approximation error does \emph{not} vanish as $N$ grows because individuals belong to bounded groups (see Assumption \ref{as:manymarkets}).\footnote{As opposed to, for example, the context studied by \cite{auerbach2019measuring}.} Moreover, because $\mathbf{y}$ is a function of $\mathbf{G}$ (but not of $\ddot{\mathbf{G}}$), we typically have $\mathbb{E}(\mathbf{Gy})_i|\mathbf{Z}_i\neq\mathbb{E}(\ddot{\mathbf{G}}\mathbf{y})_i|\mathbf{Z}_i$ for some vector of instruments $\mathbf{z}_i$ and all $i$.


In Proposition \ref{prop:bias_nocontext} of the Online Appendix \ref{sec:appendix_otherresults}, we show, using an argument very similar to that of \cite{andrews2017measuring}, that the asymptotic bias induced by $\mathbb{E}\eta_i|\mathbf{z}_i\neq 0$ can be bounded, and simulations show that it can be very small for carefully constructed vectors of instruments, which can be useful in practice.

In any case, in our main result below, we show that we can include the bias directly in the moment function; this provides a consistent estimator of $\boldsymbol{\theta}$.

\subsection{Main Result}
Let $\tilde{\boldsymbol{\theta}}=[c,\boldsymbol{\beta}',\boldsymbol{\gamma}']'$. We maintain Assumptions \ref{as:alpha}--\ref{as:partial} and impose the regularity Assumptions \ref{as:regularity}--\ref{as:weigth} and the identification Assumptions \ref{as:convex} and \ref{as:globalmin} presented in Appendix \ref{sec:appendix_proofs}. 

\begin{theorem}[SGMM]\label{prop:non_observed} $ $

[Conditions] Let $\dot{\mathbf{Z}}^{(r)}=[\mathbf{1},\mathbf{X},\dot{\mathbf{G}}^{(r)}\mathbf{X},(\dot{\mathbf{G}}^{(r)})^2\mathbf{X},(\dot{\mathbf{G}}^{(r)})^3\mathbf{X},...]$ and $\ddot{\mathbf{V}}^{(s)}=[\mathbf{1},\mathbf{X},\ddot{\mathbf{G}}^{(s)}\mathbf{X}]$. Consider also the following (simulated) moment function:
\begin{equation}\label{eq:moment}
\mathbf{m}_{R,S,T}(\boldsymbol{\theta})=\frac{1}{RST}\sum_{r=1}^R\sum_{s=1}^S\sum_{t=1}^T\dot{\mathbf{Z}}^{(r)\prime}_i\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})_i\left(\mathbf{y}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}\ddot{\mathbf{V}}^{(s)}\tilde{\boldsymbol{\theta}}\right)\right]
\end{equation}

[Result] For any positive integers $R$, $S$, and $T$, the (simulated) GMM estimator based on (\ref{eq:moment}) is consistent.
\end{theorem}

Theorem \ref{prop:non_observed} presents conditions for the consistency of our two-step estimator. In particular, similar to a standard simulated GMM \citep{gourieroux1996simulation}, consistency holds for a finite number of simulations. Our estimator therefore does not suffer from the curse of dimensionality faced by \cite{chandrasekhar2011econometrics}.\footnote{The unconditional moment condition in \cite{chandrasekhar2011econometrics} is based on the (Monte Carlo) integration of the moment condition $\mathbb{E}(\mathbf{Z}^{(s)\prime}\boldsymbol{\varepsilon}|\mathbf{G})$ over $\mathbf{G}$.}

To understand the intuition behind the use of the moment function (\ref{eq:moment}), let us replace $\mathbf{y}=(\mathbf{I}-\alpha\mathbf{G})^{-1}(\mathbf{V}\tilde{\boldsymbol{\theta}}+\boldsymbol{\varepsilon})$ in Equation (\ref{eq:moment}). In doing so, we can rewrite the term inside the triple summation in (\ref{eq:moment}) as a sum of two terms. First, $\dot{\mathbf{Z}}^{(r)\prime}_i\boldsymbol{\varepsilon}_i$, which would be the standard moment function if $\mathbf{G}$ was observed (e.g. \cite{bramoulle2009identification}), and second:
\begin{equation}\label{eq:bias_corr}
\dot{\mathbf{Z}}^{(r)\prime}_i\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})_i\left((\mathbf{I}-\alpha{\mathbf{G}})^{-1}{\mathbf{V}}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}\ddot{\mathbf{V}}^{(s)}\right)\tilde{\boldsymbol{\theta}}\right].
\end{equation}
That second term can be viewed as the bias-correction term of the moment function.

We show that the expectations of both terms are equal to $0$ as $N$ grows to $\infty$. For the first term, this is true because the simulated network is exogenous. For the second term, this is true because $\mathbf{G}$, $\dot{\mathbf{G}}$, $\ddot{\mathbf{G}}$, and $\dddot{\mathbf{G}}$ are asymptotically drawn from the same distribution.

For the special case in which $\mathbf{G}$ is observed, one could substitute $\dot{\mathbf{G}}^{(r)}=\ddot{\mathbf{G}}^{(s)}=\dddot{\mathbf{G}}^{(t)}=\mathbf{G}$ for all $r,s,t$, and the first term would simply be $\mathbf{Z}'_i\boldsymbol{\varepsilon}_i$, whereas the second term would be exactly equal to $\mathbf{0}$.

Note that Theorem \ref{prop:non_observed} is valid whether or not $\mathbf{Gy}$ and $\mathbf{GX}$ are observed because the moment function (\ref{eq:moment}) does not use information on $\mathbf{Gy}$ or $\mathbf{GX}$. It is of course possible to include this additional information if either one is observed.

For example, assume that $\mathbf{GX}$ is observed and replace $\ddot{\mathbf{V}}$ with $\mathbf{V}$ in (\ref{eq:bias_corr}). After some algebra, we obtain: \begin{equation}\label{eq:gxobswrong}
    \dot{\mathbf{Z}}^{(r)\prime}_i\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})_i(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}[\alpha(\mathbf{G}-\ddot{\mathbf{G}})\mathbf{y}]\right]
\end{equation}
and a term that is equal to zero in expectation.

We can show that the last term in brackets corresponds to the source of the asymptotic bias because of the approximation error of $\mathbf{Gy}$ by $\ddot{\mathbf{G}}\mathbf{y}$ (see Proposition \ref{prop:bias_nocontext} of the Online Appendix). Whereas Equation (\ref{eq:gxobswrong}) cannot directly be substituted for (\ref{eq:moment}) in Theorem \ref{prop:non_observed}, it is possible to construct moment functions for the particular cases for which $\mathbf{GX}$ or $\mathbf{Gy}$ is observed. These cases can be found in Corollary \ref{prop:GXobs} and \ref{prop:Gyobs} of the Online Appendix.

\subsubsection{Asymptotic Normality}
Although Theorem \ref{prop:non_observed} shows the consistency of the estimator, it remains silent about its asymptotic distribution. In Appendix \ref{sec:varestim}, we present how to estimate the asymptotic variance of the estimator, irrespective of the asymptotic distribution. The estimation includes the sampling uncertainty, the estimating uncertainty of $\hat{\boldsymbol{\rho}}$, and the simulating uncertainty (which decreases as $R$, $S$, and $T$ grow). Note, however, that asymptotic normality cannot always be guaranteed because of the dependence of the estimator on $\hat{\boldsymbol{\rho}}$, estimated in the first stage (see Assumption \ref{as:partial}).

An important special case for which asymptotic normality is achieved is when the estimator of the network formation process can be written as an m-estimator; thus, the estimator in Theorem \ref{prop:non_observed} can be written as the second stage of a two-stage m-estimator.\footnote{See Appendix \ref{sec:asymptnorm} for a more detailed discussion.} This is the case for network formation models in Examples \ref{ex:sampled}, \ref{ex:censored}, and \ref{ex:misclass}.

Note that a minor technical concern comes from the discontinuity of the moment function in $\boldsymbol{\rho}$ for a finite number of simulations. To see why, let us rewrite $\dot{\mathbf{G}}=f(\{\dot{a}_{ij}\}_{ij})=f(\{\mathbbm{1}[P_{ij}(1|\hat{\boldsymbol{\rho}})\geq \dot{u}_{ij}]\}_{ij})$, where $\dot{u}_{ij}\sim_{iid}U[0,1]$, and similarly for $\ddot{\mathbf{G}}$ and $\dddot{\mathbf{G}}$. This is only a variable change and does not introduce any additional assumptions; however, it shows that using a finite number of network draws, the moment function is not everywhere continuous in $\boldsymbol{\rho}$ because of the indicator function. This is similar to the estimator in \cite{mcfadden1989method}, and asymptotic normality results (for m-estimators) can be found in \cite{newey1994large} and \cite{andrews1994empirical}.\footnote{An alternative is to smooth the moment function (i.e. $\mathbbm{1}[x\geq 0]\approx I(x/h_N)$, see e.g. \cite{horowitz1998bootstrap}) where $h_N\rightarrow 0$ fast enough so that the approximation becomes asymptotically negligible. The selection of the bandwidth in practice is challenging. Here, we suggest applying the same function used in particular by \cite{horowitz1998bootstrap}, which is conveniently available in our R package. Specifically: $I(x)=\mathbbm{1}\{-1\leq x\leq 1\}[0.5+\frac{105}{64}(x-\frac{5}{3}x^3 +\frac{7}{5}x^5-\frac{3}{7}x^7)]+\mathbbm{1}\{x>1\}$, which was also used in particular by \cite{kaplan2017smoothed} and \cite{de2019smoothed}.}

While asymptotic normality holds for m-estimators, it cannot always be guaranteed. In general, researchers may not always understand perfectly the asymptotic properties of the used network formation estimator. Indeed, recall that Assumption \ref{as:partial} only imposes the consistency of $\hat{\boldsymbol{\rho}}$ and does not discuss the convergence rate or asymptotic framework in detail. For some network formation models, these may be difficult to formalize.

An example is latent space models based on ARD (see Example \ref{ex:ard}). As discussed in Section \ref{sec:ard}, \cite{alidaee2020recovering} propose a penalized regression, whereas \cite{breza2017using} propose a Bayesian estimator. Neither estimator can be written directly as an m-estimator, and the convergence rates in a many-networks asymptotic framework (see our Assumption \ref{as:manymarkets}) remain poorly understood.

That said, one can always use a bootstrap procedure to characterize sampling uncertainty, which in the case of ARD is computationally feasible because of the estimator proposed by \cite{alidaee2020recovering}.\footnote{See Appendix \ref{sec:varestim} for details.} Alternatively, the Bayesian estimator proposed by \cite{breza2017using} produces draws from the posterior distribution of $\boldsymbol{\rho}$, which can be used to characterize the sampling uncertainty of the first stage. In Section \ref{sec:ard}, we study the finite sample properties of our approach using network formation models estimated on aggregated relational data.

%The sufficient rate so that the approximation does not impact the asymptotic variance depends on $I(\cdot)$ chosen as well as on the function $f$ linking the interaction matrix $\mathbf{G}$ to the adjacency matrix $\mathbf{A}$. In particular, the rate at which $h_N\rightarrow 0$ must be fast enough so that $\sqrt{N}\mathbb{E}\mathbf{m}_{R,S,T}(\boldsymbol{\theta}_0,\boldsymbol{\rho}_0)=o(1)$, but not too fast as to prevent the consistent estimation of the asymptotic variance-covariance matrix.\footnote{See in particular Lemma 4 and Assumption 11 (and associated discussion in Appendix B.3) in \cite{de2019smoothed}.} The determination of the convergence rate in our context is not trivial as our moment function is more complex than the one, and is left for future research.\footnote{Note that even with the knowledge of the appropriate convergence rate, 

%Note that smoothing is only necessary for a finite number of simulations since,
%$$
%\mathbf{m}_{R,S,T}(\boldsymbol{\theta})\rightarrow \sum_{\dot{\mathbf{G}}}\sum_{\ddot{\mathbf{G}}}\sum_{\dddot{\mathbf{G}}}\dot{\mathbf{Z}}^{\prime}_i\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}})_i\left(\mathbf{y}-(\mathbf{I}-\alpha\ddot{\mathbf{G}})^{-1}\ddot{\mathbf{V}}\tilde{\boldsymbol{\theta}}\right)\right]P(\dot{\mathbf{G}}|\hat{\boldsymbol{\rho}})P(\ddot{\mathbf{G}}|\hat{\boldsymbol{\rho}})P(\dddot{\mathbf{G}}|\hat{\boldsymbol{\rho}}),
%$$
%as $R$, $S$, and $T$ grow to infinity by a LLN. The moment function is in that case continuous in $\hat{\boldsymbol{\rho}}$.



\subsection{Finite Sample Performance Using ARD}\label{sec:ard}
In this section, we study the small sample performance of the estimator presented in Section \ref{sec:iv} when the researcher only has access to ARD (as in Example \ref{ex:ard}). First, we simulate network data using the model proposed by \cite{breza2017using} and simulate outcomes using the linear-in-means model (\ref{eq:linearinmean}) conditional on the simulated networks. Second, we estimate the network formation model using the Bayesian estimator proposed by \cite{breza2017using} (yielding $\hat{\boldsymbol{\rho}}_B$) and using the classical estimator proposed by \cite{alidaee2020recovering} (yielding $\hat{\boldsymbol{\rho}}_A$). Third, we estimate the linear-in-means model using the estimators presented in Proposition \ref{prop:bias_nocontext} and Theorem \ref{prop:non_observed} based on $\hat{\boldsymbol{\rho}}_A$ and $\hat{\boldsymbol{\rho}}_B$.

Recall that
\begin{equation}\label{eq:ard}
P(a_{ij}=1)\propto\exp\{\nu_i+\nu_j+\zeta \mathbf{z}_i'\mathbf{z}_j\},    
\end{equation}
where $\nu_i$, $\nu_j$, $\zeta$, $\mathbf{z}_i$, and $\mathbf{z}_j$ are not observed by the econometrician but follow parametric distributions. We refer the interested reader to \cite{mccormick2015latent}, \cite{breza2017using}, and \cite{breza2019consistently} for a formal discussion of the model, including its identification and consistent estimation. %Here, we discuss the intuition using a simple analogy.

%Suppose that individuals are located according to their geographical position on Earth. Suppose also that there are a fixed number of cities on Earth in which individuals can live. The econometrician does not know the individuals' locations on Earth nor do they know the location of the cities. In model (\ref{eq:ard}), $\mathbf{z}_i$ represent $i$'s position on Earth. However, the econometrician has access to ARD for a subset of the population, i.e. answers to questions such as, ``How many of your friends live in city $A$?''

%To understand the intuition behind the identification of the model, consider the following example: suppose that individual $i$ has many friends living in city $A$. Then, city $A$ is likely located close to $i$'s location. Similarly, if many individuals have many friends living in city $A$, then city $A$ is likely a large city. Finally, if $i$ has many friends from many cities, $i$ likely has a large $\nu_i$.

To study the finite sample performance of our instrumental strategy in this context, we simulate 20 groups, each having 250 individuals. Within each subpopulation, we simulate the ARD responses and a series of observable characteristics. The details of the Monte Carlo simulations can be found in the Online Appendix.

Importantly, the model in (\ref{eq:ard}) is based on a single population framework. Thus, the network formation model must be estimated separately for each of the 20 groups. With only 250 individuals in each group, we therefore expect significant small-sample bias.

We contrast the estimator proposed by \cite{breza2017using} with that of \cite{alidaee2020recovering}. Whereas \cite{breza2017using} present a parametric Bayesian estimator, \cite{alidaee2020recovering} propose a (nonparametric) penalized regression based on a low-rank assumption. One main advantage of the estimator proposed in \cite{alidaee2020recovering} is that it allows for a wider class of model and ensures that the estimation is fast and easily implementable.\footnote{The authors developed user-friendly packages in R and Python. See \cite{alidaee2020recovering} for links and details.} Note, however, that their method only yields a consistent estimator of $\hat{P}(\mathbf{A})$ if the true network is effectively low rank.

Very intuitively, the low-rank assumption implies that linking probabilities were generated from a small number of parameters. %; for example, in the example above, knowing individuals' gregariousness parameters $\nu_i$ and city in which they live would allow a prediction of the linking probabilities.
Importantly, the model (\ref{eq:ard}) is not necessarily low rank; for example, if the individuals' latent positions (i.e. the $\mathbf{z}_i$'s) are uniformly distributed, then the model may not be low rank and the method proposed by \cite{alidaee2020recovering} would perform poorly. If, however, individuals' latent positions are located around a few focal points, then the model might be low-rank because knowledge of these focal points may have high predictive power.

We compare the performance of both estimators as we vary the concentration parameter (that is, $\kappa$; see the Online Appendix for details). This has the effect of changing the \emph{effective rank} of the linking probabilities: increasing $\kappa$ decreases the effective rank.\footnote{We refer the interested reader to \cite{alidaee2020recovering} for a formal discussion of the effective rank and its importance for their estimator.} We therefore expect the estimator proposed by \cite{alidaee2020recovering} to perform better for larger values of $\kappa$.

A summary of the results is presented in Tables \ref{tab:gx:obs:short} and \ref{tab:gx:unobs:short}. The complete results can be found in Tables \ref{tab:gx:obs:full} and \ref{tab:gx:unobs:full} of the Online Appendix. Table \ref{tab:gx:obs:short} presents the results for the special case where $\mathbf{GX}$ are observed in the data. The table displays the performance of our simulated GMM (see Corollary \ref{prop:GXobs}) when the network formation model is estimated by \cite{breza2017using} and \cite{alidaee2020recovering}. 

When $\kappa=0$, the network formation is not low rank. This disproportionately affects the estimator of \cite{alidaee2020recovering}. When $\kappa=15$, the estimators proposed by \cite{breza2017using} and \cite{alidaee2020recovering} perform similarly.

We now turn to the more general case where $\mathbf{GX}$ are not observed. Table \ref{tab:gx:unobs:short} presents the performance of our SGMM estimator (Theorem \ref{prop:non_observed}) when the network formation process is estimated using the estimators proposed by \cite{breza2017using} and \cite{alidaee2020recovering} and when we assume that the researcher knows the true distribution of the network.

We see that the performance of our estimator is strongly affected by the quality of the first-stage network formation estimator. When based on either the estimator proposed by \cite{breza2017using} or \cite{alidaee2020recovering}, for $\kappa=0$ or $\kappa=15$, our SGMM estimator performs poorly.

The poor performance of our SGMM estimator in a context where both $\mathbf{Gy}$ and $\mathbf{GX}$ are unobserved was anticipated. This occurs for two main reasons. \emph{First}, the consistency of the network formation estimator in \cite{breza2019consistently} holds as the size of each subpopulation goes to infinity, whereas the consistency of our estimator holds as the number of (bounded) subpopulations goes to infinity. This should affect the performance of our estimator, when based on \emph{estimated} network formation models but not when based on the true distribution of the network.

\emph{Second}, as discussed in Example \ref{ex:ard}, ARD provides very little information about the realized network structure in the data (as opposed to censoring issues, for example; see Example \ref{ex:censored}). Then, if the true distribution is vague in the sense that most predicted probabilities are away from $0$ or $1$, we expect the estimation to be imprecise. This is what happens when $\kappa=15$, where our estimation based on the true distribution of the network is very imprecise in a context where the network affects the outcome through both $\mathbf{Gy}$ and $\mathbf{GX}$.

In the next section, we present a likelihood-based estimator, which uses more information on the data-generating process of the outcome to improve the precision of the estimation.


\renewcommand{\arraystretch}{.95}
\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD and observed $\bG\bX$} 
\label{tab:gx:obs:short}
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}ld{4}c}
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Parameter              & \multicolumn{2}{c}{Breza et al.} & \multicolumn{2}{c}{Alidaee et al.} \\
                       & \multicolumn{1}{c}{Mean}           & \multicolumn{1}{c}{Std. Dev}        & \multicolumn{1}{c}{Mean}            & \multicolumn{1}{c}{Std. Dev}         \\
 
\hline\\[-1.8ex] 
                      \multicolumn{5}{c}{$\kappa=0$}       \\\hline 
                       \hline\\[-1.8ex] 
                       
 %                       \multicolumn{5}{c}{IV (Proposition \ref{prop:bias_nocontext})}    \\
%                       \\[-1.8ex] 
%$\alpha = 0.4$         & 0.392              & (0.009)              & 0.372               & (0.027)               \\
%\\[-1.8ex]
%Sargan test            & 1.217              & (1.761)              & 7.779               & (10.386)              \\
%F-test (Weak inst.)    & 4259.622           & (1140.825)           & 597.055             & (251.886)             \\\hline\\[-1.8ex] 

                       \multicolumn{5}{c}{SGMM (Corollary \ref{prop:GXobs})}                      \\
                       \\[-1.8ex]
                       
   $\alpha = 0.4$         & 0.392              & (0.010)               & 0.492               & (0.057)               \\                    
                       
                       
                       \hline\\
                                        \multicolumn{5}{c}{$\kappa=15$}      \\\hline 
                       \hline\\[-1.8ex] 
                       
 %                       \multicolumn{5}{c}{IV (Proposition \ref{prop:bias_nocontext})}    \\
 %                      \\[-1.8ex] 
%$\alpha = 0.4$         & 0.400              & (0.007)              & 0.399               & (0.007)               \\
%\\[-1.8ex]
%Sargan test            & 1.063              & (1.496)              & 2.608               & (1.496)               \\
%F-test (Weak inst.)    & 5306.551           & (1519.394)           & 1767.274            & (1519.394)            \\\hline\\[-1.8ex] 
                                        \multicolumn{5}{c}{SGMM (Corollary \ref{prop:GXobs})}                   \\                  \\[-1.8ex]                              $\alpha = 0.4$         & 0.400              & (0.009)              & 0.428               & (0.009)               \\
 
\bottomrule     
\end{tabular}
\begin{tablenotes}[para,flushleft]
\footnotesize Note: For each case, we generated 20 independent subnetworks of 250 individuals each. In each subnetwork, the spherical coordinates of individuals were generated from a von Mises--Fisher distribution with a location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in the Online Appendix \ref{sec:ardsetting}. Predicted probabilities were computed using the mean of the posterior distribution. We chose the weight associated with the nuclear norm penalty to minimize the RMSE through cross-validation. This value of $\lambda=600$ is smaller than the recommended value in \cite{alidaee2020recovering}. See Table \ref{tab:gx:obs:full} in the Online Appendix for the estimated values of the other parameters.
\end{tablenotes}
\end{threeparttable}
\end{table}




\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD and unobserved $\bG\bX$ (SGMM, Theorem \ref{prop:non_observed}) }
\label{tab:gx:unobs:short}
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}ld{4}cd{4}c}
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Parameter       & \multicolumn{2}{l}{Breza et al.} & \multicolumn{2}{l}{Alidaee et al.} & \multicolumn{2}{l}{True distribution} \\
                       & \multicolumn{1}{c}{Mean}           & \multicolumn{1}{c}{Std. Dev}        & \multicolumn{1}{c}{Mean}            & \multicolumn{1}{c}{Std. Dev}        & \multicolumn{1}{c}{Mean}            & \multicolumn{1}{c}{Std. Dev}       \\\hline\\[-1.8ex] 
                \multicolumn{7}{c}{$\kappa = 0$}                                                    \\
                \\[-1.8ex]
$\alpha = 0.4$  & 0.717          & (0.463)         & 0.700           & (0.268)          & 0.400            & (0.056)            
\\\hline\\
                 \multicolumn{7}{c}{$\kappa = 15$}                                                   \\
                 \\[-1.8ex]
$\alpha = 0.4$  & 0.603          & (0.069)         & 0.870           & (0.202)          & 0.434            & (0.394)            \\

\bottomrule     
\end{tabular}
\begin{tablenotes}[para,flushleft]
\footnotesize Note: For each case, we generated 20 independent subnetworks of 250 individuals each. In each subnetwork, the spherical coordinates of individuals were generated from a von Mises--Fisher distribution with a location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in the Online Appendix. Predicted probabilities were computed using the mean of the posterior distribution. See Table \ref{tab:gx:unobs:full} in the Online Appendix for the estimated values of the other parameters. Instruments were built using only second-degree peers, i.e. $\mathbf{G^2X}$.
\end{tablenotes}
\end{threeparttable}
\end{table}
\renewcommand{\arraystretch}{1}


==> archives/forQE/model.tex <==
\section{The Model}\label{sec:linearinmean}
We now formally present our model. We first describe the \emph{linear-in-means} model \citep{manski1993identification,bramoulle2009identification}, arguably the most widely used model for studying peer effects in networks (see \cite{bramoulle2019peer} for a recent review). We then introduce our main assumption, characterizing what is known about the structure of the network.

\subsection{The Linear-in-Means Model}

Let $\mathbf{A}$ represent the $N\times N$ \emph{adjacency matrix} of the network. We assume a directed network: $a_{ij}\in \{0,1\}$, where $a_{ij}=1$ if $i$ is linked to $j$. We normalize $a_{ii}=0$ for all $i$ and let $n_i=\sum_j a_{ij}$ denote the number of links of $i$.
Let $\mathbf{G}=f(\mathbf{A})$, the $N\times N$ \emph{interaction matrix} for some function $f$. Unless otherwise stated, we assume that $\mathbf{G}$ is a row-normalization of the adjacency matrix $\mathbf{A}$.\footnote{In such a case, $g_{ij}=a_{ij}/n_i$ whenever $n_i>0$, whereas $g_{ij}=0$ otherwise.} Most of our results hold for any function $f$, which preserves the independence among groups (see Assumption \ref{as:manymarkets} below).

We focus on the following model:
\begin{equation}\label{eq:linearinmean}
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\mathbf{Gy}+{\mathbf{GX}}\boldsymbol{\gamma}+\boldsymbol{\varepsilon},
\end{equation}
where $\mathbf{y}$ is a vector of an outcome of interest (e.g. academic achievement), $c$ is a constant, $\mathbf{X}$ is a matrix of observable characteristics (e.g. age, gender...), and $\boldsymbol{\varepsilon}$ is a vector of errors.\footnote{Note that \cite{boucher2020binary} recently showed that (\ref{eq:linearinmean}) is valid (coherent, complete, and microfounded), even when $y_i$ is binary.} The parameter $\alpha$ therefore captures the impact of the average outcome of one's peers on their behavior (the endogenous peer effect). The parameter $\boldsymbol{\beta}$ captures the impact of one's characteristics on their behavior (the individual effects). The parameter $\boldsymbol{\gamma}$ captures the impact of the average characteristics of one's peers on their behavior (the contextual peer effects).

The following set of assumptions summarizes our setup.
\begin{assumption}\label{as:alpha} $|\alpha|<1/\Vert \mathbf{G}\Vert$ for some submultiplicative norm $\Vert \cdot\Vert$.
\end{assumption}
\begin{assumption}\label{as:manymarkets} The population is partitioned into $M>1$ groups, where the size $N_r$ of each group $r=1,...,M$ is bounded. The probability of a link between individuals of different groups is equal to $0$.
\end{assumption}
\begin{assumption}\label{as:nosampling} For each group, the outcome and individual characteristics are observed (i.e. $(\mathbf{y}_r,\mathbf{X}_r)$,  $r=1,...,M$, are observed).\footnote{For any vector/matrix, we use the subscript $r$ to denote the subvector/submatrix restricted to group $r$.}
\end{assumption}
\begin{assumption}\label{as:exonet} Exogeneity: $\mathbb{E}[\boldsymbol{\varepsilon}_r|\mathbf{X}_r]=\mathbf{0}$ for all $r=1,...,M$.
\end{assumption}

Assumption \ref{as:alpha} ensures that the model is coherent and that there exists a unique vector $\mathbf{y}$ compatible with (\ref{eq:linearinmean}). When $\mathbf{G}$ is row-normalized, $|\alpha|<1$ is sufficient. Assumption \ref{as:manymarkets} is introduced for exposition purposes; for example, the data could consist of a collection of small villages \citep{banerjee2013diffusion} or schools \citep{calvo2009peer}. Our methods extend to alternative assumptions such as those proposed by \cite{lee2004asymptotic} and \cite{lee2010specification}.\footnote{The authors assume that the adjacency matrix $\mathbf{A}$ is bounded in row- and column-sums.} In particular, Assumption \ref{as:manymarkets} implies a ``many markets'' asymptotic framework, meaning that the number of groups $M$ goes to infinity as the number of individuals $N$ goes to infinity.

Assumption \ref{as:nosampling} implies that the data is composed of a subset of fully sampled groups.\footnote{Contrary to \cite{liu2017peer} or \cite{wang2013estimation}, for example.} A similar assumption is made by \cite{breza2017using}. Note that Assumption \ref{as:exonet} does not impose restrictions on the dependence between the errors and the network structure. We detail the network formation process in the next section.

\subsection{Partial Network Information}

In this paper, we relax the costly assumption that the adjacency matrix $\mathbf{A}$ is observed. We assume instead that sufficient information about the network is observed so that a network formation model can be estimated.

More formally, we let $\mathcal{A}$ denote the observed information about the true network structure. That is, $\mathcal{A}$ is a function of the true network $\mathbf{A}$ and potentially of individuals' characteristics (see Example \ref{ex:ard}). We impose no particular structure on $\mathcal{A}$ but discuss important examples below (see Examples \ref{ex:sampled}--\ref{ex:ard}).

We assume that links are generated as follows:
\begin{equation}\label{eq:gennetfor}
P(a_{ij})\equiv P(a_{ij}|\boldsymbol{\rho}_0)\propto \exp\{a_{ij}Q(\boldsymbol{\rho}_0,\mathbf{w}_{ij})\}, 
\end{equation}
where $Q$ is some known, twice continuously differentiable function, $\mathbf{w}_{ij}=\mathbf{w}_{ij}(\mathbf{X})$ is a vector of observed characteristics for the pair $ij$, and $\boldsymbol{\rho}_0$ is the true value of $\boldsymbol{\rho}$, a vector of parameters to be estimated. Note that the assumption that the set of observed characteristics of the pairs $\mathbf{w}_{ij}$ are function of $\mathbf{X}$ implies that the network is \emph{exogenous}. We omit the dependence of $P(a_{ij})$ on $\mathbf{w}_{ij}$ to simplify the notation.


As will be made clear, our estimation strategy requires that the econometrician be able to draw samples from (a consistent estimator) $P(\mathbf{A})$. Thus, and for the sake of simplicity, we focus on distributions that are conditionally independent across links (i.e. $P(a_{ij}|\mathbf{A}_{-ij})=P(a_{ij})$), as in (\ref{eq:gennetfor}), although this is not formally required.\footnote{A prime example of a network distribution that is not conditionally independent is the distribution for an exponential random graph model (ERGM), e.g. \cite{mele2017}. Of course, in these cases, the specification of the marginal distribution (\ref{eq:gennetfor}) must be replaced by a specification of the joint distribution $P(\mathbf{A})$. Our ability to accommodate for such model depends on what is known about the true network, i.e. $\mathcal{A}$. In particular, we need that $P(\mathbf{A}|\boldsymbol{\rho},\mathcal{A})$ be computationally tractable and be such that Assumption \ref{as:partial} below holds for non-trivial $\mathcal{A}$. A specific case of ERGM that could be estimated with partial-network data is that in \cite{boucher2017my}, which requires asking sampled pairs of individuals about the number of links they have.}

We now present our main assumption.
\begin{assumption}[Partial Network Information]\label{as:partial} Given network information $\mathcal{A}$ and the parametric model (\ref{eq:gennetfor}), there exists an estimator $\hat{\boldsymbol{\rho}}_N$, such that $\hat{\boldsymbol{\rho}}_N\rightarrow_p \boldsymbol{\rho}_0$ as $N\rightarrow\infty$.
\end{assumption}

Assumption \ref{as:partial} implies that, using (\ref{eq:gennetfor}), the researcher has access to ``sufficient information'' about the network structure to obtain a consistent estimator of the distribution of the true network $P(\mathbf{A})$. We denote such a consistent estimator by $\hat{P}(\mathbf{A})\equiv P(\mathbf{A}|\hat{\boldsymbol{\rho}},\mathcal{A})$. We omit the dependence on $\mathcal{A}$ to simplify the notation when this does not create confusion. Note that we can use $\hat{P}(\mathbf{A})$ to obtain the consistent estimator $\hat{P}(\mathbf{G})$ because $\mathbf{G}=f(\mathbf{A})$ for some known function $f$.\footnote{Because $\mathbf{A}$ takes a finite number of values, so does $\mathbf{G}$, and $P(\mathbf{G})$ is a multinomial distribution. As such, it is a continuous function of the distribution $P(\mathbf{A})$, irrespective of the function $f$ linking $\mathbf{A}$ and $\mathbf{G}$.}

Importantly, it should be noted that even if the econometrician has access to a consistent estimator of the distribution of the true network, it \emph{does not} imply that they could simply proxy $\mathbf{G}$ in (\ref{eq:linearinmean}) using a draw $\tilde{\mathbf{G}}$ from the distribution $\hat{P}(\mathbf{G})$. The reason is that for any vector $\mathbf{z}$, $\tilde{\mathbf{G}}\mathbf{z}$ generally does not converge to ${\mathbf{G}}\mathbf{z}$ as the number of individuals $N$ goes to infinity. In other words, knowledge of $\hat{P}(\mathbf{G})$ and $\mathbf{z}$ is not sufficient to obtain a consistent estimator of $\mathbf{Gz}$. To see why, note that $(\mathbf{Gz})_i=\sum_{j=1}^Ng_{ij}z_j$. Under Assumption \ref{as:manymarkets}, the set of $j$, such that $g_{ij}\neq 0$, is bounded; thus, a consistent estimator of $P(\mathbf{G})$ is not sufficient to obtain a consistent estimator of $\mathbf{GX}$. This is also true under the alternative assumptions in \cite{lee2004asymptotic} and \cite{de2018identifying},\footnote{\cite{lee2004asymptotic}  requires that $\mathbf{G}$ be bounded in row- and column-sums (in absolute value), whereas \cite{de2018identifying} assume that $\mathbf{A}$ is bounded in row-sums.}, but it contrasts from models based on a large network asymptotic framework (e.g. \cite{auerbach2022identification}).

Assumption \ref{as:partial} covers a large range of cases in which networks are partially observed. We specifically discuss four leading examples in which Assumption \ref{as:partial} holds: \emph{sampled networks} (Example \ref{ex:sampled}), \emph{censored networks }(Example \ref{ex:censored}), \emph{misclassified network links} (Example \ref{ex:misclass}), and \emph{aggregated relational data} (Example \ref{ex:ard}).

\begin{example}[Sampled Networks]\label{ex:sampled}
Suppose that we observe the realizations of $a_{ij}$ for a random sample of $m$ pairs (e.g. \cite{chandrasekhar2011econometrics}). Here $\mathcal{A}$ can be represented by an $N\times N$ binary matrix $\mathbf{A}^{obs}$. \cite{conley2010learning} present such a sampling scheme and ask individuals about their relationship with a random sample of other individuals; for example, ``Do you know person X?''

Such a setup is sufficient to consistently estimate flexible network formation models, such as that in \cite{graham2017econometric}. A simpler example would be to assume that the network formation model (\ref{eq:gennetfor}) is equal to $P(a_{ij}=1)\propto\exp\{\mathbf{w}_{ij}\boldsymbol{\rho}\}$. In this case, a simple logistic regression provides a consistent estimator of $\boldsymbol{\rho}$.

Given this consistent estimator for $\boldsymbol{\rho}$ and the assumed parametric model, we can compute an estimator for the distribution of the true network $\hat{P}(\mathbf{A})=P(\mathbf{A}|\hat{\boldsymbol{\rho}},\mathcal{A})$. Here, $\hat{P}(a_{ij})=a_{ij}^{obs}$ for any sampled link $ij$, while $\hat{P}(a_{ij})\propto\exp\{a_{ij}\mathbf{w}_{ij}\hat{\boldsymbol{\rho}}\}$ for the remaining unsampled links.
\end{example}

\begin{example}[Censored Network Data]\label{ex:censored}
As discussed in \cite{griffith2019namefriends}, network data is often censored. This typically arises when surveyed individuals are asked to name only $T>1$ links (among the $N$ possible links they may have). Here, $\mathcal{A}$ can be represented by an $N\times N$ binary matrix $\mathbf{A}^{obs}$. We can use censored network data to estimate a network formation model, such as $P(a_{ij}=1)\propto\exp\{\mathbf{w}_{ij}\boldsymbol{\rho}\}$.

For simplicity, let us assume as in \cite{griffith2019namefriends} that each link has the same probability of being censored. Then, the parameters in $\boldsymbol{\rho}$ (other than the constant) are identified from the observed ratios $\sum_{ij}a_{ij}{w}^k_{ij}/\sum_{ij}{w}^k_{ij}$ (for observable characteristic $k$), as these sufficient statistics are not biased by censoring. To identify the constant, note that we can compute the likelihood of the censored degree distribution (i.e. $n_i=\sum_ja_{ij}$). Letting $\lbrace\mathbf{w}_{ij}\rbrace_j=[\mathbf{w}_{i1},...,\mathbf{w}_{iN}]$, we have $P(n_i=t|\lbrace\mathbf{w}_{ij}\rbrace_j;\boldsymbol{\rho})$ for observed $t<T$ and $P(n_i\geq T|\lbrace\mathbf{w}_{ij}\rbrace_j;\boldsymbol{\rho})$ for observed $t=T$, which allows identifying the constant.

Once such an estimator of $\boldsymbol{\rho}$ is obtained, we can compute an estimator for the distribution of the true network $\hat{P}(\mathbf{A})=P(\mathbf{A}|\hat{\boldsymbol{\rho}},\mathcal{A})$. In particular, ${P}(a_{ij}|\hat{\boldsymbol{\rho}},a_{ij}^{obs}=1)=1$ because observed links necessarily exist. Also note that for all individuals $i$, such that $n_i<T$, we have ${P}(a_{ij}|\hat{\boldsymbol{\rho}},a_{ij}^{obs})=a_{ij}^{obs}$ for all $j$, as their network data are not censored. Here, the structural model is only used to obtain the probability of links that are not observed for individuals whose links are potentially censored, i.e. ${P}(a_{ij}|\hat{\boldsymbol{\rho}},a_{ij}^{obs}=0)\propto \exp\{a_{ij}\mathbf{w}_{ij}\hat{\boldsymbol{\rho}}\}$ for all $ij$, such that $n_i\geq T$.

\end{example}

\begin{example}[Misclassification]\label{ex:misclass}
\cite{hardy2019estimating} study cases in which networks are observed but may include misclassified links (i.e. false positives and false negatives). Here, $\mathcal{A}$ can be represented by an $N\times N$ binary matrix $\mathbf{A}^{mis}$. The (consistent) estimation of (\ref{eq:gennetfor}) in such a context follows directly from the existing literature on misclassification in binary outcome models, e.g. \cite{hausman1998misclassification}.

Let $q_1$ be the probability of false positives and $q_0$ be the probability of false negatives (both being elements of $\boldsymbol{\rho}$). The estimator for the distribution of the true network is given by $P(a_{ij}=1|\hat{\boldsymbol{\rho}},a_{ij}^{mis})=a_{ij}^{mis}(1-\hat{q}_1) + (1-a_{ij}^{mis})\hat{q}_0$.
\end{example}

\begin{example}[Aggregated Relational Data]\label{ex:ard}
Aggregated relational data (ARD) are obtained from survey questions such as, ``How many friends with trait `X' do you have?'' Here, $\mathcal{A}$ can be represented by an $N\times K$ matrix of integer values, where $K$ is the number of traits that individuals were asked about.

Building on \cite{mccormick2015latent}, \cite{breza2017using} proposed a novel approach for the estimation of network formation models using only ARD. They assume:
\begin{equation}\label{eq:exard}
P(a_{ij}=1)\propto\exp\{\nu_i+\nu_j+\zeta \mathbf{z}_i'\mathbf{z}_j\},    
\end{equation}
where $\nu_i$, $\nu_j$, $\zeta$, $\mathbf{z}_i$, and $\mathbf{z}_j$ are not observed by the econometrician but follow parametric distributions. Here, parameters $\nu_i$ and $\nu_j$ can be interpreted as $i$ and $j$'s propensities to create links, irrespective of the identity of the other individual involved. The other component, $\zeta \mathbf{z}_i'\mathbf{z}_j$, is meant to capture homophily (like attracts like) on an abstract latent space (e.g. \cite{hoff2002latent}).

\cite{breza2017using} show that it is possible to use ARD to recover the values of the variables in (\ref{eq:exard}). In particular, letting $\boldsymbol{\rho}=[\{\nu_i\}_i,\{\mathbf{z}_i\}_i,\zeta]$, \cite{breza2019consistently} provide sufficient conditions for the consistent estimation of $\boldsymbol{\rho}$.

Contrary to Examples \ref{ex:sampled}--\ref{ex:misclass}, ARD does not provide information on any specific links; \footnote{That is, unless ARD includes the degree distribution with some individuals reporting having no links at all.} therefore, the predicted distribution of the true network is $P(a_{ij}|\hat{\boldsymbol{\rho}},\mathcal{A})=P(a_{ij}|\hat{\boldsymbol{\rho}})$, which is given by Equation (\ref{eq:exard}). Here, it is worth emphasizing that the observed network information (i.e. ARD) is not very informative about the particular network structure in the data. In this sense, it could be viewed as a worst-case scenario.
\end{example}

==> archives/forQE/summarychanges.tex <==
\noindent\textbf{Summary of the changes}

The main comments from the editor and referees were, to our understanding, that (1) the text was lacking focus with respect to (in particular) which estimator was to be used, and that (2) our proof of the main theorem had some gaps. We agree with both comments and have made the following main changes to the manuscript.

\begin{enumerate}
    \item Proposition 1 (when $\mathbf{Gy}$ and $\mathbf{GX}$ are observed) and Proposition 2 (biased GMM estimator) were judged of weaker interest by the referees. We agree. We moved these two propositions to the Online Appendix. This left us more space to discuss our main result and to focus the narrative of the paper around the key messages/results.
    \item The main comment regarding our Theorem 1 was our claim about asymptotic normality, which we based on the CLT by Withers (1980). We agree that we cannot guarantee asymptotic normality without imposing very high-level assumptions. We have removed this claim from Theorem 1 (which now only focuses on consistency) and now discuss sufficient conditions for asymptotic normality in the text (see Section 3.1.1). Since asymptotic normality (when it holds) follows from known results, we feel that this approach is more transparent with respect to our contribution and that it allows the reader to understand more clearly when asymptotic normality holds or not.
    
    The main threat to asymptotic normality comes from the properties of the first stage network formation estimator, which may not be an m-estimator. There are numerous interesting network formation models, and some have asymptotic properties that we have yet to fully understand (at least in our context, using a many-groups asymptotic framework). Such is the case for latent space models estimated using aggregated relational data (our Example 4).

    \item We now use our empirical application to further discuss the distinctions between our two main estimators (i.e. the SGMM and the Bayesian ones). We also add counterfactual simulations of the centrality vectors---typically used to target policies--- and discuss the policy implications in more detail.
    
    \item Finally, we moved the proof of Theorem 1 to the Appendix (away from the Online Appendix).
\end{enumerate}

==> archives/model_bkp.tex <==
\section{The Model}\label{sec:linearinmean}
We now formally present our model. We first describe the \emph{linear-in-means} model, \citep{manski1993identification,bramoulle2009identification} arguably the most widely used model for studying peer effects in networks (see \cite{bramoulle2019peer} for a recent review). We then introduce our main assumption, characterizing what is known about the structure of the network.

\subsection{The Linear-in-Means Model}

Let $\mathbf{A}$ represent the $N\times N$ \emph{adjacency matrix} of the network. We assume a directed network: $a_{ij}\in \{0,1\}$, where $a_{ij}=1$ if $i$ is linked to $j$. We normalize $a_{ii}=0$ for all $i$ and let $n_i=\sum_j a_{ij}$ denote the number of links of $i$.
Let $\mathbf{G}=f(\mathbf{A})$, the $N\times N$ \emph{interaction matrix} for some function $f$. Unless otherwise stated, we assume that $\mathbf{G}$ is a row-normalization of the adjacency matrix $\mathbf{A}$.\footnote{In such a case, $g_{ij}=a_{ij}/n_i$ whenever $n_i>0$, while $g_{ij}=0$ otherwise.} Our results extend to alternative specifications of $f$.

We focus on the following model:
\begin{equation}\label{eq:linearinmean}
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\mathbf{Gy}+{\mathbf{GX}}\boldsymbol{\gamma}+\boldsymbol{\varepsilon},
\end{equation}
where $\mathbf{y}$ is a vector of an outcome of interest (e.g. academic achievement), $c$ is a constant, $\mathbf{X}$ is a matrix of observable characteristics (e.g. age, gender...), and $\boldsymbol{\varepsilon}$ is a vector of errors. The parameter $\alpha$ therefore captures the impact of the average outcome of one's peers on their behaviour (the endogenous peer effect). The parameter $\boldsymbol{\beta}$ captures the impact of one's characteristics on their behaviour (the individual effects). The parameter $\boldsymbol{\gamma}$ captures the impact of the average characteristics of one's peers on their behaviour (the contextual peer effects).

 The next assumption summarizes our set-up.
\begin{assumption}\label{as:main}\begin{singlespace}
We maintain the following assumptions:\begin{enumerate}[label={(\theassumption.\arabic*)},ref={\theassumption.\arabic*}]
    \item \label{as:alpha} $|\alpha|<1/\Vert \mathbf{G}\Vert$ for some submultiplicative norm $\Vert \cdot\Vert$.
    \item \label{as:manymarkets} The population is partitioned in $M>1$ groups, where the size $N_r$ of each group $r=1,...,M$ is bounded. The probability of a link between individuals of different groups is equal to $0$.
    \item \label{as:nosampling} For each group, the outcome and individual characteristics are observed, i.e. $(\mathbf{y}_r,\mathbf{X}_r)$,  $r=1,...,M$, are observed.
    \item \label{as:exonet} The network is exogenous in the sense that $\mathbb{E}[\boldsymbol{\varepsilon}|\mathbf{X},\mathbf{G}]=\mathbf{0}$.
\end{enumerate}
\end{singlespace}
\end{assumption}
Assumption \ref{as:alpha} ensures that the model is coherent and that there exists a unique vector $\mathbf{y}$ compatible with (\ref{eq:linearinmean}). When $\mathbf{G}$ is row-normalized, $|\alpha|<1$ is sufficient. Assumption \ref{as:manymarkets} is introduced for exposition purposes. For example, the data could consist in a collection of small villages \citep{banerjee2013diffusion}, or schools \citep{calvo2009peer}. Our methods extend to alternative assumptions such as the ones proposed by \cite{lee2004asymptotic} and \cite{lee2010specification}.\footnote{The authors assume that the adjacency matrix $\mathbf{A}$ is bounded in row- and column-sums.}

Assumption \ref{as:nosampling} implies that the data is composed of a subset of fully sampled groups.\footnote{Contrary to \cite{liu2017peer} or \cite{wang2013estimation}, for example.} A similar assumption is made by \cite{breza2017using}. Note that we assume that the network is exogenous (Assumption \ref{as:exonet}) mostly to clarify the presentation of the estimators. In Section \ref{sec:endogenous}, we discuss how recent advances for the estimation of peer effects in endogenous networks can be adapted to our context.

\subsection{Partial Network Information}

In this paper, relax the costly assumption that the adjacency matrix $\mathbf{A}$ is observed. We assume instead that enough information about the network is observed so that a network formation model can be estimated.

More formally, we let $\mathcal{A}$ denote the observed information about the true network structure. That is, $\mathcal{A}$ is a function of the true network $\mathbf{A}$, and potentially of individuals' characteristics (see Example \ref{ex:ard}). We impose no particular structure on $\mathcal{A}$, but discuss important examples below (see Examples \ref{ex:sampled}--\ref{ex:ard}).

We assume that links are generated as follows:
\begin{equation}\label{eq:gennetfor}
P(a_{ij})\equiv P(a_{ij}|\boldsymbol{\rho}_0)\propto \exp\{a_{ij}Q(\boldsymbol{\rho}_0,\mathbf{w}_{ij})\}, 
\end{equation}
where $Q$ is some known continuous function, $\mathbf{w}_{ij}$ is a vector of observed characteristics for the pair $ij$, and $\boldsymbol{\rho}_0$ is the true value of $\boldsymbol{\rho}$, a vector of parameters to be estimated. Note that we omit the dependence of $P(a_{ij})$ on $\mathbf{w}_{ij}$ to simplify the notation.

As will be made clear, our estimation strategy requires that the econometrician be able to draw samples from (a consistent estimate) $P(\mathbf{A})$. As such, and for the sake of simplicity, we focus on distributions that are conditionally independent across links (i.e. $P(a_{ij}|\mathbf{A}_{-ij})=P(a_{ij})$), as in (\ref{eq:gennetfor}), although this is not formally required.\footnote{A prime example of a network distribution that is not conditionally independent is the distribution for an exponential random graph model (ERGM), e.g. \cite{Mele2017}.}

We now present our main assumption.
\begin{assumption}[Partial Network Information]\label{as:partial} Given network information $\mathcal{A}$ and the parametric model (\ref{eq:gennetfor}), there exists an estimator $\hat{\boldsymbol{\rho}}_N$, such that $\hat{\boldsymbol{\rho}}_N\rightarrow_p \boldsymbol{\rho}_0$ as $N\rightarrow\infty$.
\end{assumption}

Assumption \ref{as:partial} implies that, using (\ref{as:partial}), the researcher has access to ``enough information'' about the network structure to obtain a consistent estimator of the distribution of the true network $P(\mathbf{A})$. We denote such a consistent estimator by $\hat{P}(\mathbf{A})\equiv P(\mathbf{A}|\hat{\boldsymbol{\rho}},\mathcal{A})$. We omit the dependence on $\mathcal{A}$ to simplify the notation when this does not create confusion. Note that we can use $\hat{P}(\mathbf{A})$ to obtain the consistent estimate $\hat{P}(\mathbf{G})$, since $\mathbf{G}=f(\mathbf{A})$ for some known function $f$.\footnote{Since $\mathbf{A}$ takes a finite number of values, so does $\mathbf{G}$, and $P(\mathbf{G})$ has a multinomial distribution.}

Importantly, it should be noted that even if the econometrician has access to a consistent estimate of the distribution of the true network, it \emph{does not} imply that they could simply proxy $\mathbf{G}$ in (\ref{eq:linearinmean}) using a draw $\tilde{\mathbf{G}}$ from the distribution $\hat{P}(\mathbf{G})$. The reason is that for any vector $\mathbf{z}$, $\tilde{\mathbf{G}}\mathbf{z}$ generally does not converge to ${\mathbf{G}}\mathbf{z}$ as the number of individuals $N$ goes to infinity. In other words, knowledge of $\hat{P}(\mathbf{G})$ and $\mathbf{z}$ is not sufficient to obtain a consistent estimate of $\mathbf{Gz}$. To see why, note that $(\mathbf{Gz})_i=\sum_{j=1}^Ng_{ij}z_j$. Under Assumption \ref{as:manymarkets}, the set of $j$ such that $g_{ij}\neq 0$ is bounded, so a consistent estimate of $P(\mathbf{G})$ is not sufficient to obtain a consistent estimate of $\mathbf{GX}$. This is also true under the alternative assumptions in \cite{lee2004asymptotic} or \cite{de2018identifying}.\footnote{\cite{lee2004asymptotic}  requires that $\mathbf{G}$ be bounded in row- and column-sums (in absolute value), while \cite{de2018identifying} assume that $\mathbf{A}$ is bounded in row-sums. An exception is the graphon games approach proposed by \cite{parise2019graphon}, although their method has yet to be implemented to the estimation of network formation games.}

Assumption \ref{as:partial} covers a large range of cases in which networks are partially observed. We specifically discuss four leading examples in which Assumption \ref{as:partial} holds: \emph{sampled networks} (Example \ref{ex:sampled}), \emph{censored networks }(Example \ref{ex:censored}), \emph{misclassified network links} (Example \ref{ex:misclass}), and \emph{aggregated relational data} (Example \ref{ex:ard}).

\medskip
\begin{testexample}[Sampled Networks][label={ex:sampled}]
Suppose that we observe the realizations of $a_{ij}$ for a random sample of $m$ pairs (e.g. \cite{chandrasekhar2011econometrics}). Here $\mathcal{A}$ can be represented by a $N\times N$ binary matrix $\mathbf{A}^{obs}$. \cite{conley2010learning} present such a sampling scheme and ask individuals about their relation with a random sample of other individuals. For example: ``Do you know person X?''

Such a setup is sufficient to consistently estimate flexible network formation models such as the one in \cite{graham2017econometric}. A simpler example would be to assume that the network formation model (\ref{eq:gennetfor}) is equal to: $P(a_{ij}=1)\propto\exp\{\mathbf{w}_{ij}\boldsymbol{\rho}\}$. In this case, a simple logistic regression provides a consistent estimator of $\boldsymbol{\rho}$.

Given this consistent estimator for $\boldsymbol{\rho}$ and the assumed parametric model, we can compute an estimator for the distribution of the true network $\hat{P}(\mathbf{A})=P(\mathbf{A}|\hat{\boldsymbol{\rho}},\mathcal{A})$. Here, $\hat{P}(a_{ij})=a_{ij}^{obs}$ for any sampled link $ij$, while $\hat{P}(a_{ij})\propto\exp\{\mathbf{w}_{ij}\hat{\boldsymbol{\rho}}\}$ for the remaining un-sampled links.
\end{testexample}

\medskip
\begin{testexample}[Censored Network Data][label={ex:censored}]
As discussed in \cite{griffith2019namefriends}, network data is often censored. This typically arise when surveyed individuals are asked to name only $T>1$ links (among the $N$ possible links they may have). Here $\mathcal{A}$ can be represented by a $N\times N$ binary matrix $\mathbf{A}^{obs}$. \cite{griffith2019namefriends} shows that estimating peer effects using a censored network leads to biased estimates. Nonetheless, we can use censored network data to estimate a network formation models such as, for example: $P(a_{ij}=1)\propto\exp\{\mathbf{w}_{ij}\boldsymbol{\rho}\}$.

For simplicity, lets assume as in \cite{griffith2019namefriends} that each link has the same probability of being censored. Then, the parameters in $\boldsymbol{\rho}$ (other than the constant) are identified from the observed ratios $\sum_{ij}a_{ij}\mathbf{w}_{ij}/\sum_{ij}\mathbf{w}_{ij}$ since these sufficient statistics are not biased by censoring. In order to identify the constant, note that we can easily compute the likelihood of the censored degree distribution (i.e. $n_i=\sum_ja_{ij}$). That is: $P(n_i=t|\mathbf{W};\boldsymbol{\rho})$ for observed $t<T$ and $P(n_i\geq T|\mathbf{W};\boldsymbol{\rho})$ for observed $t=T$, which allow to identify the constant.\footnote{A simple alternative, when only few individuals' data is censored, is to estimate the model only on individuals for which $n_i<T$. We follow this stragety in Section \ref{sec:addhealth}.}

Once such estimator of $\boldsymbol{\rho}$ is obtained, we can compute an estimator for the distribution of the true network $\hat{P}(\mathbf{A})=P(\mathbf{A}|\hat{\boldsymbol{\rho}},\mathcal{A})$. In particular, ${P}(a_{ij}|\hat{\boldsymbol{\rho}},a_{ij}^{obs}=1)=1$ since observed links necessarily exist. Also note that for all individuals $i$ such that $n_i<T$, we have ${P}(a_{ij}|\hat{\boldsymbol{\rho}},a_{ij}^{obs})=a_{ij}^{obs}$ for all $j$ since their network data is not censored. Here, the structural model is only used in order to get the probability of links that are not observed, for individuals whose links are potentially censored, i.e. ${P}(a_{ij}|\hat{\boldsymbol{\rho}},a_{ij}^{obs}=0)\propto \exp\{\mathbf{w}_{ij}\hat{\boldsymbol{\rho}}\}$ for all $ij$ such that $n_i\geq T$.



\end{testexample}

\medskip
\begin{testexample}[Misclassification][label={ex:misclass}]
\cite{hardy2019estimating} study cases in which networks are observed, but may include misclassified links (i.e. false positives and false negatives). Here, $\mathcal{A}$ can be represented by a $N\times N$ binary matrix $\mathbf{A}^{mis}$. The (consistent) estimation of (\ref{eq:gennetfor}) in such context follows directly from the existing literature on misclassification in binary outcome models, e.g. \cite{hausman1998misclassification}.

Let $q_1$ be the probability of false positives and $q_0$ be the probability of false negatives (both being elements of $\boldsymbol{\rho}$). The estimator for the distribution of the true network is given by: $P(a_{ij}=1|\hat{\boldsymbol{\rho}},a_{ij}^{mis})=a_{ij}^{mis}(1-\hat{q}_1) + (1-a_{ij}^{mis})\hat{q}_0$.
\end{testexample}

\medskip
\begin{testexample}[Aggregated Relational Data][label={ex:ard}]
Aggregated relational data (ARD) are obtained from survey questions such as: ``How many friends with trait `X' do you have?'' Here, $\mathcal{A}$ can be represented by a $N\times K$ matrix of integer values, where $K$ is the number of traits individuals were asked about.

Building on \cite{mccormick2015latent}, \cite{breza2017using} proposed a novel approach for the estimation of network formation models using only ARD. They assume that:
\begin{equation}\label{eq:exard}
P(a_{ij}=1)\propto\exp\{\nu_i+\nu_j+\zeta \mathbf{z}_i'\mathbf{z}_j\},    
\end{equation}
where $\nu_i$, $\nu_j$, $\zeta$, $\mathbf{z}_i$, and $\mathbf{z}_j$ are not observed by the econometrician but follow parametric distributions. Here, parameters $\nu_i$ and $\nu_j$ can be interpreted as $i$ and $j$'s propensity to create links, irrespective of the identity of the other individual involved. The other component, $\zeta \mathbf{z}_i'\mathbf{z}_j$, is meant to capture homophily (like attracts like) on an abstract latent space (e.g. \cite{hoff2002latent}).

\cite{breza2017using} show that it is possible to use aggregate relational data (ARD) to recover the values of the variables in (\ref{eq:exard}). In particular, letting $\boldsymbol{\rho}=[\{\nu_i\}_i,\{\mathbf{z}_i\}_i,\zeta]$, \cite{breza2019consistently} provide sufficient conditions for the consistent estimation of $\boldsymbol{\rho}$.

Contrary to Examples \ref{ex:sampled}--\ref{ex:misclass}, ARD does not provide information on any specific links.\footnote{That is, unless ARD include the degree distribution with some individuals reporting having no links at all.} As such, the predicted distribution of the true network is $P(a_{ij}|\hat{\boldsymbol{\rho}},\mathcal{A})=P(a_{ij}|\hat{\boldsymbol{\rho}})$, which is given by Equation (\ref{eq:exard}).
\end{testexample}

In the next sections, we present two estimation strategies that are valid under Assumption \ref{as:partial}, and thus applying to Examples \ref{ex:sampled}--\ref{ex:ard}. 



==> archives/shortversion/addhealth.tex <==

\section{Imperfectly Measured Networks}\label{sec:addhealth}

In this section, we assume that the econometrician has access to network data but that the data may contain errors. To show how our method can be used to address these issues, we consider a simple example where we are interested in estimating peer effects on adolescents' academic achievements.

We use the widely used AddHealth database and show that network data errors have a first-order impact on the estimated peer effects. Specifically, we focus on a subset of schools from the ``In School'' sample that each have less than 200 students. Table \ref{tab:sumstats} displays the summary statistics.

\begin{table}[!htbp] 
   \centering 
  \caption{Summary statistics.} 
  \label{tab:sumstats} 
\begin{tabular}{@{\extracolsep{5pt}} lld{3}ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
\multicolumn{2}{l}{Statistic} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline \\[-1.8ex] 
\multicolumn{2}{l}{Female} & 0.540 & 0.498 & 0 & 1 \\ 
\multicolumn{2}{l}{Hispanic}  & 0.157 & 0.364 & 0 & 0 \\ 
\multicolumn{2}{l}{Race} &  &  &  &  \\ 
 & White & 0.612 & 0.487 & 0 & 1 \\ 
 & Black & 0.246 & 0.431 & 0 & 0 \\ 
 & Asian & 0.022 & 0.147 & 0 & 0 \\ 
 & Other & 0.088 & 0.283 & 0 & 0 \\ 
\multicolumn{2}{l}{Mother's education}  &  &  &  &  \\ 
 & High & 0.310 & 0.462 & 0 & 1 \\ 
 & <High & 0.193 & 0.395 & 0 & 0 \\ 
 & >High & 0.358 & 0.480 & 0 & 1 \\ 
 & Missing & 0.139 & 0.346 & 0 & 0 \\ 
\multicolumn{2}{l}{Mother's job}  &  &  &  &  \\ 
 & Stay-at-home & 0.225 & 0.417 & 0 & 0 \\ 
 & Professional & 0.175 & 0.380 & 0 & 0 \\ 
 & Other & 0.401 & 0.490 & 0 & 1 \\ 
 & Missing & 0.199 & 0.399 & 0 & 0 \\ 
\multicolumn{2}{l}{Age}  & 13.620 & 1.526 & 13 & 14 \\ 
\multicolumn{2}{l}{GPA}  & 2.912    &0.794    &2.333      &3.5\\ 
\hline \\[-1.8ex] 
\multicolumn{6}{l}{%
  \begin{minipage}{11.6cm}%
    \footnotesize{Note: We only keep the 33 schools having less than 200 students from the In-School sample. The variable GPA is computed by taking the average grade for English, Mathematics, History, and Science, letting $A=4$, $B=3$, $C=2$, and $D=1$. Thus, higher scores indicate better academic achievement.}
  \end{minipage}%
  }
\end{tabular} 

\end{table} 

Most of the papers estimating peer effects that use this particular database have taken the network structure as given. One notable exception is \cite{griffith2019namefriends}, looking at censoring: students can only report up to five male and five female friends. We also allow for censoring but show that censoring is not the most important issue with the Add Health data. To understand why, we discuss the organization of the data.

Each adolescent is assigned a unique identifier. The data includes ten variables for the ten potential friendships (maximum of five male and five female friends). These variables can contain missing values (no friendship was reported), an error code (the named friend could not be found in the database), or an identifier for the reported friends. This data is then used to generate the network's adjacency matrix $\mathbf{A}$.

Of course, error codes cannot be matched to any particular adolescent; as well, even in the case where the friendship variable refers to a valid identifier, the referred adolescent may still be absent from the database. A prime example is when the referred adolescent has been removed from the database by the researcher, perhaps due to other missing variables for these particular individuals. These missing links are quantitatively important as they account for roughly 30\% of the total number of links (7,830 missing for 17,993 observed links). Figure \ref{fig:misfr} displays the distribution of the number of ``unmatched named friends.''\footnote{We focus on within-school friendships; thus, nominations outside of school are not treated as ``unmatched friends.''}
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.6]{graphs/Missing.pdf}
    \caption{Frequencies of the number of missing links per adolescent.}
    \label{fig:misfr}
\end{figure}

To use the methodology developed in Section \ref{sec:genestim}, we first need to estimate a network formation model using the observed network data. In this section, we assume that links are generated using a simple logistic framework, i.e.
$$
P(a_{ij}=1)\propto\exp\{\mathbf{w}_{ij}\boldsymbol{\rho}\},
$$
where $\mathbf{w}_{ij}$ is built to capture homophily on the observed characteristics of $i$ and $j$ (see Table \ref{tab:application}). We estimate the network formation model on the set of individuals who nominate strictly less than five male and five female friends and for which we observe no ``unmatched friends.'' For these students, we know for sure that their friendship data is complete. Under a missing at random assumption, the estimation is consistent.

Table \ref{tab:application} presents the estimation results for the network formation model (panel \emph{Network Formation}), as well as for the peer effect model (panel \emph{Peer Effect Model}, column \emph{Reconstructed Network}). We also present the results for the (inconsistent) estimation of the peer effect model under the assumption that the observed network is the true one (panel \emph{Peer Effect Model}, column \emph{Observed Network}).

We find evidence of homophily on all observed covariates, which is coherent with the literature (e.g. \cite{currarini2010identifying,boucher2017my,mele2020does}). The bias on the peer effects' coefficients (endogenous and contextual) is qualitatively important (and statistically significant). The estimated endogenous peer effect using the reconstructed network is 1.6 times larger than the one estimated assuming that the observed network is the true network. The reconstructed network also allows capturing a positive effect of having a high proportion of Hispanic friends on academic achievement.

The contribution of censoring to these biases is insignificant. In Table \ref{tab:appendapplication} of the Online Appendix, we report estimates for two alternative cases: one in which we disregard censoring and another in which censoring is the only data issue. The impact of controlling for censoring is almost null, coherent with the fact that only about 5\% of the observations are potentially censored.

Our exercise shows that data errors are a first-order concern when using the Add Health database. We do not argue, however, that our estimated coefficients in Table \ref{tab:application} are necessarily causal because the friendship network is likely endogenous (e.g. \cite{goldsmith2013social,hsieh2018smoking,hsieh2019specification}). The estimation of peer effects with partial endogenous network data is left for future research but is discussed in the next section.

\begin{table}[]
\small
\centering
\caption{Posterior distribution.} 
\label{tab:application} 
  \begin{adjustbox}{max width=0.85\textwidth}
\begin{tabular}{lld{5}d{3}d{3}d{5}d{3}d{3}}
\\[-1.8ex]
\toprule
      &       & \multicolumn{3}{c}{Observed network} & \multicolumn{3}{c}{Reconstructed network} \\\hline\hline
\multicolumn{2}{l}{Statistic} & \multicolumn{1}{c}{Mean}  & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{\textit{t}-stat} & \multicolumn{1}{c}{Mean}  & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{\textit{t}-stat} \\\hline\\[-1.8ex]
\midrule
                          & \multicolumn{7}{c}{\textbf{Peer effect model}}  \\ \\[-2ex]
\multicolumn{2}{l}{Peer effects}                       & 0.350***    & (0.024)    & 14.809    & 0.564***      & (0.044)      & 12.842     \\
\multicolumn{2}{l}{\textbf{Own effects}}               &             &            &           &               &              &            \\
\multicolumn{2}{l}{Female}                      & 0.144***   & (0.029)    & 5.018    & 0.120***     & (0.031)      & 3.822     \\
\multicolumn{2}{l}{Hispanic}                    & -0.083**     & (0.042)    & -1.980     & -0.145**       & (0.047)      & 3-.090      \\
\multicolumn{2}{l}{Race (White)}                &             &            &           &               &              &            \\
                          & Black               & -0.230***    & (0.045)    & -5.070     & -0.210***      & (0.055)      & -3.787      \\
                          & Asian               & -0.091       & (0.089)    & -1.024     & -0.115         & (0.089)      & -1.286      \\
                          & Other               & 0.055      & (0.051)    & 1.064    & 0.036        & (0.052)      & 0.686     \\
\multicolumn{2}{l}{Mother's education (High)}            &             &            &           &               &              &            \\
                          & \textless high      & -0.122**     & (0.039)    & -3.147     & -0.126**       & (0.039)      & -3.201      \\
                          & \textgreater high   & 0.140***   & (0.034)    & 4.131    & 0.109**      & (0.034)      & 3.208     \\
                          & missing             & -0.060       & (0.050)    & -1.182     & -0.065         & (0.051)      & -1.277      \\
\multicolumn{2}{l}{Mother's job (Stay-at-home)}         &             &            &           &               &              &            \\
                          & Professional        & 0.080*     & (0.045)    & 1.793    & 0.078*       & (0.044)      & 1.759     \\
                          & Other               & 0.003      & (0.035)    & 0.078    & -0.006         & (0.035)      & -0.168      \\
                          & Missing             & -0.066       & (0.047)    & -1.400     & -0.068         & (0.048)      & -1.427      \\
\multicolumn{2}{l}{Age}                         & -0.073***    & (0.010)    & -7.606     & -0.078***      & (0.011)      & -7.168      \\
\multicolumn{2}{l}{\textbf{Contextual effects}}          &             &            &           &               &              &            \\
\multicolumn{2}{l}{Female}                      & 0.011      & (0.049)    & 0.221    & 0.072        & (0.092)      & 0.779     \\
\multicolumn{2}{l}{Hispanic}                    & 0.060      & (0.069)    & 0.868    & 0.353**      & (0.115)      & 3.081     \\
\multicolumn{2}{l}{Race (White)}                &             &            &           &               &              &            \\
                          & Black               & 0.050      & (0.058)    & 0.865    & 0.058        & (0.075)      & 0.769     \\
                          & Asian               & 0.209      & (0.186)    & 1.126    & 0.518        & (0.579)      & 0.895     \\
                          & Other               & -0.137       & (0.089)    & -1.537     & -0.230         & (0.185)      & -1.241      \\
\multicolumn{2}{l}{Mother's education (High)}            &             &            &           &               &              &            \\
                          & \textless High      & -0.269***    & (0.070)    & -3.841     & -0.363**       & (0.158)      & -2.290      \\
                          & \textgreater High   & 0.072      & (0.059)    & 1.213    & 0.062        & (0.114)      & 0.540     \\
                          & Missing             & -0.077       & (0.093)    & -0.835     & -0.025         & (0.197)      & -0.128      \\
\multicolumn{2}{l}{Mother's job (Stay-at-home)}         &             &            &           &               &              &            \\
                          & Professional        & -0.110       & (0.080)    & -1.373     & 0.032        & (0.157)      & 0.204     \\
                          & Other               & -0.101*      & (0.060)    & -1.686     & -0.051         & (0.114)      & -0.451      \\
                          & Missing             & -0.093       & (0.085)    & -1.086     & -0.006         & (0.188)      & -0.029      \\
\multicolumn{2}{l}{Age}                         & 0.066***   & (0.006)    & 11.323   & 0.091***     & (0.010)      & 9.228     \\
\midrule
SE$^2$     &                     & 0.523       &            &           & 0.515         &              &            \\\\[-1.8ex]
\midrule
                          & \multicolumn{7}{c}{\textbf{Network formation model}}                                                            \\\\[-2ex]
\multicolumn{2}{l}{Same sex}                    &             &            &           & 0.456***      & (0.016)      & 28.208     \\
\multicolumn{2}{l}{Both Hispanic}               &             &            &           & 0.343***      & (0.023)      & 14.739     \\
\multicolumn{2}{l}{Both White}                  &             &            &           & 0.320***      & (0.022)      & 14.741     \\
\multicolumn{2}{l}{Both Black}                  &             &            &           & 1.167***      & (0.032)      & 36.121     \\
\multicolumn{2}{l}{Both Asian}                  &             &            &           & 0.278***      & (0.043)      & 6.502      \\
\multicolumn{2}{l}{Mothers education \textless High}    &             &            &           & 0.178***      & (0.018)      & 10.063     \\
\multicolumn{2}{l}{Mothers education \textgreater High} &             &            &           & 0.075***      & (0.016)      & 4.756      \\
\multicolumn{2}{l}{Mothers job Professional}       &             &            &           & -0.130***     & (0.017)      & -7.544     \\
\multicolumn{2}{l}{Age absolute difference}           &             &            &           & -0.648***     & (0.010)      & -64.105   \\
\bottomrule
\\
\multicolumn{8}{l}{%
  \begin{minipage}{16cm}%
  \vspace{0.1cm}
    \footnotesize{Note: \textit{N} = 3,126. Observed links = 17,993. Proportion of inferred network data = 77.7\%. Significance levels: $^{***} = 1$\%,   $^{**} = 5$\%, $^* = 10$\%. The explained variable is computed by taking the average grade for English, Mathematics, History, and Science, letting $A=4$, $B=3$, $C=2$, and $D=1$. Thus, higher scores indicate better academic achievement.}
  \end{minipage}%
}\\
\end{tabular} 
\end{adjustbox}
\end{table} 

==> archives/shortversion/bayesian.tex <==

\section{Estimation Using Bayesian Inference}\label{sec:genestim}

In the previous section, we showed that in a context in which $\mathbf{Gy}$ and $\mathbf{GX}$ are unobserved, and that the distribution of the network is imprecise, the SGMM estimator can be imprecise. In this section, we therefore present a likelihood-based estimator. Accordingly, greater structure must be imposed on the errors $\boldsymbol{\varepsilon}$.\footnote{One could also use our estimator to solve a classical estimator such as a GMM estimator,  like that proposed by \cite{chandrasekhar2011econometrics}, using either the approach proposed by \cite{chernozhukov2003mcmc}, or the Bayesian empirical likelihood approach by \cite{chib2018bayesian}.}

To clarify the exposition, we will focus on the network adjacency matrix $\mathbf{A}$ rather than the interaction matrix $\mathbf{G}$. Of course, this is without any loss of generality. Given parametric assumptions for $\boldsymbol{\varepsilon}$, one can write the log-likelihood of the outcome as:\footnote{Note that under Assumption \ref{as:manymarkets}, the likelihood can be factorized across groups.}
\begin{equation}\label{eq:likelihood}
\ln \mathcal{P}(\mathbf{y}|\mathbf{A},\boldsymbol{\theta}),    
\end{equation}
where $\boldsymbol{\theta}=[\alpha,\boldsymbol{\beta}',\boldsymbol{\gamma}',\boldsymbol{\sigma}']'$, $\boldsymbol{\sigma}$ are unknown parameters from the distribution of $\boldsymbol{\varepsilon}$. Note that $\mathbf{y}=(\mathbf{I}_N-\alpha\mathbf{G})^{-1}(c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+{\mathbf{GX}}\boldsymbol{\gamma}+\boldsymbol{\varepsilon})$ and $(\mathbf{I}_N-\alpha\mathbf{G})^{-1}$ exist under our Assumption \ref{as:alpha}.

If the adjacency matrix $\mathbf{A}$ was observed, then $\boldsymbol{\theta}$ could be estimated using a simple maximum likelihood estimator (as in \cite{lee2010specification}) or using Bayesian inference (as in \cite{goldsmith2013social}).

Since $\mathbf{A}$ is not observed, an alternative would be to focus on the unconditional likelihood, i.e.
$$
\ln \mathcal{P}(\mathbf{y}|\boldsymbol{\theta})=\ln \sum_\mathbf{A}\mathcal{P}(\mathbf{y}|\mathbf{A},\boldsymbol{\theta})P(\mathbf{A}).
$$
A similar strategy is proposed by \cite{chandrasekhar2011econometrics} using a GMM estimator.

One particular issue with estimating $\ln \mathcal{P}(\mathbf{y}|\boldsymbol{\theta})$ is that the summation is not tractable. Indeed, the sum is over the set of possible adjacency matrices, which contain $2^{N(N-1)}$ elements. Then, simply simulating networks from $P(\mathbf{A})$ (or rather from $\hat{P}(\mathbf{A})$) as proposed by \cite{chandrasekhar2011econometrics}, and taking the average likely lead to poor approximations. A classical way to address this issue is to use an EM algorithm \citep{dempster1977maximum}. Although valid, we found that the Bayesian estimator proposed in this section is less restrictive and numerically outperforms its classical counterpart.

For concreteness, we will assume that $\boldsymbol{\varepsilon}\sim\mathcal{N}(0,\sigma^2\mathbf{I}_N)$; however, it should be noted that our approach is valid for a number of alternative assumptions, as long as it yeilds a computationally tractable likelihood. We have, for $\mathbf{G}=f(\mathbf{A})$,
\begin{eqnarray*}
\ln \mathcal{P}(\mathbf{y}|\mathbf{A},\boldsymbol{\theta})&=&-N\ln(\sigma)+\ln|\mathbf{I}_N-\alpha\mathbf{G}|-\frac{N}{2}\ln(\pi)\\&&-\frac{1}{2\sigma^2}[(\mathbf{I}_N-\alpha\mathbf{G})\mathbf{y}-c\mathbf{1}_N-\mathbf{X}\boldsymbol{\beta}-\mathbf{GX}\boldsymbol{\gamma}]'\cdot\\ &&[(\mathbf{I}_N-\alpha\mathbf{G})\mathbf{y}-c\mathbf{1}_N-\mathbf{X}\boldsymbol{\beta}-\mathbf{GX}\boldsymbol{\gamma}].
\end{eqnarray*}
Since $\mathbf{A}$ is not observed, we follow \cite{tanner1987calculation} and \cite{albert1993bayesian}, and we use data augmentation to evaluate the posterior distribution of $\boldsymbol{\theta}$. That is, instead of focusing on the posterior $p(\boldsymbol{\theta}|\mathbf{y},\mathbf{A})$, we focus on the posterior $p(\boldsymbol{\theta},\mathbf{A}|\mathbf{y},\mathcal{A})$, treating $\mathbf{A}$ as another set of unknown parameters. Note that we now make  the dependence on $\mathcal{A}$ explicit for clarity.

Indeed, the identification of the model rests on the a priori information of $\mathbf{A}$. A sensible prior for $\mathbf{A}$ is the consistent estimator of its distribution, i.e. $\hat{P}(\mathbf{A}|\mathcal{A})\equiv P(\mathbf{A}|\hat{\boldsymbol{\rho}},\mathcal{A})$. One may wish, however, to also use the information regarding the sampling uncertainty around $\hat{P}(\mathbf{A}|\mathcal{A})$. This is very similar to inference for two-step estimators in a classical setting: estimation uncertainty in the first stage must be accounted for to provide valid inference in the second stage (see \cite{cameron2005microeconometrics}, Section 6.6, for a discussion).

Let $\pi(\boldsymbol{\rho}|\mathcal{A})$ be the prior density on $\boldsymbol{\rho}$. How to obtain $\pi(\boldsymbol{\rho}|\mathcal{A})$, depending on whether $\hat{\boldsymbol{\rho}}$ is obtained using a Bayesian or classical setting, is discussed in Examples \ref{ex:prior_distr} and \ref{ex:prior_post} below. Given $\pi(\boldsymbol{\rho}|\mathcal{A})$, it is possible to obtain draws from the posterior distribution $p(\boldsymbol{\rho},\mathbf{A}|\mathbf{y},\mathcal{A})$ using the following MCMC:
\begin{algorithm}\label{algo:mcmc} The MCMC goes as follows for $t=1,...,T$, starting from any $\mathbf{A}_0,\boldsymbol{\theta}_0$, and $\boldsymbol{\rho}_0$.
\begin{enumerate}
    \item Draw $\boldsymbol{\rho}^*$ from the proposal distribution $q_\rho(\boldsymbol{\rho}^*|\boldsymbol{\rho}_{t-1})$ and accept $\boldsymbol{\rho}^*$ with probability
    $$
    \min\left\lbrace 1,\frac{P(\mathbf{A}_{t-1}|\boldsymbol{\rho}^*,\mathcal{A})q_\rho(\boldsymbol{\rho}_{t-1}|\boldsymbol{\rho}^*)\pi(\boldsymbol{\rho}^*|\mathcal{A})}
    {P(\mathbf{A}_{t-1}|\boldsymbol{\rho}_{t-1},\mathcal{A})q_\rho(\boldsymbol{\rho}^*|\boldsymbol{\rho}_{t-1})\pi(\boldsymbol{\rho}_{t-1}|\mathcal{A})} \right\rbrace.
    $$
    \item Propose $\mathbf{A}^*$ from the proposal distribution $q_A(\mathbf{A}^*|\mathbf{A}_{t-1})$ and accept $\mathbf{A}^*$ with probability
    $$
    \min\left\lbrace 1,\frac{\mathcal{P}(\mathbf{y}|\boldsymbol{\theta}_{t-1},\mathbf{A}^*)q_A(\mathbf{A}_{t-1}|\mathbf{A}^*)P(\mathbf{A}^*|{\boldsymbol{\rho}_{t-1}},\mathcal{A})}{\mathcal{P}(\mathbf{y}|\boldsymbol{\theta}_{t-1},\mathbf{A}_{t-1})q_A(\mathbf{A}^*|\mathbf{A}_{t-1})P(\mathbf{A}_{t-1}|{\boldsymbol{\rho}_{t-1}},\mathcal{A})} \right\rbrace.
    $$
    \item Draw $\alpha^*$ from the proposal $q_\alpha(\cdot|\alpha_{t-1})$ and accept $\alpha^*$ with probability
    $$
    \min\left\lbrace 1,\frac{\mathcal{P}(\mathbf{y}|\mathbf{A}_{t};\boldsymbol{\beta}_{t-1},\boldsymbol{\gamma}_{t-1},\alpha^*)q_\alpha(\alpha_{t - 1}|\alpha^*)\pi(\alpha^*)}{\mathcal{P}(\mathbf{y}|\mathbf{A}_{t};\boldsymbol{\theta}_{t-1})q_\alpha(\alpha^*|\alpha_{t-1})\pi(\alpha_{t-1})}\right\rbrace.
    $$
    \item Draw $[\boldsymbol{\beta,\gamma},\sigma]$ from their conditional distributions.
\end{enumerate}
\end{algorithm}

As discussed, Step 1 accounts for the sampling uncertainty around the true value of $\boldsymbol{\rho}$. If the true value of $\boldsymbol{\rho}$ was known (instead of being estimated) Step 1 would not be required. Step 1 shows that the flexibility of the network formation model comes at a cost. For example, \cite{graham2017econometric} and \cite{breza2017using} propose network formation models for which the number of parameters is $O(N_r)$. In turn, this large number of parameters increases the computational cost of Step 1.


\begin{example}[Priors from the Asymptotic Distribution of $\boldsymbol{\rho}$]\label{ex:prior_distr}
In a classical setting, and under the usual assumptions, the estimation of (\ref{eq:gennetfor}) produces a estimator $\hat{\boldsymbol{\rho}}$ of $\boldsymbol{\rho}_0$ as well as an estimator of the asymptotic variance of $\hat{\boldsymbol{\rho}}$, i.e. $\hat{\mathbf{V}}(\hat{\boldsymbol{\rho}})$. In this case, we define the prior density $\pi(\boldsymbol{\rho})$ as the density of a multivariate normal distribution with mean $\hat{\boldsymbol{\rho}}$ and variance-covariance matrix $\hat{\mathbf{V}}(\hat{\boldsymbol{\rho}})$.
\end{example}

\begin{example}[Priors from the Posterior Distribution of $\boldsymbol{\rho}$]\label{ex:prior_post}
In a Bayesian setting, the estimation of $\boldsymbol{\rho}$ from the network formation model (\ref{eq:gennetfor}) results in draws from the posterior distribution of $\boldsymbol{\rho}$. It is therefore natural to use such a posterior distribution as the prior distribution of $\mathbf{A}$ for the estimation based on (\ref{eq:likelihood}). Performing such a sequential Bayesian updating approach comes with a well-known numerical issue.\footnote{See \cite{thijssen2020approximating} for a recent discussion.}

Indeed, the evaluation of the acceptance ratio in Step 1 of Algorithm \ref{algo:mcmc} below requires the evaluation of the density of $\boldsymbol{\rho}$ at different values. Ideally, one would use the draws from the posterior distribution of $\boldsymbol{\rho}$ from the first step (network formation model) and perform a nonparametric kernel density estimation of the posterior distribution. However, when the dimension of $\boldsymbol{\rho}$ is large, the kernel density estimation may be infeasible in practice.

This is especially true for very flexible network formation models, such as the one proposed by \cite{breza2017using}, for which the number of parameters to estimate is $O(N_r)$. In such a case, it might be more reasonable to use a more parametric approach or to impose additional restrictions on the dependence structure of $\boldsymbol{\rho}$ across dimensions.\footnote{For example, if we assume that the posterior distribution of $\boldsymbol{\rho}$ is jointly normal, the estimation of the mean and variance-covariance matrix is straightforward, even in a high-dimensional setting. Simulations (not reported) suggest that this approach performs well in practice.}
\end{example}


Detailed distributions for Steps 3 and 4 can be found in the Online Appendix. Step 2, however, involves requires some discussion. Indeed, the idea is the following: given the prior information $P(\textbf{A}|\boldsymbol{\rho}_{t-1},\mathcal{A})$, one must be able to draw samples from the posterior distribution of $\mathbf{A}$, given $\mathbf{y}$. This is not a trivial task.

In particular, there is no general rule for selecting the network proposal distribution $q_A(\cdot\vert\cdot)$. A natural candidate is a Gibbs sampling algorithm for each link, i.e. change only one link $ij$ at every step $t$ and propose $a_{ij}$ according to its marginal distribution, i.e. $a_{ij}\sim P(\cdot|\mathbf{A}_{-ij},\mathbf{y},\mathcal{A})$, where $\mathbf{A}_{-ij} = \{a_{kl}; k \ne i, l \ne j\}$. In this case, the proposal is always accepted.
%$$
%a_{ij}\sim P(\cdot|\mathbf{A}_{-ij},\mathbf{y},\mathcal{A})=\frac{\mathcal{P}(\mathbf{y}|a_{ij},\mathbf{A}_{-ij})P(a_{ij}|\mathbf{A}_{-ij};\tilde{\boldsymbol{\rho}},\mathcal{A})}{\mathcal{P}(\mathbf{y}|1,\mathbf{A}_{-ij})P(a_{ij}=1|\mathbf{A}_{-ij};\tilde{\boldsymbol{\rho}},\mathcal{A})+\mathcal{P}(\mathbf{y}|0,\mathbf{A}_{-ij})P(a_{ij}=0|\mathbf{A}_{-ij};\tilde{\boldsymbol{\rho}},\mathcal{A})},
%$$

However, it has been argued that Gibbs sampling could lead to slow convergence (e.g. \cite{snijders2002markov}, \cite{chatterjee2013estimating}), especially when the network is \emph{sparse} or exhibits a high level of \emph{clustering}. For example, \cite{mele2017} and \cite{bhamidi2008mixing} propose different blocking techniques that are meant to improve convergence.

Here, however, achieving Step 2 involves an additional computational issue because evaluating the likelihood ratio in Step 1 requires comparing the determinants $|\mathbf{I}-\alpha f(\mathbf{A}^*)|$ for each proposed $\mathbf{A}^*$, which is computationally intensive. In particular, taking $\mathbf{G}^*=f(\mathbf{A}^*)$ to be a row-normalization of $\mathbf{A}^*$, changing a single element of $\mathbf{A}^*$ results in a change in the entire corresponding row of $\mathbf{G}^*$. Still, comparing the determinant of two matrices that differ only in a single row is relatively fast. Moreover, when $\mathbf{G}=\mathbf{A}$, \cite{hsieh2019structural} propose a blocking technique that facilitates the computation of the determinant.

In any case, note that the computational complexity of Step 2 depends strongly on $P(\textbf{A}|\boldsymbol{\rho}_{t-1},\mathcal{A})$, which is a function of the assumed network formation model (\ref{eq:gennetfor}) and of the observed information about the network structure $\mathcal{A}$. For censored network data, for example, most of the network structure is observed (see Example \ref{ex:censored}). This implies that $P(a_{ij}|\boldsymbol{\rho}_{t-1},\mathcal{A})\in\{0,1\}$ for most pairs $ij$. As such, few entries of $\mathbf{A}$ must be updated in Step 2. The opposite is true for ARD (see Example \ref{ex:ard}) for which all entries of $\mathbf{A}$ must be updated.

Then, the appropriate blocking technique depends strongly on $P(\textbf{A}|\boldsymbol{\rho}_{t-1},\mathcal{A})$ as well as on the assumed distribution for $\boldsymbol{\varepsilon}$. For the simulations and estimations presented in this paper, we use the Gibbs sampling algorithm for each link, adapting the strategy proposed by \cite{hsieh2019structural} to our setting (see Proposition \ref{prop:det} in the Online Appendix. This can be viewed as a \emph{worse-case} scenario. Nonetheless, the Gibbs sampler performs reasonably well in practice, even for ARD;\footnote{Simulations available upon request.} however, we encourage researchers to try other updating schemes if Gibbs sampling performs poorly in their specific contexts. In particular, we present a blocking technique in the Online Appendix that is also implemented in our R package \texttt{PartialNetwork}.\footnote{Available at: \url{https://github.com/ahoundetoungan/PartialNetwork}}

It is important to note that the complexity of Step 2 is not limited to our Bayesian approach. Classical estimators, such as GMM estimators, face a similar challenge in requiring the integration over the entire set of networks. The strategy used here is to rely on a Metropolis--Hastings algorithm, a strategy that has also been successfully implemented in the related literature on ERGMs (e.g. \cite{snijders2002markov,mele2017,mele2020does,badev2018nash,hsieh2019structural,hsieh2019specification}).

Finally, note that for simple network formation models, it is possible to jointly estimate $\boldsymbol{\rho}$ and $\boldsymbol{\theta}$ within the same MCMC instead of using the two-step procedure described above. In that case, Step 1 can simply be replaced by:
\begin{enumerate}
    \item[1'.]  Draw $\boldsymbol{\rho}^*$ from the proposal distribution $q_\rho(\boldsymbol{\rho}^*|\boldsymbol{\rho}_{t-1})$ and accept $\boldsymbol{\rho}^*$ with probability
    $$
    \min\left\lbrace 1,\frac{P(\mathbf{A}_{t-1}|\boldsymbol{\rho}^*,\mathcal{A})P(\mathcal{A}|\boldsymbol{\rho}^*)q_\rho(\boldsymbol{\rho}_{t-1}|\boldsymbol{\rho}^*)\pi(\boldsymbol{\rho}^*)}
    {P(\mathbf{A}_{t-1}|\boldsymbol{\rho}_{t-1},\mathcal{A})P(\mathcal{A}|\boldsymbol{\rho}_{t-1})q_\rho(\boldsymbol{\rho}^*|\boldsymbol{\rho}_{t-1})\pi(\boldsymbol{\rho}_{t-1})} \right\rbrace.
    $$
\end{enumerate}
Here, $P(\mathcal{A}|\boldsymbol{\rho}^*)$ is the likelihood of the network information $\mathcal{A}$ assuming the network formation model in (\ref{eq:gennetfor}). Note that $\pi(\boldsymbol{\rho})$, the prior density on $\boldsymbol{\rho}$, no longer depends on $\mathcal{A}$ and can be chosen arbitrarily (e.g. uniform).

This approach would work well for simple models, such as the ones discussed in Examples \ref{ex:sampled} and \ref{ex:misclass}. It is impractical, however, for more involved models, such as the one proposed by \cite{breza2017using}.


==> archives/shortversion/bkp/IV_old.tex <==


\section{Estimation Using Instrumental Variables}\label{sec:iv}

We now present our instrumental variable strategy. To understand the underlying intuition, note that it is not necessary to observe the complete network structure to observe $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$. For example, one could simply obtain ${\mathbf{Gy}}$ from survey data, ``What is the average value of your friends' $y$?''

However, even observing $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$, the model (\ref{eq:linearinmean}) cannot be simply estimated using simple linear regression. The reason is that ${\mathbf{Gy}}$ is endogenous; thus, a linear regression would produce biased estimates (e.g. \cite{manski1993identification}, \cite{bramoulle2009identification}).

The typical instrumental approach to deal with this endogeneity is to use instruments based on the structural model, i.e. instruments constructed using second-degree peers (e.g. $\mathbf{G}^2\mathbf{X}$, see \cite{bramoulle2009identification}). These are less likely to be found in survey data. Indeed, we could doubt the informativeness of questions such as, ``What is the average value of your friends' average value of their friends' $x$?''

Propositions \ref{prop:gamma0} and \ref{prop:gammanot0} describe how to construct valid instruments when the researcher observes  $\mathbf{y}$, $\mathbf{X}$, and ${\mathbf{GX}}$. To clearly expose the argument, we first start by discussing the special case where there are no contextual effects: $\boldsymbol{\gamma}=\mathbf{0}$. The model in (\ref{eq:linearinmean}) can therefore be rewritten as: 
$$
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\mathbf{Gy}+\boldsymbol{\varepsilon}.
$$
The following proposition holds.\footnote{Proofs of Propositions \ref{prop:gamma0} and \ref{prop:gammanot0} can be found in Appendix \ref{sec:appendix_proofs}.}
\begin{proposition}\label{prop:gamma0}
Assume that $\boldsymbol{\gamma}=\mathbf{0}$. There are two cases:\begin{enumerate}
\item Suppose that $\mathbf{Gy}$ is observed and let $\boldsymbol{H}$ be an interaction matrix, correlated with $\mathbf{G}$, and such that $\mathbb{E}[\boldsymbol{\varepsilon}|\mathbf{X},\mathbf{H}]=\mathbf{0}$. Then, $\mathbf{H}\mathbf{X}$, $\mathbf{H}^2\mathbf{X}$,... are valid instruments.
\item Suppose that $\mathbf{Gy}$ \emph{is not} observed and let $\dot{\mathbf{G}}$ and $\ddot{\mathbf{G}}$ be two independent draws from the distribution $\hat{P}(\mathbf{G})$. Then, $\dot{\mathbf{G}}\mathbf{X}$, $\dot{\mathbf{G}}^2\mathbf{X}$,... are valid instruments when $\ddot{\mathbf{G}}\mathbf{y}$ is used as a proxy for $\mathbf{Gy}$, as $N\rightarrow\infty$.
\end{enumerate}
\end{proposition}

First, suppose that $\mathbf{Gy}$ is observed directly from the data. Then, any instrument correlated with the usual instruments $\mathbf{GX},\mathbf{G}^2\mathbf{X}$,..., while being exogenous, are valid. Note that a special case of the first part of Proposition \ref{prop:gamma0} is when $\mathbf{H}$ is drawn from $\hat{P}(\mathbf{G})$. However, the instrument remains valid if the researcher uses a \emph{mispecified} estimator of the distribution ${P}(\mathbf{G})$.\footnote{We would like to thank Chih-Sheng Hsieh and Arthur Lewbel for discussions on this important point.} A similar strategy is used by \cite{kelejian2014estimation} and \cite{lee2020key} in a different context. Of course, the specification error on $P(\mathbf{G})$ must be independent of $\boldsymbol{\varepsilon}$. In Section \ref{sec:ard}, we discuss the importance of this robustness feature in a context in which the network formation process could be misspecified or subject to small sample biases.\footnote{Note, however, that if the specification error is too large, the correlation between $\mathbf{Gy}$ and $\mathbf{H}\mathbf{X}$ will likely be small, leading to a problem of weak instruments. It is also worth noting that the first part of Proposition \ref{prop:gamma0} does not depend on the assumption that groups are entirely sampled (i.e. Assumption \ref{as:nosampling}).}

When $\mathbf{Gy}$ is \emph{not} observed directly, however, specification errors typically produce invalid instruments. As stated in Part 2 of Proposition \ref{prop:gamma0}, the estimation also requires two independent draws from $\hat{P}(\mathbf{G})$ instead of just one. To see why, let us rewrite the model as:
$$
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\ddot{\mathbf{G}}\mathbf{y}+[\boldsymbol{\eta}+\boldsymbol{\varepsilon}],
$$
where $\boldsymbol{\eta}=\alpha[\mathbf{G}\mathbf{y}-\ddot{\mathbf{G}}\mathbf{y}]$ is the error due to the approximation of $\mathbf{Gy}$. Suppose also that $\dot{\mathbf{G}}\mathbf{X}$ is used as an instrument for $\mathbf{Gy}$.

The validity of the instrument therefore requires $\mathbb{E}[\boldsymbol{\eta}+\boldsymbol{\varepsilon}|\mathbf{X},\dot{\mathbf{G}}\mathbf{X}]=0$, and in particular: $$\mathbb{E}[\mathbf{G}\mathbf{y}|\mathbf{X},\dot{\mathbf{G}}\mathbf{X}]=\mathbb{E}[\ddot{\mathbf{G}}\mathbf{y}|\mathbf{X},\dot{\mathbf{G}}\mathbf{X}],$$
which is true since $\mathbf{G}$ and $\ddot{\mathbf{G}}$ have the same asymptotic distribution.

Of course, Proposition \ref{prop:gamma0} assumes that there are no contextual effects. We show that a similar result holds when $\boldsymbol{\gamma}\neq \mathbf{0}$. To estimate (\ref{eq:linearinmean}) using an instrumental variable approach, however, we must assume that ${\mathbf{GX}}$ are \emph{observed}. The reason is that there are no natural, strong instruments for ${\mathbf{GX}}$.\footnote{Indeed, the strengths of the instruments in Proposition \ref{prop:gamma0} come from the fact that $\mathbf{GX}$ are strong instruments for $\mathbf{Gy}$ when $\mathbf{G}$ is observed. Proxying $\mathbf{GX}$ with $\ddot{\mathbf{G}}\mathbf{X}$ and instrumenting with $\dot{\mathbf{G}}\mathbf{X}$ would be valid. However, the explanatory power of $\dot{\mathbf{G}}\mathbf{X}$, conditional on $\ddot{\mathbf{G}}\mathbf{X}$, would be much too weak to be of any practical use.} In Section \ref{sec:genestim}, we present an alternative estimation strategy that does not require the observation of $\mathbf{GX}$.

\begin{proposition}\label{prop:gammanot0}
Assume that $\mathbf{GX}$ are observed. There are two cases:\begin{enumerate}
\item Suppose that $\mathbf{Gy}$ is observed and let $\boldsymbol{H}$ be an interaction matrix, correlated with $\mathbf{G}$, and such that $\mathbb{E}[\boldsymbol{\varepsilon}|\mathbf{X},\mathbf{H}]=\mathbf{0}$. Then, $\mathbf{H}^2\mathbf{X}$, $\mathbf{H}^3\mathbf{X}$,... are valid instruments.
\item Suppose that $\mathbf{Gy}$ \emph{is not} observed and let $\dot{\mathbf{G}}$ and $\ddot{\mathbf{G}}$ be two independent draws from the distribution $\hat{P}(\mathbf{G})$. Then, $\dot{\mathbf{G}}^2\mathbf{X}$, $\dot{\mathbf{G}}^3\mathbf{X}$,... are valid instruments when $\ddot{\mathbf{G}}\mathbf{y}$ is used as a proxy for $\mathbf{Gy}$, if $\ddot{\mathbf{G}}\mathbf{X}$ are added as additional explanatory variables and as $N\rightarrow\infty$.
\end{enumerate}
\end{proposition}
The first part of Proposition \ref{prop:gammanot0} is a simple extension of the first part of Proposition \ref{prop:gamma0}. The second part of Proposition \ref{prop:gammanot0} requires more discussion. Essentially, it states that $\dot{\mathbf{G}}^2\mathbf{X}$, $\dot{\mathbf{G}}^3\mathbf{X}$, ... are valid instruments when the following \emph{expanded model} is estimated:
\begin{equation}\label{eq:expanded}
    \mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha{\ddot{\mathbf{G}}\mathbf{y}}+{\mathbf{GX}}\boldsymbol{\gamma}+\ddot{\mathbf{G}}\mathbf{X}\check{\boldsymbol{\gamma}}+\boldsymbol{\eta}+\boldsymbol{\varepsilon},
\end{equation}
where the true value of $\check{\boldsymbol{\gamma}}$ is $\mathbf{0}$.

To understand why the introduction of $\ddpt{\mathbf{G}}\mathbf{X}\check{\boldsymbol{\gamma}}$ is needed, recall that the constructed instrument must be uncorrelated with the approximation error $\boldsymbol{\eta}$. This correlation is conditional on the explanatory variables, which contain $\mathbf{G}$. In particular, it implies that generically, $$\mathbb{E}[\mathbf{G}\mathbf{y}|\mathbf{X},\mathbf{GX},\dot{\mathbf{G}}^2\mathbf{X}]\neq\mathbb{E}[\ddot{\mathbf{G}}\mathbf{y}|\mathbf{X},\mathbf{GX},\dot{\mathbf{G}}^2\mathbf{X}].$$

However, adding the auxiliary variable $\ddot{\mathbf{G}}\mathbf{X}$ as a covariate is sufficient to restore the result, i.e. as $N\rightarrow\infty$: $$\mathbb{E}[\mathbf{G}\mathbf{y}|\mathbf{X},\mathbf{GX},\dot{\mathbf{G}}^2\mathbf{X}, \ddot{\mathbf{G}}\mathbf{X}]=\mathbb{E}[\ddot{\mathbf{G}}\mathbf{y}|\mathbf{X},\mathbf{GX},\dot{\mathbf{G}}^2\mathbf{X}, \ddot{\mathbf{G}}\mathbf{X}].$$


Proposition \ref{prop:gamma0} and Proposition \ref{prop:gammanot0} therefore show that the estimation of (\ref{eq:linearinmean}) is possible, even with very limited information about the network structure. Note, however, that the validity of the constructed instruments only holds asymptotically. In Section \ref{sec:ard}, we study the finite sample properties of our approach using network formation models estimated on aggregated relational data (\cite{breza2017using}; see Example \ref{ex:ard}). Before, however, we briefly discuss how one can adapt this estimation strategy while allowing for group-level unobservables.

Indeed, a common assumption is that each group in the population is affected by a common shock, unobserved by the econometrician (e.g. \cite{bramoulle2009identification}). As such, for each group $r=1,...,M$, we have: $\mathbf{y}_r=c_r\mathbf{1}_r+\mathbf{X}_r\boldsymbol{\beta}+\alpha\mathbf{G}_r\mathbf{y}_r+{\mathbf{G}_r\mathbf{X}_r}\boldsymbol{\gamma}+\boldsymbol{\varepsilon}_r$, where $c_r$ is not observed, $\mathbf{1}_r$ is an $N_r$-dimensional vector of ones, $N_r$ is the size of the group r, $\bG_r$ is the subinteraction matrix in the group r, and $\bepsilon_r$ is the vector of error terms in the group r.

Under Assumption \ref{as:manymarkets}, it is not possible to obtain a consistent estimator of $\{c_r\}_{r=1}^m$ because the number of observations used to estimate each $c_r$ is bounded. This is known as the \emph{incidental parameter problem}.\footnote{See \cite{lancaster2000incidental} for a review.} A common strategy is to use deviations from the group average and estimate the model in deviations (e.g. \cite{bramoulle2009identification}).

Let $\mathbf{J}=diag\{\mathbf{I}_{N_r}-\frac{1}{N_r}\mathbf{1}_r\mathbf{1}'_r\}$ be the group-differentiating matrix, where $\mathbf{I}_{N_r}$ is the identified matrix of dimension $N_r$. The operator \emph{diag} generates a blog-diagonal matrix in which each group is a block.\footnote{Then, $\mathbf{Jw}$ gives $\mathbf{w}$ minus the group average of $\mathbf{w}$.} We can rewrite: $\mathbf{Jy}=\mathbf{JX}\boldsymbol{\beta}+\alpha{\mathbf{JG}\mathbf{y}}+{\mathbf{JGX}}\boldsymbol{\gamma}+\boldsymbol{J\varepsilon}$. Note that the results of Propositions \ref{prop:gamma0} and \ref{prop:gammanot0} extend directly, using instruments in deviation with the group average.

\subsection{Finite Sample Performance Using ARD}\label{sec:ard}
In this section, we study the small sample performance of the estimator presented in Section \ref{sec:iv} when the researcher only has access to ARD (as in Example \ref{ex:ard}). First, we simulate network data using the model proposed by \cite{breza2017using} and simulate outcomes using the linear in means model (\ref{eq:linearinmean}) conditional on the simulated networks. Second, we estimate the network formation model using the Bayesian estimator proposed by \cite{breza2017using} (yielding $\hat{\boldsymbol{\rho}}_B$), as well as using the classical estimator proposed by \cite{alidaee2020recovering} (yielding $\hat{\boldsymbol{\rho}}_A$). Third, we estimate the linear-in-means model, using our IV estimator based on $\hat{\boldsymbol{\rho}}_A$ and $\hat{\boldsymbol{\rho}}_B$.

Recall that
\begin{equation}\label{eq:ard}
P(a_{ij}=1)\propto\exp\{\nu_i+\nu_j+\zeta \mathbf{z}_i'\mathbf{z}_j\},    
\end{equation}
where $\nu_i$, $\nu_j$, $\zeta$, $\mathbf{z}_i$, and $\mathbf{z}_j$ are not observed by the econometrician but follow parametric distributions. We refer the interested reader to \cite{mccormick2015latent}, \cite{breza2017using}, and \cite{breza2019consistently} for a formal discussion of the model, including its identification and consistent estimation. Here, we discuss the intuition using a simple analogy.

Suppose that individuals are located according to their geographical position on Earth. Suppose also that there are a fixed number of cities on Earth in which individuals can live. The econometrician does not know the individuals' locations on Earth nor do they know the location of the cities. In model (\ref{eq:ard}), $\mathbf{z}_i$ represent $i$'s position on Earth. However, the econometrician has access to ARD for a subset of the population, i.e. answers to questions such as, ``How many of your friends live in city $A$?''

To understand the intuition behind the identification of the model, consider the following example: suppose that individual $i$ has many friends living in city $A$. Then, city $A$ is likely located close to $i$'s location. Similarly, if many individuals have many friends living in city $A$, then city $A$ is likely a large city. Finally, if $i$ has many friends from many cities, $i$ likely has a large $\nu_i$.

To study the finite sample performance of our instrumental strategy in this context, we simulate 20 groups of 250 individuals each. Within each subpopulation, we simulate the ARD responses as well as a series of observable characteristics (e.g. cities). The details of the Monte Carlo simulations can be found in Appendix \ref{sec:ardsetting}.

Importantly, the model in (\ref{eq:ard}) is based on a single population framework. Thus, the network formation model must be estimated separately for each of the 20 groups. With only 250 individuals in each group, we therefore expect significant small-sample bias.

We contrast the estimator proposed by \cite{breza2017using} with the one proposed by \cite{alidaee2020recovering}. Whereas \cite{breza2017using} present a parametric Bayesian estimator, \cite{alidaee2020recovering} propose a (nonparametric) penalized regression based on a low-rank assumption. One main advantage of their estimator is that it allows for a wider class of model and ensures that the estimation is fast and easily implementable.\footnote{The authors developed user-friendly packages in R and Python. See their paper for links and details.} Note, however, that their method only yields a consistent estimator of $\hat{P}(\mathbf{A})$ if the true network is effectively low rank.

Very intuitively, the low-rank assumption implies that linking probabilities were generated from a small number of parameters; for example, in the example above, knowing individuals' gregariousness parameters $\nu_i$ and city in which they live would allow a prediction of the linking probabilities.

Importantly, the model (\ref{eq:ard}) is not necessarily low rank; for example, if the individuals' locations on Earth (i.e. the $\mathbf{z}_i$'s) are uniformly distributed and there are only very few  large cities, then the model produced is not low rank and the method proposed by \cite{alidaee2020recovering} performs poorly. Intuitively, in such a case, the fact that individual $i$ lives in city $A$ poorly explains the linking probabilities. 

We compare the performance of both estimators as we vary the concentration parameter for the individuals' locations on Earth (that is, $\kappa$, see Appendix \ref{sec:ardsetting} for details). This has the effect of changing the \emph{effective rank} of the linking probabilities: increasing $\kappa$ decreases the effective rank.\footnote{We refer the interested reader to \cite{alidaee2020recovering} for a formal discussion of the effective rank and of its importance for their estimator.} We therefore expect the estimator proposed by \cite{alidaee2020recovering} to perform better for larger values of $\kappa$.

Results are presented in Tables \ref{tab:breza} and \ref{tab:alidaee}. When $\mathbf{Gy}$ is observed, both estimators perform extremely well. In light of Propositions \ref{prop:gamma0} and \ref{prop:gammanot0}, this is expected, as the IV estimator is valid even under misspecification. When $\mathbf{Gy}$ is not observed, results are more nuanced. First, note that for all specifications, the introduction of the non-pertinent variables $\ddot{\mathbf{G}}\mathbf{X}$ contaminates the estimation of $\boldsymbol{\gamma}$. This occurs because ${\mathbf{G}}\mathbf{X}$ and $\ddot{\mathbf{G}}\mathbf{X}$ are highly correlated.\footnote{This is a small sample issue which is not due to the assumed network formation model and would arise even if the linking probabilities were known (instead of being estimated).} Note, however, that the estimated values for $\boldsymbol{\gamma}+\check{\boldsymbol{\gamma}}$ are centered on the true value. Second, the bias of the estimated endogenous peer effect (i.e. $\alpha$) goes to zero when the linking probabilities are of lower rank, with an advantage for the estimator proposed by  \cite{breza2017using}. This is expected because the model is correctly specified and the estimator is parametric. 

Overall, our IV estimator can be successfully implemented in small samples, using either the estimator proposed by \cite{breza2017using} or by \cite{alidaee2020recovering}, both of which only rely on the observation of ARD.

\renewcommand{\arraystretch}{.9}
\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD - network distribution estimated following \cite{breza2017using} } 
\label{tab:breza}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}d{4}d{4}d{4}d{4}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 0$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1ex]                                             
$\alpha=0.4$    & 0.400  & 0.007 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$                & 5.000  & 0.021 & 4.986   & 5.000  & 5.014   \\
$\gamma_2=-3$              & -3.001 & 0.031 & -3.021  & -3.000 & -2.980  \\  
F-test (Weak inst.) & 3144.574&	874.400&	2492.881&	3075.955&	3672.449 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                                          
$\alpha=0.4$ & 0.371  & 0.013 & 0.363   & 0.372  & 0.380   \\
$\gamma_1=5$            & 5.396  & 0.021 & 5.383   & 5.397  & 5.410   \\
$\gamma_2=-3$          & -2.400 & 0.041 & -2.428  & -2.400 & -2.371  \\
$\hat{\gamma}_1=0$          & -0.380 & 0.028 & -0.400  & -0.382 & -0.362  \\
$\hat{\gamma}_2=0$           & -0.553 & 0.044 & -0.584  & -0.551 & -0.525  \\
F-test (Weak inst.) & 3193.940&	760.793&	2642.815&	3153.048&	3666.220 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 10$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                                              
$\alpha=0.4$   & 0.400  & 0.006 & 0.396   & 0.400  & 0.404   \\
$\gamma_1=5$                & 5.001  & 0.019 & 4.988   & 5.001  & 5.014   \\
$\gamma_2=-3$             & -3.000 & 0.031 & -3.020  & -3.000 & -2.978  \\
F-test (Weak inst.) & 5905.596&	1876.836&	4519.460&	5766.601&	7158.739 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                                          
$\alpha=0.4$ & 0.400  & 0.007 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$            & 5.392  & 0.019 & 5.379   & 5.393  & 5.405   \\
$\gamma_2=-3$          & -2.397 & 0.037 & -2.421  & -2.398 & -2.373  \\
$\hat{\gamma}_1=0$           & -0.391 & 0.022 & -0.405  & -0.390 & -0.375  \\
$\hat{\gamma}_2=0$          & -0.604 & 0.038 & -0.630  & -0.605 & -0.579  \\
F-test (Weak inst.) & 5176.649&	1507.532&	4058.393&	5087.275&	6243.500 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 20$, $N=250$, $M=20$}                                                            \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                                             
$\alpha=0.4$    & 0.400  & 0.006 & 0.396   & 0.400  & 0.404   \\
$\gamma_1=5$                & 5.000  & 0.020 & 4.986   & 4.999  & 5.013   \\
$\gamma_2=-3$            & -3.001 & 0.031 & -3.021  & -3.001 & -2.981  \\
F-test (Weak inst.) &6104.999&	1927.633&	4734.460&	5937.815&	7246.355 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]   
$\alpha=0.4$ & 0.400  & 0.007 & 0.396   & 0.400  & 0.405   \\
$\gamma_1=5$            & 5.390  & 0.019 & 5.377   & 5.390  & 5.403   \\
$\gamma_2=-3$          & -2.398 & 0.036 & -2.422  & -2.398 & -2.375  \\
$\hat{\gamma}_1=0$           & -0.390 & 0.022 & -0.405  & -0.390 & -0.376  \\
$\hat{\gamma}_2=0$          & -0.604 & 0.036 & -0.628  & -0.604 & -0.579 \\ 
F-test (Weak inst.) & 5321.702&	1524.973&	4272.790&	5199.232&	6235.250 \\ 
\hline \\[-1.8ex] 


\multicolumn{6}{l}{%
  \begin{minipage}{15cm}%
    \footnotesize{Note: In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with a location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in Appendix \ref{sec:ardsetting}. Predicted probabilities are computed using the mean of the posterior distribution. F-test is the Fisher-statistic of the Weak instruments test. We do not report the estimated values for $c$ and $\boldsymbol{\beta}$ to keep the table readable, but they are available upon request. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.}
  \end{minipage}%
}\end{tabular}
\end{table}

\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD - network distribution estimated following \cite{alidaee2020recovering} } 
\label{tab:alidaee}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}d{4}d{4}d{4}d{4}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 0$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1ex]                                
$\alpha=0.4$     & 0.400  & 0.012 & 0.393   & 0.400  & 0.407   \\
$\gamma_1=5$             & 5.000  & 0.029 & 4.980   & 4.999  & 5.019   \\
$\gamma_2=-3$             & -3.000 & 0.032 & -3.021  & -3.000 & -2.978  \\
F-test (Weak inst.) & 798.971&	340.558&	560.817&	749.132&	990.407\\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                          
$\alpha=0.4$ & 0.371  & 0.024 & 0.357   & 0.373  & 0.387   \\
$\gamma_1=5$              & 5.504  & 0.036 & 5.479   & 5.503  & 5.528   \\
$\gamma_2=-3$            & -2.480 & 0.057 & -2.517  & -2.480 & -2.441  \\
$\hat{\gamma}_1=0$           & -0.364 & 0.031 & -0.385  & -0.363 & -0.344  \\
$\hat{\gamma}_2=0$          & -0.302 & 0.070 & -0.349  & -0.304 & -0.254  \\
F-test (Weak inst.) & 590.248&	253.853&	409.497&	572.210&	721.788 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 10$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                              
$\alpha=0.4$    & 0.400  & 0.009 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$         & 4.999  & 0.022 & 4.985   & 4.999  & 5.014   \\
$\gamma_2=-3$                & -3.000 & 0.032 & -3.022  & -3.001 & -2.978 \\
F-test (Weak inst.) & 1697.514&	741.478&	1179.079&	1593.284&	2127.582\\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                          
$\alpha=0.4$  & 0.395  & 0.021 & 0.388   & 0.397  & 0.405   \\
$\gamma_1=5$            & 5.396  & 0.027 & 5.378   & 5.394  & 5.412   \\
$\gamma_2=-3$            & -2.412 & 0.045 & -2.439  & -2.410 & -2.383  \\
$\hat{\gamma}_1=0$          & -0.385 & 0.032 & -0.404  & -0.387 & -0.370  \\
$\hat{\gamma}_2=0$           & -0.462 & 0.117 & -0.534  & -0.483 & -0.414  \\
F-test (Weak inst.) &1303.291&	586.429&	895.070&	1227.426&	1652.148\\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 20$, $N=250$, $M=20$}                                                            \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                              
$\alpha=0.4$     & 0.400  & 0.008 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$                & 5.000  & 0.021 & 4.985   & 5.000  & 5.013   \\
$\gamma_2=-3$             & -2.999 & 0.032 & -3.020  & -2.999 & -2.979   \\
F-test (Weak inst.) & 2685.354&	978.512&	1998.396&	2601.996&	3268.714 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]   
$\alpha=0.4$ & 0.399  & 0.010 & 0.393   & 0.400  & 0.406   \\
$\gamma_1=5$        & 5.391  & 0.020 & 5.378   & 5.391  & 5.404   \\
$\gamma_2=-3$             & -2.400 & 0.039 & -2.425  & -2.400 & -2.374  \\
$\hat{\gamma}_1=0$           & -0.391 & 0.022 & -0.406  & -0.391 & -0.376  \\
$\hat{\gamma}_2=0$          & -0.573 & 0.047 & -0.605  & -0.575 & -0.544 \\ 
F-test (Weak inst.) & 2191.313&	774.366&	1656.355&	2130.681&	2668.781\\ 
\hline \\[-1.8ex] 



\multicolumn{6}{l}{%
  \begin{minipage}{15cm}%
    \footnotesize{Note: In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in Appendix \ref{sec:ardsetting}. We chose the weight associated with the nuclear norm penalty to minimize the RMSE through cross-validation. This value of $\lambda=600$ is smaller than the recommended value in \cite{alidaee2020recovering}. F-test is the Fisher-statistic of the Weak instruments test. We do not report the estimated values for $c$ and $\boldsymbol{\beta}$ to keep the table readable, but they are available upon request. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.}
  \end{minipage}%
}\end{tabular}
\end{table}
\renewcommand{\arraystretch}{1}

==> archives/shortversion/bkp/iv_old__1_.tex <==


\section{Estimation Using Instrumental Variables}\label{sec:iv}

We now present our instrumental variable strategy. To understand the underlying intuition, note that it is not necessary to observe the complete network structure to observe $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$. For example, one could simply obtain ${\mathbf{Gy}}$ from survey data, ``What is the average value of your friends' $y$?''

However, even observing $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$, the model (\ref{eq:linearinmean}) cannot be simply estimated using simple linear regression. The reason is that ${\mathbf{Gy}}$ is endogenous; thus, a linear regression would produce biased estimates (e.g. \cite{manski1993identification}, \cite{bramoulle2009identification}).

The typical instrumental approach to deal with this endogeneity is to use instruments based on the structural model, i.e. instruments constructed using second-degree peers (e.g. $\mathbf{G}^2\mathbf{X}$, see \cite{bramoulle2009identification}). These are less likely to be found in survey data. Indeed, we could doubt the informativeness of questions such as, ``What is the average value of your friends' average value of their friends' $x$?''

However, the above discussion is encouraging. When researchers observe $[\mathbf{y}, \mathbf{X}, {\mathbf{GX}},{\mathbf{Gy}}]$, information about the network is only used as a mean to construct a valid instrument, e.g. following \citet{bramoulle2009identification}. We propose one simple way to construct such an instrument in Proposition \ref{prop:all_observed} below.

\begin{proposition}\label{prop:all_observed}
[Conditions] Suppose that $\mathbf{GX}$ and $\mathbf{Gy}$ are observed and define the matrix $\mathbf{Z}=[\mathbf{1},\mathbf{X},\mathbf{GX},\mathbf{H}^2\mathbf{X},\mathbf{H}^3\mathbf{X}...]$. Let $\boldsymbol{H}$ be a matrix such that: (1) at least one column of $\mathbf{H}^k\mathbf{X}$ is correlated with $\mathbf{G}\mathbf{y}$, conditional on $[\mathbf{1},\mathbf{X},\mathbf{GX}]$ for $k\geq 2$, and (2) $\mathbb{E}[\boldsymbol{\varepsilon}|\mathbf{X},\mathbf{H}]=\mathbf{0}$.

[Results] Then, under classical assumptions (e.g. \cite{cameron2005microeconometrics}, Proposition 6.1), the (linear) GMM estimator based on the moment function $\frac{1}{N}\sum_i\mathbf{Z}_i'\boldsymbol{\varepsilon}_i=\mathbf{0}$ is consistent and asymptotically normally distributed with the usual asymptotic variance-covariance matrix.
\end{proposition}

Condition (1) is the relevancy condition, while condition (2) is the exogeneity condition. While Proposition \ref{prop:all_observed} holds for any matrix $\mathbf{H}$ such that conditions (1) and (2), the most sensible example is when $\mathbf{H}$ is constructed using a draw from $\hat{P}(\mathbf{G})$. A similar strategy is used by \cite{kelejian2014estimation}, \cite{konig2019r} and \cite{lee2020key} in a different context.

Importantly, the moment conditions remain valid even when the researcher uses a \emph{mispecified} estimator of the distribution ${P}(\mathbf{G})$, as long as the specification error on $P(\mathbf{G})$ does not induce a correlation with $\boldsymbol{\varepsilon}$.\footnote{We would like to thank Chih-Sheng Hsieh and Arthur Lewbel for discussions on this important point.} This could be of great practical importance, especially if the estimation of $\hat{P}(\mathbf{G})$ suffers from small sample bias. We provide an example in Section \ref{sec:ard} below.

We now turn to the more general case where $\mathbf{Gy}$ and $\mathbf{GX}$ are not observed. To simplify the notation, for the remainder of this section, we define $\lbrace \dot{\mathbf{G}}^{(s)}\rbrace_{s=1}^S$ and $\lbrace \ddot{\mathbf{G}}^{(t)}\rbrace_{t=1}^T$ be two sequences of independent draws from $\hat{P}(\mathbf{G})$. We will also let $\dot{\mathbf{G}}$ and $\ddot{\mathbf{G}}$ be single draws from $\hat{P}(\mathbf{G})$.

To understand why we cannot simply proxy $\mathbf{Gy}$ and $\mathbf{GX}$ using draws form $\hat{P}(\mathbf{G})$, consider the simple case for which $\boldsymbol{\gamma}=\mathbf{0}$, so the observation of $\mathbf{GX}$ is inconsequential. We have:
$$
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\ddot{\mathbf{G}}\mathbf{y}+[\boldsymbol{\eta}+\boldsymbol{\varepsilon}],
$$
where $\ddot{\mathbf{G}}$ is drawn from $\hat{P}(\mathbf{G})$, and $\boldsymbol{\eta}=\alpha[\mathbf{G}-\ddot{\mathbf{G}}]\mathbf{y}$ is the error due to the approximation of $\mathbf{Gy}$ by $\ddot{\mathbf{G}}\mathbf{y}$. Importantly, the approximation error does \emph{not} vanish as $n$ grows, due to the fact that individuals belong to bounded groups (see Assumption \ref{as:manymarkets}).\footnote{CITE Eric's paper.}

Our moment condition exploit the fact, however, that as $n$ grows, $\ddot{\mathbf{G}}$ and $ {\mathbf{G}}$ are drawn from the same distribution. Then, we can construct an instrument using \emph{another} draw  $\dot{\mathbf{G}}$ from $\hat{P}(\mathbf{G})$, say $\dot{\mathbf{G}}\mathbf{X}$. The intuition is that, as $n$ grows, the dependence between  $\dot{\mathbf{G}}$ and $ \ddot{\mathbf{G}}$ is the same as the dependence between  $\dot{\mathbf{G}}$ and  ${\mathbf{G}}$. This observation however, does not directly implies that $\dot{\mathbf{G}}\mathbf{X}$ is a valid instrument for $\ddot{\mathbf{G}}\mathbf{y}$ because $\dot{\mathbf{G}}\mathbf{X}$ is correlated with $\boldsymbol{\eta}$. This is due to the fact that $\mathbf{y}$ is a function of the true network $\mathbf{G}$, and as such, the correlation between columns of $\dot{\mathbf{G}}\mathbf{X}$ and $\mathbf{Gy}$ is not the same as the correlation between columns of $\dot{\mathbf{G}}\mathbf{X}$ and $\ddot{\mathbf{G}}\mathbf{y}$.\footnote{In an earlier version of this paper, we suggested such an approach. Although inconsistent, the bias in practice is very small. We discuss this point in Appendix.}

That being said we can bound the asymptotic bias, similarly to what is done in \cite{andrews2017measuring}. Proposition \ref{prop:bias_nocontext} formalizes.
\begin{proposition}\label{prop:bias_nocontext}
[Conditions] Assume that $\boldsymbol{\gamma}=\mathbf{0}$. Let $\ddot{\mathbf{S}}=[\mathbf{1},\mathbf{X},\ddot{\mathbf{G}}\mathbf{y}]$ and $\dot{\mathbf{Z}}=[\mathbf{1},\mathbf{X},\dot{\mathbf{G}}\mathbf{X},\dot{\mathbf{G}}^2\mathbf{X},...]$. Denote by $\hat{\boldsymbol{\theta}}$ the linear GMM estimator based on the (pseudo) moment function $\frac{1}{N}\sum_i \dot{\mathbf{Z}}_i[\boldsymbol{\eta}_i+\boldsymbol{\varepsilon}_i]$, and define the sensitivity matrix ${\mathbf{M}}=[\ddot{\mathbf{S}}'\dot{\mathbf{Z}}\mathbf{W}\dot{\mathbf{Z}}'\ddot{\mathbf{S}}]^{-1}\ddot{\mathbf{S}}'\dot{\mathbf{Z}}\mathbf{W}$.

[Result] Then, under classical assumptions (see proof), the asymptotic bias of $\hat{\boldsymbol{\theta}}_k$ is at most $Plim\sum_l |{\mathbf{M}}_{k,l}|b_l$, for all $k$, and where $b_l=|\alpha|^3(2Var_i(\sum_j\dot{\mathbf{Z}}_{jl}\ddot{\mathbf{G}}_{ji}))^{1/2}\max_i|y_i|$. Moreover, letting $\mathbf{W}=\mathbf{I}$ reduces the overall bias in the sense of minimizing the Froenius norm of ${\mathbf{M}}$.
\end{proposition}
Note that $Var_i(\sum_j\dot{\mathbf{Z}}_{jl}\ddot{\mathbf{G}}_{ji})$ decreases as the size $N_r$ of each group $r$ grows. We therefore expect the bias to be small for groups of medium sizes (such as small villages, see REF). The argument is very similar to the one in \cite{andrews2017measuring}, although here perturbation with respect to the true model is not \textit{local}.\footnote{See page 1562 in \cite{andrews2017measuring}.} We also show that we expect $\mathbf{W}=\mathbf{I}$ to minimize the overall bias. Our result therefore provides a theoretical justification for the simulations in \cite{onishi2021sample} who show that the using the identity matrix to weight the moments greatly reduce the bias in the context studied by \cite{andrews2017measuring}.

A similar result holds when we do not impose $\boldsymbol{\gamma}=\mathbf{0}$, although only when $\mathbf{GX}$ is observed.

\begin{corollary}\label{cor:bias}
Assume that $\mathbf{GX}$ is observed, then the results of Proposition \ref{prop:bias_nocontext} hold, with $b_l=|\alpha|^2(2Var_i(\sum_j\dot{\mathbf{Z}}_{jl}\ddot{\mathbf{G}}_{ji}))^{1/2}\max_i|y_i|$ for $\ddot{\mathbf{S}}=[\mathbf{1},\mathbf{X},\mathbf{GX},\ddot{\mathbf{G}}\mathbf{y}]$ and $\dot{\mathbf{Z}}=[\mathbf{1},\mathbf{X},\mathbf{GX},\ddot{\mathbf{G}}\mathbf{X},\dot{\mathbf{G}}^2\mathbf{X},\dot{\mathbf{G}}^3\mathbf{X},...]$.
\end{corollary}
Note that the instrument $\ddot{\mathbf{Z}}$ now includes the term $\ddot{\mathbf{G}}\mathbf{X}$, which is constructed using the same draw that is used to contruct the proxy variable $\ddot{\mathbf{G}}\mathbf{y}$. This is done to ensure that the columns of $\ddot{\mathbf{Z}}'\mathbf{G}$ and the columns of $\ddot{\mathbf{Z}}'\ddot{\mathbf{G}}$ have the same asymptotic distribution.\footnote{This also explains why the observation of $\mathbf{GX}$ is required.}

Following Proposition \ref{prop:bias_nocontext} and Corollary \ref{cor:bias}, if the maximal bias is small in practice, researchers may choose to use the pseudo GMM estimators and to report the maximal bias. However, if the maximal bias is large, we show that we can include the bias directly in the moment function, which provides a consistent estimator of $\boldsymbol{\theta}$. Let $\tilde{\boldsymbol{\theta}}=[c,\boldsymbol{\beta}',\boldsymbol{\gamma}']'$.

\begin{theorem}\label{prop:non_observed} [Conditions] Let $\dot{\mathbf{Z}}^{(s)}=[\mathbf{1},\mathbf{X},\dot{\mathbf{G}}^{(s)}\mathbf{X},(\dot{\mathbf{G}}^{(s)})^2\mathbf{X},(\dot{\mathbf{G}}^{(s)})^3\mathbf{X},...]$ and $\ddot{\mathbf{V}}^{(t)}=[\mathbf{1},\mathbf{X},\ddot{\mathbf{G}}^{(t)}\mathbf{X}]$. Consider also the following (simulated) moment function:
\begin{equation}\label{eq:moment}
\mathbb{E}(\frac{1}{ST}\sum_{t=1}^T\sum_{s=1}^S\dot{\mathbf{Z}}^{(s)\prime}_i(\mathbf{I}-\alpha\dot{\mathbf{G}}^{(s)})_i\left(\mathbf{y}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(t)})^{-1}\ddot{\mathbf{V}}^{(t)}\tilde{\boldsymbol{\theta}}\right))=\mathbf{0}
\end{equation}

[Result] For any $S$ and $T$, the (simulated) GMM estimator based on (\ref{eq:moment}) is consistent and asymptotically normal, i.e.  $\sqrt{N}(\hat{\boldsymbol{\theta}}-\boldsymbol{\theta}_0+\Delta\boldsymbol{\theta}^*)\overset{d}{\to}N(\mathbf{0},\mathbf{V})$, where $\Delta\boldsymbol{\theta}^*$ and $\mathbf{V}$ are defined in (\ref{eq:thetastar}) and (\ref{var:gmm}) in Appendix and where $\Delta\boldsymbol{\theta}^*\rightarrow 0$ as $N\rightarrow\infty$.
\end{theorem}
Here the asymptotic variance $\mathbf{V}$ includes the sampling uncertainty, the estimating uncertainty of $\hat{\boldsymbol{\rho}}$, as well as the simulating uncertainty (which decreases as $S$ and $T$ grow). The term $\Delta\boldsymbol{\theta}^*$ allows to center the distribution of $\hat{\boldsymbol{\theta}}$ for finite $N$, much like for the asymptotic distribution of penalized likelihood models (e.g. \cite{fan2001variable} or \cite{fan2004nonconcave}).

Importantly, and similar to standard methods of simulated moments (e.g. \cite{gourieroux1993simulation}), the estimation is consistent even for a finite number of simulations (i.e. $S$ and $T$ are finite). Our estimator therefore does not suffer from the curse of dimensionality faced by \cite{chandrasekhar2011econometrics}.\footnote{The unconditional moment condition in \cite{chandrasekhar2011econometrics} is based on the integration of the moment condition $\mathbb{E}(\mathbf{Z}^{(s)\prime}\boldsymbol{\varepsilon}|\mathbf{G})$ over $\mathbf{G}$. See our discussion in REFERENCES"}

To understand the intuition behind the use of the moment function (\ref{eq:moment}), let us replace $\mathbf{y}=(\mathbf{I}-\alpha\mathbf{G})^{-1}(\mathbf{V}\tilde{\boldsymbol{\theta}}+\boldsymbol{\varepsilon})$ in equation (\ref{eq:moment}). In doing so, we can rewrite the term inside the double summation in (\ref{eq:moment}) as a sum of two terms.\footnote{The double summation in (\ref{eq:moment}) is not essential and (\ref{eq:moment}) could be replaced by $\mathbb{E}\frac{1}{S}\sum_{t=1}^T\dot{\mathbf{Z}}^{(s)\prime}(\mathbf{I}-\alpha\dot{\mathbf{G}}^{(s)})\left(\mathbf{y}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}\ddot{\mathbf{V}}^{(s)}\tilde{\boldsymbol{\theta}}\right)=\mathbf{0}$. The efficiency loss in practice could however be important.} First, $\dot{\mathbf{Z}}^{(s)\prime}\boldsymbol{\varepsilon}$, which would be the standard moment condition if $\mathbf{G}$ was observed (e.g. \cite{bramoulle2009identification}), and second: $$ \dot{\mathbf{Z}}^{(s)\prime}(\mathbf{I}-\alpha\dot{\mathbf{G}}^{(s)})\left((\mathbf{I}-\alpha{\mathbf{G}})^{-1}{\mathbf{V}}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}\ddot{\mathbf{V}}^{(t)}\right)\tilde{\boldsymbol{\theta}}.$$
We show that both terms are equal to $0$ in expectation as $N$ grows to $\infty$. For the first term, this is true since the simulated network is exogenous. For the second term, this is true because $\mathbf{G}$, $\dot{\mathbf{G}}$ and $\ddot{\mathbf{G}}$ are asymptotically drawn from the same distribution.

For the special case in which $\mathbf{G}$ is observed, one could substitute $\dot{\mathbf{G}}^{(s)}=\mathbf{G}$ and $\ddot{\mathbf{G}}^{(t)}=\mathbf{G}$ for all $s,t$ and the first term would simply be $\mathbf{Z}'\boldsymbol{\varepsilon}$, while the second term would be exactly equal to $\mathbf{0}$.

Note that Theorem \ref{prop:non_observed} is valid whether or not $\mathbf{Gy}$ and $\mathbf{GX}$ are observed since the moment function (\ref{eq:moment}) does not use information on $\mathbf{Gy}$ or $\mathbf{GX}$. Proposition \ref{prop:GXobs} and Proposition \ref{prop:Gyobs} below present specific moment function that use $\mathbf{Gy}$ or $\mathbf{GX}$, if they are observed.

\begin{proposition}\label{prop:GXobs}
Assume that $\mathbf{GX}$ is observed, but that $\mathbf{Gy}$ is not observed. Let $\lbrace \dot{\mathbf{G}}^{(s)}\rbrace_{s=1}^S$ and $\lbrace \ddot{\mathbf{G}}^{(t)}\rbrace_{t=1}^T$ be two sequences of independent draws from $\hat{P}(\mathbf{G})$. Let $\dot{\mathbf{Z}}^{(s)}=[\mathbf{1},\mathbf{X},{\mathbf{G}}\mathbf{X},\dot{\mathbf{G}}^{s}{\mathbf{G}}\mathbf{X},(\dot{\mathbf{G}}^{(s)})^2{\mathbf{G}}\mathbf{X},...]$,
$\ddot{\mathbf{Z}}^{(s,t)}=[\mathbf{1},\mathbf{X},\ddot{\mathbf{G}}^{(t)}\mathbf{X},\dot{\mathbf{G}}^{s}\ddot{\mathbf{G}}^{(t)}\mathbf{X},(\dot{\mathbf{G}}^{(s)})^2\ddot{\mathbf{G}}^{(t)}\mathbf{X},...]$, $\mathbf{V}=[\mathbf{1},\mathbf{X},\mathbf{G}\mathbf{X}]$, and $\ddot{\mathbf{V}}^{(t)}=[\mathbf{1},\mathbf{X},\ddot{\mathbf{G}}^{(t)}\mathbf{X}]$. Then, the simulated GMM estimator based on
\begin{eqnarray}\label{eq:Gyobs}
\mathbb{E}(\frac{1}{S}\sum_{s=1}^S\dot{\mathbf{Z}}_i^{(s)\prime}(\mathbf{I}-\alpha\dot{\mathbf{G}}^{(s)})_i\mathbf{y} -
\frac{1}{ST}\sum_{t=1}^T\sum_{s=1}^S (\dot{\mathbf{Z}}^{(s)\prime}\mathbf{V}-\ddot{\mathbf{Z}}^{(s,t)\prime}\ddot{\mathbf{V}}^{(t)})_i\tilde{\boldsymbol{\theta}}\nonumber\\ -\frac{1}{ST}\sum_{t=1}^T\sum_{s=1}^S  \ddot{\mathbf{Z}}^{(s,t)\prime}_i(\mathbf{I}-\alpha\dot{\mathbf{G}}^{(s)})_i(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(t)})^{-1}\ddot{\mathbf{V}}^{(t)}\tilde{\boldsymbol{\theta}}) =\mathbf{0}
\end{eqnarray}
is consistent and asymptotically normally distributed with asymptotic variance-covariance matrix defined in ????.
\end{proposition}

\begin{proposition}\label{prop:Gyobs}
Assume that $\mathbf{Gy}$ is observed, but that $\mathbf{GX}$ is not observed. Let $\lbrace \dot{\mathbf{G}}^{(s)}\rbrace_{s=1}^S$ and $\lbrace \ddot{\mathbf{G}}^{(t)}\rbrace_{t=1}^T$ be two sequences of independent draws from $\hat{P}(\mathbf{G})$. Let $\dot{\mathbf{Z}}^{(s)}=[\mathbf{1},\mathbf{X},\dot{\mathbf{G}}^{(s)}\mathbf{X},(\dot{\mathbf{G}}^{(s)})^2\mathbf{X},...]$, and $\ddot{\mathbf{V}}^{(t)}=[\mathbf{1},\mathbf{X},\ddot{\mathbf{G}}^{(t)}\mathbf{X}]$. Then, the simulated GMM estimator based on
\begin{eqnarray}\label{eq:GXobs}
\mathbb{E}(\frac{1}{S}\sum_{s=1}^S\dot{\mathbf{Z}}_i^{(s)\prime}(\mathbf{I}-\alpha\mathbf{G})_i\mathbf{y} -
\frac{1}{ST}\sum_{t=1}^T\sum_{s=1}^S \dot{\mathbf{Z}}^{(s)\prime}_i\ddot{\mathbf{V}}^{(t)}_i\tilde{\boldsymbol{\theta}})=\mathbf{0}
\end{eqnarray}
is consistent and asymptotically normally distributed with asymptotic variance-covariance matrix defined in ????.
\end{proposition}

The logic behind Proposition \ref{prop:GXobs} is exactly the same as the one for Proposition \ref{prop:non_observed}. The objective is to use $\lbrace\dot{\mathbf{G}}^{(s)}\rbrace_{s=1}^S$ and $\lbrace \ddot{\mathbf{G}}^{(t)}\rbrace_{t=1}^T$ in order to write the moment condition as a sum of random variables with the same expected value. As for \ref{prop:non_observed}, if $\mathbf{G}$ was observed, we could substitute $\dot{\mathbf{G}}^{(s)}=\mathbf{G}$ and $\ddot{\mathbf{G}}^{(t)}=\mathbf{G}$ for all $s,t$, and the first summation in the moment condition (\ref{eq:GXobs}) would simply reduce to $\mathbb{E}\mathbf{Z}'\boldsymbol{\varepsilon}$, while the other remaining summations would be exactly $0$.


Proposition \ref{prop:all_observed}, Proposition \ref{prop:non_observed} and \ref{prop:GXobs} therefore show that the estimation of (\ref{eq:linearinmean}) is possible, even with very limited information about the network structure. In Section \ref{sec:ard}, we study the finite sample properties of our approach using network formation models estimated on aggregated relational data (\cite{breza2017using}; see Example \ref{ex:ard}). Before, however, we briefly discuss how one can adapt this estimation strategy while allowing for group-level unobservables.

Indeed, a common assumption is that each group in the population is affected by a common shock, unobserved by the econometrician (e.g. \cite{bramoulle2009identification}). As such, for each group $r=1,...,M$, we have: $\mathbf{y}_r=c_r\mathbf{1}_r+\mathbf{X}_r\boldsymbol{\beta}+\alpha\mathbf{G}_r\mathbf{y}_r+{\mathbf{G}_r\mathbf{X}_r}\boldsymbol{\gamma}+\boldsymbol{\varepsilon}_r$, where $c_r$ is not observed, $\mathbf{1}_r$ is an $N_r$-dimensional vector of ones, $N_r$ is the size of the group r, $\bG_r$ is the subinteraction matrix in the group r, and $\bepsilon_r$ is the vector of error terms in the group r.

Under Assumption \ref{as:manymarkets}, it is not possible to obtain a consistent estimator of $\{c_r\}_{r=1}^m$ because the number of observations used to estimate each $c_r$ is bounded. This is known as the \emph{incidental parameter problem}.\footnote{See \cite{lancaster2000incidental} for a review.} A common strategy is to use deviations from the group average and estimate the model in deviations (e.g. \cite{bramoulle2009identification}).

Let $\mathbf{J}=diag\{\mathbf{I}_{N_r}-\frac{1}{N_r}\mathbf{1}_r\mathbf{1}'_r\}$ be the group-differentiating matrix, where $\mathbf{I}_{N_r}$ is the identified matrix of dimension $N_r$. The operator \emph{diag} generates a blog-diagonal matrix in which each group is a block.\footnote{Then, $\mathbf{Jw}$ gives $\mathbf{w}$ minus the group average of $\mathbf{w}$.} We can rewrite: $\mathbf{Jy}=\mathbf{JX}\boldsymbol{\beta}+\alpha{\mathbf{JG}\mathbf{y}}+{\mathbf{JGX}}\boldsymbol{\gamma}+\boldsymbol{J\varepsilon}$. Note that the results of Propositions \ref{prop:all_observed}--\ref{prop:GXobs} extend directly, using instruments in deviation with the group average.

\subsection{Finite Sample Performance Using ARD}\label{sec:ard}
In this section, we study the small sample performance of the estimator presented in Section \ref{sec:iv} when the researcher only has access to ARD (as in Example \ref{ex:ard}). First, we simulate network data using the model proposed by \cite{breza2017using} and simulate outcomes using the linear in means model (\ref{eq:linearinmean}) conditional on the simulated networks. Second, we estimate the network formation model using the Bayesian estimator proposed by \cite{breza2017using} (yielding $\hat{\boldsymbol{\rho}}_B$), as well as using the classical estimator proposed by \cite{alidaee2020recovering} (yielding $\hat{\boldsymbol{\rho}}_A$). Third, we estimate the linear-in-means model, using our IV estimator based on $\hat{\boldsymbol{\rho}}_A$ and $\hat{\boldsymbol{\rho}}_B$.

Recall that
\begin{equation}\label{eq:ard}
P(a_{ij}=1)\propto\exp\{\nu_i+\nu_j+\zeta \mathbf{z}_i'\mathbf{z}_j\},    
\end{equation}
where $\nu_i$, $\nu_j$, $\zeta$, $\mathbf{z}_i$, and $\mathbf{z}_j$ are not observed by the econometrician but follow parametric distributions. We refer the interested reader to \cite{mccormick2015latent}, \cite{breza2017using}, and \cite{breza2019consistently} for a formal discussion of the model, including its identification and consistent estimation. Here, we discuss the intuition using a simple analogy.

Suppose that individuals are located according to their geographical position on Earth. Suppose also that there are a fixed number of cities on Earth in which individuals can live. The econometrician does not know the individuals' locations on Earth nor do they know the location of the cities. In model (\ref{eq:ard}), $\mathbf{z}_i$ represent $i$'s position on Earth. However, the econometrician has access to ARD for a subset of the population, i.e. answers to questions such as, ``How many of your friends live in city $A$?''

To understand the intuition behind the identification of the model, consider the following example: suppose that individual $i$ has many friends living in city $A$. Then, city $A$ is likely located close to $i$'s location. Similarly, if many individuals have many friends living in city $A$, then city $A$ is likely a large city. Finally, if $i$ has many friends from many cities, $i$ likely has a large $\nu_i$.

To study the finite sample performance of our instrumental strategy in this context, we simulate 20 groups of 250 individuals each. Within each subpopulation, we simulate the ARD responses as well as a series of observable characteristics (e.g. cities). The details of the Monte Carlo simulations can be found in Appendix \ref{sec:ardsetting}.

Importantly, the model in (\ref{eq:ard}) is based on a single population framework. Thus, the network formation model must be estimated separately for each of the 20 groups. With only 250 individuals in each group, we therefore expect significant small-sample bias.

We contrast the estimator proposed by \cite{breza2017using} with the one proposed by \cite{alidaee2020recovering}. Whereas \cite{breza2017using} present a parametric Bayesian estimator, \cite{alidaee2020recovering} propose a (nonparametric) penalized regression based on a low-rank assumption. One main advantage of their estimator is that it allows for a wider class of model and ensures that the estimation is fast and easily implementable.\footnote{The authors developed user-friendly packages in R and Python. See their paper for links and details.} Note, however, that their method only yields a consistent estimator of $\hat{P}(\mathbf{A})$ if the true network is effectively low rank.

Very intuitively, the low-rank assumption implies that linking probabilities were generated from a small number of parameters; for example, in the example above, knowing individuals' gregariousness parameters $\nu_i$ and city in which they live would allow a prediction of the linking probabilities.

Importantly, the model (\ref{eq:ard}) is not necessarily low rank; for example, if the individuals' locations on Earth (i.e. the $\mathbf{z}_i$'s) are uniformly distributed and there are only very few  large cities, then the model produced is not low rank and the method proposed by \cite{alidaee2020recovering} performs poorly. Intuitively, in such a case, the fact that individual $i$ lives in city $A$ poorly explains the linking probabilities. 

We compare the performance of both estimators as we vary the concentration parameter for the individuals' locations on Earth (that is, $\kappa$, see Appendix \ref{sec:ardsetting} for details). This has the effect of changing the \emph{effective rank} of the linking probabilities: increasing $\kappa$ decreases the effective rank.\footnote{We refer the interested reader to \cite{alidaee2020recovering} for a formal discussion of the effective rank and of its importance for their estimator.} We therefore expect the estimator proposed by \cite{alidaee2020recovering} to perform better for larger values of $\kappa$.

Results are presented in Tables \ref{tab:breza} and \ref{tab:alidaee}. When $\mathbf{Gy}$ is observed, both estimators perform extremely well. In light of Propositions \ref{prop:gamma0} and \ref{prop:gammanot0}, this is expected, as the IV estimator is valid even under misspecification. When $\mathbf{Gy}$ is not observed, results are more nuanced. First, note that for all specifications, the introduction of the non-pertinent variables $\ddot{\mathbf{G}}\mathbf{X}$ contaminates the estimation of $\boldsymbol{\gamma}$. This occurs because ${\mathbf{G}}\mathbf{X}$ and $\ddot{\mathbf{G}}\mathbf{X}$ are highly correlated.\footnote{This is a small sample issue which is not due to the assumed network formation model and would arise even if the linking probabilities were known (instead of being estimated).} Note, however, that the estimated values for $\boldsymbol{\gamma}+\check{\boldsymbol{\gamma}}$ are centered on the true value. Second, the bias of the estimated endogenous peer effect (i.e. $\alpha$) goes to zero when the linking probabilities are of lower rank, with an advantage for the estimator proposed by  \cite{breza2017using}. This is expected because the model is correctly specified and the estimator is parametric. 

Overall, our IV estimator can be successfully implemented in small samples, using either the estimator proposed by \cite{breza2017using} or by \cite{alidaee2020recovering}, both of which only rely on the observation of ARD.

\renewcommand{\arraystretch}{.9}
\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD - network distribution estimated following \cite{breza2017using} } 
\label{tab:breza}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}d{4}d{4}d{4}d{4}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 0$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1ex]                                             
$\alpha=0.4$    & 0.400  & 0.007 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$                & 5.000  & 0.021 & 4.986   & 5.000  & 5.014   \\
$\gamma_2=-3$              & -3.001 & 0.031 & -3.021  & -3.000 & -2.980  \\  
F-test (Weak inst.) & 3144.574&	874.400&	2492.881&	3075.955&	3672.449 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                                          
$\alpha=0.4$ & 0.371  & 0.013 & 0.363   & 0.372  & 0.380   \\
$\gamma_1=5$            & 5.396  & 0.021 & 5.383   & 5.397  & 5.410   \\
$\gamma_2=-3$          & -2.400 & 0.041 & -2.428  & -2.400 & -2.371  \\
$\hat{\gamma}_1=0$          & -0.380 & 0.028 & -0.400  & -0.382 & -0.362  \\
$\hat{\gamma}_2=0$           & -0.553 & 0.044 & -0.584  & -0.551 & -0.525  \\
F-test (Weak inst.) & 3193.940&	760.793&	2642.815&	3153.048&	3666.220 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 10$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                                              
$\alpha=0.4$   & 0.400  & 0.006 & 0.396   & 0.400  & 0.404   \\
$\gamma_1=5$                & 5.001  & 0.019 & 4.988   & 5.001  & 5.014   \\
$\gamma_2=-3$             & -3.000 & 0.031 & -3.020  & -3.000 & -2.978  \\
F-test (Weak inst.) & 5905.596&	1876.836&	4519.460&	5766.601&	7158.739 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                                          
$\alpha=0.4$ & 0.400  & 0.007 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$            & 5.392  & 0.019 & 5.379   & 5.393  & 5.405   \\
$\gamma_2=-3$          & -2.397 & 0.037 & -2.421  & -2.398 & -2.373  \\
$\hat{\gamma}_1=0$           & -0.391 & 0.022 & -0.405  & -0.390 & -0.375  \\
$\hat{\gamma}_2=0$          & -0.604 & 0.038 & -0.630  & -0.605 & -0.579  \\
F-test (Weak inst.) & 5176.649&	1507.532&	4058.393&	5087.275&	6243.500 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 20$, $N=250$, $M=20$}                                                            \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                                             
$\alpha=0.4$    & 0.400  & 0.006 & 0.396   & 0.400  & 0.404   \\
$\gamma_1=5$                & 5.000  & 0.020 & 4.986   & 4.999  & 5.013   \\
$\gamma_2=-3$            & -3.001 & 0.031 & -3.021  & -3.001 & -2.981  \\
F-test (Weak inst.) &6104.999&	1927.633&	4734.460&	5937.815&	7246.355 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]   
$\alpha=0.4$ & 0.400  & 0.007 & 0.396   & 0.400  & 0.405   \\
$\gamma_1=5$            & 5.390  & 0.019 & 5.377   & 5.390  & 5.403   \\
$\gamma_2=-3$          & -2.398 & 0.036 & -2.422  & -2.398 & -2.375  \\
$\hat{\gamma}_1=0$           & -0.390 & 0.022 & -0.405  & -0.390 & -0.376  \\
$\hat{\gamma}_2=0$          & -0.604 & 0.036 & -0.628  & -0.604 & -0.579 \\ 
F-test (Weak inst.) & 5321.702&	1524.973&	4272.790&	5199.232&	6235.250 \\ 
\hline \\[-1.8ex] 


\multicolumn{6}{l}{%
  \begin{minipage}{15cm}%
    \footnotesize{Note: In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with a location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in Appendix \ref{sec:ardsetting}. Predicted probabilities are computed using the mean of the posterior distribution. F-test is the Fisher-statistic of the Weak instruments test. We do not report the estimated values for $c$ and $\boldsymbol{\beta}$ to keep the table readable, but they are available upon request. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.}
  \end{minipage}%
}\end{tabular}
\end{table}

\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD - network distribution estimated following \cite{alidaee2020recovering} } 
\label{tab:alidaee}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}d{4}d{4}d{4}d{4}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 0$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1ex]                                
$\alpha=0.4$     & 0.400  & 0.012 & 0.393   & 0.400  & 0.407   \\
$\gamma_1=5$             & 5.000  & 0.029 & 4.980   & 4.999  & 5.019   \\
$\gamma_2=-3$             & -3.000 & 0.032 & -3.021  & -3.000 & -2.978  \\
F-test (Weak inst.) & 798.971&	340.558&	560.817&	749.132&	990.407\\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                          
$\alpha=0.4$ & 0.371  & 0.024 & 0.357   & 0.373  & 0.387   \\
$\gamma_1=5$              & 5.504  & 0.036 & 5.479   & 5.503  & 5.528   \\
$\gamma_2=-3$            & -2.480 & 0.057 & -2.517  & -2.480 & -2.441  \\
$\hat{\gamma}_1=0$           & -0.364 & 0.031 & -0.385  & -0.363 & -0.344  \\
$\hat{\gamma}_2=0$          & -0.302 & 0.070 & -0.349  & -0.304 & -0.254  \\
F-test (Weak inst.) & 590.248&	253.853&	409.497&	572.210&	721.788 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 10$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                              
$\alpha=0.4$    & 0.400  & 0.009 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$         & 4.999  & 0.022 & 4.985   & 4.999  & 5.014   \\
$\gamma_2=-3$                & -3.000 & 0.032 & -3.022  & -3.001 & -2.978 \\
F-test (Weak inst.) & 1697.514&	741.478&	1179.079&	1593.284&	2127.582\\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                          
$\alpha=0.4$  & 0.395  & 0.021 & 0.388   & 0.397  & 0.405   \\
$\gamma_1=5$            & 5.396  & 0.027 & 5.378   & 5.394  & 5.412   \\
$\gamma_2=-3$            & -2.412 & 0.045 & -2.439  & -2.410 & -2.383  \\
$\hat{\gamma}_1=0$          & -0.385 & 0.032 & -0.404  & -0.387 & -0.370  \\
$\hat{\gamma}_2=0$           & -0.462 & 0.117 & -0.534  & -0.483 & -0.414  \\
F-test (Weak inst.) &1303.291&	586.429&	895.070&	1227.426&	1652.148\\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 20$, $N=250$, $M=20$}                                                            \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                              
$\alpha=0.4$     & 0.400  & 0.008 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$                & 5.000  & 0.021 & 4.985   & 5.000  & 5.013   \\
$\gamma_2=-3$             & -2.999 & 0.032 & -3.020  & -2.999 & -2.979   \\
F-test (Weak inst.) & 2685.354&	978.512&	1998.396&	2601.996&	3268.714 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]   
$\alpha=0.4$ & 0.399  & 0.010 & 0.393   & 0.400  & 0.406   \\
$\gamma_1=5$        & 5.391  & 0.020 & 5.378   & 5.391  & 5.404   \\
$\gamma_2=-3$             & -2.400 & 0.039 & -2.425  & -2.400 & -2.374  \\
$\hat{\gamma}_1=0$           & -0.391 & 0.022 & -0.406  & -0.391 & -0.376  \\
$\hat{\gamma}_2=0$          & -0.573 & 0.047 & -0.605  & -0.575 & -0.544 \\ 
F-test (Weak inst.) & 2191.313&	774.366&	1656.355&	2130.681&	2668.781\\ 
\hline \\[-1.8ex] 



\multicolumn{6}{l}{%
  \begin{minipage}{15cm}%
    \footnotesize{Note: In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in Appendix \ref{sec:ardsetting}. We chose the weight associated with the nuclear norm penalty to minimize the RMSE through cross-validation. This value of $\lambda=600$ is smaller than the recommended value in \cite{alidaee2020recovering}. F-test is the Fisher-statistic of the Weak instruments test. We do not report the estimated values for $c$ and $\boldsymbol{\beta}$ to keep the table readable, but they are available upon request. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.}
  \end{minipage}%
}\end{tabular}
\end{table}
\renewcommand{\arraystretch}{1}

==> archives/shortversion/bkp/iv_old_last.tex <==


\section{Estimation Using Instrumental Variables}\label{sec:iv}

We now present our instrumental variable strategy. To understand the underlying intuition, note that it is not necessary to observe the complete network structure to observe $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$. For example, one could simply obtain ${\mathbf{Gy}}$ from survey data, ``What is the average value of your friends' $y$?''

However, even observing $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$, the model (\ref{eq:linearinmean}) cannot be simply estimated using simple linear regression. The reason is that ${\mathbf{Gy}}$ is endogenous; thus, a linear regression would produce biased estimates (e.g. \cite{manski1993identification}, \cite{bramoulle2009identification}).

The typical instrumental approach to deal with this endogeneity is to use instruments based on the structural model, i.e. instruments constructed using second-degree peers (e.g. $\mathbf{G}^2\mathbf{X}$, see \cite{bramoulle2009identification}). These are less likely to be found in survey data. Indeed, we could doubt the informativeness of questions such as, ``What is the average value of your friends' average value of their friends' $x$?''

Propositions \ref{prop:gamma0} and \ref{prop:gammanot0} describe how to construct valid instruments when the researcher observes  $\mathbf{y}$, $\mathbf{X}$, and ${\mathbf{GX}}$. To clearly expose the argument, we first start by discussing the special case where there are no contextual effects: $\boldsymbol{\gamma}=\mathbf{0}$. The model in (\ref{eq:linearinmean}) can therefore be rewritten as: 
$$
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\mathbf{Gy}+\boldsymbol{\varepsilon}.
$$
The following proposition holds.\footnote{Proofs of Propositions \ref{prop:gamma0} and \ref{prop:gammanot0} can be found in Appendix \ref{sec:appendix_proofs}.}
\begin{proposition}\label{prop:gamma0}
Assume that $\boldsymbol{\gamma}=\mathbf{0}$. There are two cases:\begin{enumerate}
\item Suppose that $\mathbf{Gy}$ is observed and let $\boldsymbol{H}$ be an interaction matrix, correlated with $\mathbf{G}$, and such that $\mathbb{E}[\boldsymbol{\varepsilon}|\mathbf{X},\mathbf{H}]=\mathbf{0}$. Then, $\mathbf{H}\mathbf{X}$, $\mathbf{H}^2\mathbf{X}$,... are valid instruments.
\item Suppose that $\mathbf{Gy}$ \emph{is not} observed and let $\dot{\mathbf{G}}$ and $\ddot{\mathbf{G}}$ be two independent draws from the distribution $\hat{P}(\mathbf{G})$. Then, $\dot{\mathbf{G}}\mathbf{X}$, $\dot{\mathbf{G}}^2\mathbf{X}$,... are valid instruments when $\ddot{\mathbf{G}}\mathbf{y}$ is used as a proxy for $\mathbf{Gy}$, as $N\rightarrow\infty$.
\end{enumerate}
\end{proposition}

First, suppose that $\mathbf{Gy}$ is observed directly from the data. Then, any instrument correlated with the usual instruments $\mathbf{GX},\mathbf{G}^2\mathbf{X}$,..., while being exogenous, are valid. Note that a special case of the first part of Proposition \ref{prop:gamma0} is when $\mathbf{H}$ is drawn from $\hat{P}(\mathbf{G})$. However, the instrument remains valid if the researcher uses a \emph{mispecified} estimator of the distribution ${P}(\mathbf{G})$.\footnote{We would like to thank Chih-Sheng Hsieh and Arthur Lewbel for discussions on this important point.} A similar strategy is used by \cite{kelejian2014estimation} and \cite{lee2020key} in a different context. Of course, the specification error on $P(\mathbf{G})$ must be independent of $\boldsymbol{\varepsilon}$. In Section \ref{sec:ard}, we discuss the importance of this robustness feature in a context in which the network formation process could be misspecified or subject to small sample biases.\footnote{Note, however, that if the specification error is too large, the correlation between $\mathbf{Gy}$ and $\mathbf{H}\mathbf{X}$ will likely be small, leading to a problem of weak instruments. It is also worth noting that the first part of Proposition \ref{prop:gamma0} does not depend on the assumption that groups are entirely sampled (i.e. Assumption \ref{as:nosampling}).}

When $\mathbf{Gy}$ is \emph{not} observed directly, however, specification errors typically produce invalid instruments. As stated in Part 2 of Proposition \ref{prop:gamma0}, the estimation also requires two independent draws from $\hat{P}(\mathbf{G})$ instead of just one. To see why, let us rewrite the model as:
$$
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\ddot{\mathbf{G}}\mathbf{y}+[\boldsymbol{\eta}+\boldsymbol{\varepsilon}],
$$
where $\boldsymbol{\eta}=\alpha[\mathbf{G}\mathbf{y}-\ddot{\mathbf{G}}\mathbf{y}]$ is the error due to the approximation of $\mathbf{Gy}$. Suppose also that $\dot{\mathbf{G}}\mathbf{X}$ is used as an instrument for $\mathbf{Gy}$.

The validity of the instrument therefore requires $\mathbb{E}[\boldsymbol{\eta}+\boldsymbol{\varepsilon}|\mathbf{X},\dot{\mathbf{G}}\mathbf{X}]=0$, and in particular: $$\mathbb{E}[\mathbf{G}\mathbf{y}|\mathbf{X},\dot{\mathbf{G}}\mathbf{X}]=\mathbb{E}[\ddot{\mathbf{G}}\mathbf{y}|\mathbf{X},\dot{\mathbf{G}}\mathbf{X}],$$
which is true since $\mathbf{G}$ and $\ddot{\mathbf{G}}$ have the same asymptotic distribution.

Of course, Proposition \ref{prop:gamma0} assumes that there are no contextual effects. We show that a similar result holds when $\boldsymbol{\gamma}\neq \mathbf{0}$. To estimate (\ref{eq:linearinmean}) using an instrumental variable approach, however, we must assume that ${\mathbf{GX}}$ are \emph{observed}. The reason is that there are no natural, strong instruments for ${\mathbf{GX}}$.\footnote{Indeed, the strengths of the instruments in Proposition \ref{prop:gamma0} come from the fact that $\mathbf{GX}$ are strong instruments for $\mathbf{Gy}$ when $\mathbf{G}$ is observed. Proxying $\mathbf{GX}$ with $\ddot{\mathbf{G}}\mathbf{X}$ and instrumenting with $\dot{\mathbf{G}}\mathbf{X}$ would be valid. However, the explanatory power of $\dot{\mathbf{G}}\mathbf{X}$, conditional on $\ddot{\mathbf{G}}\mathbf{X}$, would be much too weak to be of any practical use.} In Section \ref{sec:genestim}, we present an alternative estimation strategy that does not require the observation of $\mathbf{GX}$.

\begin{proposition}\label{prop:gammanot0}
Assume that $\mathbf{GX}$ are observed. There are two cases:\begin{enumerate}
\item Suppose that $\mathbf{Gy}$ is observed and let $\boldsymbol{H}$ be an interaction matrix, correlated with $\mathbf{G}$, and such that $\mathbb{E}[\boldsymbol{\varepsilon}|\mathbf{X},\mathbf{H}]=\mathbf{0}$. Then, $\mathbf{H}^2\mathbf{X}$, $\mathbf{H}^3\mathbf{X}$,... are valid instruments.
\item Suppose that $\mathbf{Gy}$ \emph{is not} observed and let $\dot{\mathbf{G}}$ and $\ddot{\mathbf{G}}$ be two independent draws from the distribution $\hat{P}(\mathbf{G})$. Then, $\dot{\mathbf{G}}^2\mathbf{X}$, $\dot{\mathbf{G}}^3\mathbf{X}$,... are valid instruments when $\ddot{\mathbf{G}}\mathbf{y}$ is used as a proxy for $\mathbf{Gy}$, if $\ddot{\mathbf{G}}\mathbf{X}$ are added as additional explanatory variables and as $N\rightarrow\infty$.
\end{enumerate}
\end{proposition}
The first part of Proposition \ref{prop:gammanot0} is a simple extension of the first part of Proposition \ref{prop:gamma0}. The second part of Proposition \ref{prop:gammanot0} requires more discussion. Essentially, it states that $\dot{\mathbf{G}}^2\mathbf{X}$, $\dot{\mathbf{G}}^3\mathbf{X}$, ... are valid instruments when the following \emph{expanded model} is estimated:
\begin{equation}\label{eq:expanded}
    \mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha{\ddot{\mathbf{G}}\mathbf{y}}+{\mathbf{GX}}\boldsymbol{\gamma}+\ddot{\mathbf{G}}\mathbf{X}\check{\boldsymbol{\gamma}}+\boldsymbol{\eta}+\boldsymbol{\varepsilon},
\end{equation}
where the true value of $\check{\boldsymbol{\gamma}}$ is $\mathbf{0}$.

To understand why the introduction of $\ddpt{\mathbf{G}}\mathbf{X}\check{\boldsymbol{\gamma}}$ is needed, recall that the constructed instrument must be uncorrelated with the approximation error $\boldsymbol{\eta}$. This correlation is conditional on the explanatory variables, which contain $\mathbf{G}$. In particular, it implies that generically, $$\mathbb{E}[\mathbf{G}\mathbf{y}|\mathbf{X},\mathbf{GX},\dot{\mathbf{G}}^2\mathbf{X}]\neq\mathbb{E}[\ddot{\mathbf{G}}\mathbf{y}|\mathbf{X},\mathbf{GX},\dot{\mathbf{G}}^2\mathbf{X}].$$

However, adding the auxiliary variable $\ddot{\mathbf{G}}\mathbf{X}$ as a covariate is sufficient to restore the result, i.e. as $N\rightarrow\infty$: $$\mathbb{E}[\mathbf{G}\mathbf{y}|\mathbf{X},\mathbf{GX},\dot{\mathbf{G}}^2\mathbf{X}, \ddot{\mathbf{G}}\mathbf{X}]=\mathbb{E}[\ddot{\mathbf{G}}\mathbf{y}|\mathbf{X},\mathbf{GX},\dot{\mathbf{G}}^2\mathbf{X}, \ddot{\mathbf{G}}\mathbf{X}].$$


Proposition \ref{prop:gamma0} and Proposition \ref{prop:gammanot0} therefore show that the estimation of (\ref{eq:linearinmean}) is possible, even with very limited information about the network structure. Note, however, that the validity of the constructed instruments only holds asymptotically. In Section \ref{sec:ard}, we study the finite sample properties of our approach using network formation models estimated on aggregated relational data (\cite{breza2017using}; see Example \ref{ex:ard}). Before, however, we briefly discuss how one can adapt this estimation strategy while allowing for group-level unobservables.

Indeed, a common assumption is that each group in the population is affected by a common shock, unobserved by the econometrician (e.g. \cite{bramoulle2009identification}). As such, for each group $r=1,...,M$, we have: $\mathbf{y}_r=c_r\mathbf{1}_r+\mathbf{X}_r\boldsymbol{\beta}+\alpha\mathbf{G}_r\mathbf{y}_r+{\mathbf{G}_r\mathbf{X}_r}\boldsymbol{\gamma}+\boldsymbol{\varepsilon}_r$, where $c_r$ is not observed, $\mathbf{1}_r$ is an $N_r$-dimensional vector of ones, $N_r$ is the size of the group r, $\bG_r$ is the subinteraction matrix in the group r, and $\bepsilon_r$ is the vector of error terms in the group r.

Under Assumption \ref{as:manymarkets}, it is not possible to obtain a consistent estimator of $\{c_r\}_{r=1}^m$ because the number of observations used to estimate each $c_r$ is bounded. This is known as the \emph{incidental parameter problem}.\footnote{See \cite{lancaster2000incidental} for a review.} A common strategy is to use deviations from the group average and estimate the model in deviations (e.g. \cite{bramoulle2009identification}).

Let $\mathbf{J}=diag\{\mathbf{I}_{N_r}-\frac{1}{N_r}\mathbf{1}_r\mathbf{1}'_r\}$ be the group-differentiating matrix, where $\mathbf{I}_{N_r}$ is the identified matrix of dimension $N_r$. The operator \emph{diag} generates a blog-diagonal matrix in which each group is a block.\footnote{Then, $\mathbf{Jw}$ gives $\mathbf{w}$ minus the group average of $\mathbf{w}$.} We can rewrite: $\mathbf{Jy}=\mathbf{JX}\boldsymbol{\beta}+\alpha{\mathbf{JG}\mathbf{y}}+{\mathbf{JGX}}\boldsymbol{\gamma}+\boldsymbol{J\varepsilon}$. Note that the results of Propositions \ref{prop:gamma0} and \ref{prop:gammanot0} extend directly, using instruments in deviation with the group average.

\subsection{Finite Sample Performance Using ARD}\label{sec:ard}
In this section, we study the small sample performance of the estimator presented in Section \ref{sec:iv} when the researcher only has access to ARD (as in Example \ref{ex:ard}). First, we simulate network data using the model proposed by \cite{breza2017using} and simulate outcomes using the linear in means model (\ref{eq:linearinmean}) conditional on the simulated networks. Second, we estimate the network formation model using the Bayesian estimator proposed by \cite{breza2017using} (yielding $\hat{\boldsymbol{\rho}}_B$), as well as using the classical estimator proposed by \cite{alidaee2020recovering} (yielding $\hat{\boldsymbol{\rho}}_A$). Third, we estimate the linear-in-means model, using our IV estimator based on $\hat{\boldsymbol{\rho}}_A$ and $\hat{\boldsymbol{\rho}}_B$.

Recall that
\begin{equation}\label{eq:ard}
P(a_{ij}=1)\propto\exp\{\nu_i+\nu_j+\zeta \mathbf{z}_i'\mathbf{z}_j\},    
\end{equation}
where $\nu_i$, $\nu_j$, $\zeta$, $\mathbf{z}_i$, and $\mathbf{z}_j$ are not observed by the econometrician but follow parametric distributions. We refer the interested reader to \cite{mccormick2015latent}, \cite{breza2017using}, and \cite{breza2019consistently} for a formal discussion of the model, including its identification and consistent estimation. Here, we discuss the intuition using a simple analogy.

Suppose that individuals are located according to their geographical position on Earth. Suppose also that there are a fixed number of cities on Earth in which individuals can live. The econometrician does not know the individuals' locations on Earth nor do they know the location of the cities. In model (\ref{eq:ard}), $\mathbf{z}_i$ represent $i$'s position on Earth. However, the econometrician has access to ARD for a subset of the population, i.e. answers to questions such as, ``How many of your friends live in city $A$?''

To understand the intuition behind the identification of the model, consider the following example: suppose that individual $i$ has many friends living in city $A$. Then, city $A$ is likely located close to $i$'s location. Similarly, if many individuals have many friends living in city $A$, then city $A$ is likely a large city. Finally, if $i$ has many friends from many cities, $i$ likely has a large $\nu_i$.

To study the finite sample performance of our instrumental strategy in this context, we simulate 20 groups of 250 individuals each. Within each subpopulation, we simulate the ARD responses as well as a series of observable characteristics (e.g. cities). The details of the Monte Carlo simulations can be found in Appendix \ref{sec:ardsetting}.

Importantly, the model in (\ref{eq:ard}) is based on a single population framework. Thus, the network formation model must be estimated separately for each of the 20 groups. With only 250 individuals in each group, we therefore expect significant small-sample bias.

We contrast the estimator proposed by \cite{breza2017using} with the one proposed by \cite{alidaee2020recovering}. Whereas \cite{breza2017using} present a parametric Bayesian estimator, \cite{alidaee2020recovering} propose a (nonparametric) penalized regression based on a low-rank assumption. One main advantage of their estimator is that it allows for a wider class of model and ensures that the estimation is fast and easily implementable.\footnote{The authors developed user-friendly packages in R and Python. See their paper for links and details.} Note, however, that their method only yields a consistent estimator of $\hat{P}(\mathbf{A})$ if the true network is effectively low rank.

Very intuitively, the low-rank assumption implies that linking probabilities were generated from a small number of parameters; for example, in the example above, knowing individuals' gregariousness parameters $\nu_i$ and city in which they live would allow a prediction of the linking probabilities.

Importantly, the model (\ref{eq:ard}) is not necessarily low rank; for example, if the individuals' locations on Earth (i.e. the $\mathbf{z}_i$'s) are uniformly distributed and there are only very few  large cities, then the model produced is not low rank and the method proposed by \cite{alidaee2020recovering} performs poorly. Intuitively, in such a case, the fact that individual $i$ lives in city $A$ poorly explains the linking probabilities. 

We compare the performance of both estimators as we vary the concentration parameter for the individuals' locations on Earth (that is, $\kappa$, see Appendix \ref{sec:ardsetting} for details). This has the effect of changing the \emph{effective rank} of the linking probabilities: increasing $\kappa$ decreases the effective rank.\footnote{We refer the interested reader to \cite{alidaee2020recovering} for a formal discussion of the effective rank and of its importance for their estimator.} We therefore expect the estimator proposed by \cite{alidaee2020recovering} to perform better for larger values of $\kappa$.

Results are presented in Tables \ref{tab:breza} and \ref{tab:alidaee}. When $\mathbf{Gy}$ is observed, both estimators perform extremely well. In light of Propositions \ref{prop:gamma0} and \ref{prop:gammanot0}, this is expected, as the IV estimator is valid even under misspecification. When $\mathbf{Gy}$ is not observed, results are more nuanced. First, note that for all specifications, the introduction of the non-pertinent variables $\ddot{\mathbf{G}}\mathbf{X}$ contaminates the estimation of $\boldsymbol{\gamma}$. This occurs because ${\mathbf{G}}\mathbf{X}$ and $\ddot{\mathbf{G}}\mathbf{X}$ are highly correlated.\footnote{This is a small sample issue which is not due to the assumed network formation model and would arise even if the linking probabilities were known (instead of being estimated).} Note, however, that the estimated values for $\boldsymbol{\gamma}+\check{\boldsymbol{\gamma}}$ are centered on the true value. Second, the bias of the estimated endogenous peer effect (i.e. $\alpha$) goes to zero when the linking probabilities are of lower rank, with an advantage for the estimator proposed by  \cite{breza2017using}. This is expected because the model is correctly specified and the estimator is parametric. 

Overall, our IV estimator can be successfully implemented in small samples, using either the estimator proposed by \cite{breza2017using} or by \cite{alidaee2020recovering}, both of which only rely on the observation of ARD.

\renewcommand{\arraystretch}{.9}
\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD - network distribution estimated following \cite{breza2017using} } 
\label{tab:breza}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}d{4}d{4}d{4}d{4}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 0$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1ex]                                             
$\alpha=0.4$    & 0.400  & 0.007 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$                & 5.000  & 0.021 & 4.986   & 5.000  & 5.014   \\
$\gamma_2=-3$              & -3.001 & 0.031 & -3.021  & -3.000 & -2.980  \\  
F-test (Weak inst.) & 3144.574&	874.400&	2492.881&	3075.955&	3672.449 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                                          
$\alpha=0.4$ & 0.371  & 0.013 & 0.363   & 0.372  & 0.380   \\
$\gamma_1=5$            & 5.396  & 0.021 & 5.383   & 5.397  & 5.410   \\
$\gamma_2=-3$          & -2.400 & 0.041 & -2.428  & -2.400 & -2.371  \\
$\hat{\gamma}_1=0$          & -0.380 & 0.028 & -0.400  & -0.382 & -0.362  \\
$\hat{\gamma}_2=0$           & -0.553 & 0.044 & -0.584  & -0.551 & -0.525  \\
F-test (Weak inst.) & 3193.940&	760.793&	2642.815&	3153.048&	3666.220 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 10$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                                              
$\alpha=0.4$   & 0.400  & 0.006 & 0.396   & 0.400  & 0.404   \\
$\gamma_1=5$                & 5.001  & 0.019 & 4.988   & 5.001  & 5.014   \\
$\gamma_2=-3$             & -3.000 & 0.031 & -3.020  & -3.000 & -2.978  \\
F-test (Weak inst.) & 5905.596&	1876.836&	4519.460&	5766.601&	7158.739 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                                          
$\alpha=0.4$ & 0.400  & 0.007 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$            & 5.392  & 0.019 & 5.379   & 5.393  & 5.405   \\
$\gamma_2=-3$          & -2.397 & 0.037 & -2.421  & -2.398 & -2.373  \\
$\hat{\gamma}_1=0$           & -0.391 & 0.022 & -0.405  & -0.390 & -0.375  \\
$\hat{\gamma}_2=0$          & -0.604 & 0.038 & -0.630  & -0.605 & -0.579  \\
F-test (Weak inst.) & 5176.649&	1507.532&	4058.393&	5087.275&	6243.500 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 20$, $N=250$, $M=20$}                                                            \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                                             
$\alpha=0.4$    & 0.400  & 0.006 & 0.396   & 0.400  & 0.404   \\
$\gamma_1=5$                & 5.000  & 0.020 & 4.986   & 4.999  & 5.013   \\
$\gamma_2=-3$            & -3.001 & 0.031 & -3.021  & -3.001 & -2.981  \\
F-test (Weak inst.) &6104.999&	1927.633&	4734.460&	5937.815&	7246.355 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]   
$\alpha=0.4$ & 0.400  & 0.007 & 0.396   & 0.400  & 0.405   \\
$\gamma_1=5$            & 5.390  & 0.019 & 5.377   & 5.390  & 5.403   \\
$\gamma_2=-3$          & -2.398 & 0.036 & -2.422  & -2.398 & -2.375  \\
$\hat{\gamma}_1=0$           & -0.390 & 0.022 & -0.405  & -0.390 & -0.376  \\
$\hat{\gamma}_2=0$          & -0.604 & 0.036 & -0.628  & -0.604 & -0.579 \\ 
F-test (Weak inst.) & 5321.702&	1524.973&	4272.790&	5199.232&	6235.250 \\ 
\hline \\[-1.8ex] 


\multicolumn{6}{l}{%
  \begin{minipage}{15cm}%
    \footnotesize{Note: In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with a location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in Appendix \ref{sec:ardsetting}. Predicted probabilities are computed using the mean of the posterior distribution. F-test is the Fisher-statistic of the Weak instruments test. We do not report the estimated values for $c$ and $\boldsymbol{\beta}$ to keep the table readable, but they are available upon request. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.}
  \end{minipage}%
}\end{tabular}
\end{table}

\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD - network distribution estimated following \cite{alidaee2020recovering} } 
\label{tab:alidaee}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}d{4}d{4}d{4}d{4}} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 0$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1ex]                                
$\alpha=0.4$     & 0.400  & 0.012 & 0.393   & 0.400  & 0.407   \\
$\gamma_1=5$             & 5.000  & 0.029 & 4.980   & 4.999  & 5.019   \\
$\gamma_2=-3$             & -3.000 & 0.032 & -3.021  & -3.000 & -2.978  \\
F-test (Weak inst.) & 798.971&	340.558&	560.817&	749.132&	990.407\\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                          
$\alpha=0.4$ & 0.371  & 0.024 & 0.357   & 0.373  & 0.387   \\
$\gamma_1=5$              & 5.504  & 0.036 & 5.479   & 5.503  & 5.528   \\
$\gamma_2=-3$            & -2.480 & 0.057 & -2.517  & -2.480 & -2.441  \\
$\hat{\gamma}_1=0$           & -0.364 & 0.031 & -0.385  & -0.363 & -0.344  \\
$\hat{\gamma}_2=0$          & -0.302 & 0.070 & -0.349  & -0.304 & -0.254  \\
F-test (Weak inst.) & 590.248&	253.853&	409.497&	572.210&	721.788 \\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 10$, $N=250$, $M=20$}                                                             \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                              
$\alpha=0.4$    & 0.400  & 0.009 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$         & 4.999  & 0.022 & 4.985   & 4.999  & 5.014   \\
$\gamma_2=-3$                & -3.000 & 0.032 & -3.022  & -3.001 & -2.978 \\
F-test (Weak inst.) & 1697.514&	741.478&	1179.079&	1593.284&	2127.582\\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]                          
$\alpha=0.4$  & 0.395  & 0.021 & 0.388   & 0.397  & 0.405   \\
$\gamma_1=5$            & 5.396  & 0.027 & 5.378   & 5.394  & 5.412   \\
$\gamma_2=-3$            & -2.412 & 0.045 & -2.439  & -2.410 & -2.383  \\
$\hat{\gamma}_1=0$          & -0.385 & 0.032 & -0.404  & -0.387 & -0.370  \\
$\hat{\gamma}_2=0$           & -0.462 & 0.117 & -0.534  & -0.483 & -0.414  \\
F-test (Weak inst.) &1303.291&	586.429&	895.070&	1227.426&	1652.148\\ 
\hline\\[-1.8ex] 

\multicolumn{6}{c}{$\kappa = 20$, $N=250$, $M=20$}                                                            \\
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is observed}\\\\[-1.8ex]                              
$\alpha=0.4$     & 0.400  & 0.008 & 0.395   & 0.400  & 0.405   \\
$\gamma_1=5$                & 5.000  & 0.021 & 4.985   & 5.000  & 5.013   \\
$\gamma_2=-3$             & -2.999 & 0.032 & -3.020  & -2.999 & -2.979   \\
F-test (Weak inst.) & 2685.354&	978.512&	1998.396&	2601.996&	3268.714 \\\\[-1.8ex]
\multicolumn{6}{c}{$\boldsymbol{G}\boldsymbol{y}$ is not observed}\\\\[-1.8ex]   
$\alpha=0.4$ & 0.399  & 0.010 & 0.393   & 0.400  & 0.406   \\
$\gamma_1=5$        & 5.391  & 0.020 & 5.378   & 5.391  & 5.404   \\
$\gamma_2=-3$             & -2.400 & 0.039 & -2.425  & -2.400 & -2.374  \\
$\hat{\gamma}_1=0$           & -0.391 & 0.022 & -0.406  & -0.391 & -0.376  \\
$\hat{\gamma}_2=0$          & -0.573 & 0.047 & -0.605  & -0.575 & -0.544 \\ 
F-test (Weak inst.) & 2191.313&	774.366&	1656.355&	2130.681&	2668.781\\ 
\hline \\[-1.8ex] 



\multicolumn{6}{l}{%
  \begin{minipage}{15cm}%
    \footnotesize{Note: In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in Appendix \ref{sec:ardsetting}. We chose the weight associated with the nuclear norm penalty to minimize the RMSE through cross-validation. This value of $\lambda=600$ is smaller than the recommended value in \cite{alidaee2020recovering}. F-test is the Fisher-statistic of the Weak instruments test. We do not report the estimated values for $c$ and $\boldsymbol{\beta}$ to keep the table readable, but they are available upon request. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.}
  \end{minipage}%
}\end{tabular}
\end{table}
\renewcommand{\arraystretch}{1}

==> archives/shortversion/discussion.tex <==
%\section{Discussion}\label{sec:discussion}

%In this paper, we proposed two types of estimators of peer effects given that the researcher only has access to partial network information. In this section, we discuss how these proposed estimators can be adapted if the underlying network is endogenous and discuss the implications of our results for survey design.

%\subsection{Endogenous Networks}\label{sec:endogenous} In this paper, we assumed away any endogeneity of the network structure (Assumption \ref{as:exonet}). As discussed in Section \ref{sec:linearinmean}, this is done for the purposes of presentation. Indeed, there are multiple ways to introduce, and correct for, endogenous networks, which lead to many possible models and estimators. In this section, we discuss how existing endogenous network corrections can be adapted to our setting. Specifically, we assume that there exists some unobserved variable correlated with both the network $\mathbf{A}$ and the outcome $\mathbf{y}$. This violates Assumption \ref{as:exonet}.

%A first remark is that our ability to accommodate such an unobserved variable depends on the flexibility of the used network formation model. Indeed, some models can obtain estimates of the unobserved heterogeneity (e.g. \cite{breza2017using} or \cite{graham2017econometric}). In such cases, one could simply include the estimated unobserved variables as additional explanatory variables. In particular, the approach followed by \cite{houndetoungan2020count} could be adapted to our context. \cite{johnsson2017estimation} discuss this approach as well as other control-function approaches in detail. Since their instrumental variable estimator is based on the higher-order link relations (i.e. $\mathbf{G}^2\mathbf{X},\mathbf{G}^3\mathbf{X},...$), is is possible that the estimator presented in  Section \ref{sec:iv} could be adapted to their setting.

%However, these approaches may not be entirely satisfactory because they assume that the network formation is estimated consistently, independent of the peer-effect model.\footnote{See, for example, Assumption 1 and Assumptions 6--11 in \cite{johnsson2017estimation}.} The Bayesian estimator presented in Section \ref{sec:genestim} allows for more flexibility. Indeed, one could expand Algorithm \ref{algo:mcmc} and include unobserved latent variables, as has been done, for instance, by \cite{goldsmith2013social}, \cite{hsieh2018smoking}, and \cite{hsieh2019specification}) in contexts where the network is observed. The exploration of such models, in particular their identification and computational complexity, goes far beyond the scope of the current paper and is left for future (exciting) research.

%\subsection{Survey Design} As discussed in Section \ref{sec:iv}, the performance of our SGMM estimators improves if the researcher observes $\mathbf{GX}$. Also, as discussed in Section \ref{sec:ard}, \cite{breza2017using} and \cite{alidaee2020recovering} propose using ARD to estimate network formation models. Importantly, although ARD responses and $\mathbf{GX}$ are similar, they are not equivalent. For example, consider a binary variable (e.g. gender). One can obtain $\mathbf{GX}$ by asking questions such as, ``What fraction of your friends are female?'' For ARD, the question would be, ``How many of your friends are female?'' This suggests asking two questions: one related to the number of female friends and another related to the number of friends.\footnote{\cite{breza2017using} do not require information on the number of friends, although this significantly helps the estimation.}

%For continuous variables (e.g. age), this creates additional issues. One can obtain $\mathbf{GX}$ by asking about the average age of one's friends, but ARD questions must be discrete: ``How many of your friends are in the same age group as you?'' Then, in practice, an approach could be to ask individuals about the number of friends they have and the number of friends they have from multiple age groups: ``How many of your friends are between X and Y years old?'' Using this strategy allows construction of both the ARD and $\mathbf{GX}$.

%Recall that an implication of Propositions \ref{prop:all_observed} is that asking directly for $\mathbf{Gy}$ in the survey leads to a more robust estimation strategy. Indeed, the constructed instruments are valid even if the network formation model is misspecified. We therefore encourage researchers to design their survey questions to elicit ARD as well as $\mathbf{Gy}$ and $\mathbf{GX}$.

\subsection{Next Steps} In this paper, we proposed two estimators where peer effects can be estimated without having knowledge of the entire network structure. We found that, perhaps surprisingly, even very partial information on network structure is sufficient. Nonetheless, many important challenges remain, in particular with respect to the study of compatible models of network formation, which can be estimated under nonrandom sampling, for example.


==> archives/shortversion/intro.tex <==
\section{Introduction}
There is a large and growing literature on the impact of peer effects in social networks.\footnote{For recent reviews, see \cite{boucher2015some}, \cite{bramoulle2019peer}, \cite{breza2016}, and \cite{de2015econometrics}.} However, since eliciting network data is expensive \citep{breza2017using}, relatively few data sets contain comprehensive network information, and existing ones are prone to data errors. Despite some recent contributions, existing methodologies for the estimation of peer effects with incomplete or erroneous network data either focus on a specific kind of sampling or errors, or they are highly computationally demanding.

In this paper, we propose a unifying framework that allows for the estimation of peer effects under the widely used linear-in-means model (e.g. \cite{manski1993identification,bramoulle2009identification}) when the researcher does not observe the entire network structure. Our methodology is computationally attractive and flexible enough to cover cases in which, for example, network data are sampled \citep{chandrasekhar2011econometrics,liu2013estimation}, censored \citep{griffith2019namefriends}, missclassified \citep{hardy2019estimating,lewbel2019social}, or summarized by aggregated relational data (ARD; \cite{breza2017using,alidaee2020recovering}). Our central assumption is that the researcher is able to estimate a network formation model using some partial information about the network structure. Leveraging recent contributions on the estimation of network formation models, we show that this assumption is sufficient to identify and estimate peer effects.

We propose two estimators. First, we present a computationally attractive estimator based on a simulated generalized method of moment (SGMM). The moments are built using draws from the (estimated) network formation model. We study the finite sample properties of our SGMM estimator in the context of ARD using Monte Carlo simulations. We show that the estimator performs very well when the distribution of the true network is relatively informative about the realized network structure in the data. Second, we present a flexible Bayesian estimator allowing to exploit the entire structure of the data generating process. Although the computational cost is greater, we exploit recent computational advances in the literature (e.g. \cite{mele2017,hsieh2019structural}) and show that the estimator can be successfully implemented on common-sized data sets. In particular, we use our estimator to study peer effects on academic achievement using the widely used Add Health database. We find that data errors have first-order downward bias on the estimated endogenous effect.

Our SGMM estimator is inspired by the literature on error-in-variable models with repeated observations.\footnote{See \cite{bound2001measurement} for a review and \cite{chen2011nonlinear} for a review focused on nonlinear models.} Using a network formation model, we obtain a consistent estimator of the distribution of the true network. We then use this estimated distribution to obtain different draws from the distribution of the network.
Our moment condition can be seen as a biased-corrected version of the instrumental strategy proposed by \cite{bramoulle2009identification}, in which we substitute the true network with the draws from the estimated distribution. We show that our moment conditions are asymptotically valid for any fixed number of draws from the estimated distribution of the network. This property implies a significant reduction in the computational cost of the method, compared to methods based on the integration of the moment conditions (e.g. \cite{chandrasekhar2011econometrics}).

Importantly, our SGMM strategy requires only the (partial) observation of a \emph{single} cross-section, as opposed to, for example, the approach of \cite{zhang2020spillovers}. This feature is due to two main properties of the model. First, we can consistently estimate the distribution of the mismeasured variable (i.e. the network) using a single (partial) observation of the variable. Second, in the absence of measurement error, valid instruments for the endogenous peer variable are available \citep{bramoulle2009identification}.

We explore the finite sample properties of our instrumental variable estimator using Monte Carlo simulations. We consider the case in which the researcher only has access to aggregated relational data (ARD). In particular, we show that our SGMM estimator can be successfully combined with the network formation estimators proposed by \cite{breza2017using} and \cite{alidaee2020recovering}. As long as ARD are sufficiently informative in regard to the linking probabilities, our SGMM estimator successfully recovers the model's parameters.

Our Bayesian estimator is based on the likelihood and therefore uses more information about the structure of the model, leading to more precise estimates. In the context of this estimator, the estimated distribution for the network acts as a prior distribution, and the inferred network structure is updated through a Markov chain Monte Carlo (MCMC) algorithm. Our approach relies on data augmentation \citep{tanner1987calculation}, which treats the network as an additional set of parameters to be estimated. This approach saves us from integrating over the $2^{N(N-1)}$ potential networks compatible with the data, which would create an important computational issue. In particular, our MCMC builds on recent developments from the empirical literature on network formation (e.g. \cite{mele2017,hsieh2019structural,hsieh2019specification}). We show that the computational cost of our estimator is reasonable and that it can easily be applied to standard data sets.

We study the impact of errors in adolescents' friendship network data for the estimation of peer effects in education \citep{calvo2009peer}. We show that the widely used Add Health database features many missing links---around 30\% of the within-school friendship nominations are coded with error---and that these data errors strongly bias the estimated peer effects. Specifically, we estimate a model of peer effects on students' academic achievement. Our Bayesian estimator probabilistically reconstructs the missing links, and we obtain a consistent estimator of peer effects. The bias due to data errors is qualitatively important. Our estimated endogenous peer effect coefficient is 1.6 times larger than the one obtained by assuming that the data contains no errors.

\subsection*{Related Literature}
This paper contributes to the recent literature on the estimation of peer effects when the network is either not entirely observed or is observed with noise. In particular, our framework is valid when network data are either sampled, censored, misclassified, or consist of aggregate relational data.\footnote{For related literature that studies the estimation of peer effects when researchers have no network data, see \cite{manresa2016estimating,de2018recovering,souza2014estimating,lewbel2019social}.} We unify these strands in the literature and provide a flexible and computationally tractable framework for estimating peer effects with incomplete or erroneous network data.

\emph{Sampled networks and censoring:} \cite{chandrasekhar2011econometrics} show that models estimated using sampled networks are generally biased. They propose an analytical correction as well as a two-step general method of moment (GMM) estimator. \cite{liu2013estimation} shows that when the interaction matrix is not row-normalized, instrumental variable estimators based on an out-degree distribution are valid, even with sampled networks. \cite{hsieh2018non} focus on a regression model that depends on global network statistics. They propose analytical corrections to account for nonrandom sampling of the network (see also \cite{chen2013impact}). \cite{thirkettleidentification} also focuses on global network statistics, assuming that the researcher only observes a random sample of links. Using a structural network formation model, he derives bounds on the identified set for both the network formation model and the network statistic of interest. Finally, \cite{zhang2020spillovers} studies program evaluation in a context in which networks are locally sampled and affected by a single type measurement error (either false positives or false negatives, but not both). Assuming that the researcher has access to two measurements of the network for each sampled unit, she presents a nonparametric estimator of the treatment and spillover effects.

Relatedly, \cite{griffith2019namefriends} explores the impact of imposing an upper bound to the number of links when eliciting network data, e.g. ``Name your five best friends.'' He shows, analytically and through simulations, that these bounds may bias the estimates significantly. He presents a bias-correction method and explores the impact of censoring using two empirical applications. He finds that censoring underestimates peer effects.

We contribute to this literature by proposing two simple and flexible estimators for the estimation of peer effects based on the linear-in-means model (as opposed to network statistics as in \cite{hsieh2016social} and \cite{thirkettleidentification}). Our estimators do not require many observations of the sampled network (contrary to \cite{zhang2020spillovers}). Similar to \cite{griffith2019namefriends}, we find---using the Add Health database---that sampling leads to an underestimation of peer effects, although we find that censoring has negligible impact in the context of peer effects on academic achievement.

Our Bayesian estimator is similar in spirit to the two-stage GMM estimator proposed by \cite{chandrasekhar2011econometrics}, but it is computationally advantageous. Indeed, their GMM estimator is based on an unconditional moment condition, which requires integrating over the entire set of networks that are compatible in the data. In \cite{chandrasekhar2011econometrics}, there are $2^{N(N-1)-M}$ such networks, where $M$ is the number of sampled pairs of individuals. Even for small networks, the computational cost is substantial whenever sampling is nontrivial. Our SGMM estimator does not suffer from this computational cost and can produce precise estimates with as little as three network simulations. While our Bayesian estimator is more computationally demanding, we exploit recent developments from the empirical literature on network formation (e.g. \cite{mele2017,hsieh2019structural}) and show that it is computationally tractable, even when no link is sampled (e.g. with ARD), which would otherwise  require integrating over the $2^{N(N-1)}$ networks compatible with the data.

\emph{Misclassification:} \cite{hardy2019estimating} look at the estimation of (discrete) treatment effects when the network is observed noisily. Specifically, they assume that observed links are affected by iid errors and present an expectation maximization (EM) algorithm that allows for a consistent estimator of the treatment effect. \cite{lewbel2019social} show that the estimation of the linear-in-means model is consistent and that inference is valid if the expected number of misclassified links grows at a rate slower than $O(\sqrt{N})$.

Our model allows for misclassification of all links with positive probability. As in \cite{hardy2019estimating}, we use a network formation model to estimate the probability of false positives and false negatives. However, our two-stage strategy---estimating the network formation model and then the peer effect model---allows for greater flexibility. In particular, our network formation model is allowed to flexibly depend on covariates. This is empirically important, as networks typically feature homophily on observed characteristics (e.g. \cite{currarini2010identifying,bramoulle2012homophily}).

\emph{Aggregate relational data:} \cite{breza2017using} propose to estimate network effects using aggregate relation data (ARD). These are obtained from such survey questions as, ``How many of your friends have trait X?'' They present a network formation model that can be estimated using only ARD. They show the validity of their methodology using two empirical applications in which the outcome of interest depends on the summary statistics of the network. \cite{alidaee2020recovering} present an alternative estimator allowing to recover nonparametrically the linking probability through ARD. Using a low-rank assumption, they present a simple penalized regression.

We show that these recent methodologies can also be applied to the study of peer effects using the linear-in-means model, which significantly expands the scope of the potential applications of these approaches. In particular, we study the finite sample performance of our SGMM estimator using Monte Carlo simulations and show that we can successfully recover the simulated parameters when combined with the network formation estimators proposed by \cite{breza2017using} or by \cite{alidaee2020recovering}.

A main contribution of this paper is that our estimators can be applied to each of the previously mentioned data issues or to their combination. Our two-step approach---first estimating the network formation and then the peer effects---is flexible and computationally attractive. To reduce the implementation costs, we also present an easy-to-use R package---named \texttt{PartialNetwork}---for applying our estimators. The package allows replicating all simulations and empirical applications in the paper, including the estimator proposed by \cite{breza2017using}. The package is available online at: \url{https://github.com/ahoundetoungan/PartialNetwork}. Additional implementation examples are provided in the vignette accompanying the package. For example, we show that the implementation of our Bayesian estimator, combined with the estimator for ARD proposed by \cite{breza2017using}, is straightforward and computationally tractable.

The remainder of the paper is organized as follows. In Section 2, we present the econometric model as well as the main assumptions. In Section 3, we present our SGMM estimator and study its performance when combined with the estimators for ARD proposed by \cite{breza2017using} and \cite{alidaee2020recovering}. In Section 4, we present our Bayesian estimation strategy. In Section 5, we present our application to peer effects on academic achievement. Section 6 concludes.% with a discussion of the main results, limits, and challenges for future research.


==> archives/shortversion/iv.tex <==
\section{Simulated Generalized Method of Moment Estimators}\label{sec:iv}

In this section, we present estimator based on a Simulated Generalized Method of Moments. The key observation underlying our approach is that it is not necessary to observe the complete network structure to observe $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$. For example, one could simply obtain ${\mathbf{Gy}}$ from survey data, ``What is the average value of your friends' $y$?''

However, even observing $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$, the model (\ref{eq:linearinmean}) cannot be simply estimated using simple linear regression. The reason is that ${\mathbf{Gy}}$ is endogenous; thus, a linear regression would produce biased estimates (e.g. \cite{manski1993identification}, \cite{bramoulle2009identification}).

The typical instrumental approach to deal with this endogeneity is to use instruments based on the structural model, i.e. instruments constructed using second-degree peers (e.g. $\mathbf{G}^2\mathbf{X}$, see \cite{bramoulle2009identification}). These are less likely to be found in survey data. Indeed, we could doubt the informativeness of questions such as, ``What is the average value of your friends' average value of their friends' $x$?''

However, the above discussion is encouraging. When researchers observe $[\mathbf{y}, \mathbf{X}, {\mathbf{GX}},{\mathbf{Gy}}]$, information about the network is only used as a mean to construct a valid instrument, e.g. following \citet{bramoulle2009identification}. Then, if $\mathbf{GX}$ and $\mathbf{Gy}$ are observed, the following simple estimator can be used.

\begin{proposition}\label{prop:all_observed}
[Conditions] Suppose that $\mathbf{GX}$ and $\mathbf{Gy}$ are observed. Let $\boldsymbol{H}$ be a matrix such that: (1) at least one column of $\mathbf{H}^k\mathbf{X}$ is (strongly) correlated with $\mathbf{G}\mathbf{y}$, conditional on $[\mathbf{1},\mathbf{X},\mathbf{GX}]$ for $k\geq 2$, and (2) $\mathbb{E}[\boldsymbol{\varepsilon}|\mathbf{X},\mathbf{H}]=\mathbf{0}$. Finally,  define the matrix $\mathbf{Z}=[\mathbf{1},\mathbf{X},\mathbf{GX},\mathbf{H}^2\mathbf{X},\mathbf{H}^3\mathbf{X}...]$.

[Results] Then, under classical assumptions (e.g. \cite{cameron2005microeconometrics}, Proposition 6.1), the (linear) GMM estimator based on the moment function $\frac{1}{N}\sum_i\mathbf{Z}_i'\boldsymbol{\varepsilon}_i$ is consistent and asymptotically normally distributed with the usual asymptotic variance-covariance matrix.
\end{proposition}

Condition (1) is the relevancy condition, while condition (2) is the exogeneity condition.\footnote{While (for simplicity) in Proposition \ref{prop:all_observed}, we use the entire matrix $\mathbf{X}$ in order to generate the instruments $\mathbf{HX}$, in practice, one should avoid including instruments (i.e. columns of $\mathbf{HX}$) that are weakly correlated with $\mathbf{Gy}$.} While Proposition \ref{prop:all_observed} holds for any matrix $\mathbf{H}$ such that conditions (1) and (2), the most sensible example in our context is when $\mathbf{H}$ is constructed using a draw from $\hat{P}(\mathbf{G})$. A similar strategy is used by \cite{kelejian2014estimation}, \cite{konig2019r} and \cite{lee2020key} in a different context.

Importantly, the moment conditions remain valid even when the researcher uses a \emph{mispecified} estimator of the distribution ${P}(\mathbf{G})$, as long as the specification error on $P(\mathbf{G})$ does not induce a correlation with $\boldsymbol{\varepsilon}$.\footnote{We would like to thank Chih-Sheng Hsieh and Arthur Lewbel for discussions on this important point.} This could be of great practical importance, especially if the estimation of $\hat{P}(\mathbf{G})$ suffers from small sample bias.% We provide an example in Section \ref{sec:ard} below.

\subsection{The General Case}
We now turn to the more general case where $\mathbf{Gy}$ and $\mathbf{GX}$ are not observed. To simplify the notation, for the remainder of this section, we define $\lbrace \dot{\mathbf{G}}^{(r)}\rbrace_{r=1}^R$, $\lbrace \ddot{\mathbf{G}}^{(s)}\rbrace_{s=1}^S$ and $\lbrace \dddot{\mathbf{G}}^{(t)}\rbrace_{t=1}^T$ as sequences of independent draws from $\hat{P}(\mathbf{G})$. We will also let $\dot{\mathbf{G}}$, $\ddot{\mathbf{G}}$, and $\dddot{\mathbf{G}}$ be single independent draws from $\hat{P}(\mathbf{G})$.

Before presenting our estimation strategy, we want to emphasize that we cannot simply proxy $\mathbf{Gy}$ and $\mathbf{GX}$ using draws form $\hat{P}(\mathbf{G})$. To see why, consider the simple case for which $\boldsymbol{\gamma}=\mathbf{0}$, so the observation of $\mathbf{GX}$ is inconsequential. We have, substituting $\mathbf{Gy}$ with $\ddot{\mathbf{G}}\mathbf{y}$:
$$
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\ddot{\mathbf{G}}\mathbf{y}+[\boldsymbol{\eta}+\boldsymbol{\varepsilon}],
$$
where $\boldsymbol{\eta}=\alpha[\mathbf{G}-\ddot{\mathbf{G}}]\mathbf{y}$ is the error due to the approximation of $\mathbf{Gy}$ by $\ddot{\mathbf{G}}\mathbf{y}$. Importantly, the approximation error does \emph{not} vanish as $n$ grows, due to the fact that individuals belong to bounded groups (see Assumption \ref{as:manymarkets}).\footnote{As opposed, for example, to the context studied by \cite{auerbach2019measuring}.} Moreover, since $\mathbf{y}$ is a function of $\mathbf{G}$ (but not of $\ddot{\mathbf{G}}$), we typically have $\mathbb{E}(\mathbf{Gy})_i|\mathbf{z}_i\neq\mathbb{E}(\ddot{\mathbf{G}}\mathbf{y})_i|\mathbf{z}_i$ for some vector of instruments $\mathbf{z}_i$ and all $i$.


Proposition \ref{prop:bias_nocontext} below however shows that the asymptotic bias induced by $\mathbb{E}\eta_i|\mathbf{z}_i\neq 0$ can be bounded, and be very small in practice for carefully constructed vectors of instruments.

\subsubsection{Asymptotically Biased Estimator}
Before presenting our main result (Theorem \ref{prop:non_observed}), we present a simple, asymptotically biased, linear GMM estimator. The presentation of such this estimator is useful for two reasons. First, simulations show that the asymptotic bias turns out to be negligible in many cases, especially for moderate group sizes. Moreover, the estimator is computationally attractive since the estimator can be written in closed-form. Second, the estimator helps to understand the logic underlying the estimator defined in Theorem \ref{prop:non_observed}, which we can view as a bias-corrected version of this simple linear GMM estimator. Proposition \ref{prop:bias_nocontext} formalizes.

\begin{proposition}\label{prop:bias_nocontext}
[Conditions] Assume that $\mathbf{GX}$ is observed. Let $\ddot{\mathbf{S}}=[\mathbf{1},\mathbf{X},\mathbf{GX},\ddot{\mathbf{G}}\mathbf{X},\ddot{\mathbf{G}}\mathbf{y}]$ and $\dot{\mathbf{Z}}=[\mathbf{1},\mathbf{X},\mathbf{GX},\ddot{\mathbf{G}}\mathbf{X},\dot{\mathbf{G}}^2\mathbf{X},\dot{\mathbf{G}}^3\mathbf{X},...]$. Denote by $\hat{\boldsymbol{\theta}}$ the linear GMM estimator based on the (pseudo) moment function $\frac{1}{N}\sum_i \dot{\mathbf{Z}}_i[\boldsymbol{\eta}_i+\boldsymbol{\varepsilon}_i]$, and define the sensitivity matrix\newline ${\mathbf{M}}_N=[(\ddot{\mathbf{S}}'\dot{\mathbf{Z}}/N)\mathbf{W}(\dot{\mathbf{Z}}'\ddot{\mathbf{S}}/N)]^{-1}(\ddot{\mathbf{S}}'\dot{\mathbf{Z}}/N)\mathbf{W}$.

[Result] Then, under classical assumptions (see proof), the asymptotic bias of $\hat{\boldsymbol{\theta}}$ is given by $\alpha \mathbf{M}_0 \plim[\dot{\mathbf{Z}}'({\mathbf{G}}-\ddot{\mathbf{G}})\mathbf{y}/N]$. Moreover, letting $\mathbf{W}=\mathbf{I}$ minimizes the asymptotic bias in the sense of minimizing the Frobenius norm of $\mathbf{M}$.
\end{proposition}
While there are no obvious way to get a consistent estimate of the asymptotic bias (because $\mathbf{y}$ is a function of $\mathbf{G}$) simulations show that the bias is very small in practice.\footnote{See Section \ref{sec:ard} below.} 

The intuition behind Proposition \ref{prop:bias_nocontext} comes from the literature on error-in-variable models with repeated observations (e.g. \cite{bound2001measurement}). The instrumental variable uses two independent draws from the (estimated) distribution of the true network. One draw is used to proxy the unobserved variable (i.e. $\mathbf{Gy}$), while the other is used to proxy the instrument (i.e. $\mathbf{G}\mathbf{X}$). This approach greatly reduces the bias as compared to a situation in which only one draw would be used.\footnote{Simulations available uppon request.}

The argument in Proposition \ref{prop:bias_nocontext} is very similar to the one in \cite{andrews2017measuring}, although here perturbation with respect to the true model is not \textit{local}.\footnote{See page 1562 in \cite{andrews2017measuring}.} We also show that we expect $\mathbf{W}=\mathbf{I}$ to minimize the asymptotic bias. Our result therefore provides a theoretical justification for the simulations in \cite{onishi2021sample} who show that the using the identity matrix to weight the moments greatly reduce the bias in the context studied by \cite{andrews2017measuring}.


Conceptually, Proposition \ref{prop:bias_nocontext} states that the simple linear GMM estimator $\hat{\boldsymbol{\theta}}$ is such $\hat{\boldsymbol{\theta}}=\boldsymbol{\theta_0}+F(\boldsymbol{\theta}_0)$ for some known function $F$. It is therefore possible to use this insight to define a consistent estimator of $\boldsymbol{\theta}_0$. This is what we do in Theorem \ref{prop:non_observed} below.

\subsubsection{Main Result}
We show that we can include the bias directly in the moment function, which provides a consistent estimator of $\boldsymbol{\theta}$. Let $\tilde{\boldsymbol{\theta}}=[c,\boldsymbol{\beta}',\boldsymbol{\gamma}']'$.

\begin{theorem}\label{prop:non_observed} [Conditions] Let $\dot{\mathbf{Z}}^{(r)}=[\mathbf{1},\mathbf{X},\dot{\mathbf{G}}^{(r)}\mathbf{X},(\dot{\mathbf{G}}^{(r)})^2\mathbf{X},(\dot{\mathbf{G}}^{(r)})^3\mathbf{X},...]$ and $\ddot{\mathbf{V}}^{(s)}=[\mathbf{1},\mathbf{X},\ddot{\mathbf{G}}^{(s)}\mathbf{X}]$. Consider also the following (simulated) moment function:
\begin{equation}\label{eq:moment}
\frac{1}{RST}\sum_{r=1}^R\sum_{s=1}^S\sum_{t=1}^T\dot{\mathbf{Z}}^{(r)\prime}_i\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})_i\left(\mathbf{y}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}\ddot{\mathbf{V}}^{(s)}\tilde{\boldsymbol{\theta}}\right)\right]
\end{equation}

[Result] For any positive integers $R$, $S$ and $T$, the (simulated) GMM estimator based on (\ref{eq:moment}) is consistent and asymptotically normal, i.e.  $\sqrt{N}(\hat{\boldsymbol{\theta}}-\boldsymbol{\theta}_0+\Delta\boldsymbol{\theta}^*)\overset{d}{\to}N(\mathbf{0},\mathbf{V})$, where $\Delta\boldsymbol{\theta}^*$ and $\mathbf{V}$ are defined in (\ref{eq:thetastar}) and (\ref{var:gmm}) in the Online Appendix and where $\Delta\boldsymbol{\theta}^*\rightarrow 0$ as $N\rightarrow\infty$.
\end{theorem}
Here the asymptotic variance $\mathbf{V}$ includes the sampling uncertainty, the estimating uncertainty of $\hat{\boldsymbol{\rho}}$, as well as the simulating uncertainty (which decreases as $R$, $S$ and $T$ grow). The term $\Delta\boldsymbol{\theta}^*$ is introduced due to the fact the our moment condition is equal to zero only asymptotically, and it therefore allows to center the distribution of $\hat{\boldsymbol{\theta}}$ for finite $N$. Similar corrections can be found for penalized likelihood models (e.g. \cite{fan2001variable}, \cite{fan2004nonconcave}, \cite{dzemski2019empirical})

Importantly, and similar to standard methods of simulated moments (e.g. \cite{gourieroux1993simulation}), the estimation is consistent even for a finite number of simulations (i.e. $R$, $S$, and $T$ are finite). Our estimator therefore does not suffer from the curse of dimensionality faced by \cite{chandrasekhar2011econometrics}.\footnote{The unconditional moment condition in \cite{chandrasekhar2011econometrics} is based on the (Monte Carlo) integration of the moment condition $\mathbb{E}(\mathbf{Z}^{(s)\prime}\boldsymbol{\varepsilon}|\mathbf{G})$ over $\mathbf{G}$. Suppose that there are $m$ pairs of individuals with unknown link status, there would be $2^m$ network structures to integrate from.}

To understand the intuition behind the use of the moment function (\ref{eq:moment}), let us replace $\mathbf{y}=(\mathbf{I}-\alpha\mathbf{G})^{-1}(\mathbf{V}\tilde{\boldsymbol{\theta}}+\boldsymbol{\varepsilon})$ in equation (\ref{eq:moment}). In doing so, we can rewrite the term inside the triple summation in (\ref{eq:moment}) as a sum of two terms. First, $\dot{\mathbf{Z}}^{(r)\prime}_i\boldsymbol{\varepsilon}_i$, which would be the standard moment function if $\mathbf{G}$ was observed (e.g. \cite{bramoulle2009identification}), and second:
\begin{equation}\label{eq:bias_corr}
\dot{\mathbf{Z}}^{(r)\prime}_i\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})_i\left((\mathbf{I}-\alpha{\mathbf{G}})^{-1}{\mathbf{V}}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}\ddot{\mathbf{V}}^{(s)}\right)\tilde{\boldsymbol{\theta}}\right].
\end{equation}
That second term can be viewed as the bias-correction term of the moment function.

We show that the expectation both terms are equal to $0$ as $N$ grows to $\infty$. For the first term, this is true since the simulated network is exogenous. For the second term, this is true because $\mathbf{G}$, $\dot{\mathbf{G}}$, $\ddot{\mathbf{G}}$ and $\dddot{\mathbf{G}}$ are asymptotically drawn from the same distribution.

For the special case in which $\mathbf{G}$ is observed, one could substitute $\dot{\mathbf{G}}^{(r)}=\ddot{\mathbf{G}}^{(s)}=\dddot{\mathbf{G}}^{(t)}=\mathbf{G}$ for all $r,s,t$ and the first term would simply be $\mathbf{Z}'_i\boldsymbol{\varepsilon}_i$, while the second term would be exactly equal to $\mathbf{0}$.

Note that Theorem \ref{prop:non_observed} is valid whether or not $\mathbf{Gy}$ and $\mathbf{GX}$ are observed since the moment function (\ref{eq:moment}) does not use information on $\mathbf{Gy}$ or $\mathbf{GX}$. It is of course possible to include this additional information, if either one is observed.

For example, assume that $\mathbf{GX}$ is observed, and replace $\ddot{\mathbf{V}}$ with $\mathbf{V}$ in (\ref{eq:bias_corr}). After some algebra, we obtain:\footnote{See the Online Appendix} \begin{equation}\label{eq:gxobswrong}
    \dot{\mathbf{Z}}^{(r)\prime}_i\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})_i(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}[\alpha(\mathbf{G}-\ddot{\mathbf{G}})\mathbf{y}]\right],
\end{equation}
plus a term that is equal to zero in expectation.

We can see that the last term in bracket corresponds to the source of the asymptotic bias in Proposition \ref{prop:bias_nocontext}: the approximation error of $\mathbf{Gy}$ by $\ddot{\mathbf{G}}\mathbf{y}$. The instruments used are however different and, here, are such that (\ref{eq:gxobswrong}) does not converge to $0$ as $N$ grows. As for Proposition \ref{prop:bias_nocontext}, this is due to the fact that $\mathbf{y}$ is a function of $\mathbf{G}$. It is however possible to construct moment functions for the particular cases for which $\mathbf{GX}$ or $\mathbf{Gy}$ are observed. These can be found in Corollary \ref{prop:GXobs} and \ref{prop:Gyobs} of the Online Appendix.

The results of this Section show that the estimation of (\ref{eq:linearinmean}) is possible, even with very limited information about the network structure. In Section \ref{sec:ard}, we study the finite sample properties of our approach using network formation models estimated on aggregated relational data (\cite{breza2017using}; see Example \ref{ex:ard}). %Before, however, we briefly discuss how one can adapt this estimation strategy while allowing for group-level unobservables.

%Indeed, a common assumption is that each group in the population is affected by a common shock, unobserved by the econometrician (e.g. \cite{bramoulle2009identification}). As such, for each group $r=1,...,M$, we have: $\mathbf{y}_r=c_r\mathbf{1}_r+\mathbf{X}_r\boldsymbol{\beta}+\alpha\mathbf{G}_r\mathbf{y}_r+{\mathbf{G}_r\mathbf{X}_r}\boldsymbol{\gamma}+\boldsymbol{\varepsilon}_r$, where $c_r$ is not observed, $\mathbf{1}_r$ is an $N_r$-dimensional vector of ones, $N_r$ is the size of the group r, $\bG_r$ is the subinteraction matrix in the group r, and $\bepsilon_r$ is the vector of error terms in the group r.

%Under Assumption \ref{as:manymarkets}, it is not possible to obtain a consistent estimator of $\{c_r\}_{r=1}^m$ because the number of observations used to estimate each $c_r$ is bounded. This is known as the \emph{incidental parameter problem}.\footnote{See \cite{lancaster2000incidental} for a review.} A common strategy is to use deviations from the group average and estimate the model in deviations (e.g. \cite{bramoulle2009identification}).

%Let $\mathbf{J}=diag\{\mathbf{I}_{N_r}-\frac{1}{N_r}\mathbf{1}_r\mathbf{1}'_r\}$ be the group-differentiating matrix, where $\mathbf{I}_{N_r}$ is the identified matrix of dimension $N_r$. The operator \emph{diag} generates a blog-diagonal matrix in which each group is a block.\footnote{Then, $\mathbf{Jw}$ gives $\mathbf{w}$ minus the group average of $\mathbf{w}$.} We can rewrite: $\mathbf{Jy}=\mathbf{JX}\boldsymbol{\beta}+\alpha{\mathbf{JG}\mathbf{y}}+{\mathbf{JGX}}\boldsymbol{\gamma}+\boldsymbol{J\varepsilon}$. Note that the results of this Section extend directly, using variables in deviation with the group average. Simulation results presented in the Online Appendix confirm that SGMM estimator performs well in the presence of group heterogeneity.

\subsection{Finite Sample Performance Using ARD}\label{sec:ard}
In this section, we study the small sample performance of the estimator presented in Section \ref{sec:iv} when the researcher only has access to ARD (as in Example \ref{ex:ard}). First, we simulate network data using the model proposed by \cite{breza2017using} and simulate outcomes using the linear in means model (\ref{eq:linearinmean}) conditional on the simulated networks. Second, we estimate the network formation model using the Bayesian estimator proposed by \cite{breza2017using} (yielding $\hat{\boldsymbol{\rho}}_B$), as well as using the classical estimator proposed by \cite{alidaee2020recovering} (yielding $\hat{\boldsymbol{\rho}}_A$). Third, we estimate the linear-in-means model, using our the estimators presented in Proposition \ref{prop:bias_nocontext} and Theorem \ref{prop:non_observed}, based on $\hat{\boldsymbol{\rho}}_A$ and $\hat{\boldsymbol{\rho}}_B$.

Recall that
\begin{equation}\label{eq:ard}
P(a_{ij}=1)\propto\exp\{\nu_i+\nu_j+\zeta \mathbf{z}_i'\mathbf{z}_j\},    
\end{equation}
where $\nu_i$, $\nu_j$, $\zeta$, $\mathbf{z}_i$, and $\mathbf{z}_j$ are not observed by the econometrician but follow parametric distributions. We refer the interested reader to \cite{mccormick2015latent}, \cite{breza2017using}, and \cite{breza2019consistently} for a formal discussion of the model, including its identification and consistent estimation. %Here, we discuss the intuition using a simple analogy.

%Suppose that individuals are located according to their geographical position on Earth. Suppose also that there are a fixed number of cities on Earth in which individuals can live. The econometrician does not know the individuals' locations on Earth nor do they know the location of the cities. In model (\ref{eq:ard}), $\mathbf{z}_i$ represent $i$'s position on Earth. However, the econometrician has access to ARD for a subset of the population, i.e. answers to questions such as, ``How many of your friends live in city $A$?''

%To understand the intuition behind the identification of the model, consider the following example: suppose that individual $i$ has many friends living in city $A$. Then, city $A$ is likely located close to $i$'s location. Similarly, if many individuals have many friends living in city $A$, then city $A$ is likely a large city. Finally, if $i$ has many friends from many cities, $i$ likely has a large $\nu_i$.

To study the finite sample performance of our instrumental strategy in this context, we simulate 20 groups of 250 individuals each. Within each subpopulation, we simulate the ARD responses as well as a series of observable characteristics. The details of the Monte Carlo simulations can be found in the Online Appendix.

Importantly, the model in (\ref{eq:ard}) is based on a single population framework. Thus, the network formation model must be estimated separately for each of the 20 groups. With only 250 individuals in each group, we therefore expect significant small-sample bias.

We contrast the estimator proposed by \cite{breza2017using} with the one proposed by \cite{alidaee2020recovering}. Whereas \cite{breza2017using} present a parametric Bayesian estimator, \cite{alidaee2020recovering} propose a (nonparametric) penalized regression based on a low-rank assumption. One main advantage of their estimator is that it allows for a wider class of model and ensures that the estimation is fast and easily implementable.\footnote{The authors developed user-friendly packages in R and Python. See their paper for links and details.} Note, however, that their method only yields a consistent estimator of $\hat{P}(\mathbf{A})$ if the true network is effectively low rank.

Very intuitively, the low-rank assumption implies that linking probabilities were generated from a small number of parameters.%; for example, in the example above, knowing individuals' gregariousness parameters $\nu_i$ and city in which they live would allow a prediction of the linking probabilities.
Importantly, the model (\ref{eq:ard}) is not necessarily low rank; for example, if the individuals' locations on Earth (i.e. the $\mathbf{z}_i$'s) are uniformly distributed and there are only very few  large cities, then the model produced is not low rank and the method proposed by \cite{alidaee2020recovering} performs poorly. Intuitively, in such a case, the fact that individual $i$ lives in city $A$ poorly explains the linking probabilities. 

We compare the performance of both estimators as we vary the concentration parameter (that is, $\kappa$, see the Online Appendix for details). This has the effect of changing the \emph{effective rank} of the linking probabilities: increasing $\kappa$ decreases the effective rank.\footnote{We refer the interested reader to \cite{alidaee2020recovering} for a formal discussion of the effective rank and of its importance for their estimator.} We therefore expect the estimator proposed by \cite{alidaee2020recovering} to perform better for larger values of $\kappa$.

A summary of the results is presented in Tables \ref{tab:gx:obs:short} and \ref{tab:gx:unobs:short}. The complete results can be found in Tables \ref{tab:gx:obs:full} and \ref{tab:gx:unobs:full} of the Online Appendix. Table \ref{tab:gx:obs:short} presents the results for the special case where $\mathbf{GX}$ are observed in the data. The table displays the performance of the simple (biased) estimator in Proposition \ref{prop:bias_nocontext} and that of our simulated GMM (see Corollary \ref{prop:GXobs}) when the network formation model is estimated by \cite{breza2017using} and \cite{alidaee2020recovering}. 

When $\kappa=0$, the network formation is not low-rank. This disproportionately affects the estimator of \cite{alidaee2020recovering}. Although asymptotically biased, the performance of the IV in Proposition \ref{prop:bias_nocontext} is very good and even seems to outperform our SGMM when using the estimator proposed by \cite{alidaee2020recovering}. Moreover, the overidentification test points (on average) to a violation of the exclusion restriction.

When $\kappa=15$ the estimators proposed by \cite{breza2017using} and \cite{alidaee2020recovering} perform similarly and so do our estimators. Both the IV and SGMM estimators recover the true value of $\alpha$.

We now turn to the more general case where $\mathbf{GX}$ are not observed. Note that in that case, Proposition \ref{prop:bias_nocontext} does not apply. Table \ref{tab:gx:unobs:short} presents the performance of our SGMM estimator (Theorem \ref{prop:non_observed}) when the network formation process is estimated using the estimators proposed by \cite{breza2017using} and \cite{alidaee2020recovering}, as well as when we assume that the researcher knows the true distribution of the network.

We see that the performance of our estimator, is strongly affected by the quality of the first-stage network formation estimator. When based on either the estimator proposed by \cite{breza2017using} or \cite{alidaee2020recovering}, for $\kappa=0$ or $\kappa=15$, our SGMM estimator performs poorly.

This poor performance of our SGMM estimator in a context where both $\mathbf{Gy}$ and $\mathbf{GX}$ are unobserved was anticipated. This is due to two main reasons. \emph{First}, the consistency of the network formation estimator in \cite{breza2019consistently} holds as the size of each sub-population goes to infinity, while the consistency of our estimator holds as the number of (bounded) sub-populations goes to infinity. This should affect the performance of our estimator, when based on \emph{estimated} network formation models, but when based on the true distribution of the network.

\emph{Second}, as discussed in Example \ref{ex:ard}, ARD provides very little information about the realized network structure in the data (as opposed, for example, as for censoring issues, see Example \ref{ex:censored}). Then, if the true distribution is vague in the sense that most predicted probabilities are away from $0$ or $1$, we expect the estimation to be imprecise. This is what happens when $\kappa=15$, where our estimation based on the true distribution of the network is very imprecise, in a context where the network affects the outcome through both $\mathbf{Gy}$ and $\mathbf{GX}$.

In the next section, we present a likelihood based estimator, which uses more information on the data generating process of the outcome, in order to improve the precision of the estimation.


\renewcommand{\arraystretch}{.95}
\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD and observed $\bG\bX$} 
\label{tab:gx:obs:short}
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}ld{4}c}
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Parameter              & \multicolumn{2}{c}{Breza et al.} & \multicolumn{2}{c}{Alidaee et al.} \\
                       & \multicolumn{1}{c}{Mean}           & \multicolumn{1}{c}{Std. Dev}        & \multicolumn{1}{c}{Mean}            & \multicolumn{1}{c}{Std. Dev}         \\
 
\hline\\[-1.8ex] 
                      \multicolumn{5}{c}{$\kappa=0$}       \\\hline 
                       \hline\\[-1.8ex] 
                       
                        \multicolumn{5}{c}{IV (Proposition \ref{prop:bias_nocontext})}    \\
                       \\[-1.8ex] 
$\alpha = 0.4$         & 0.392              & (0.009)              & 0.372               & (0.027)               \\
\\[-1.8ex]
Sargan test            & 1.217              & (1.761)              & 7.779               & (10.386)              \\
F-test (Weak inst.)    & 4259.622           & (1140.825)           & 597.055             & (251.886)             \\\hline\\[-1.8ex] 

                       \multicolumn{5}{c}{SGMM (Corollary \ref{prop:GXobs})}                      \\
                       \\[-1.8ex]
                       
   $\alpha = 0.4$         & 0.392              & (0.010)               & 0.492               & (0.057)               \\                    
                       
                       
                       \hline\\
                                        \multicolumn{5}{c}{$\kappa=15$}      \\\hline 
                       \hline\\[-1.8ex] 
                       
                        \multicolumn{5}{c}{IV (Proposition \ref{prop:bias_nocontext})}    \\
                       \\[-1.8ex] 
$\alpha = 0.4$         & 0.400              & (0.007)              & 0.399               & (0.007)               \\
\\[-1.8ex]
Sargan test            & 1.063              & (1.496)              & 2.608               & (1.496)               \\
F-test (Weak inst.)    & 5306.551           & (1519.394)           & 1767.274            & (1519.394)            \\\hline\\[-1.8ex] 
                                        \multicolumn{5}{c}{SGMM (Corollary \ref{prop:GXobs})}                   \\                  \\[-1.8ex]                              $\alpha = 0.4$         & 0.400              & (0.009)              & 0.428               & (0.009)               \\
 
\bottomrule     
\end{tabular}
\begin{tablenotes}[para,flushleft]
\footnotesize Note: For each case, we generated 20 independent subnetworks of 250 individuals each. In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with a location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in the Online Appendix \ref{sec:ardsetting}. Predicted probabilities are computed using the mean of the posterior distribution. Sargan test is the statistic of the overidentification test. F-test is the Fisher-statistic of the Weak instruments test. We chose the weight associated with the nuclear norm penalty to minimize the RMSE through cross-validation. This value of $\lambda=600$ is smaller than the recommended value in \cite{alidaee2020recovering}. See Table \ref{tab:gx:obs:full} for the estimated values of the other parameters. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.
\end{tablenotes}
\end{threeparttable}
\end{table}




\begin{table}[!htbp]
\centering 
\small
\caption{Simulation results with ARD and unobserved $\bG\bX$ (SGMM, Theorem \ref{prop:non_observed}) }
\label{tab:gx:unobs:short}
\begin{threeparttable}
\begin{tabular}{@{\extracolsep{5pt}}ld{4}ld{4}cd{4}c}
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Parameter       & \multicolumn{2}{l}{Breza et al.} & \multicolumn{2}{l}{Alidaee et al.} & \multicolumn{2}{l}{True distribution} \\
                       & \multicolumn{1}{c}{Mean}           & \multicolumn{1}{c}{Std. Dev}        & \multicolumn{1}{c}{Mean}            & \multicolumn{1}{c}{Std. Dev}        & \multicolumn{1}{c}{Mean}            & \multicolumn{1}{c}{Std. Dev}       \\\hline\\[-1.8ex] 
                \multicolumn{7}{c}{$\kappa = 0$}                                                    \\
                \\[-1.8ex]
$\alpha = 0.4$  & 0.717          & (0.463)         & 0.700           & (0.268)          & 0.400            & (0.056)            
\\\hline\\
                 \multicolumn{7}{c}{$\kappa = 15$}                                                   \\
                 \\[-1.8ex]
$\alpha = 0.4$  & 0.603          & (0.069)         & 0.870           & (0.202)          & 0.434            & (0.394)            \\

\bottomrule     
\end{tabular}
\begin{tablenotes}[para,flushleft]
\footnotesize Note: For each case, we generated 20 independent subnetworks of 250 individuals each. In each subnetwork, the spherical coordinates of individuals are generated from a von Mises--Fisher distribution with a location parameter $(1, 0, 0)$ and intensity parameter $\kappa$. Details of the simulation exercise can be found in the Online Appendix. Predicted probabilities are computed using the mean of the posterior distribution. Sargan test is the statistic of the overidentification test. F-test is the Fisher-statistic of the Weak instruments test.  See Table \ref{tab:gx:unobs:full} for the estimated values of the other parameters. Instruments are build using only second-degree peers, i.e. $\mathbf{G^2X}$.
\end{tablenotes}
\end{threeparttable}
\end{table}
\renewcommand{\arraystretch}{1}


==> archives/shortversion/model.tex <==
\section{The Model}\label{sec:linearinmean}
We now formally present our model. We first describe the \emph{linear-in-means} model \citep{manski1993identification,bramoulle2009identification}, arguably the most widely used model for studying peer effects in networks (see \cite{bramoulle2019peer} for a recent review). We then introduce our main assumption, characterizing what is known about the structure of the network.

\subsection{The Linear-in-Means Model}

Let $\mathbf{A}$ represent the $N\times N$ \emph{adjacency matrix} of the network. We assume a directed network: $a_{ij}\in \{0,1\}$, where $a_{ij}=1$ if $i$ is linked to $j$. We normalize $a_{ii}=0$ for all $i$ and let $n_i=\sum_j a_{ij}$ denote the number of links of $i$.
Let $\mathbf{G}=f(\mathbf{A})$, the $N\times N$ \emph{interaction matrix} for some function $f$. Unless otherwise stated, we assume that $\mathbf{G}$ is a row-normalization of the adjacency matrix $\mathbf{A}$.\footnote{In such a case, $g_{ij}=a_{ij}/n_i$ whenever $n_i>0$, whereas $g_{ij}=0$ otherwise.} Most of our results hold for any function $f$ which preserves the independence among groups (see Assumption \ref{as:manymarkets} below).

We focus on the following model:
\begin{equation}\label{eq:linearinmean}
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\mathbf{Gy}+{\mathbf{GX}}\boldsymbol{\gamma}+\boldsymbol{\varepsilon},
\end{equation}
where $\mathbf{y}$ is a vector of an outcome of interest (e.g. academic achievement), $c$ is a constant, $\mathbf{X}$ is a matrix of observable characteristics (e.g. age, gender...), and $\boldsymbol{\varepsilon}$ is a vector of errors.\footnote{Note that \cite{boucher2020binary} recently showed that (\ref{eq:linearinmean}) is valid (coherent, complete, and microfounded), even when $y_i$ is binary.} The parameter $\alpha$ therefore captures the impact of the average outcome of one's peers on their behavior (the endogenous peer effect). The parameter $\boldsymbol{\beta}$ captures the impact of one's characteristics on their behavior (the individual effects). The parameter $\boldsymbol{\gamma}$ captures the impact of the average characteristics of one's peers on their behavior (the contextual peer effects).

The following set of assumptions summarizes our setup.
\begin{assumption}\label{as:alpha} $|\alpha|<1/\Vert \mathbf{G}\Vert$ for some submultiplicative norm $\Vert \cdot\Vert$.
\end{assumption}
\begin{assumption}\label{as:manymarkets} The population is partitioned into $M>1$ groups, where the size $N_r$ of each group $r=1,...,M$ is bounded. The probability of a link between individuals of different groups is equal to $0$.
\end{assumption}
\begin{assumption}\label{as:nosampling} For each group, the outcome and individual characteristics are observed, i.e. $(\mathbf{y}_r,\mathbf{X}_r)$,  $r=1,...,M$, are observed.
\end{assumption}
\begin{assumption}\label{as:exonet} Exogeneity: $\mathbb{E}[\boldsymbol{\varepsilon}|\mathbf{X}]=\mathbf{0}$.
\end{assumption}

Assumption \ref{as:alpha} ensures that the model is coherent and that there exists a unique vector $\mathbf{y}$ compatible with (\ref{eq:linearinmean}). When $\mathbf{G}$ is row-normalized, $|\alpha|<1$ is sufficient. Assumption \ref{as:manymarkets} is introduced for exposition purposes; for example, the data could consist of a collection of small villages \citep{banerjee2013diffusion} or schools \citep{calvo2009peer}. Our methods extend to alternative assumptions such as those proposed by \cite{lee2004asymptotic} and \cite{lee2010specification}.\footnote{The authors assume that the adjacency matrix $\mathbf{A}$ is bounded in row- and column-sums.}

Assumption \ref{as:nosampling} implies that the data is composed of a subset of fully sampled groups.\footnote{Contrary to \cite{liu2017peer} or \cite{wang2013estimation}, for example.} A similar assumption is made by \cite{breza2017using}. Note that Assumption \ref{as:exonet} does not impose restrictions on the dependence between the errors and the network structure. We present the network formation process in details in the next section.

\subsection{Partial Network Information}

In this paper, we relax the costly assumption that the adjacency matrix $\mathbf{A}$ is observed. We assume instead that sufficient information about the network is observed so that a network formation model can be estimated.

More formally, we let $\mathcal{A}$ denote the observed information about the true network structure. That is, $\mathcal{A}$ is a function of the true network $\mathbf{A}$ and potentially of individuals' characteristics (see Example \ref{ex:ard}). We impose no particular structure on $\mathcal{A}$ but discuss important examples below (see Examples \ref{ex:sampled}--\ref{ex:ard}).

We assume that links are generated as follows:
\begin{equation}\label{eq:gennetfor}
P(a_{ij})\equiv P(a_{ij}|\boldsymbol{\rho}_0)\propto \exp\{a_{ij}Q(\boldsymbol{\rho}_0,\mathbf{w}_{ij})\}, 
\end{equation}
where $Q$ is some known continuous function, $\mathbf{w}_{ij}=\mathbf{w}_{ij}(\mathbf{X})$ is a vector of observed characteristics for the pair $ij$, and $\boldsymbol{\rho}_0$ is the true value of $\boldsymbol{\rho}$, a vector of parameters to be estimated. Note that the assumption that the set of observed characteristics of the pairs $\mathbf{w}_{ij}$ are function of $\mathbf{X}$ implies that the network is \emph{exogenous}. We omit the dependence of $P(a_{ij})$ on $\mathbf{w}_{ij}$ to simplify the notation.


As will be made clear, our estimation strategy requires that the econometrician be able to draw samples from (a consistent estimator) $P(\mathbf{A})$. Thus, and for the sake of simplicity, we focus on distributions that are conditionally independent across links (i.e. $P(a_{ij}|\mathbf{A}_{-ij})=P(a_{ij})$), as in (\ref{eq:gennetfor}), although this is not formally required.\footnote{A prime example of a network distribution that is not conditionally independent is the distribution for an exponential random graph model (ERGM), e.g. \cite{mele2017}.}

We now present our main assumption.
\begin{assumption}[Partial Network Information]\label{as:partial} Given network information $\mathcal{A}$ and the parametric model (\ref{eq:gennetfor}), there exists an estimator $\hat{\boldsymbol{\rho}}_N$, such that $\hat{\boldsymbol{\rho}}_N\rightarrow_p \boldsymbol{\rho}_0$ as $N\rightarrow\infty$.
\end{assumption}

Assumption \ref{as:partial} implies that, using (\ref{as:partial}), the researcher has access to ``sufficient information'' about the network structure to obtain a consistent estimator of the distribution of the true network $P(\mathbf{A})$. We denote such a consistent estimator by $\hat{P}(\mathbf{A})\equiv P(\mathbf{A}|\hat{\boldsymbol{\rho}},\mathcal{A})$. We omit the dependence on $\mathcal{A}$ to simplify the notation when this does not create confusion. Note that we can use $\hat{P}(\mathbf{A})$ to obtain the consistent estimator $\hat{P}(\mathbf{G})$, since $\mathbf{G}=f(\mathbf{A})$ for some known function $f$.\footnote{Since $\mathbf{A}$ takes a finite number of values, so does $\mathbf{G}$, and $P(\mathbf{G})$ is a multinomial distribution. As such it is a continuous function of the distribution $P(\mathbf{A})$, irrespective of the function $f$ linking $\mathbf{A}$ and $\mathbf{G}$.}

Importantly, it should be noted that even if the econometrician has access to a consistent estimator of the distribution of the true network, it \emph{does not} imply that they could simply proxy $\mathbf{G}$ in (\ref{eq:linearinmean}) using a draw $\tilde{\mathbf{G}}$ from the distribution $\hat{P}(\mathbf{G})$. The reason is that for any vector $\mathbf{z}$, $\tilde{\mathbf{G}}\mathbf{z}$ generally does not converge to ${\mathbf{G}}\mathbf{z}$ as the number of individuals $N$ goes to infinity. In other words, knowledge of $\hat{P}(\mathbf{G})$ and $\mathbf{z}$ is not sufficient to obtain a consistent estimator of $\mathbf{Gz}$. To see why, note that $(\mathbf{Gz})_i=\sum_{j=1}^Ng_{ij}z_j$. Under Assumption \ref{as:manymarkets}, the set of $j$ such that $g_{ij}\neq 0$ is bounded, so a consistent estimator of $P(\mathbf{G})$ is not sufficient to obtain a consistent estimator of $\mathbf{GX}$. This is also true under the alternative assumptions in \cite{lee2004asymptotic} and \cite{de2018identifying},\footnote{\cite{lee2004asymptotic}  requires that $\mathbf{G}$ be bounded in row- and column-sums (in absolute value), whereas \cite{de2018identifying} assume that $\mathbf{A}$ is bounded in row-sums.} but it contrasts from models based on a large network asymptotic (e.g. \cite{auerbach2022identification}).

Assumption \ref{as:partial} covers a large range of cases in which networks are partially observed. We specifically discuss four leading examples in which Assumption \ref{as:partial} holds: \emph{sampled networks} (Example \ref{ex:sampled}), \emph{censored networks }(Example \ref{ex:censored}), \emph{misclassified network links} (Example \ref{ex:misclass}), and \emph{aggregated relational data} (Example \ref{ex:ard}).

\begin{example}[Sampled Networks]\label{ex:sampled}
Suppose that we observe the realizations of $a_{ij}$ for a random sample of $m$ pairs (e.g. \cite{chandrasekhar2011econometrics}). Here $\mathcal{A}$ can be represented by an $N\times N$ binary matrix $\mathbf{A}^{obs}$. \cite{conley2010learning} present such a sampling scheme and ask individuals about their relationship with a random sample of other individuals, for example, ``Do you know person X?''

Such a setup is sufficient to consistently estimate flexible network formation models such as the one in \cite{graham2017econometric}. A simpler example would be to assume that the network formation model (\ref{eq:gennetfor}) is equal to $P(a_{ij}=1)\propto\exp\{\mathbf{w}_{ij}\boldsymbol{\rho}\}$. In this case, a simple logistic regression provides a consistent estimator of $\boldsymbol{\rho}$.

Given this consistent estimator for $\boldsymbol{\rho}$ and the assumed parametric model, we can compute an estimator for the distribution of the true network $\hat{P}(\mathbf{A})=P(\mathbf{A}|\hat{\boldsymbol{\rho}},\mathcal{A})$. Here, $\hat{P}(a_{ij})=a_{ij}^{obs}$ for any sampled link $ij$, while $\hat{P}(a_{ij})\propto\exp\{a_{ij}\mathbf{w}_{ij}\hat{\boldsymbol{\rho}}\}$ for the remaining unsampled links.
\end{example}

\begin{example}[Censored Network Data]\label{ex:censored}
As discussed in \cite{griffith2019namefriends}, network data is often censored. This typically arises when surveyed individuals are asked to name only $T>1$ links (among the $N$ possible links they may have). Here, $\mathcal{A}$ can be represented by an $N\times N$ binary matrix $\mathbf{A}^{obs}$. We can use censored network data to estimate a network formation model such as $P(a_{ij}=1)\propto\exp\{\mathbf{w}_{ij}\boldsymbol{\rho}\}$, for example.

For simplicity, let us assume as in \cite{griffith2019namefriends} that each link has the same probability of being censored. Then, the parameters in $\boldsymbol{\rho}$ (other than the constant) are identified from the observed ratios $\sum_{ij}a_{ij}{w}^k_{ij}/\sum_{ij}{w}^k_{ij}$ (for observable characteristic $k$), as these sufficient statistics are not biased by censoring. To identify the constant, note that we can easily compute the likelihood of the censored degree distribution (i.e. $n_i=\sum_ja_{ij}$). That is $P(n_i=t|\mathbf{W};\boldsymbol{\rho})$ for observed $t<T$ and $P(n_i\geq T|\mathbf{W};\boldsymbol{\rho})$ for observed $t=T$, which allows identifying the constant.\footnote{A simple alternative, when the data of only a few individuals is censored, is to estimate the model only for individuals for whom $n_i<T$. We follow this strategy in Section \ref{sec:addhealth}.}

Once such estimator of $\boldsymbol{\rho}$ is obtained, we can compute an estimator for the distribution of the true network $\hat{P}(\mathbf{A})=P(\mathbf{A}|\hat{\boldsymbol{\rho}},\mathcal{A})$. In particular, ${P}(a_{ij}|\hat{\boldsymbol{\rho}},a_{ij}^{obs}=1)=1$ because observed links necessarily exist. Also note that for all individuals $i$, such that $n_i<T$, we have ${P}(a_{ij}|\hat{\boldsymbol{\rho}},a_{ij}^{obs})=a_{ij}^{obs}$ for all $j$, as their network data are not censored. Here, the structural model is only used to obtain the probability of links that are not observed for individuals whose links are potentially censored, i.e. ${P}(a_{ij}|\hat{\boldsymbol{\rho}},a_{ij}^{obs}=0)\propto \exp\{a_{ij}\mathbf{w}_{ij}\hat{\boldsymbol{\rho}}\}$ for all $ij$, such that $n_i\geq T$.

\end{example}

\begin{example}[Misclassification]\label{ex:misclass}
\cite{hardy2019estimating} study cases in which networks are observed but may include misclassified links (i.e. false positives and false negatives). Here, $\mathcal{A}$ can be represented by an $N\times N$ binary matrix $\mathbf{A}^{mis}$. The (consistent) estimation of (\ref{eq:gennetfor}) in such a context follows directly from the existing literature on misclassification in binary outcome models, e.g. \cite{hausman1998misclassification}.

Let $q_1$ be the probability of false positives and $q_0$ be the probability of false negatives (both being elements of $\boldsymbol{\rho}$). The estimator for the distribution of the true network is given by $P(a_{ij}=1|\hat{\boldsymbol{\rho}},a_{ij}^{mis})=a_{ij}^{mis}(1-\hat{q}_1) + (1-a_{ij}^{mis})\hat{q}_0$.
\end{example}

\begin{example}[Aggregated Relational Data]\label{ex:ard}
Aggregated relational data (ARD) are obtained from survey questions such as, ``How many friends with trait `X' do you have?'' Here, $\mathcal{A}$ can be represented by an $N\times K$ matrix of integer values, where $K$ is the number of traits that individuals were asked about.

Building on \cite{mccormick2015latent}, \cite{breza2017using} proposed a novel approach for the estimation of network formation models using only ARD. They assume:
\begin{equation}\label{eq:exard}
P(a_{ij}=1)\propto\exp\{\nu_i+\nu_j+\zeta \mathbf{z}_i'\mathbf{z}_j\},    
\end{equation}
where $\nu_i$, $\nu_j$, $\zeta$, $\mathbf{z}_i$, and $\mathbf{z}_j$ are not observed by the econometrician but follow parametric distributions. Here, parameters $\nu_i$ and $\nu_j$ can be interpreted as $i$ and $j$'s propensities to create links, irrespective of the identity of the other individual involved. The other component, $\zeta \mathbf{z}_i'\mathbf{z}_j$, is meant to capture homophily (like attracts like) on an abstract latent space (e.g. \cite{hoff2002latent}).

\cite{breza2017using} show that it is possible to use aggregate relational data (ARD) to recover the values of the variables in (\ref{eq:exard}). In particular, letting $\boldsymbol{\rho}=[\{\nu_i\}_i,\{\mathbf{z}_i\}_i,\zeta]$, \cite{breza2019consistently} provide sufficient conditions for the consistent estimation of $\boldsymbol{\rho}$.

Contrary to Examples \ref{ex:sampled}--\ref{ex:misclass}, ARD does not provide information on any specific links; \footnote{That is, unless ARD include the degree distribution with some individuals reporting having no links at all.} therefore, the predicted distribution of the true network is $P(a_{ij}|\hat{\boldsymbol{\rho}},\mathcal{A})=P(a_{ij}|\hat{\boldsymbol{\rho}})$, which is given by Equation (\ref{eq:exard}). Here, it is worth emphasizing that the observed network information (i.e. ARD) is not very informative about the particular network structure in the data. In this sense, it could be viewed as a worse case scenario.
\end{example}

==> archives/shortversion__copy_/addhealth.tex <==

\section{Imperfectly Measured Networks}\label{sec:addhealth}

In this section, we assume that the econometrician has access to network data but that the data may contain errors. To show how our method can be used to address these issues, we consider a simple example where we are interested in estimating peer effects on adolescents' academic achievements.

We use the widely used AddHealth database and show that network data errors have a first-order impact on the estimated peer effects. Specifically, we focus on a subset of schools from the ``In School'' sample that each have less than 200 students. Table \ref{tab:sumstats} displays the summary statistics.

\begin{table}[!htbp] 
   \centering 
  \caption{Summary statistics.} 
  \label{tab:sumstats} 
\begin{tabular}{@{\extracolsep{5pt}} lld{3}ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
\multicolumn{2}{l}{Statistic} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} \\ 
\hline \\[-1.8ex] 
\multicolumn{2}{l}{Female} & 0.540 & 0.498 & 0 & 1 \\ 
\multicolumn{2}{l}{Hispanic}  & 0.157 & 0.364 & 0 & 0 \\ 
\multicolumn{2}{l}{Race} &  &  &  &  \\ 
 & White & 0.612 & 0.487 & 0 & 1 \\ 
 & Black & 0.246 & 0.431 & 0 & 0 \\ 
 & Asian & 0.022 & 0.147 & 0 & 0 \\ 
 & Other & 0.088 & 0.283 & 0 & 0 \\ 
\multicolumn{2}{l}{Mother's education}  &  &  &  &  \\ 
 & High & 0.310 & 0.462 & 0 & 1 \\ 
 & <High & 0.193 & 0.395 & 0 & 0 \\ 
 & >High & 0.358 & 0.480 & 0 & 1 \\ 
 & Missing & 0.139 & 0.346 & 0 & 0 \\ 
\multicolumn{2}{l}{Mother's job}  &  &  &  &  \\ 
 & Stay-at-home & 0.225 & 0.417 & 0 & 0 \\ 
 & Professional & 0.175 & 0.380 & 0 & 0 \\ 
 & Other & 0.401 & 0.490 & 0 & 1 \\ 
 & Missing & 0.199 & 0.399 & 0 & 0 \\ 
\multicolumn{2}{l}{Age}  & 13.620 & 1.526 & 13 & 14 \\ 
\multicolumn{2}{l}{GPA}  & 2.912    &0.794    &2.333      &3.5\\ 
\hline \\[-1.8ex] 
\multicolumn{6}{l}{%
  \begin{minipage}{11.6cm}%
    \footnotesize{Note: We only keep the 33 schools having less than 200 students from the In-School sample. The variable GPA is computed by taking the average grade for English, Mathematics, History, and Science, letting $A=4$, $B=3$, $C=2$, and $D=1$. Thus, higher scores indicate better academic achievement.}
  \end{minipage}%
  }
\end{tabular} 

\end{table} 

Most of the papers estimating peer effects that use this particular database have taken the network structure as given. One notable exception is \cite{griffith2019namefriends}, looking at censoring: students can only report up to five male and five female friends. We also allow for censoring but show that censoring is not the most important issue with the Add Health data. To understand why, we discuss the organization of the data.

Each adolescent is assigned a unique identifier. The data includes ten variables for the ten potential friendships (maximum of five male and five female friends). These variables can contain missing values (no friendship was reported), an error code (the named friend could not be found in the database), or an identifier for the reported friends. This data is then used to generate the network's adjacency matrix $\mathbf{A}$.

Of course, error codes cannot be matched to any particular adolescent; as well, even in the case where the friendship variable refers to a valid identifier, the referred adolescent may still be absent from the database. A prime example is when the referred adolescent has been removed from the database by the researcher, perhaps due to other missing variables for these particular individuals. These missing links are quantitatively important as they account for roughly 30\% of the total number of links (7,830 missing for 17,993 observed links). Figure \ref{fig:misfr} displays the distribution of the number of ``unmatched named friends.''\footnote{We focus on within-school friendships; thus, nominations outside of school are not treated as ``unmatched friends.''}
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.6]{graphs/Missing.pdf}
    \caption{Frequencies of the number of missing links per adolescent.}
    \label{fig:misfr}
\end{figure}

To use the methodology developed in Section \ref{sec:genestim}, we first need to estimate a network formation model using the observed network data. In this section, we assume that links are generated using a simple logistic framework, i.e.
$$
P(a_{ij}=1)\propto\exp\{\mathbf{w}_{ij}\boldsymbol{\rho}\},
$$
where $\mathbf{w}_{ij}$ is built to capture homophily on the observed characteristics of $i$ and $j$ (see Table \ref{tab:application}). We estimate the network formation model on the set of individuals who nominate strictly less than five male and five female friends and for which we observe no ``unmatched friends.'' For these students, we know for sure that their friendship data is complete. Under a missing at random assumption, the estimation is consistent.

Table \ref{tab:application} presents the estimation results for the network formation model (panel \emph{Network Formation}), as well as for the peer effect model (panel \emph{Peer Effect Model}, column \emph{Reconstructed Network}). We also present the results for the (inconsistent) estimation of the peer effect model under the assumption that the observed network is the true one (panel \emph{Peer Effect Model}, column \emph{Observed Network}).

We find evidence of homophily on all observed covariates, which is coherent with the literature (e.g. \cite{currarini2010identifying,boucher2017my,mele2020does}). The bias on the peer effects' coefficients (endogenous and contextual) is qualitatively important (and statistically significant). The estimated endogenous peer effect using the reconstructed network is 1.6 times larger than the one estimated assuming that the observed network is the true network. The reconstructed network also allows capturing a positive effect of having a high proportion of Hispanic friends on academic achievement.

The contribution of censoring to these biases is insignificant. In Table \ref{tab:appendapplication} of the Online Appendix, we report estimates for two alternative cases: one in which we disregard censoring and another in which censoring is the only data issue. The impact of controlling for censoring is almost null, coherent with the fact that only about 5\% of the observations are potentially censored.

Our exercise shows that data errors are a first-order concern when using the Add Health database. We do not argue, however, that our estimated coefficients in Table \ref{tab:application} are necessarily causal because the friendship network is likely endogenous (e.g. \cite{goldsmith2013social,hsieh2018smoking,hsieh2019specification}). The estimation of peer effects with partial endogenous network data is left for future research but is discussed in the next section.

\begin{table}[]
\small
\centering
\caption{Posterior distribution.} 
\label{tab:application} 
  \begin{adjustbox}{max width=0.85\textwidth}
\begin{tabular}{lld{5}d{3}d{3}d{5}d{3}d{3}}
\\[-1.8ex]
\toprule
      &       & \multicolumn{3}{c}{Observed network} & \multicolumn{3}{c}{Reconstructed network} \\\hline\hline
\multicolumn{2}{l}{Statistic} & \multicolumn{1}{c}{Mean}  & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{\textit{t}-stat} & \multicolumn{1}{c}{Mean}  & \multicolumn{1}{c}{Std. Dev.} & \multicolumn{1}{c}{\textit{t}-stat} \\\hline\\[-1.8ex]
\midrule
                          & \multicolumn{7}{c}{\textbf{Peer effect model}}  \\ \\[-2ex]
\multicolumn{2}{l}{Peer effects}                       & 0.350***    & (0.024)    & 14.809    & 0.564***      & (0.044)      & 12.842     \\
\multicolumn{2}{l}{\textbf{Own effects}}               &             &            &           &               &              &            \\
\multicolumn{2}{l}{Female}                      & 0.144***   & (0.029)    & 5.018    & 0.120***     & (0.031)      & 3.822     \\
\multicolumn{2}{l}{Hispanic}                    & -0.083**     & (0.042)    & -1.980     & -0.145**       & (0.047)      & 3-.090      \\
\multicolumn{2}{l}{Race (White)}                &             &            &           &               &              &            \\
                          & Black               & -0.230***    & (0.045)    & -5.070     & -0.210***      & (0.055)      & -3.787      \\
                          & Asian               & -0.091       & (0.089)    & -1.024     & -0.115         & (0.089)      & -1.286      \\
                          & Other               & 0.055      & (0.051)    & 1.064    & 0.036        & (0.052)      & 0.686     \\
\multicolumn{2}{l}{Mother's education (High)}            &             &            &           &               &              &            \\
                          & \textless high      & -0.122**     & (0.039)    & -3.147     & -0.126**       & (0.039)      & -3.201      \\
                          & \textgreater high   & 0.140***   & (0.034)    & 4.131    & 0.109**      & (0.034)      & 3.208     \\
                          & missing             & -0.060       & (0.050)    & -1.182     & -0.065         & (0.051)      & -1.277      \\
\multicolumn{2}{l}{Mother's job (Stay-at-home)}         &             &            &           &               &              &            \\
                          & Professional        & 0.080*     & (0.045)    & 1.793    & 0.078*       & (0.044)      & 1.759     \\
                          & Other               & 0.003      & (0.035)    & 0.078    & -0.006         & (0.035)      & -0.168      \\
                          & Missing             & -0.066       & (0.047)    & -1.400     & -0.068         & (0.048)      & -1.427      \\
\multicolumn{2}{l}{Age}                         & -0.073***    & (0.010)    & -7.606     & -0.078***      & (0.011)      & -7.168      \\
\multicolumn{2}{l}{\textbf{Contextual effects}}          &             &            &           &               &              &            \\
\multicolumn{2}{l}{Female}                      & 0.011      & (0.049)    & 0.221    & 0.072        & (0.092)      & 0.779     \\
\multicolumn{2}{l}{Hispanic}                    & 0.060      & (0.069)    & 0.868    & 0.353**      & (0.115)      & 3.081     \\
\multicolumn{2}{l}{Race (White)}                &             &            &           &               &              &            \\
                          & Black               & 0.050      & (0.058)    & 0.865    & 0.058        & (0.075)      & 0.769     \\
                          & Asian               & 0.209      & (0.186)    & 1.126    & 0.518        & (0.579)      & 0.895     \\
                          & Other               & -0.137       & (0.089)    & -1.537     & -0.230         & (0.185)      & -1.241      \\
\multicolumn{2}{l}{Mother's education (High)}            &             &            &           &               &              &            \\
                          & \textless High      & -0.269***    & (0.070)    & -3.841     & -0.363**       & (0.158)      & -2.290      \\
                          & \textgreater High   & 0.072      & (0.059)    & 1.213    & 0.062        & (0.114)      & 0.540     \\
                          & Missing             & -0.077       & (0.093)    & -0.835     & -0.025         & (0.197)      & -0.128      \\
\multicolumn{2}{l}{Mother's job (Stay-at-home)}         &             &            &           &               &              &            \\
                          & Professional        & -0.110       & (0.080)    & -1.373     & 0.032        & (0.157)      & 0.204     \\
                          & Other               & -0.101*      & (0.060)    & -1.686     & -0.051         & (0.114)      & -0.451      \\
                          & Missing             & -0.093       & (0.085)    & -1.086     & -0.006         & (0.188)      & -0.029      \\
\multicolumn{2}{l}{Age}                         & 0.066***   & (0.006)    & 11.323   & 0.091***     & (0.010)      & 9.228     \\
\midrule
SE$^2$     &                     & 0.523       &            &           & 0.515         &              &            \\\\[-1.8ex]
\midrule
                          & \multicolumn{7}{c}{\textbf{Network formation model}}                                                            \\\\[-2ex]
\multicolumn{2}{l}{Same sex}                    &             &            &           & 0.456***      & (0.016)      & 28.208     \\
\multicolumn{2}{l}{Both Hispanic}               &             &            &           & 0.343***      & (0.023)      & 14.739     \\
\multicolumn{2}{l}{Both White}                  &             &            &           & 0.320***      & (0.022)      & 14.741     \\
\multicolumn{2}{l}{Both Black}                  &             &            &           & 1.167***      & (0.032)      & 36.121     \\
\multicolumn{2}{l}{Both Asian}                  &             &            &           & 0.278***      & (0.043)      & 6.502      \\
\multicolumn{2}{l}{Mothers education \textless High}    &             &            &           & 0.178***      & (0.018)      & 10.063     \\
\multicolumn{2}{l}{Mothers education \textgreater High} &             &            &           & 0.075***      & (0.016)      & 4.756      \\
\multicolumn{2}{l}{Mothers job Professional}       &             &            &           & -0.130***     & (0.017)      & -7.544     \\
\multicolumn{2}{l}{Age absolute difference}           &             &            &           & -0.648***     & (0.010)      & -64.105   \\
\bottomrule
\\
\multicolumn{8}{l}{%
  \begin{minipage}{16cm}%
  \vspace{0.1cm}
    \footnotesize{Note: \textit{N} = 3,126. Observed links = 17,993. Proportion of inferred network data = 77.7\%. Significance levels: $^{***} = 1$\%,   $^{**} = 5$\%, $^* = 10$\%. The explained variable is computed by taking the average grade for English, Mathematics, History, and Science, letting $A=4$, $B=3$, $C=2$, and $D=1$. Thus, higher scores indicate better academic achievement.}
  \end{minipage}%
}\\
\end{tabular} 
\end{adjustbox}
\end{table} 

==> iv_backup_parts.tex <==

\section{Temporary}
Once the network distribution is estimated, a simple and intuitive (but invalid) approach to estimating peer effects is to replace the true network in the classical moment function of the linear-in-means peer effects model \citep[see][]{bramoulle2009identification} with a simulated network from the estimated distribution. What follows also holds if one simulates many networks and takes the average of corresponding moment functions.

For each group $m$, this approach leads to the moment function:
\[
\dot{\mathbf m}_m (\boldsymbol{\theta}) = \dot{\mathbf Z}_m^{\prime}(\mathbf y_m - \alpha \dot{\mathbf G}_m \mathbf y_m - c\mathbf{1}_m - \mathbf X_m\boldsymbol{\beta} - \dot{\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}),
\]
where $\boldsymbol{\theta} = (\alpha, ~c, ~\boldsymbol{\beta}^{\prime}, ~\boldsymbol{\gamma}^{\prime})^{\prime}$, $\dot{\mathbf G}_m = f(\dot{\mathbf A}_m)$, $\dot{\mathbf A}_m$ is the simulated network from the estimated distribution, and $\mathbf 1_m$ is an $n_m$-dimensional vector of ones. By substituting $\mathbf y_m$ with its specification given in \eqref{eq:linearinmean}, we obtain:
\begin{align}
\begin{split}
    \dot{\mathbf m}_m (\boldsymbol{\theta}) &= \dot{\mathbf Z}_m^{\prime} \big[(\mathbf I_m - \alpha \dot{\mathbf G}_m )(\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}(c_0\mathbf{1}_m + \mathbf X_m\boldsymbol{\beta}_0 + {\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}_0 + \boldsymbol{\varepsilon}_m)\\
    &\hspace{1.5cm} - c\mathbf{1}_m - \mathbf X_m\boldsymbol{\beta} - \dot{\mathbf G}_m\mathbf X_m\boldsymbol{\gamma} \big],
\end{split} \label{eq:dotm}
\end{align}
where the subscript $0$ denotes the true parameter values, and $\mathbf I_m$ is the $n_m \times n_m$ identity matrix. Although $\mathbb{E}[\boldsymbol{\varepsilon}_m|\mathbf{X}_m,\mathcal{A}_m]=\mathbf{0}$ (Assumption \ref{as:exonet}), it is clear that $\mathbb{E}[\dot{\mathbf m}_m (\boldsymbol{\theta}_0)] \neq \mathbf{0}$ in general (even asymptotically), unless $\dot{\mathbf G}_m = \mathbf G_m$ for all $m$. Indeed, $\dot{\mathbf G}_m$ is not a consistent estimator of $\mathbf G_m$. Importantly, this issue is not resolved by simulating multiple $\dot{\mathbf G}_m$ and averaging the corresponding moment functions $\dot{\mathbf m}_m (\boldsymbol{\theta})$.


We denote by \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) the term in square brackets in \eqref{eq:dotm}, so that \( \dot{\mathbf{m}}_m (\boldsymbol{\theta}) = \dot{\mathbf{Z}}_m^{\prime} \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \). The sources of the inconsistency of \( \dot{\mathbf{m}}_m \) are twofold. First, \( \dot{\mathbf{Z}}_m \) and \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}_0) \) are correlated, as they depend on the same simulation \( \dot{\mathbf{G}}_m \). Second, even if \( \dot{\mathbf{Z}}_m \) and \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}_0) \) were independent, \( \mathbb{E}(\dot{\boldsymbol{\varepsilon}}_m | \mathbf{X}_m, \mathcal{A}_m) \neq \mathbf{0} \) (even asymptotically) because \( \dot{\mathbf{G}}_m \) is not a consistent estimator of \( \mathbf{G}_m \). For a moment function of the form \( \dot{\mathbf{Z}}_m^{\prime} \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \), the desired properties are that \( \dot{\mathbf{Z}}_m \) and \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) are independent and that \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) is centered (conditional on the observable exogenous variables).



To address the first issue, it is sufficient to use two different simulations for \( \dot{\mathbf{Z}}_m \) and \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \). We then replace \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) with some \( \ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \), which has the same expression as \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) with the difference that \( \dot{\mathbf{G}}_m \) is replaced with a new simulated network \( \ddot{\mathbf{G}}_m \). This guarantees that \( \dot{\mathbf{Z}}_m \) and \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) are independent conditional on \( \mathbf{X}_m \) and \( \mathcal{A}_m \). We thus have a new moment function, which is \( \ddot{\mathbf{m}}_m (\boldsymbol{\theta}) = \dot{\mathbf{Z}}_m^{\prime} \ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \).


As now \( \mathbb{E} (\ddot{\mathbf{m}}_m (\boldsymbol{\theta})|\mathbf{X}_m, \mathcal{A}_m) = \mathbb{E} (\dot{\mathbf{Z}}_m^{\prime}|\mathbf{X}_m, \mathcal{A}_m) \mathbb{E} [\ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta})|\mathbf{X}_m, \mathcal{A}_m] \), we only need to "force" \( \mathbb{E} (\ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}_0)) \) to be zero to establish consistency. To achieve this, we can replace \( \ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \) with the \textit{unfeasible} debiased equivalent \( \ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) - \mathbb{E} [\ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta})|\mathbf{X}_m, \mathcal{A}_m, \ddot{\mathbf{G}}_m, \mathbf{G}_m] \). This debiasing approach is unfeasible since the removed bias is conditional on the unobserved true network matrix \( \mathbf{G}_m \) and the true parameters. We condition on \( \mathbf{G}_m \) only to make the computation of the removed bias easier. The resulting expression then depends on \( \mathbf{G}_m \), which can be approximated using a third simulated network.


From \eqref{eq:dotm}, we have:
\begin{align}
    &\mathbb E [\ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta})|\mathbf{X}_m,\mathcal{A}_m, \ddot{\mathbf G}_m, \mathbf G_m]  = (\mathbf I_m - \alpha \ddot{\mathbf G}_m )(\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}(c_0\mathbf{1}+ \mathbf X_m\boldsymbol{\beta}_0 + {\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}_0) \nonumber\\
    &\hspace{5.5cm}- c\mathbf{1}_m- \mathbf X_m\boldsymbol{\beta} - \ddot{\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}, \nonumber\\
    &\ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) - \mathbb E [\ddot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta})|\mathbf{X}_m,\mathcal{A}_m, \ddot{\mathbf G}_m, \mathbf G_m] = (\mathbf I_m - \alpha \ddot{\mathbf G}_m)\mathbf y_m -c\mathbf{1}_m- \mathbf X_m\boldsymbol{\beta} - \ddot{\mathbf G}_m\mathbf X_m\boldsymbol{\gamma} \nonumber\\
    & ~- (\mathbf I_m - \alpha \ddot{\mathbf G}_m )(\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}(c_0\mathbf{1}+ \mathbf X_m\boldsymbol{\beta}_0 + {\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}_0) + c\mathbf{1}_m- \mathbf X_m\boldsymbol{\beta} - \ddot{\mathbf G}_m\mathbf X_m\boldsymbol{\gamma},\nonumber \\
    &= (\mathbf I_m - \alpha \ddot{\mathbf G}_m)(\mathbf y_m - (\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}(c_0\mathbf{1}+ \mathbf X_m\boldsymbol{\beta}_0 + {\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}_0) \label{eq:debaisederror}
\end{align}
The feasible equivalent of \eqref{eq:debaisederror} that can lead to similar properties asymptotically is:
$$
    (\mathbf{I}_m - \alpha \ddot{\mathbf{G}}_m)\left(\mathbf{y}_m - (\mathbf{I}_m - \alpha \dddot{\mathbf{G}}_m)^{-1}(c\mathbf{1} + \mathbf{X}_m \boldsymbol{\beta} + \dddot{\mathbf{G}}_m \mathbf{X}_m \boldsymbol{\gamma})\right).
$$
We replace \( \mathbf{G}_m \) with a new independent simulation to preserve the independence between \( \mathbf{G}_m \) and the first two initial simulated networks. Our consistent moment function then becomes:
\begin{equation} \label{eq:moment:3simu}
\dot{\mathbf{Z}}_m^{\prime}(\mathbf{I}_m - \alpha \ddot{\mathbf{G}}_m)\left(\mathbf{y}_m - (\mathbf{I}_m - \alpha \dddot{\mathbf{G}}_m)^{-1}(c\mathbf{1} + \mathbf{X}_m \boldsymbol{\beta} + \dddot{\mathbf{G}}_m \mathbf{X}_m \boldsymbol{\gamma})\right).
\end{equation}


Another approach is to directly correct the bias of the initial function \( \dot{\mathbf{m}}_m (\boldsymbol{\theta}) = \dot{\mathbf{Z}}_m^{\prime} \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}) \). In this case, an unfeasible debiased moment function can be:
\begin{align}
    &\dot{\mathbf m}_m (\boldsymbol{\theta}) - \mathbb{E}[\dot{\mathbf m}_m (\boldsymbol{\theta})|\mathbf{X}_m, \mathcal{A}_m, \dot{\mathbf{G}}_m, \mathbf{G}_m] = \nonumber\\
    &\dot{\mathbf Z}_m^{\prime}(\mathbf I_m - \alpha \dot{\mathbf G}_m ) \big[\mathbf y_m - (\mathbf I_m - \alpha_0 \mathbf G_m )^{-1}(c_0\mathbf{1}_m + \mathbf X_m\boldsymbol{\beta}_0 + {\mathbf G}_m\mathbf X_m\boldsymbol{\gamma}_0)\big].\nonumber
\end{align}
The feasible equivalent of this moment function is thus:
\begin{equation} \label{eq:moment:2simu}
\dot{\mathbf Z}_m^{\prime}(\mathbf I_m - \alpha \dot{\mathbf G}_m ) \big[\mathbf y_m - (\mathbf I_m - \alpha \ddot{\mathbf G}_m )^{-1}(c\mathbf{1}_m + \mathbf X_m\boldsymbol{\beta} + \ddot{\mathbf G}_m\mathbf X_m\boldsymbol{\gamma})\big].
\end{equation}
While both moment functions \eqref{eq:moment:3simu} and \eqref{eq:moment:2simu} lead to consistent estimators, it can be shown that \eqref{eq:moment:3simu} is more efficient because its variance is lower. The intuition is as follows. Bias correction is generally associated with a loss of efficiency. With \( \dot{\mathbf{m}}_m (\boldsymbol{\theta}) \), we mechanically correct both the bias stemming from the dependence between \( \dot{\mathbf{Z}}_m \) and \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}_0) \), as well as the bias due to the fact that \( \dot{\boldsymbol{\varepsilon}}_m(\boldsymbol{\theta}_0) \) is not centered. In contrast, our proposed moment function \eqref{eq:moment:3simu} no longer suffers from the first bias, and we only correct for the second bias mechanically.

Both moment functions have the form \(\dot{\mathbf Z}_m^{\prime}\mathbf u_m\) and \(\dot{\mathbf Z}_m^{\prime}\tilde{\mathbf u}_m\), where \(\mathbf u_m\) and \(\tilde{\mathbf u}_m\) are the terms that post-multiply \(\dot{\mathbf Z}_m^{\prime}\) in \eqref{eq:moment:3simu} and \eqref{eq:moment:2simu}, respectively. Although \(\mathbf u_m\) and \(\tilde{\mathbf u}_m\) have different expressions, they share the same distribution. Indeed, \(\mathbf u_m\) can be written as a function of \(\ddot{\mathbf G}_m\) and \(\dddot{\mathbf G}_m\), whereas \(\tilde{\mathbf u}_m\) can be written as the same function of \(\dot{\mathbf G}_m\) and \(\ddot{\mathbf G}_m\). Since the simulated networks have the same distribution, it follows that \(\mathbf u_m\) and \(\tilde{\mathbf u}_m\) also have the same distribution.

We aim to compare the variance of \(\dot{\mathbf Z}_m^{\prime}\mathbf u_m\) to the variance of \(\dot{\mathbf Z}_m^{\prime}\tilde{\mathbf u}_m\) in a situation where \(\mathbf u_m\) and \(\tilde{\mathbf u}_m\) have the same distribution, \(\tilde{\mathbf u}_m\) is correlated with \(\dot{\mathbf Z}\), and \(\mathbf u_m\) is independent of \(\dot{\mathbf Z}\), conditional on \(\mathbf{X}_m\) and \(\mathcal{A}_m\). Indeed, \(\dot{\mathbf Z}\) and \(\tilde{\mathbf u}_m\) are correlated because they depend on the same simulated network \(\dot{\mathbf G}_m\).

To simplify the comparison of the variances of \(\dot{\mathbf Z}_m^{\prime}\mathbf u_m\) and \(\dot{\mathbf Z}_m^{\prime}\tilde{\mathbf u}_m\), we assume that \(\dot{\mathbf Z}_m\), \(\mathbf u_m\), and \(\tilde{\mathbf u}_m\) are scalars. (It is possible to generalize the result by applying what follows to each entry of the variances, but the notation would become cumbersome.) Let \(\mathbb{V}_1\) and \(\mathbb{V}_2\) be the variances of \(\dot{\mathbf Z}_m^{\prime}\mathbf u_m\) and \(\dot{\mathbf Z}_m^{\prime}\tilde{\mathbf u}_m\), respectively, conditional on \(\mathbf{X}_m\) and \(\mathcal{A}_m\). We have:
\begin{align*}
    \mathbb{V}_2 - \mathbb{V}_1 &= \mathbb{E}(\dot{\mathbf Z}_m^2\tilde{\mathbf u}_m^2|\mathbf{X}_m, \mathcal{A}_m) -  \mathbb{E}(\dot{\mathbf Z}_m^2\mathbf u_m^2|\mathbf{X}_m, \mathcal{A}_m),\\
    \mathbb{V}_2 - \mathbb{V}_1 &= \mathbb{E}(\dot{\mathbf Z}_m^2\tilde{\mathbf u}_m^2|\mathbf{X}_m, \mathcal{A}_m) -  \mathbb{E}(\dot{\mathbf Z}_m^2|\mathbf{X}_m, \mathcal{A}_m)\mathbb{E}(\mathbf u_m^2|\mathbf{X}_m, \mathcal{A}_m),\\
    \mathbb{V}_2 - \mathbb{V}_1 &= \mathbb{E}(\dot{\mathbf Z}_m^2\tilde{\mathbf u}_m^2|\mathbf{X}_m, \mathcal{A}_m) -  \mathbb{E}(\dot{\mathbf Z}_m^2|\mathbf{X}_m, \mathcal{A}_m)\mathbb{E}(\tilde{\mathbf u}_m^2|\mathbf{X}_m, \mathcal{A}_m),\\
    \mathbb{V}_2 - \mathbb{V}_1 &= \operatorname{Cov}(\dot{\mathbf Z}_m^2, ~\tilde{\mathbf u}_m^2|\mathbf{X}_m, \mathcal{A}_m).
\end{align*}
In the third equality, we replace 
\(\mathbb{E}(\mathbf{u}_m^2 \mid \mathbf{X}_m, \mathcal{A}_m)\) 
with 
\(\mathbb{E}(\tilde{\mathbf{u}}_m^2 \mid \mathbf{X}_m, \mathcal{A}_m)\) 
because \(\mathbf{u}_m\) and \(\tilde{\mathbf{u}}_m\) share the same distribution. 
Thus, the moment function with two simulated networks performs better if 
\(\dot{\mathbf{Z}}_m^2\) and \(\tilde{\mathbf{u}}_m^2\) are positively correlated, 
conditional on \(\mathbf{X}_m\) and \(\mathcal{A}_m\). 
This is straightforward to see when there are no contextual effects, 
as both \(\dot{\mathbf{Z}}_m\) and \(\tilde{\mathbf{u}}_m\) are linear in \(\dot{\mathbf{G}}_m\). 
Moreover, \(\dot{\mathbf{Z}}_m^2\) and \(\tilde{\mathbf{u}}_m^2\) remain positively correlated 
regardless of the sign of \(\alpha\).




\section{Simulated Generalized Method of Moment Estimators}\label{sec:iv}


%Note that we can use $\hat{P}(\mathbf{A}_m)$ implicitly defines the analog $\hat{P}(\mathbf{G}_m)$ because $\mathbf{G}_m=f(\mathbf{A}_m)$ for some known function $f$.\footnote{Because $\mathbf{A}_m$ takes a finite number of values (the size of group $m$ is bounded), so does $\mathbf{G}_m$, (thus $\mathbf{A}_m$ and $\mathbf{G}_m$ have multinomial distributions). Then, $P(\mathbf{G}_m)$ is a continuous function of $P(\mathbf{A}_m)$, irrespective of the function $f$ linking $\mathbf{A}_m$ and $\mathbf{G}_m$.}


In this section, we present an estimator based on a Simulated Generalized Method of Moments (SGMM). The key observation underlying our approach is that it is not necessary to observe the complete network structure to observe $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$. For example, one could simply obtain ${\mathbf{Gy}}$ from survey data, ``What is the average value of your friends' $y$?''

However, even observing $\mathbf{y}$, $\mathbf{X}$, ${\mathbf{GX}}$, and ${\mathbf{Gy}}$, the model (\ref{eq:linearinmean}) cannot be simply estimated using simple linear regression. The reason is that ${\mathbf{Gy}}$ is endogenous; thus, a linear regression would produce biased estimates (e.g. \cite{manski1993identification}, \cite{bramoulle2009identification}).

The typical instrumental approach to deal with this endogeneity is to use instruments based on the structural model, i.e. instruments constructed using second-degree peers (e.g. $\mathbf{G}^2\mathbf{X}$, see \cite{bramoulle2009identification}). These are less likely to be found in survey data. Indeed, we could doubt the informativeness of questions such as, ``What is the average value of your friends' average value of their friends' $x$?''

However, the above discussion is encouraging. When researchers observe $[\mathbf{y}, \mathbf{X}]$ and $[{\mathbf{GX}},{\mathbf{Gy}}]$, information about the network is only used as a means to construct a valid instrument, e.g. following \citet{bramoulle2009identification}. Then, if $\mathbf{GX}$ and $\mathbf{Gy}$ are observed, the estimation of peer effects is possible using any exogeneous (strong) predictor of the true network structure, as in \cite{kelejian2014estimation}, \cite{konig2019r}, and \cite{lee2020key}.\footnote{See Proposition \ref{prop:all_observed} of the Online Appendix \ref{sec:appendix_otherresults} for a formal statement. In particular, one needs a predictor of the network such that the resulting instrument is not correlated with $\boldsymbol{\varepsilon}$ and is strongly correlated with $\mathbf{Gy}$.}

The problem is more challenging when $\mathbf{Gy}$ and $\mathbf{GX}$ are not observed.



Finally, for any matrix $\mathbf{B}$, we will use $\mathbf{B}_i$ to denote the $i$th row of $\mathbf{B}$.

Before presenting our estimation strategy, we want to emphasize that we cannot simply proxy $\mathbf{Gy}$ and $\mathbf{GX}$ using draws from $\hat{P}(\mathbf{G})$. To see why, consider the simple case for which $\boldsymbol{\gamma}=\mathbf{0}$, so that the observation of $\mathbf{GX}$ is inconsequential. We have, substituting $\mathbf{Gy}$ with $\ddot{\mathbf{G}}\mathbf{y}$,
$$
\mathbf{y}=c\mathbf{1}+\mathbf{X}\boldsymbol{\beta}+\alpha\ddot{\mathbf{G}}\mathbf{y}+[\boldsymbol{\eta}+\boldsymbol{\varepsilon}],
$$
where $\boldsymbol{\eta}=\alpha[\mathbf{G}-\ddot{\mathbf{G}}]\mathbf{y}$ is the error due to the approximation of $\mathbf{Gy}$ by $\ddot{\mathbf{G}}\mathbf{y}$. Importantly, the approximation error does \emph{not} vanish as $N$ grows because individuals belong to bounded groups (see Assumption \ref{as:manymarkets}).\footnote{As opposed to, for example, the context studied by \cite{auerbach2019measuring}.} Moreover, because $\mathbf{y}$ is a function of $\mathbf{G}$ (but not of $\ddot{\mathbf{G}}$), we typically have $\mathbb{E}(\mathbf{Gy})_i|\mathbf{Z}_i\neq\mathbb{E}(\ddot{\mathbf{G}}\mathbf{y})_i|\mathbf{Z}_i$ for some vector of instruments $\mathbf{z}_i$ and all $i$.


In Proposition \ref{prop:bias_nocontext} of the Online Appendix \ref{sec:appendix_otherresults}, we show, using an argument very similar to that of \cite{andrews2017measuring}, that the asymptotic bias induced by $\mathbb{E}\eta_i|\mathbf{z}_i\neq 0$ can be bounded, and simulations show that it can be very small for carefully constructed vectors of instruments, which can be useful in practice.

In any case, in our main result below, we show that we can include the bias directly in the moment function; this provides a consistent estimator of $\boldsymbol{\theta}$.

\subsection{Main Result}
Let $\tilde{\boldsymbol{\theta}}=[c,\boldsymbol{\beta}',\boldsymbol{\gamma}']'$.  We present the following simulated general method of moment estimator. Theorem \ref{prop:non_observed} defines the moment function and shows the consistency of the estimator. Theorem ?? shows the asymptotic normality for a large class of first-stage estimators. 

\begin{theorem}[SGMM - Consistency]\label{prop:non_observed} Suppose that Assumptions \ref{as:alpha}--\ref{as:partial} and regularity conditions \ref{as:regularity}--\ref{as:Wm} hold. Suppose also that the identification condition \ref{as:identification} hold

[Conditions] Let $\dot{\mathbf{Z}}^{(r)}_m=[\mathbf{1},\mathbf{X}_m,\dot{\mathbf{G}}^{(r)}_m\mathbf{X}_m,(\dot{\mathbf{G}}^{(r)}_m)^2\mathbf{X}_m,(\dot{\mathbf{G}}_m^{(r)})^3\mathbf{X}_m,...]$ and $\ddot{\mathbf{V}}_m^{(s)}=[\mathbf{1},\mathbf{X}_m,\ddot{\mathbf{G}}_m^{(s)}\mathbf{X}_m]$. Consider also the following (simulated) moment function:
\begin{equation}\label{eq:moment}
\bar{\mathbf{m}}_{M}(\boldsymbol{\theta})=\frac{1}{M}\sum_m\frac{1}{RST}\sum_{rst}\dot{\mathbf{Z}}^{(r)\prime}_m\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})_m\left(\mathbf{y}_m-(\mathbf{I}-\alpha\ddot{\mathbf{G}}_m^{(s)})^{-1}\ddot{\mathbf{V}}_m^{(s)}\tilde{\boldsymbol{\theta}}\right)\right]
\end{equation}

[Result] For any positive integers $R$, $S$, and $T$, the (simulated) GMM estimator based on (\ref{eq:moment}) is consistent and asymptotically normally distributed.
\end{theorem}



To understand the intuition behind the use of the moment function (\ref{eq:moment}), let us replace $\mathbf{y}=(\mathbf{I}-\alpha\mathbf{G})^{-1}(\mathbf{V}\tilde{\boldsymbol{\theta}}+\boldsymbol{\varepsilon})$ in Equation (\ref{eq:moment}), considering a single group and ignoring the subscript $m$. In doing so, we can rewrite the term inside the triple summation in (\ref{eq:moment}) as a sum of two terms. First, $\dot{\mathbf{Z}}^{(r)\prime}\boldsymbol{\varepsilon}$, which would be the standard moment function if $\mathbf{G}$ was observed (e.g. \cite{bramoulle2009identification}), and second:
\begin{equation}\label{eq:bias_corr}
\dot{\mathbf{Z}}^{(r)\prime}\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})\left((\mathbf{I}-\alpha{\mathbf{G}})^{-1}{\mathbf{V}}-(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}\ddot{\mathbf{V}}^{(s)}\right)\tilde{\boldsymbol{\theta}}\right].
\end{equation}
That second term can be viewed as the bias-correction term of the moment function.

We show that the expectations of both terms are equal to $0$ as $M$ grows to $\infty$. For the first term, this is true because the simulated network is exogenous. For the second term, this is true because $\mathbf{G}$, $\dot{\mathbf{G}}$, $\ddot{\mathbf{G}}$, and $\dddot{\mathbf{G}}$ are asymptotically drawn from the same distribution.

For the special case in which $\mathbf{G}$ is observed, one could substitute $\dot{\mathbf{G}}^{(r)}=\ddot{\mathbf{G}}^{(s)}=\dddot{\mathbf{G}}^{(t)}=\mathbf{G}$ for all $r,s,t$, and the first term would simply be $\mathbf{Z}'\boldsymbol{\varepsilon}$, whereas the second term would be exactly equal to $\mathbf{0}$.

Note that Theorem \ref{prop:non_observed} is valid whether or not $\mathbf{Gy}$ and $\mathbf{GX}$ are observed because the moment function (\ref{eq:moment}) does not use information on $\mathbf{Gy}$ or $\mathbf{GX}$. It is of course possible to include this additional information if either one is observed.

For example, assume that $\mathbf{GX}$ is observed and replace $\ddot{\mathbf{V}}$ with $\mathbf{V}$ in (\ref{eq:bias_corr}). After some algebra, we obtain: \begin{equation}\label{eq:gxobswrong}
    \dot{\mathbf{Z}}^{(r)\prime}\left[(\mathbf{I}-\alpha\dddot{\mathbf{G}}^{(t)})(\mathbf{I}-\alpha\ddot{\mathbf{G}}^{(s)})^{-1}[\alpha(\mathbf{G}-\ddot{\mathbf{G}})\mathbf{y}]\right]
\end{equation}
and a term that is equal to zero in expectation.

We can show that the last term in brackets corresponds to the source of the asymptotic bias because of the approximation error of $\mathbf{Gy}$ by $\ddot{\mathbf{G}}\mathbf{y}$ (see Proposition \ref{prop:bias_nocontext} of the Online Appendix). Whereas Equation (\ref{eq:gxobswrong}) cannot directly be substituted for (\ref{eq:moment}) in Theorem \ref{prop:non_observed}, it is possible to construct moment functions for the particular cases for which $\mathbf{GX}$ or $\mathbf{Gy}$ is observed. These cases can be found in Corollary \ref{prop:GXobs} and \ref{prop:Gyobs} of the Online Appendix.


